Variable-Frequency Model Learning and Predictive Control for Jumping Maneuvers on Legged Robots

Achieving both target accuracy and robustness in dynamic maneuvers with long flight phases, such as high or long jumps, has been a significant challenge for legged robots. To address this challenge, we propose a novel learning-based control approach consisting of model learning and model predictive control (MPC) utilizing a variable-frequency scheme. Compared to existing MPC techniques, we learn a model directly from experiments, accounting not only for leg dynamics but also for modeling errors and unknown dynamics mismatch in hardware and during contact. Additionally, learning the model with variable-frequency allows us to cover the entire flight phase and final jumping target, enhancing the prediction accuracy of the jumping trajectory. Using the learned model, we also design variable-frequency to effectively leverage different jumping phases and track the target accurately. In a total of 92 jumps on Unitree A1 robot hardware, we verify that our approach outperforms other MPCs using fixed frequency or nominal model, reducing the jumping distance error 2 to 8 times. We also achieve jumping distance errors of less than 3 percent during continuous jumping on uneven terrain with randomly placed perturbations of random heights (up to 4 cm or 27 percent the robot standing height). Our approach obtains distance errors of 1 to 2 cm on 34 single and continuous jumps with different jumping targets and model uncertainties. Code is available at https://github.com/DRCL-USC/Learning MPC Jumping.

==> Sections/diff.tex <==
\section{Introduction}
\redst{Aggressive maneuvers with legged robots, such as jumping \cite{QuannICRA19,RL_jump_bipedal}, back-flipping \cite{unitreeH1}, and barrel rolls \cite{chuongjump3D}, have received significant attention recently, and have been successfully demonstrated using trajectory optimization \cite{QuannICRA19,chuongjump3D,matthew_mit2021_1,ChignoliICRA2021}, model-based control \cite{YanranDingTRO,continuous_jump_bipedal,GabrielICRA2021,park2017high, ZhitaoIROS22,fullbody_MPC}, and learning-based control \cite{zhuang2023robot, RL_jump_bipedal,yang2023cajun,vassil_drl,jumpingrl,lokesh_ogmp}.} 
\IEEEPARstart{A}{ggressive} jumping maneuvers with legged robots have received significant attention recently, and have been successfully demonstrated using trajectory optimization \cite{QuannICRA19,chuongjump3D,matthew_mit2021_1,ChignoliICRA2021}, model-based control \cite{YanranDingTRO,continuous_jump_bipedal,GabrielICRA2021,park2017high, ZhitaoIROS22,fullbody_MPC}, and learning-based control \cite{zhuang2023robot, RL_jump_bipedal,yang2023cajun,vassil_drl,jumpingrl,lokesh_ogmp}.
Unlike walking or running, aggressive motions are particularly challenging due to \textit{(1)} the extreme underactuation in the mid-air phase (the robot mainly relies on the force control during contact to regulate its global position and orientation), \textit{(2)} significant dynamics model error and uncertainty that are inherently hard to model accurately, especially with contact and hardware load during extreme motions, and \textit{(3)} the trade-off between model accuracy and efficient computation for real-time execution. Achieving both target accuracy and robustness for long-flight maneuvers, such as high or long jumps, therefore still presents an open challenge. 
In this work, we address this challenge by developing a real-time MPC for quadruped jumping using a robot dynamics model learned from experiments.
% In this work, we address this challenge by developing a
% real-time MPC with dynamics model learned from experiments, demonstrated via an example of quadruped jumping.

%developing a real-time model predictive control policy with adaptive frequency and accurate learned robot dynamics from data.

% Recent advancements in model-based approaches, notably MPC, have proven effective in realizing robust acrobatic motions \cite{GabrielICRA2021,park2017high, YanranDingTRO,continuous_jump}. 

% In the realm of model-based control and optimization, the main challenge of modeling choice to realize jumping tasks is how to compromise between model accuracy and online control. 
%a varied selection of models
% \rep{Many advanced control and optimization frameworks with different dynamics formulations have been proposed to realize jumping maneuvers}.

% \TD{What does it mean to be full-nonlinear dynamics? Does that mean it accounts for the leg dynamics? This is because we just mentioned in the previous paragraph that some parts of the dynamics are hard to model but here, it might make an impression to readers that full dynamics are available to use.} 

\rebut{Many control and optimization techniques have been developed for jumping motions.}\redst{Various dynamics models have been proposed for control and optimization of aggressive robot maneuvers.} \rebut{Trajectory optimization (TO) with full-body nonlinear dynamics is normally utilized to generate long-flight trajectories in an offline fashion (e.g., \cite{QuannICRA19,chuongjump3D}).}
% However, since the optimization is very high dimensional and objectives are highly nonlinear, solutions are normally obtained offline. 
% For efficient computation, many offline trajectory optimization frameworks adopt reduced-order models such as spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid} or standard single-rigid-body dynamic (SRBD) \cite{ChignoliICRA2021, ZhitaoIROS22}.
\redst{Many frameworks sacrifice model accuracy for very efficient computation by using simplified models such as spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid} or single-rigid-body dynamic (SRBD) \cite{NMPC_3D_hopping, ZhitaoIROS22, GabrielICRA2021, park2017high,YanranDingTRO} that lumps the trunk and legs into a unified body.}
\rebut{Many MPC approaches sacrifice model accuracy to achieve robust maneuvers by using simplified models that treat the trunk and legs as a unified body \cite{NMPC_3D_hopping,ZhitaoIROS22,GabrielICRA2021, park2017high,YanranDingTRO}. 
% Iterative learning control (ILC) can tackle model uncertainties and unknown dynamics by gradually improving the tracking accuracy over trials \cite{Kai_ILC_biped_ICRA15, Kai_ILC_TRO,pronking_ILC, ILC_continuous_pronking}. 
Our recent iterative learning control (ILC) work \cite{chuong_ilc_jump} handles model uncertainty to realize long-flight jumps via multi-stage optimization that optimizes the control policy after each jump offline until reaching a target accurately. It also relies on a simplified model for computational efficiency. However, this work focuses on target jumping rather than robustness, e.g. requiring the same initial condition for all trials. Different from existing works, we learn a robot dynamics model from experiments and develop real-time MPC using the learned dynamics to achieve both target accuracy and robustness in continuous quadruped jumping.}
% Many methods sacrifice model accuracy for real-time performance by using simplified models such as nominal single-rigid-body dynamics (SRBD) \cite{NMPC_3D_hopping,ZhitaoIROS22,GabrielICRA2021, park2017high,YanranDingTRO} that combine the trunk and legs as a unified body. 
% To consider the effect of leg dynamics, Zhou \textit{et al.} \cite{ZiyiZhouRAL} recently propose a linearized variant of the full centroidal dynamics, incorporating joint information to centroidal model of quadruped jumping \cite{ZiyiZhouRAL}; He \textit{et al.} \cite{He2024} exploit centroidal inertia decomposition model to regulate angular momentum during flight phase of bipedal jumping. In most existing works, the effects of model mismatch or unknown dynamics in hardware and contact on the accuracy of aggressive maneuvers, however, have not been well explored and modeled effectively. 
\redst{Recently, designing models that both consider leg dynamics and enable real-time execution has gained considerable attention. Zhou \textit{et al.} \cite{ZiyiZhouRAL} propose a linearized variant of the full centroidal dynamics, incorporating joint information in a centroidal model of quadruped jumping. He \textit{et al.} \cite{He2024} exploit a centroidal inertia decomposition model to regulate angular momentum during the flight phase of bipedal jumping. However, developing a model that can account for model mismatch with hardware and dynamics uncertainty as well as effectively predict long flight phases, which is important for control policies to enhance both target accuracy and jumping robustness, is still an open challenge.}
% \rebut{Iterative learning control (ILC) is another effective strategy to deal with model uncertainties and unknown dynamics by gradually improve the tracking accuracy over time \cite{Kai_ILC_biped_ICRA15, Kai_ILC_TRO,pronking_ILC, ILC_continuous_pronking}. Our recent ILC paper \cite{chuong_ilc_jump} aims to realize target accuracy for long-flight jumps via multi-stage optimization that off-line adjusts the control after each jump. It also allows using one reference for many targets. However, this work focuses on target jumping rather than robustness, e.g. requiring the same initial condition for all trials. Different from existing work, we propose to learn the robot dynamics from experiments and develop real-time MPC for the learned dynamics, achieving both target accuracy and robustness for aggressive maneuvers, such as continuous jumping.} 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{figures/Introduction/Introduction-v6-traj-v2.pdf}%	
    % The Unitree A1 robot is able to jump on box with target error of $1~cm$ and orientation error less than $10^0$ degree upon landing.
    % during prediction horizons ($\Delta t_{\calF} > \Delta t_{\calC}$). 
    \caption{A Unitree A1 robot performs \textit{continuous jumps} on unknown uneven terrain, achieving both target accuracy and robustness. The target distance for each jump is $0.6$ m. The flight phase covers a vertical height of up to $4 \times$ the robot's normal height. \rebut{MPC with a nominal single rigid-body model is used to collect data for training a neural-network residual dynamics model following using a variable-frequency scheme. The learned model is then used in a variable-frequency MPC to execute jumping motions. The variable-frequency scheme varies the time step sizes in the contact phase ($\Delta t_{\calC}$) and flight phase ($\Delta t_{\calF}$) to dedicate more model capacity and more MPC optimization steps to the contact phase, which improves the jumping robustness and accuracy. The green dashed line is the actual robot trajectory.} Supplemental video: \url{https://youtu.be/yUqI_MBOC6Q}.}
    \label{fig:introduction}
\vspace{-0.6cm} 
\end{figure}
% \rebut{However, developing an approach that can account for model mismatch with hardware and dynamics uncertainty as well as effectively predict long flight phases, which is important for control policies to enhance both target accuracy and jumping robustness, is still an open challenge.}
% that combines the trunk and legs into a unified body. 
% which usually ignores the change in the centroidal inertia due to the limb movements. 
% To reason the effect of leg dynamics, the authors in \cite{KeMechatronics23} abstract the legged robots as a standard SRBD for the base and point masses for the legs. This choice reduces a certain complexity to the model for offline planning, compared to the full-order model resolution.
% , or centroidal dynamics with kinematic constraints \cite{matthew_mit2021_1, ChignoliICRA2022}. 
% To reason the effect of leg dynamics, recent work \cite{KeMechatronics23} abstracts the legged robots as a standard SRB for the base and point masses for the legs.
% These reduced-order models are utilized for offline planning to generate reference trajectories for long-flight maneuvers, which then be tracked by additional real-time control.
% However, incorporating joint information to reason about the centroidal inertia is non-trivial with these models, which limits their ability to generate angular-momentum-rich motions using limb movements such as jumping.
% The lumped-leg SRBM attempted to augment the standard SRBM
% by approximating the time-varying inertia tensor; however, neither use the full capabilities of the joint motions.
% Many optimization frameworks sacrifice model accuracy for very efficient computation by assuming the robot dynamics as a single rigid body (SRB) dynamics (\cite{ChignoliICRA2021, ZhitaoIROS22}), or centroidal dynamics with kinematic constraints (\cite{matthew_mit2021_1, ChignoliICRA2022}), which ignore the dynamic effect of all legs in the whole-body jumping motions.
% To leverage the limb movement, the authors in \cite{KeMechatronics23} abstract the legged robots as a SRB for the base and point masses for the legs. However, leveraging leg motions typically adds a certain complexity to the model, thus this is mainly utilized for offline planning. 
% Recently, there have been increasing efforts to achieve real-time control with models that account for non-constant leg inertia.
% These simplified models have also been widely adopted for online control pipelines for jumping \cite{GabrielICRA2021,park2017high, YanranDingTRO}. 
% However, incorporating leg configuration to reason about the centroidal inertia is non-trivial with these models. 

% These simplifications consider the effect of leg dynamics partially or ignore it in the whole-body linear and angular momentum. 
% Thus, it may compromise target jumping accuracy for real-time control.
% However, since these simplifications ignore the dynamic effect of all legs in the whole-body linear and angular momentum, adopting these models may compromise target accuracy as well as success rates when translating highly agile motions to hardware.
% To enable real-time execution, the complexity of the dynamics has been simplified and led to the introduction of various models. Single rigid body model (SRBM) ....(\cite{NMPC_3D_hopping, YanranDingTRO, GabrielICRA2021}), spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid}, . Such simplification normally ignores the dynamic effects of legs.
% In summary, the main challenge of modeling choice is how to compromise between model accuracy and online control.
% In this work, we attempt to address this problem by proposing a well-balanced middle-ground model that is able to leverage the effect of legged dynamics, but can be efficiently utilized for real-time control and optimization.
% Difference from previous work, we develop
% a learning-base model that can represent the effect of leg
% dynamics in the whole-body linear and angular momentum
% of the robot trajectories, while it is efficiently utilized for
% real-time control and optimization

% In this work, we propose a dynamics model learned from data, which considers not only the effects of leg dynamics but also model mismatch with the real robot hardware.



% \note{Dynamic learning}
Learning robot models from experiments to capture complex dynamics effects and account for model errors with real hardware has become a popular approach \cite{ bauersfeld2021neurobem,hewing2019cautious,saviolo2022physics,duong23porthamiltonian}.
% A recent line of work aims to learn dynamic models entirely from real-world data, with a primary investigation of dynamical systems without contact \cite{salzmann2023real, bauersfeld2021neurobem,hewing2019cautious,saviolo2022physics}. 
% Compared to Deep Reinforcement Learning which often requires millions of timesteps of simulation interactions and bridging sim-to-real gaps \cite{jumpingrl,yang2023cajun, RL_jump_bipedal,zhang2024wococo,unitreeH1}, directly learning real-world models via residual dynamics can require a smaller number of data points \cite{bauersfeld2021neurobem, salzmann2023real}
% directly learning real-world models for control is able to address these challenges. In addition, by exploiting the residual dynamics of a nominal model, it can even require a smaller number of data points to effectively learn the model \cite{bauersfeld2021neurobem, salzmann2023real}
% Compared to learning the full model, learning the residual dynamics of a nominal model simplifies the learning tasks and allows describing the model augmentation using only a smaller number of data points. 
Many frameworks learn residual dynamics using neural networks \cite{bauersfeld2021neurobem, salzmann2023real} or Gaussian processes \cite{hewing2019cautious, cao2017gaussian} and use MPC to control the learned systems \cite{salzmann2023real, pohlodek2022hilompc} to improve tracking errors.
Most existing works, however, primarily investigate dynamical systems without contact. Recently, Sun et al. \cite{sun2021online} proposed a notable method to learn a linear residual model, addressing unknown dynamics during walking stabilization.
% , \rebut{but not considering the effect of leg dynamics.} 
\redst{Nevertheless, the method is designed for walking stabilization specifically and does not leverage the effect of leg dynamics.} 
\rebut{Pandala et al. \cite{Pandala_robustMPC}  propose to close the gap between reduced- and full-order models by using deep reinforcement learning to learn unmodeled dynamics, which are used in MPC to realize robust walking on various terrains. Meanwhile, we use supervised learning to learn unmodelled dynamics with real data from hardware.} 
\redst{Compared to existing works, learning dynamics for aggressive maneuvers with long-flight periods on legged robots presents some challenges,}
\rebut{Also, we learn dynamics for maneuvers with long-flight periods to tackle} \textit{(1)} the switching between multiple dynamic models due to contact, including flight phase where control action has very little effect on the body dynamics, \textit{(2)} disturbances and uncertainty in dynamic modeling due to hard impact in jumping, and \textit{(3)} the effect of intermittent control at contact transitions on state predictions. 


% \TD{We haven't defined adaptive frequency until the next paragraph. Also, I don't think that adaptive frequency affects the comparison of our approach with others here. So maybe we can omit it.}

% enhancing target jumping accuracy for dynamic maneuvers with extended flight phases.

% \rep{ Compared to the abundance of work that exists for learning the dynamics, the literature for learning the dynamic maneuvers of systems with contact, such as jumping on legged robots, is comparatively sparse and consists of unique challenges such as \textit{(1)}  the period of extreme underactuation, \textit{(2)} complex contact dynamics, and \textit{(3)} the effect of intermittent control at contact transitions to state predictions. To address these challenges, we propose a residual learning model for legged robots and design the learning in an adaptive frequency scheme to realize the model for enhancing target jumping accuracy for dynamic maneuvers with extended flight phases.}
% Most of the work, however, mainly focuses on learning systems without contact such as aerial robots \cite{bauersfeld2021neurobem, salzmann2023real,duong23porthamiltonian}.
% Several works augment a nominal model with a learned residual to account for uncertainties or to capture complex dynamic effects. 
% One approach is to complement a nominal model with a Gaussian process \cite{kabzan2019learning, torrente2021data, khadivar2023self}, but a key drawback is a computational complexity due to its nonparametric nature. Another approach is to use neural networks for the residual term \cite{salzmann2023real, saviolo2022physics}. 
% Khadivar et al. \cite{khadivar2023self} learn a residual inverse dynamics model for a quadratic programming-based controller to account for model uncertainties using a Gaussian process.
% Existing works discussed above, however, aims to learn the dynamics systems without contact dynamics. 
% For learning systems with contact, Sun et al. \cite{sun2021online} recently propose a notable framework to learn a time-varying linear residual model for a quadruped robot to compensate for the unmodeled dynamics online, which however mainly focuses on the walking stabilization.
% The work \cite{sun2021online} shows impressive robustness of walking motion under model uncertainties; however, leveraging the effect of leg dynamics on the model is not demonstrated.
% \note{To our knowledge, such approaches have not yet been demonstrated for modeling the legged robots.}



%MPC has recently been brought into the realm of real-time dynamic jumping control due to its ability to optimize control actions during the contact phase based on predictions of where the robot in mid-air periods

In this letter, we propose a residual learning model that uses a \rebut{variable-frequency} \redst{adaptive-frequency} scheme, \rebut{i.e., varying the coarseness of integration time step}, to address the aforementioned challenges and enhance long-term trajectory predictions over different jumping phases. MPC has been commonly used for jumping by optimizing the control inputs during the contact phase based on future state prediction during the flight phase (e.g.,\cite{GabrielICRA2021, fullbody_MPC, park2017high, YanranDingTRO,  continuous_jump}). 
% When it comes to model selection, there is typically an inherent trade-off between model accuracy and computational efficiency.
% A full-body nonlinear dynamics model can leverage the whole effect of leg dynamics on the robot trajectory; however, it normally poses a challenge to utilize this model for real-time performance due to its high nonlinearity. Therefore, it is mainly utilized for offline planning to generate complex motions with long flight phases to consider all feasible nonlinear constraints (e.g., \cite{QuannICRA19,chuongjump3D}).
% ; nevertheless, it can take a significant amount of time to converge to the optimal solution due to the model's complexity.
%\rep{When designing MPC for long flight maneuvers, a major challenge is how to utilize a limited number of the prediction horizons but still effectively cover the entire flight phase and especially the final target in the horizons, as it is the most important goal for jumping. Another challenge is to obtain an accurate model to leverage complex dynamic maneuvers, unknown dynamics, and model mismatch with real hardware in order to improve jumping accuracy, while still ensuring real-time performance.}
%in the horizons, as it is the most important goal 
A major challenge in MPC for long flight maneuvers is to utilize a limited number of prediction steps yet still effectively cover the entire flight phase and especially the final jumping target. Another challenge is to obtain an accurate model for complex dynamic maneuvers, unknown dynamics, and model mismatch with the real hardware to improve the jumping accuracy, while still ensuring real-time performance. Some recent works have addressed these challenges partially.
% how to achieve accurate trajectory prediction for the entire flight phase
% To facilitate real-time computation, 
%  to sacrifice model accuracy for 
% , as demonstrated via robust jumping tasks (e.g. 
Many methods use conventional single-rigid-body dynamic (SRBD) models, ignoring the leg dynamics, to achieve real-time execution \cite{GabrielICRA2021,continuous_jump_bipedal,YanranDingTRO}. 
% \rebut{However, the trajectory prediction error due to leg inertia can accumulate significantly over long flight periods \cite{chuongjump3D}}. 
\rebut{Using the SRBD model in the contact phase can lead to inaccurate predictions of the robot's state at take-off, which is the initial condition of the
projectile motion in the flight phase. Thus, the trajectory prediction error can accumulate significantly over long flight periods.}
% which will then 
%  a key idea of our method is to improve the model
% using learning in order to obtain more precise contact phase prediction and, hence, an accurate initial condition of the
% projectile motion during flight
Some methods account for leg inertia \cite{ZiyiZhouRAL,He2024,fullbody_MPC}, however, disturbance and uncertainty in dynamic modeling have not been considered. 
% These frameworks also focus on jumping robustness rather than accurate target jumping. 
\rebut{Recently, planning with multi-fidelity models and multi-resolution time steps has emerged as an effective strategy to enhance target accuracy and robustness \cite{heli_cafempc,Norby_adaptivempc,Heli_hierarchympc}. Li et al. \cite{Heli_hierarchympc} adopt a less accurate model in the far horizon and a more accurate but expensive model in the near future. Norby et al. \cite{Norby_adaptivempc} adapt model complexity based on the task complexity along the prediction horizon. Li et al. \cite{Heli_hierarchympc} also design multi-resolution time steps to cover the whole flight phase. While we vary the coarseness of the time step as \cite{Heli_hierarchympc}, we design a novel residual model learning approach combined with variable-frequency MPC to address the aforementioned challenges.}
% Our work is related to \cite{heli_cafempc} by way of varying the coarseness of the timesteps but with distinct ideas.  We learn the model from experimental results, which account for nonlinear legged dynamics, uncertainties, and model mismatch with the real hardware. The learning dynamics is synchronized with MPC prediction to cover contact transitions and improve the accuracy of long-term trajectory prediction.
\redst{In this work, we address these challenges by learning a dynamics model from date and designing an adaptive-frequency MPC capturing both the contact and entire flight phase in the optimization process}

\textbf{Contributions:} The contributions of this letter are summarized as follows. 
% We learn a \textit{residual dynamics model} directly from a small real experiment dataset. The model accounts for nonlinear leg dynamics, modeling errors, and unknown dynamics mismatch in hardware and during contact. We propose learning the model in an \rebut{\textit{variable-frequency scheme}} \redst{adaptive-frequency scheme} that leverages different time resolutions to capture the entire flight phase, the jumping target, and the contact transitions over a few-step horizon, thereby significantly improving the accuracy of long-term trajectory prediction. We propose learning the model in an \rebut{\textit{variable-frequency scheme}} \redst{adaptive-frequency scheme} that leverages different time resolutions to capture the entire flight phase, the jumping target, and the contact transitions over a few-step horizon, thereby significantly improving the accuracy of long-term trajectory prediction. \textit{Extensive hardware experiments} validate the effectiveness and robustness of our approach with single and consecutive jumps on uneven terrains. Comparisons with other MPC techniques using a nominal model or fixed-frequency are also provided.
% The highly dynamic jump typically requires the robot to reach its hardware limits. In these extreme condition, the accurate model is hard to achieve.
% Our work proposes a solution to tackle this problem by leveraging the advantage of supervised learning and real-time model predictive control.
% Contributions:
\begin{itemize}
  % \item We learn a \textit{residual dynamics model} directly from a small real experiment dataset. The model accounts for nonlinear leg dynamics, hardware modeling errors, and model mismatch during contact.
  \item We learn a \textit{residual dynamics model} directly from a small real experiment dataset. The model accounts for nonlinear leg dynamics, modeling errors, and unknown dynamics mismatch in hardware and during contact.
  
  % \item \rep{A residual adaptive-frequency learning model that aims not only to learn the nonlinear leg dynamics, unknown dynamics, and model mismatch from real robot hardware but also enhance long-term state predictions over different jumping phases} 
  
  % \item We introduce an \textit{adaptive-frequency scheme} that leverages different time resolution to capture the entire flight phase, the jumping target, and the contact transitions over a few-step horizon, thereby significantly improving the accuracy of long-term trajectory prediction.

    \item We propose learning the model in an \rebut{\textit{variable-frequency scheme}}\redst{adaptive-frequency scheme} that leverages different time resolutions to capture the entire flight phase, the jumping target, and the contact transitions over a few-step horizon, thereby significantly improving the accuracy of long-term trajectory prediction.
    
  % \item \rep{A residual model learning approach that learns the effect of unknown nonlinear dynamics, e.g., leg dynamics, and model mismatch from real robot hardware from real-world data in an adaptive-frequency scheme.} 
%   We propose to learn a residual model from real-world
% data and in an adaptive-frequency scheme to leverage
% the effect of leg dynamics, unknown dynamics, and
% model mismatch with the real robot hardware, as well
% as enhance target jumping accuracy.

  % The model can be efficiently utilized for real-time control and optimization of highly dynamic jumping.
  \item We develop  \rebut{\textit{variable-frequency MPC using the learned model}}\redst{adaptive-frequency MPC using the learned model} to synthesize controls that improve both target accuracy and robustness in dynamic robot maneuvers.
  
  \item \textit{Extensive hardware experiments} validate the effectiveness and robustness of our approach with single and consecutive jumps on uneven terrains. Comparisons with other MPC techniques using a nominal model or fixed-frequency are also provided.
  % \item \rep{ We also validate the framework on robust and consecutive jumping on uneven terrain consisting of perturbation of random heights ($13-27\%$ of the robot's standing height), achieving an average distance error of $1.67~cm$.}
  % \item We conduct 48 dynamic jumps .
\end{itemize}

% Our approach outperforms other MPC settings, achieving a jumping distance error of less than $3\%$ compared to the target, based on the overall performance of 20 jumps with different target locations and ground uncertainties.
\redst{Our approach outperforms other MPC settings, reducing the jumping distance error up to $8$ times. We demonstrate robust and consecutive jumping on uneven terrain with height perturbations ($13-27\%$ of the robot's standing height), achieving a distance error of $1.67$ cm on average. Testing on $34$ single and continuous jumps, our approach achieves target jumping error of less than $2$ cm ($3.5\%$) for different targets and uneven terrain.}

% This letter is organized as follows. Section \ref{sec:overview} presents the overview of the proposed system architecture. In more detail, Section \ref{sec:proposed_approach} introduces the proposed learned residual model, followed by adaptive-frequency model training and MPC execution for learned dynamics. The results of hardware experiments are reported in Section \ref{sec:results}. Finally, we summarize our conclusions and discuss directions for future research in Section \ref{sec:conclusion} .
 
% Using simplified model is evidenced to enable real-time computation; However, it normally sacrifices the target jumping accuracy. On the other hand, full-body dynamic model typically enables accurate jumping with further requirement on off-line solving
% Our work towards that goal by bringing the 
% Numerous recent advancements in robotics draw inspiration from nature, textitasizing the refinement of efficiency and precision in highly dynamic jumping maneuvers targeted at a specific point within real-world applications.

% \section{Related Work} \label{sec:related_work}

% \subsection{Model-based Control and Optimization} Recent advancements in model-based approaches, notably Model Predictive Control (MPC), have proven effective in realizing diverse acrobatic motions \cite{GabrielICRA2021,park2017high,YanranDingTRO,continuous_jump, Quad-SDK}. To facilitate real-time computation, MPC often builds up on simplified dynamics models that combine the body and legs into a unified rigid body. While this approach expedites computations, these simplifications in the robot model may compromise both accuracy and success rates when translating highly agile motions to hardware. At the other end, trajectory optimization (TO) has shown as an effective solution for improving accuracy by considering a full-body dynamics model, making it well-suited for planning acrobatic motions with long flight times \cite{QuannICRA19, matthew_mit2021_1,chuongjump3D}. Full-body trajectory optimization has very high dimensional and objectives are highly nonlinear, which often leads optimization procedures into bad local minima. However, the trajectory optimization can be slow, especially when a good initial guess is not available. Therefore, solutions are normally obtained offline with trajectory optimization.


% In the context of conventional locomotion
% strategies like walking and running, such initial guesses can
% be generated by simplified models [15], but such templates are
% not readily available for tasks that require whole-body shape
% changes like in mid-air acrobatics.

% Although both MPC and trajectory optimization offer promising solutions for dynamic jumping, they typically rely on the accuracy of the model. Nevertheless, an accurate model may hardly be achieved due to uncertainties and unmodelled dynamics involved in jumping motion. 
% For example, the interaction between foot and ground introduces various uncertainties, such as varied friction or unknown ground stiffness and damping. In addition, parameter variations (i.e. inaccurate kinematic parameters) contribute to the model accuracy as well. The authors in \cite{Zachary_RAL_online_calibration_2022} show that the actual leg length of a robot with deformable feet is likely difficult to measure due to dynamic deformation effects and rolling contacts. These problems are likely to cause inaccuracy in hardware transfer. 
% Last but not least, the jumping motion typically involves long flight maneuvers. During this aerial period, the system becomes under-actuated systems and the control has little impact on the robot trajectory during this period \cite{falling_cat}. Therefore, the trajectory errors are normally accumulated and prevent the robot from reaching desired targets at high accuracy. 


% In our prior work \cite{continuous_jump}, we combine real-time MPC
% and joint PD controller to track the reference motion from
% the trajectory optimization under unknown disturbance. The MPC is also designed based on single rigid body dynamics. However, since the predicted horizon of MPC in our prior work is limited, it would not efficient to deal with jumping with long flight time.

% \subsection{Learning-based approaches} 


% \subsection{Dynamics learning.} 

% Saviolo et al. \cite{saviolo2022physics} relax the nominal model's strict physical constraints, guiding the neural network to learn the true system dynamics from data by using soft constraints to guide the training. 










% \textbf{Variational Integrator Networks}
% MPC controllers rely on long-term predictions of the robot states given a control policy, by using an ODE solver to integrate the continuous-time dynamics over time, such as Euler approximation or Runge-Kutta methods. While such solvers are universal, they do not account for the structure or symmetry of a physical system, e.g. respecting the law of energy conservation, leading to poor long-term predictions. Instead,  variational integrators \cite{marsden2001discrete} have been used to predict the future states of a physical system by discretizing Langrange-d'Alembert principle instead of Euler-Lagrange equations, e.g. in astronomy (\todo{cite}) (\todo{search for papers in robotics as well?}). This leads to an integration rule that respects the law of energy conservation and accurately predicts the future trajectory.

% Let $\frakq$ and $\dot{\frakq}$ be the generalized coordinates and velocity. The Lagrangian of the system is defined as the difference between the kinetic energy and the potential energy:
% \begin{equation}
%     \calL(\frakq, \dot{\frakq}) = \frac{1}{2}\dot{\frakq}^\top \bfM \dot{\frakq} - V(\frakq),
% \end{equation}
% where $\bfM$ is the generalized mass, e.g. mass for linear velocity and inertia matrix for angular velocity, and $V(\frakq)$ is the potential energy. The Lagrange-d'Alembert principle states that:
% \begin{equation}
% \label{eq:Lagrange-dAlembert}
%     \delta  \int_0^T \calL(\frakq(t), \dot{\frakq}(t))dt + \int_0^T\bff(\frakq(t), \dot{\frakq}(t), \bfu(t))\delta \frakq(t)dt = 0.
% \end{equation}
% This leads to the standard Euler-Lagrange equations:
% \begin{equation}
% \label{eq:Euler-Lagrange}
%     \frac{\partial \calL(\frakq(t), \dot{\frakq}(t))}{\partial\frakq} - \frac{d}{dt}\left(\frac{\partial \calL(\frakq(t), \dot{\frakq}(t))}{\partial\dot{\frakq}}\right) + \bff(\frakq(t), \dot{\frakq}(t), \bfu(t)) = 0.
% \end{equation}
% While normal integrators discretize Eq. \eqref{eq:Euler-Lagrange}, variational integrators discretize Eq. \eqref{eq:Lagrange-dAlembert} and yield the following integration rules for $\frakq$ in $\bbR^n$:
% \begin{equation}
% \label{eq:var_int_Rn}
%     \begin{aligned}
%         \frakq_{k+1} &= \frakq_k + h\dot{\frakq}_k + \frac{h^2}{2}\bfM^{-1}(F(\frakq_k, \bfu_k) - \nabla V(\frakq_k)) \\
%         \dot{\frakq}_{k+1} &= \dot{\frakq}_k + h\bfM^{-1}(F(\frakq_k, \bfu_k) - \frac{\nabla V(\frakq_k) + \nabla V(\frakq_{k+1})}{2}),
%     \end{aligned}
% \end{equation}
% where $F(\frakq_k, \bfu_k)$ represents the average external force over the time step $h$. Havens et al. \cite{havens2021forced} model $\bfM, F$ and $V$ in Eq. \eqref{eq:var_int_Rn} by neural networks and learn them from data. Please refer to \cite{havens2021forced} and references therein for more details.

% When the coordinates $\frakq$ evolves on the $SE(3)$ manifold, the integration rules are derived to respect both the law of energy conservation and the manifold constraints as follows.
% \begin{equation}
% \label{eq:_var_int_SE3}
%     \begin{aligned}
%    & h\hat{\pi}_k   +   h \hat{\bff}_{d_k}^{R-} + (1-\alpha)h^2 \hat{\xi}_k  =  Z_k J_d - J_d Z_k^\top , \\ &
%     R_{k+1}  = R_k Z_k , \\
%     & \pi_{k+1}  = Z_k^\top \pi_k + (1-\alpha)h Z_k^\top \xi_k+ \alpha h \xi_{k+1}   + Z_k^\top \bff_{d_k}^{R-}+ \bff_{d_k}^{R+}   , \\ &
%       x_{k+1}  =  x_{k} + \frac{h}{m} \gamma_k - (1-\alpha)\frac{h^2}{m} \frac{\partial U_k}{\partial x_k} -  \frac{h}{m} R_k \bff_{d_k}^{x-}  , \\ &
%         \gamma_{k+1}  = \gamma_k - (1-\alpha)h    \frac{\partial U_k}{\partial x_k} - \alpha h \frac{\partial U_{k+1}}{\partial x_{k+1}} +  R_k \bff_{d_k}^{x-} \\ & \qquad \qquad + R_{k+1} \bff_{d_k}^{x+},
% \end{aligned}
% \end{equation}
% where $\pi_{k} = m\bfv_k$ is the linear momentum, $\gamma_k = \mathbf{J}\Omega$ is the angular momentum, and $\hat{\xi}_k = \frac{\partial  V_{k}}{\partial R_{k}}^\top R_{k} - R_{k}^\top \frac{\partial V_{k}}{\partial R_{k}}$. Our previous paper \cite{duruisseaux2022lie} model the mass $(m,\mathbf{J})$, the potential energy $V$ and the generalized force $\bff_d$ by neural networks, trained from data. Please refer to \cite{lee2008computational, duruisseaux2022lie} for more details. (\todo{Unify notations in Eq. \eqref{eq:var_int_Rn} and Eq. \eqref{eq:_var_int_SE3}}).

% \textbf{Energy-based control for jumping.} \todo{Questions}: Can we design an energy-based controller for jumping? The control input is only applied during contact phase, which is different from the setting from our previous paper \cite{Duong-RSS-21}. It is perhaps related to event-triggered control?




% \section{Problem Formulation}
% \label{sec:Method}
% % We separate as two problems: Jumping in 2D and Jumping in 3D



%  to capture the whole-body coordination

% \section{Preliminaries} \label{sec:Preliminaries}
% % We first revisit two fundamental models for quadruped locomotion.

% % \subsection{Full-body dynamics}
% % Jumping is a highly complex motion for a legged robots, requiring coordination of the whole body while respecting all physical constraints of the robots' actuators. To achieve highly accurate jumping, a full-body dynamics model is usually utilized. For quadrupedal animals, high jumping is normally restricted to a sagittal plane. Therefore, this paper will also focus on 2D motion of the robot\NA{This sentence can be moved before the subsubsection as part of the brief overview.}. The robot model thus can be considered as a rigid-body system consisting of $5$ links in the 2D plane\NA{Explain that the 5 links are the 4 legs and the body}. A jumping task is modeled as a sequence of three contact phases: double contact (all legs have contact), single contact (rear legs have contact), and flight (no legs have contact). The equations of motion can be formulated as follows \cite{QuannICRA19}:  
% % %
% % \begin{equation}\label{eq:full_dynamics_2D}
% % \begin{bmatrix}\bm{H} & -(\bm{J}_c^f)^\top \\ -(\bm{J}_c^f)^\top & \mathbf{0} \end{bmatrix} \begin{bmatrix}
% % \bm{\ddot{q}} \\ \bm{f}
% % \end{bmatrix}= \begin{bmatrix}-\bm{C}\bm{\dot q}-\bm{G} + \bm{S}\bm{\tau}+\bm{S}_{f}\bm{\tau}_{f} \\ \bm{\dot J}_{c}^f\bm{\dot q}\end{bmatrix}
% % \end{equation}
% % %
% % % \begin{subequations}\label{eq:gait_1}
% % %     \begin{align}
% % %     \bm{M} \bm{\ddot{q}}+\bm{C}\bm{\dot q}+\bm{g} &= \bm{J}_c^T \bm{f}_c +\bm{S}\bm{\tau}+\bm{S}_{f}\bm{\tau}_{f} \\
% % %     \bm{J}_c^T \bm{\ddot{q}} + \bm{\dot J}_{c}(\bfq)\bm{\dot q} &=0
% % %     \end{align}
% % % \end{subequations}
% % %
% % where $\bfq:=\left[\bfq_b;~\bfq_{j}\right]$ is a vector of generalized coordinates, in which $\bfq_b = [ x,z,q_{pitch}]$ is the body coordinates including CoM\NA{This abbreviation has not been introduced} position and body's pitch angles respectively, and $\bfq_j$\NA{Specify the dimension} is a vector of joint angles.\NA{The sentence should not end here} $\bm{H}$ is the mass matrix, $\bm{C}$ is represented for Coriolis  and centrifugal terms, $\bfA_g$\NA{This is denoted by $\bm{g}$ above} denotes gravity vector. $\bm{J}_c^f(\bfq)$\NA{It may be good to make the dependence on $\bfq$ explicit in the model above} is the spatial Jacobian respectively with the generalized coordinate $\bfq$ and expressed at the contact foot. $\bm{S}$ and $\bm{S}_{fric}$ \NA{This is denoted by $\bm{S}_{f}$ above} are distribution matrices of actuator torques $\bm{\tau}$ and the joint friction torques $\bm{\tau}_{fric}$\NA{This is denoted by $\bm{\tau}_{f}$ above}, $\bm{f}$ is the spatial contact force at the feet. The dimensions of $\bm{J}_c$ and $\bm{f}$ depend on the phase of the gait and the number of legs in contact with the ground.
% \subsection{Single rigid body dynamics}
%  This simplification considers the whole trunk and legs as a unified single rigid body subject to forces at the contact patches (e.g. \cite{park2017high,YanranDingTRO,ParkRSS15}). 
%  % which finds highly efficient to real-time control. 
%  % Although ignoring leg dynamics is a major simplification, the controller
%  % is still able to stabilize a high-DoF system and is robust
%  % to these multi-body effects.
%  % Consider a robot modeled as a single rigid body with position $\bfp \in \bbR^2$, orientation $\theta \in \mathbb{R}$. 
%  We denote the robot's generalized coordinates as $\boldsymbol{\mathfrak{q}} = \begin{bmatrix} \bfp^{\top} & \theta \end{bmatrix}^{\top} \in \mathbb{R}^{3}$, where $\bfp \in \bbR^2$ is the position of center of mass (CoM) of the body, and $\theta \in \mathbb{R}$ is the body orientation. We define the generalized velocity of the robot by $\bfzeta = \begin{bmatrix} \bfv^{\top} & \omega \end{bmatrix}^{\top} \in \mathbb{R}^3$, where $\bfv \in \mathbb{R}^2$ is the linear velocity and $\omega \in \mathbb{R}$ is the angular velocity. Both $\mathfrak{q}$ and $\bfzeta$ are expressed in the world frame. Under the control input $\bfu = \begin{bmatrix} \bff_1^{\top} & \bff_2^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{n_u}$,  robot state $\bfx = \begin{bmatrix} \boldsymbol{\mathfrak{q}}^{\top} & \bfzeta^{\top} & g\end{bmatrix}^{\top} \in \mathbb{R}^{n_x}$ is evolved by the following continuous-time state-space model:
% %
% \begin{equation} \label{eq:nominal_continuous_dynamics}
% 	\dot{\bfx}(t) = \bfA_{ct} \bfx(t) + \bfB_{ct}(\bfr) \bfu(t),
% \end{equation}
% %
% with 
% \begin{equation}
% \begin{aligned}
%     \bfA_{ct} &= 
%     \begin{bmatrix}
%         \bf0_{3} & \bfI_{3} & \bf0 \\ 
%         \bf0_{3} & \bf0_{3} & -\bfe_{3} \\ 
%         \bf0^{\top} & \bf0^{\top} & 0
%     \end{bmatrix}, 
%     \bfB_{ct}(\bfr) = 
%     \begin{bmatrix}
%         \bf0_{3\times2} & \bf0_{3\times2} \\ 
%         \bfI_{2} / m & \bfI_{2} / m \\ 
%         [\bfr_1]_{\times}/J & [\bfr_2]_{\times}/J \\ 
%         \bf0^{\top} & \bf0^{\top}
%     \end{bmatrix},
% \end{aligned}
% \end{equation}
% where $\bfA_{ct}\in \mathbb{R}^{n_x\times n_x}$, $\bfB_{ct} \in \mathbb{R}^{n_x\times n_u}$, $\bfe_3= \begin{bmatrix} 0 & -1 & 0
% \end{bmatrix}^\top$, $m$ is the body mass, $J$ is the moment inertia of the body, $\bfr_i$ is the foot $i = \{1, 2\}$ position relative to the CoM in the world frame and $[\bfr_i]_{\times}^{\top} = \begin{bmatrix} r_{iz} & -r_{ix} \end{bmatrix}^{\top} \in \mathbb{R}^2$. These relative position vectors $\bfr_i$ are combined as $\bfr$ for the sake of notation. The gravity term $g$ is added to the robot state to obtain the convenient state-space form (\ref{eq:nominal_continuous_dynamics}).
% The discrete dynamics is then propagated using the Euler forward scheme as
% \begin{equation} \label{eq:nominal_dynamics}
% 	\bfx_{k+1} = \bfA_k \bfx_{k} + \bfB_k(\bfr_k) \bfu_k,
% \end{equation}
% where $\bfA_k = \bfI_{n_x} + \bfA_{ct} \Delta t$, $\bfB_k= \bfB_{ct} \Delta t$, $\Delta t$ is sampling step.
% \begin{remark}
%     The full-body dynamic model \eqref{eq:full_dynamics_2D} is complex and, normally, not favorable for real-time control\NA{Explain more precisely what makes the model complex and unfavorable for real-time control. Is it the fact that the model is nonlinear due to the term $\bm{J}_c^f(\bfq)$ and its time derivative? Is it the fact that linearizaiton as part of MPC is not accurate?}. In addition, with even higher accuracy, this model still ignores the uncertainties and unknown dynamics. Unlike normal operations, dynamic jumping poses a unique challenge as it rapidly reaches hardware limits. In these extreme conditions, accurately modeling the hardware is challenging. On the other hand, the SRB model (E.q. \ref{eq:simplified dynamics}) is favorable for real-time control. However, this model neglects the leg dynamics, which are important to achieve accurate jumping. 
% \end{remark}
% \subsubsection{Single Rigid Body Dynamics}Another widely used model of robot dynamics is a single rigid body \cite{park2017high,YanranDingTRO,ParkRSS15}. This model treats the whole robot as a single rigid body, neglecting the leg dynamics  which finds highly efficient to real-time control.\NA{An equation should be part of a sentence.}\NA{We had denoted gravity as $\bm{g}$ before.}\NA{Why is the second equation below using $\frac{\mathrm{d}}{\mathrm{d} t}(I_b {\bm{\omega}})$ on the right-hand side? Is $I_b$ a function of the state?}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{subequations}\label{eq:simplified dynamics}
%     \begin{align} \label{eq:simplified dynamics}
%     \ddot{\bm{p}} =\frac{\sum_{i=1}^{2}\bm{f}_{i}}{m}-\bfA_g, ~~~ \frac{\mathrm{d}}{\mathrm{d} t}(I_b {\bm{\omega}}) =\sum_{i=1}^{2} \mathbf{r}_{i} \times \bm{f}_{i},
%     \end{align}
% % \end{subequations}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% where $\bm{p} =[p_x; p_z] \in \mathbb{R}^2$ is the CoM position in the world frame; $\bfr_i=[r_{ix};r_{iz}]$ and $\bm{f}_i=[f_{ix};f_{iz}]$ denotes the position of contact point relatively to CoM, and contact force at foot $i^{th}$ respectively in the world frame; $\bm{\omega}=\dot{\theta} \vec{k}$ is angular velocity of the body; $\theta$ is a pitch angle. \NA{What is $\vec{k}$? What is $I_b$?}


% We define $\bfx^s=[\bm{p};\theta;\dot{\bm{p}};\dot{\theta},a_g]$\NA{Why is gravity part of the state?} as the state of a simplified dynamics, $a_g$ is gravity, $\bfu^s=[\bm{f}_1^\top; \bm{f}_2^\top]$\NA{The notation here is weird. Why do we have ";" to separate the variables and why do we have transpose on the entries but not on the overall vector. Are we trying to obtain a column vector?}. Then, the simplified dynamics in continuous time can be rewritten as:\NA{Should we have $\bfB_{ct}$ instead of $\bfB_{ct}$?}
% \begin{equation}\label{eq:simplified_dynamics}
% \dot{\bfx}^s=\bfA_{ct}\bfx^s+\bfB_{ct}(\bfr) \bfu^s,
% \end{equation}
% where
% \\
% $\bfA_{ct}= \begin{bmatrix}
% \bm{0} & \bfI & \bm{0}\\
% \bm{0} & \bm{0} & \bm{e}_g\\
% \bm{0} & \bm{0} & \bm{0}
% \end{bmatrix}$, $\bfB_{ct}(\bfr)= \begin{bmatrix}
% \bm{0} & \bm{0}\\
% \bfI/m & \bfI/m \\
%  [\bfr_1]_{\times}/I_b &  [\bfr_2]_{\times}/I_b \\
% \bm{0} & \bm{0}
% \end{bmatrix}$, $\bm{e}_g= \begin{bmatrix} 0 & -1 & 0
% \end{bmatrix}^\top$ \\
% % $\bm{\sigma}_i= I_b^{-1} \begin{bmatrix} -r_{iz} & r_{ix}
% In discrete time, 
% \begin{equation}\label{eq:dis_simplified_dynamics}
% \bfx_{k+1}^s=\bfA\bfx_k^s+\bfB(\bfr_k) \bfu_k^s,
% \end{equation}

% \begin{remark}
%     The full-body dynamic model \eqref{eq:full_dynamics_2D} is complex and, normally, not favorable for real-time control\NA{Explain more precisely what makes the model complex and unfavorable for real-time control. Is it the fact that the model is nonlinear due to the term $\bm{J}_c^f(\bfq)$ and its time derivative? Is it the fact that linearizaiton as part of MPC is not accurate?}. In addition, with even higher accuracy, this model still ignores the uncertainties and unknown dynamics. Unlike normal operations, dynamic jumping poses a unique challenge as it rapidly reaches hardware limits. In these extreme conditions, accurately modeling the hardware is challenging. On the other hand, the SRB model (E.q. \ref{eq:simplified dynamics}) is favorable for real-time control. However, this model neglects the leg dynamics, which are important to achieve accurate jumping. 
% \end{remark}

% This motivates us to use propose Neural Network:
% \begin{itemize}
%     \item learn residual dynamics to compensate for model uncertainties and unknown dynamics.
%     \item choose to learn residual dynamics for single rigid body to enable real-time control with MPC
% \end{itemize}

% \begin{figure}[!tpb]
%       \centering
%       % \vspace{.06in}
%       % \vspace{-1em}
%       \includegraphics[width=2.7in,trim={0cm 0cm 0cm 0.5cm},clip]{figures/jumping_phases.png} \\
%       \vspace{-0.6em}
%       \caption{A generalized jumping motion in 2D. }
%       \label{fig:jumping_phases}
%       \vspace{-1.5em}
% \end{figure}
% \begin{figure}[!tpb]
%       \centering
%       % \vspace{.06in}
%       % \vspace{-1em}
%       \includegraphics[width=2in,trim={0cm 1.7cm 0cm 0cm},clip]{figures/2D_rigid.png} \\
%       \vspace{-0.em}
%       \caption{A rigid body in 2D. }
%       \label{fig:2D_rigid_body}
%       \vspace{-0.5em}
% \end{figure}
% \subsection{3D jumping}

% The single rigid body dynamics in SE(3) has a form
% \begin{subequations}\label{eq:SRB_dynamics}
%     \begin{align}
%         \ddot{\bm{p}}&=\sum_{s=1}^{n_s} \bm{f}^{s}/m-\bm{g}, \label{eq:SRB_dynamics1}\\
%         \bm{I_b} \dot{\bm{\Omega}} + \bm{\Omega} \times \bm{I_b} \bm{\Omega} &= \bfr^{-1} \sum_{s=1}^{n_s} \bm{f}^s \times (\bm{p} - \bm{p}_f^s) ,\label{eq:SRB_dynamics2}\\
%         \dot{\bfr} &= \bfr\widehat{\mathbf{\Omega}}\label{eq:SRB_dynamics3}
%     \end{align}
% \end{subequations}

% where $n_s$ is number of feet, m is the robot's mass, $\bm{\Omega} \in \mathbb{R}^3$ is angular velocity expressed in the body frame, $\bfr$ is rotation matrix of the body frame, $\bm{g}$ is the gravity acceleration; $\bm{p}, \dot{\bm{p}}, \ddot{\bm{p}} \in \mathbb{R}^3$ is the CoM position, velocity, acceleration of the body in the world frame; $\bm{f}^s \in \mathbb{R}^3$ is GRF on foot $s^{th}$;   $\bm{p}_f^s \in \mathbb{R}^3$ is $s^{th}$ foot position in the world frame. The hat map $(\hat{.}):\mathbb{R}^3  \rightarrow so(3) $ converts any vector in $\mathbb{R}^3$ to the space of skew-symmetric matrices. For the sake of notation, we define the robot's state as
% $\bfx:=\left[\bm{p}; \dot{\bm{p}}; \bm{\Omega}; \dot{\bm{\Omega}}; \bfr\right]$. 

% \section{Problem Statement}
% \label{sec:problem_statement}



% Further, we aim to design a model predictive controller that attempts to track a desired state trajectory $\bfx^*(t)$, $t \geq t_0$, for any learned realization $\tilde{\bff}_{\bftheta}$ of the robot dynamics and unknown disturbance and uncertainties\NA{We keep mentioning disturbance and uncertainty but I am not sure what this is referring to. Where in the models do we have uncertainty and disturbances?}.

% \begin{problem}
% \label{problem:setpoint_reg}
% Given an initial condition $\bfx_0$ at time $t_0$, desired state trajectory $\bfx^*(t)$, $t \geq t_0$, and learned dynamics $\tilde{\bff}_{\bftheta}$, design a model predictive control law $\bfu = \bfpi(\bfx, \bftheta, \bfx^*(t))$ for contact phases to track the whole jumping reference that involves long acrobatic period.
% \end{problem}

% In our setting, the robot kinematics need to evolve over the $SE(3)$ manifold and the dynamics $\bff(\bfx, \bfu)$ respect the law of energy conservation, when there is no control input, $\bfu = \bf0$. We embed these constraints in the structure of the parametric function $\tilde{\bff}_{\bftheta}$. We review the $SE(3)$ kinematics and Hamiltonian dynamics equations next.


% \section{Problem Statement} \label{sec:statement}
% In the following, we present the learning model with adaptive frequency and model predictive control for the learned dynamics.



% \subsection{Residual Dynamics}

% - \note{use u as control input --> uncertainties in contact, motor dynamics, hardware model --> }
% - \note{problem statement}


% \note{We consider \ref{eq:nominal_continuous_dynamics} as nominal model , then develop residual dynamics}


% Our main objective is to formulate a real-time executable MPC scheme for controlling
% quadruped robotics to perform a variety of dynamic motions. To meet the real-time require-
% ment, the optimization problem posed by the MPC has to be solved robustly at a high rate
% on the mobile embedded computer, which has limited computational resources. Hence, a
% simplified model is adopted to reduce the dimensionality of the optimization problem. Since
% the mass of all legs combined is less than 10% of the total body mass, a single rigid body
% model serves as a reasonable approximation.
\begin{figure*}
      \centering
      \includegraphics[trim = 0mm 11mm 0mm 0mm, clip, width=\linewidth]{figures/framework-v6.pdf}
      \caption{\textbf{System Architecture}. The learning procedure and MPC execution are paired with the same \rebut{integration timesteps} $\lbrace \Delta t_{\calC}, \Delta t_{\calF} \rbrace$, prediction horizon $K$, and predefined contact schedule ($cs$). The MPC and low-level joint PD controllers are updated at $40Hz$ and $1kHz$, respectively. 
      % The MPC aim to track the jumping reference $\bfx^*$ from full-body trajectory optimization \cite{QuannICRA19}.      
      % The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $
      }
      \label{fig:overview_framework}
      \vspace{-1.7em}
\end{figure*}

\section{Problem Statement} \label{sec:problem_statement}

% \NA{I think we should have a problem statement section that explains what we are trying to do before we have an overview of how we are doing it.}

Consider a legged robot modelled by state $\bfx_k$, consisting of the pose and velocity of the body's center of mass (CoM), foot positions $\bfr_k$ relative to the body's CoM, and ground force control input $\bfu_k$ at the legs, sampled at time $t_k$. We  augment the nominal SRBD model (e.g., \cite{GabrielICRA2021, park2017high,YanranDingTRO}) with a learned residual term to account for leg dynamics, model mismatch with the real robot hardware, as well as capture complex dynamic effects in contact and hardware:
%
\rebut{
\begin{equation}\label{eq:discrete_learned_model}
    \bfx_{k+1} = \bff\left(\bfx_k, \bfu_k, \bfr_{k}, \Delta t_k \right) + \delta\bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k}\right)\Delta t_k ,
\end{equation}
}
%
where $\bff$ represents the nominal SRBD model, $\delta\bff_{\bftheta}$ with parameters $\bftheta$ approximates the residual dynamics, and $\Delta t_k$ is the sampling interval. Our first objective is to learn the residual dynamics $\bff_{\bftheta}$ using a dataset of jumping trajectories.


%on the dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consisting of $D$ state sequences $\bfx^{(i)}_{0:K}$, obtained by applying control inputs $\bfu^{(i)}_{0:K}$ to the system, and $\bfr^{(i)}_{0:K}$ represents the foot positions.
% $\bff_{\bftheta}$ with state $\bfx_{0:K-1}^{(i)}$ and control $\bfu^{(i)}_{0:K-1}$ 
% \tilde{\bfx}^{(i)}_k = \tilde{\bfx}^{(i)}(t_k), \quad 
%  of $K+1$ collocation points}
% indexed by $t_{0:K}$

\begin{problem} \label{problem:dynamics_learning}
Given a set $\calD \!=\! \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ of $D$ sequences of states, foot positions, and control inputs,
% \NA{Do we need the time indices $t_{0:K}$?},
find the parameters $\bftheta$ of the residual dynamics $\delta \bff_{\bftheta}$ in \eqref{eq:discrete_learned_model} by rolling out the dynamics model and minimizing the discrepancy between the predicted state sequence $\tilde{\bfx}^{(i)}_{1:K}$ and the true state sequence $\bfx^{(i)}_{1:K}$ in $\calD$:
%
\begin{align}
\min_{\bftheta} \;&\sum_{i = 1}^D \sum_{k = 1}^K \mathcal{L} (\bfx^{(i)}_k,\tilde{\bfx}^{(i)}_k) + \calL_{\text{reg}}(\bftheta) \notag\\
\text{s.t.} \;\; & \tilde{\bfx}^{(i)}_{k+1} = \bff \left(\tilde{\bfx}^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k, \Delta t_k\right)\notag\\ 
&\qquad \qquad\qquad + \rebut{\delta \bff_{\bftheta}\left(\tilde{\bfx}^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k,\right) \Delta t_k } , \notag\\
& \tilde{\bfx}^{(i)}_0 = \bfx_{0}^{(i)}, \quad \rebut{\forall i=1,...,D,}  \label{eq:problem_formulation_unknown_env_equation}
\end{align}
%
where $\mathcal{L}$ is an error function in the state space, and $\calL_{\text{reg}}(\bftheta)$ is a regularization term to avoid overfitting. Note that it is not necessary for $\Delta t_k = t_{k+1}-t_{k}$ to be fixed.
\end{problem}

After learning to improve the accuracy of model prediction, our second objective is to use the learned model \eqref{eq:discrete_learned_model} for MPC to track a desired state trajectory $\bfx_{0:K}^*$.

\begin{problem} \label{problem:mpc_learn}
Given the dynamics model \eqref{eq:discrete_learned_model}, \rebut{a current robot state $\bfx_0$} and foot positions $\bfr_0$, a desired trajectory of states $\bfx^*_{0:K}$, foot positions $\bfr^*_{0:K}$, and control $\bfu^*_{0:K}$,
% \NA{Do we need the time indices $t_{0:K}$?},
design a control law $\bfu_0 = \bfpi(\bfx_0, \bfr_0, \bfx^*_{0:K}, \bfr^*_{0:K},\bfu^*_{0:K}; \bftheta)$ to achieve accurate and robust tracking of the desired state trajectory via shifting-horizon optimization:
%
\begin{align}
\min_{\bfu_{0:K-1}} \;& \sum_{k = 1}^K \| \bfx_k-\bfx_{k}^* \|_{\bfQ_k} + \| \bfu_{k-1}-\bfu_{k-1}^* \|_{\bfR_k} \notag\\
\text{s.t.} \;\; & \rebut{\bfx_{k+1} = \bff\left(\bfx_k, \bfu_k, \bfr_{k}, \Delta t_k \right) + \delta \bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k}\right) \Delta t_k }, \notag\\
& \bfu_k \in \calU_k, \quad \forall k=0,...,K-1, \label{eq:mpc_formulation}
\end{align}
%
where $\bfQ_k$ and $\bfR_k$ are positive definite weight matrices,
% weight matrices, i.e., diagonal matrices with positive diagonal entries,
% \NA{Do we need $\bfP_k$ to be positive semidefinite and $\bfQ_k$ to be positive definite? The usual notation is to use $\bfQ_k$ for $\bfx_k$ and $\bfR_k$ for $\bfu_k$. We should define what we mean by $\|\cdot\|_{\bfQ}$. Do we need to select $\bfu_K$? Seems that it will always be equal to $\bfu_K^*$ in the above optimization.}, 
and $\calU_{0:K-1}$ represents an input constraint set. 
% \CN{I just corrected the equation (3)}
\end{problem}

% Achieving accurate target jumping with MPC requires not only an accurate model but also consideration of the desired trajectory $\bfx_{0:K}^*,\bfr_{0:K}^*,\bfu_{0:K}^*$, including the final state upon landing. 
Achieving accurate target jumping with MPC requires not only an accurate model but also the coverage of the final state upon landing, which represents the accuracy of the jumping target. Using a fixed-frequency has shown to be efficient for locomotion tasks with limited aerial phases; however, this can face two challenges in long-flight maneuvers. On the one hand, using a fine time-step dirscretization enhances the model prediction accuracy but requires a large number of steps to capture the entire flight phase, thereby increasing the optimization size and computational cost. On the other hand, using a coarse time-step discretization allows capturing the entire flight phase efficiently but can sacrifice model prediction accuracy. For jumping tasks, different phases may require different model resolutions, e.g., fine time resolution during the contact phase but coarser time resolution during the flight phase as the model complexity is reduced due to unavailable force control and contact. Therefore, we propose to learn a model for dynamic maneuvers (Problem \ref{problem:dynamics_learning}) with an \rebut{variable-frequency scheme}\redst{adaptive-frequency scheme} that uses a coarse time discretization in the flight phase and a fine time discretization in the contact phase. Importantly, this \rebut{variable-frequency}\redst{adaptive-frequency} scheme is also synchronized with the MPC control of the learned model (Problem \ref{problem:mpc_learn}) \rebut{by utilizing the same time steps for both fitting the learned model and performing the MPC optimization. This synchronization ensures that the same discretization errors are leveraged when using the model for MPC predictions}. Thus, in our formulation $t_{0:K}$ does not have equal time steps and is a mixture of fine and coarse discretization capturing the contact and flight phases\redst{of a jumping motion}.
\rebut{Note that we use a constant time step $\Delta t_k$ during the different jumping phases. It is possible to use $\Delta t_k$ as input to the residual model neural networks. However, we need to collect a substantial amount of data for a wide range of $\Delta t_k$ to avoid overfitting, which would also increase the size of the neural network and computational cost.
% and potentially reduces the accuracy.
% However, this would require additional data for each $\Delta t_k$ to avoid overfitting.
}

% , i.e., for each $\Delta t_k$, we would need to collect a new state and control sequence


% Given the dynamics model in \eqref{eq:discrete_learned_model}, design a control law \rep{$\bfu_k = \bfpi(\bfx_k, \bfr_k, \bftheta, \bfx^*_{0:K}, \bfr^*_{0:K},\bfu^*_{0:K})$} 
% % \NA{Should this depend on $\bfr_k$ as well?}\NA{Should the policy depend on a reference control input $\bfu^*_{0:K}$ as well? It seems that trajectory optimization provides this as well.} 
% to achieve accurate and robust tracking of a desired state trajectory $\bfx_{0:K}^*$.
% %target jumping, which involves flight phase (i.e. extreme underactuated systems).
% % that involves long acrobatic period.


% \rep{Explain Adaptive frequency here}
% Jumping and Flight phase --> use adaptive frequency -->  Define of time step $t_{0:K}$, sample with different freq
% The MPC design tailor for jumping motions consisting of two distinguish phases: contact and flight phase. 



% \CN{I added this paragraph to explain the adaptive frequency; it seems a little bit long and replicates some information from the introduction. \textcolor{red}{ Please let me know if you have any suggestions}} 

%the coverage of the final state upon landing, which represents the accuracy of the jumping target. 

%for discretization normally enhances the dynamic representation, but it also requires a  large number of prediction steps to leverage the entire flight maneuvers, thereby increasing the optimization size and computational cost.

%On the other hand, adopting relaxed time steps leverage the whole flight prediction with computational efficiency but can sacrifice model accuracy\NA{I am not sure what this sentence means}.
% Using fine time-step discretization normally enhances the prediction accuracy, but it also requires a large number of prediction steps to leverage the entire light phase. This likely increases the optimization size and computational cost that can ruin the real-time performance. 





% The adaptive-frequency protocol relaxes the time steps for the discretization of flight-phase dynamics while still keeping a fine sampling time for robot dynamics in the contact phase. 

%In our formulation, $t_{0:K}$ does not necessarily have equal time intervals. It can be a mixture of fine and relaxed time steps if the horizon involves different phases. 
% Therefore, $t_{0:K}$ do not necessarily have the same length of time due to the adaptive-frequency sampling policy.


% For example, the time sequence is not sampled
% \CN{I rewrite this section to describe system overview}

\section{System Overview}
\label{sec:sys_overview}

Fig. \ref{fig:overview_framework} presents an overview of our system architecture. Our approach consists of two stages: \rebut{variable-frequency}\redst{adaptive-frequency} model learning (Sec. \ref{sec:adaptive-frequency-learning}) and \rebut{variable-frequency}\redst{adaptive-frequency} MPC (Sec. \ref{sec:adaptive-MPC}), which solve Problem~\ref{problem:dynamics_learning} and Problem~\ref{problem:mpc_learn}, respectively.
% Our approach for quadruped jumping consists of three stages
% \NA{We should give the three stages good names and use them consistently in the figures and section captions.}: data collection, adaptive-frequency model learning (Problem~\ref{problem:dynamics_learning}), and adaptive-frequency MPC (Problem~\ref{problem:mpc_learn})
% \NA{The caption of Fig.~\ref{fig:overview_framework} is not very well organized. The second sentence is already discussing paring adaptive frequencies but we have not even explained what adaptive frequency means yet. We should first provide an overview of the 3 stages: data collection, model learning, and MPC before delving into the details.}. 
% In the data collection stage (Sec. \ref{subsec:data_gen})\NA{Should we discuss only 2 stages and merge the data collection with the model learning stage? This will be better aligned both with the two problems above and with the two sections (3 and 4) that follow.}, we combine nominal MPC using a conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD\NA{Has this acronym been defined?} controller to generate diverse motions with different jumping references and disturbance. 

We synchronize the \rebut{variable-frequency scheme}\redst{adaptive-frequency scheme}  for both model learning and MPC execution with the same \textit{(1)} \rebut{variable prediction timesteps}\redst{adaptive sampling time} $\Delta t_{\calC}$ and $\Delta t_{\calF}$ for contact and flight phase, respectively, \textit{(2)} the same horizon length $K$ for all data collection, training, and MPC, and \textit{(3)} the same contact schedule.
% \NA{What is a contact schedule?}. 
Full-body trajectory optimization (TO) \cite{QuannICRA19} is utilized to generate jumping references for various targets, including body states $\bfx^*$, joint states $\lbrace \bfq_{\mathbf{J}}^*, \dot{\bfq}_{\mathbf{J}}^* \rbrace$, ground contact force $\bfu^*$, and foot positions $\bfr^*$. 
For data collection, we combine a baseline MPC using a nominal SRBD model and joint PD 
% \TD{Have we defined PD before using this abbreviation?}
controller, generating diverse motions under disturbances. For training, we design a neural network to learn the discretized residual model $\delta \bff_{\bftheta}$ with \rebut{variable}\redst{adaptive} sampling time via supervised learning. For control, we design an \rebut{variable-frequency}\redst{adaptive-frequency} MPC using the learned dynamics to track a desired reference trajectory obtained from full-body TO. 
% It works together with a high-frequency joint tracking PD controller to execute jumping motions. 
% \NA{I don't think this sentence is adding much.}. 
The feedback states from the robot include global body's CoM $\bfx$, and joint states $\bfq_{\mathbf{J}}, \dot{\bfq}_{\mathbf{J}} \in \mathbb{R}^4 $, and foot positions $\bfr \in \mathbb{R}^4$.
% \NA{The sentence is out of place here. This information should be presented earlier.}. 



% These models aim
% to predict robot states for the upcoming $K$ horizons as MPC
% schedule, which can cover contact transitions and the entire
% flight phase
% In contrast with existing methods, we use adaptive sampling time in the learning process to cover both the contact transitions and the entire flight phase within the MPC planning horizon\NA{Currently we are highlighting the adaptive frequency twice. Once during model-learning and once during MPC. It may be confusing. Should we highlight it once, e.g., just for the MPC to keep it clear in the reader's mind what the key ideas in the three stages are?}.


% Using adaptive sampling time enables MPC to cover the entire flight phase and the transition between jumping phases within planning horizons}
% \NA{Currently we are highlighting the adaptive frequency twice. Once during model-learning and once during MPC. It may be confusing. Should we highlight it once, e.g., just for the MPC to keep it clear in the reader's mind what the key ideas in the three stages are?}.
% It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. 
% The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $\NA{The information in this and the previous sentence should be moved later. They read like low-level details rather than the key novelty of the adaptive MPC}
% \todo{Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness. We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. 
% \NA{This information needs more context. What does adaptive-frequency mean? Why is it useful? Are we the first to propose it?}
% \NA{Are we the first to propose it?}

%To tackle these problems, we propose the following system architecture as depicted in Fig. \ref{fig:overview_framework}, which includes the baseline MPC with nominal SRBD for collecting data for training, the Adaptive-frequency learning (Sec. \ref{sec:adaptive_learn_model}, \ref{sec:training}), and the Adaptive-frequency MPC for the learned dynamics (Sec. \ref{sec:adaptive-MPC}). 


%Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness. We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. For data collection, we combine nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD controller, generating diverse motions with different jumping references and disturbance, as presented in Sec. \ref{subsec:data_gen}. For adaptive-frequency learning, we design neural networks to learn the discretized models for contact and flight phases with adaptive sampling time via the supervised learning, aiming to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover contact transitions and the entire flight phase. Finally, adaptive-frequency MPC is designed to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 


% % The proposed learning-based MPC framework comprises of
% % two primary parts, the Adaptive-frequency model training and the Adaptive-frequency MPC execution for the learned dynamics, which are presented in Sec. \ref{sec:training} and \ref{sec:adaptive-MPC} respectively.

% % Conventional MPC usually either adopt fixed frequency in state prediction or has not leverage of legged dynamics in dynamic model, which may limits accurate trajectory prediction for whole long flight phase. 
% Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness.
% % Unlike conventional MPC, we design a learning residual model and adaptive-frequency to leverage the effect of complex leg dynamics, unknown dynamics in contact and hardware, as well as compensate for model mismatch, which will then followed by adaptive prediction frequency design to leverage the whole flight phase inside MPC predictions. 
% % Both factors are combined as a unified model, allowing us to enhance the accuracy of trajectory prediction for long flight phase within a limited MPC horizon. 
% We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. 
% % We denote the synchronized sampling time $\Delta t_{\calC}$ and $\Delta t_{\calF}$ for contact and flight phase, $\Delta t_{\calF} > \Delta t_{\calC}$, respectively. 
% % This synchronization aims to avoid conflict in discretization. 
% % \textcolor{red}{We use the same contact schedule}
% For data collection, we combine nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD controller, generating diverse motions with different jumping references and disturbance, as presented in Sec. \ref{subsec:data_gen}. 
% % For data collection for jumping, we combine both nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) for high-level body trajectory tracking and joint PD controller for low-level joint profile tracking, generating a diverse motions with different jumping references and disturbance. 
% % presented in Sec. \ref{subsec:data_gen}. 
% For adaptive-frequency learning, we design neural networks to learn the discretized models for contact and flight phases with adaptive sampling time via the supervised learning, aiming to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover contact transitions and the entire flight phase.
% % For adaptive-frequency learning, we design neural networks with Pytorch to learn the discretized models for contact and flight phases with adaptive sampling time. The training is based on supervised learning and we aim to learn the model to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover the contact transition and the entire flight phase.
% Finally, adaptive-frequency MPC is designed to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 





%for contact and flight phase $\calD$, the nominal dynamics $\bff$, and  function $\bff_{\bftheta}$ representing residual dynamics,
% $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$, 
% a function $\bff$ representing nominal SRBD (e.g. \cite{GabrielICRA2021, park2017high,YanranDingTRO}), and a function $\bff_{\bftheta}$ representing residual dynamics, 
%we aim to optimize the parameters $\bftheta$ 



%system and unknown dynamics in the contact and hardware, which yields the discrete-time model:
% Importantly, we also aim to design model predictive control using the learned model to achieve accurate jumping under uncertainty.
% We utilize the simplified dynamics to enable real-time control but propose to learn a residual term to account for legged dynamics and other model uncertainties in contact dynamics or hardware. 
% The proposed discrete-time model with residual dynamics can be characterized as follows

% where the nominal and residual dynamics are defined as
% \begin{equation}\label{eq:discrete_learned_model}
% \begin{aligned}
%     \bff\left(\bfx_k, \bfu_k, \bfr_{k} \right) = & \bfA_k \bfx_{k} + \bfB_k(\bfr_k) \bfu_k,\\ 
%     \bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k} \right) = & 
%  \bfh_{\bftheta}(\bfx_k, \bfr_{k})  + \bfG_{\bftheta}(\bfx_k, \bfr_{k}) \bfu_k.
% \end{aligned}
% \end{equation}


% Consider a robot with state $\bfx$ consisting of its position $\bfp \in \mathbb{R}^3$, orientation $\bfR\in SO(3)$, body-frame linear velocity $\bfv \in \bbR^3$, and body-frame angular velocity $\bfomega\in \mathbb{R}^3$. 

% Let $\bfx_{k+1} = \bff(\bfx_{k}, \bfu_k)$\NA{This is a sudden jump since in the previous section we specified continuous-time models}\NA{I see that there is a cleaner formulation in green in the appendix.} characterize the robot dynamics with control input $\bfu$. We assume that the function $\bff$ represented the unknown robot dynamics in discrete time, for which we aim to approximate it using a dataset $\mathcal{D}$ of state and control trajectories\NA{Use present tense. The second part of this sentence is awkward. Rewrite.}. Specifically, let $\calD = \{t_{0:N}^{(i)}, \bfx^{(i)}_{0:N}, \bfr^{(i)}_{0:N}, \bfu^{(i)}_{0:N}\}_{i=1}^D$ consist of $D$ state sequences $\bfx^{(i)}_{0:N}$, obtained by applying appropriate\NA{What does appropriate mean?} control inputs $\bfu^{(i)}_{0:N}$ to the system, and $\bfr^{(i)}_{0:N}$ represents the foot position.
% with initial condition $\bfx^{(i)}_0$ at time $t_0^{(i)}$ and sampling its state $\bfx^{(i)}(t_n^{(i)}) =: \bfx^{(i)}_n$ at times $t_0^{(i)} < t_1^{(i)} < \ldots < t_N^{(i)}$. 
% We aim to find a function $\tilde{\bff}_{\bfbeta}$ with parameters $\bfbeta$ that approximates the residual\NA{Why residual? This idea has not been introduced.} dynamics $\bff$ on the dataset $\mathcal{D}$. To optimize the parameters $\bfbeta$, we roll out the approximate dynamics $\tilde{\bff}_{\bfbeta}$ with initial state $\bfx_0^{(i)}$ and control $\bfu^{(i)}_{0:N}$ and minimize the discrepancy between the computed state sequence $\tilde{\bfx}^{(i)}_{1:N}$ and the true state sequence $\bfx^{(i)}_{1:N}$ in $\calD$. The dynamics learning problem is summarized below.
%where a function $\bff$ representing nominal SRBD, and $\bff_{\bftheta}$ with parameters $\bftheta$ approximates the residual dynamics on the dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consisting of $D$ state sequences $\bfx^{(i)}_{0:K}$, obtained by applying control inputs $\bfu^{(i)}_{0:K}$ to the system, and $\bfr^{(i)}_{0:K}$ represents the foot positions.
% To optimize the parameters $\bftheta$, we roll out the approximate dynamics $\bff_{\bftheta}$ with initial state $\bfx_0^{(i)}$ and control $\bfu^{(i)}_{0:K}$ and minimize the discrepancy between the computed state sequence $\tilde{\bfx}^{(i)}_{1:K}$ and the true state sequence $\bfx^{(i)}_{1:K}$ in $\calD$. 
% The dynamics learning problem is stated below.

% \begin{problem}
% \label{problem:dynamics_learning}
% Given a dataset for contact and flight phase $\calD$, the nominal dynamics $\bff$, and  function $\bff_{\bftheta}$ representing residual dynamics,
% % $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$, 
% % a function $\bff$ representing nominal SRBD (e.g. \cite{GabrielICRA2021, park2017high,YanranDingTRO}), and a function $\bff_{\bftheta}$ representing residual dynamics, 
% we aim to optimize the parameters $\bftheta$ by rolling out the approximate dynamics $\bff_{\bftheta}$ with state $\bfx_{0:K-1}^{(i)}$ and control $\bfu^{(i)}_{0:K-1}$ and minimizing the discrepancy between the predicted state sequence $\tilde{\bfx}^{(i)}_{1:K}$ and the true state sequence $\bfx^{(i)}_{1:K}$ in $\calD$:
% %
% \begin{equation}
% \label{eq:problem_formulation_unknown_env_equation}
% \begin{aligned}
% \min_{\bftheta} \;&\sum_{i = 1}^D \sum_{k = 1}^K \mathcal{L} (\bfx^{(i)}_k,\tilde{\bfx}^{(i)}_k)\\
% \text{s.t.} \;\; & \tilde{\bfx}^{(i)}_{k+1} = \bff \left(\bfx^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k \right) + \bff_{\bftheta}\left(\bfx^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k \right), \\
% & \tilde{\bfx}^{(i)}_k = \tilde{\bfx}^{(i)}(t_k), \quad \tilde{\bfx}^{(i)}_0 = \bfx_{0}^{(i)}, \quad \forall k=0,...,K-1,
% \end{aligned}
% \end{equation}
% %
% where $\mathcal{L}$ is a distance metric on the state space.
% \end{problem}



%that tracks a desired state trajectory $\bfx^*(t)$, $t \geq t_0$, for the learned realization of the robot dynamics with unknown dynamics and model mismatches (\ref{eq:discrete_learned_model}).

% \begin{problem}
% \label{problem:setpoint_reg}
% Given an initial condition $\bfx_0$ at time $t_0$, desired state trajectory $\bfx^*(t)$, $t \geq t_0$, and learned realization (\ref{eq:discrete_learned_model}), design a model predictive control law $\bfu = \bfpi(\bfx, \bftheta, \bfx^*(t))$ to achieve both accurate and robust target jumping, which involves flight phase (i.e. extreme underactuated systems).
% % that involves long acrobatic period.
% \end{problem}

% To tackle these problems, we propose the following system architecture as depicted in Fig. \ref{fig:overview_framework}, which includes the baseline MPC with nominal SRBD for collecting data for training, the Adaptive-frequency learning (Sec. \ref{sec:adaptive_learn_model}, \ref{sec:training}), and the Adaptive-frequency MPC for the learned dynamics (Sec. \ref{sec:adaptive-MPC}). 

% % The proposed learning-based MPC framework comprises of
% % two primary parts, the Adaptive-frequency model training and the Adaptive-frequency MPC execution for the learned dynamics, which are presented in Sec. \ref{sec:training} and \ref{sec:adaptive-MPC} respectively.

% % Conventional MPC usually either adopt fixed frequency in state prediction or has not leverage of legged dynamics in dynamic model, which may limits accurate trajectory prediction for whole long flight phase. 
% Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness.
% % Unlike conventional MPC, we design a learning residual model and adaptive-frequency to leverage the effect of complex leg dynamics, unknown dynamics in contact and hardware, as well as compensate for model mismatch, which will then followed by adaptive prediction frequency design to leverage the whole flight phase inside MPC predictions. 
% % Both factors are combined as a unified model, allowing us to enhance the accuracy of trajectory prediction for long flight phase within a limited MPC horizon. 
% We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. 
% % We denote the synchronized sampling time $\Delta t_{\calC}$ and $\Delta t_{\calF}$ for contact and flight phase, $\Delta t_{\calF} > \Delta t_{\calC}$, respectively. 
% % This synchronization aims to avoid conflict in discretization. 
% % \textcolor{red}{We use the same contact schedule}
% For data collection, we combine nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD controller, generating diverse motions with different jumping references and disturbance, as presented in Sec. \ref{subsec:data_gen}. 
% % For data collection for jumping, we combine both nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) for high-level body trajectory tracking and joint PD controller for low-level joint profile tracking, generating a diverse motions with different jumping references and disturbance. 
% % presented in Sec. \ref{subsec:data_gen}. 
% For adaptive-frequency learning, we design neural networks to learn the discretized models for contact and flight phases with adaptive sampling time via the supervised learning, aiming to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover contact transitions and the entire flight phase.
% % For adaptive-frequency learning, we design neural networks with Pytorch to learn the discretized models for contact and flight phases with adaptive sampling time. The training is based on supervised learning and we aim to learn the model to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover the contact transition and the entire flight phase.
% Finally, adaptive-frequency MPC is designed to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 
% With the constructed adaptive residual learning model, the MPC is formulated with adaptive frequency in prediction in order to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. The real-time MPC works together with high-frequency joint tracking PD controller to execute entire dynamic jumping motion. The feedback states from robot includes global body's CoM $\bfx $, and the local joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 
% The transformation $\mathbf{J}^T \bfR^T$ converts the output of MPC controller in world frame to joint torque in the robot frame, where $\mathbf{J} (\bfq_j)^T$ is leg Jacobian and $\bfR$ is rotation matrix. 
% The references for MPC and joint PD controller are obtained from full-body TO (e.g. \cite{QuannICRA19}). 

% We implement MPC for the nominal dynamics model (\ref{eq:nominal_dynamics}) to track reference from full-body TO \cite{QuannICRA19}, generating various jumping motions to different targets. The ground disturbances (i.e. blocks under feet with random height) are added to obtain a variety set of data for training.



\section{\rebut{Variable-Frequency} Model Learning}
\label{sec:adaptive-frequency-learning}

In this section, we describe how to learn the residual dynamics $\delta \bff_{\bftheta}$ from data with \rebut{a variable-frequency}\redst{an adaptive-frequency} scheme that can cover the entire flight phase, the final state upon landing, and the contact transitions between jumping phases.


% \subsection{Overview framework}
% \NA{We should use the title of this section as an opportunity to highlight our method. We should have a better title that highlights the novelty or the name of our approach.}

% \subsection{Model Learning with Adaptive Frequency}
% - Adaptive Frequency to contact phase and flight phases
% - Neural Network, Euler integration, 
% \label{sec:training}

\subsection{Learning Dynamics with \rebut{Variable-Frequency}\redst{Adaptive Frequency}}  \label{sec:adaptive_learn_model}

% In contrast with many legged-jumping MPC frameworks using SRBD (e.g.\cite{YanranDingTRO, GabrielICRA2021,park2017high,continuous_jump_bipedal}), we propose to add learned residual terms to account for leg dynamics, model mismatch, and unknown dynamics in the contact model or hardware \NA{This sentence could be moved to the intro/related work}. 
% This model also leverage the state transition between contact and flight phase, aiming to achieve accurate trajectory prediction for real-time control and optimization.
% We utilize the simplified dynamics to enable real-time control but propose to learn a residual term to account for legged dynamics, model mismatch (e.g. kinematic parameters, or unknown dynamics in contact model or hardware. 


% We aim to develop a learned model for quadruped jumping that is able to represent the complexity of whole-body dynamics and capture the robot model uncertainties, while it is necessary compact and lightweight to be utilized for real-time feedback control\NA{I suggest toning down this sentence and making it more specific. We introduced the full-body and single-rigid-body models in the previous section. We can build on these, i.e., explain that we focus on the SRB model due to its simplicity (linearity?) for online control but aim to learn residual terms the account for the leg dynamics.}. Importantly, we also aim to design model predictive control using the learned model to achieve accurate jumping under uncertainty.

% Consider a robot with state $\bfx$ consisting of its position $\bfp \in \mathbb{R}^3$, orientation $\bfR\in SO(3)$, body-frame linear velocity $\bfv \in \bbR^3$, and body-frame angular velocity $\bfomega\in \mathbb{R}^3$. 

% Let $\bfx_{k+1} = \bff(\bfx_{k}, \bfu_k)$ characterize the robot dynamics with control input $\bfu$.
% We aim to approximate the residual dynamics using a dataset $\mathcal{D}$ of state and control trajectories. 

 % This simplifies the whole trunk and legs as a unified single rigid body subject to forces at the contact patches (e.g. \cite{park2017high,YanranDingTRO,ParkRSS15}). 
 % which finds highly efficient to real-time control. 
 % Although ignoring leg dynamics is a major simplification, the controller
 % is still able to stabilize a high-DoF system and is robust
 % to these multi-body effects.
 % Consider a robot modeled as a single rigid body with position $\bfp \in \bbR^2$, orientation $\theta \in \mathbb{R}$. 
 % \TD{I think before this sentence, we should clarify that in this paper, we only consider 2D jumping, leading to the generalized coordinates that follow. Up to this point, the state $\bfx$ is general.} 

 
We consider a 2D jumping motion on a legged robot with point foot contact, e.g., quadruped robot, with generalized coordinates $\boldsymbol{\mathfrak{q}} = \begin{bmatrix} \bfp^{\top} & \phi \end{bmatrix}^{\top} \!\in \mathbb{R}^{3}$, where $\bfp \in \bbR^2$ is the CoM's position, and $\phi \in \mathbb{R}$ is the body pitch angle. We define the generalized robot's velocity as $\bfzeta = \begin{bmatrix} \bfv^{\top} & \omega \end{bmatrix}^{\top} \in \mathbb{R}^3$, where $\bfv \in \mathbb{R}^2$ and $\omega \in \mathbb{R}$ are the linear and angular velocity. Both $\mathfrak{q}$ and $\bfzeta$ are expressed in world-frame coordinates. The robot state is $\bfx = \begin{bmatrix} \boldsymbol{\mathfrak{q}}^{\top} & \bfzeta^{\top} & g\end{bmatrix}^{\top} \in \mathbb{R}^{7}$, where the (constant) gravity acceleration $g$ is added to obtain a convenient state-space form \cite{Carlo2018}.
 % \TD{This is a bit vague. Why is it convenient?}.
% Under the control input $\bfu = \begin{bmatrix} \bff_1^{\top} & \bff_2^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{n_u}$,  robot state $\bfx = \begin{bmatrix} \boldsymbol{\mathfrak{q}}^{\top} & \bfzeta^{\top} & g\end{bmatrix}^{\top} \in \mathbb{R}^{n_x}$.
\rebut{We define $\bfR(\phi) = \begin{bmatrix}
    \text{cos}(\phi) & -\text{sin}(\phi); \text{sin}(\phi) & \text{cos}(\phi)
\end{bmatrix} \in \mathbb{R}^{2\times 2}$ as a rotation matrix of the main body, which converts $\bfr_{i,b}$ (a relative foot $i \in \{1, 2\}$ position relative to the body's CoM in the body frame) to the world frame $\bfr_{i} = \bfR\bfr_{i,b}$}. We denote $\bfr = \begin{bmatrix} \bfr_1^{\top} & \bfr_2^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{4}$\redst{, where $\bfr_i$ as the foot $i \in \{1, 2\}$ position relative to the body's CoM in the world frame}. With the force control input for the front and rear legs as $\bfu = \begin{bmatrix} \bfu_f^{\top} & \bfu_r^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{4}$, the nominal discrete-time SRBD model can be written as:
% \NA{What is the control input? What is its dimension?}
% We use discrete-time SRBD as the nominal dynamics model:
% \NA{Is it necessary for $\bfB$ to depend on $k$? Is it because we will be changing $\Delta t$? Then, perhaps, it is better to use $\Delta t_k$.}
\begin{equation}\label{eq:discrete_nominal_model}
    \bff\left(\bfx_k, \bfu_k, \bfr_{k},\Delta t_k \right)  = \bfA_k\bfx_{k} + \bfB_k(\bfr_k) \bfu_k,
\end{equation}
where $\bfA_k = \bfI_{7} + \bfA_{ct} \Delta t_k$, $\bfB_k(\bfr_k)= \bfB_{ct}(\bfr_k) \Delta t_k$, $\Delta t_k$ is the \redst{adaptive sampling time}\rebut{time step} (e.g., $\Delta t_{\calC}$ or $\Delta t_{\calF}$ for the contact or flight phase, respectively), and $\bfA_{ct}$ and $\bfB_{ct}$ are obtained from the continuous-time robot dynamics:
% \NA{Also, should we call the vector $\bfe_2$?}
%
\begin{equation}
    \bfA_{ct} = 
    \begin{bmatrix}
        \bf0 & \bfI_{3} & \bf0 \\ 
        \bf0 & \bf0 & \bfe_{3} \\ 
        \bf0 & \bf0 & 0
    \end{bmatrix}, 
    \bfB_{ct}(\bfr) = 
    \begin{bmatrix}
        \bf0 & \bf0 \\ 
        \bfI_{2} / m & \bfI_{2} / m \\ 
        [\bfr_1]_{\times}^{\top}/J & [\bfr_2]_{\times}^{\top}/J \\ 
        \bf0 & \bf0
    \end{bmatrix}, \nonumber
\end{equation}
where $\bfA_{ct}\in \mathbb{R}^{7\times 7}$, $\bfB_{ct} \in \mathbb{R}^{7\times 4}$, $\bfe_3= \begin{bmatrix} 0 & -1 & 0
\end{bmatrix}^\top$, $m$ and $J$ are mass and moment inertial of the body\redst{$m$ is the body mass, $J$ is the moment inertia of the body}, $[\bfr_i]_{\times} = \begin{bmatrix} r_{iz} & -r_{ix} \end{bmatrix}^{\top} \in \mathbb{R}^2$.
% $\bfr$\NA{Perhaps this should be introduced earlier, e.g., before eq. (3) where we define the state and input}.  
% for the sake of notation. 
% The discrete dynamics is then propagated using the Euler forward scheme as
% \begin{equation} \label{eq:nominal_dynamics}
% 	\bfx_{k+1} = \bfA_k \bfx_{k} + \bfB_k(\bfr_k) \bfu_k,
% \end{equation}
% We choose to learn a model that represents the relationship between the robot states and force control, rather than actual ground contact force which is hard to estimate accurately \cite{Zachary_RAL_online_calibration_2022} or when force sensors are not equipped, which is the case for many quadruped robots (e.g. \cite{QuannICRA19,YanranDingTRO,ChignoliICRA2022})\NA{Should this information be moved earlier where we define $\bfx_k$ and $\bfu_k$?}. In addition, this representation allows us to directly incorporate the learned model with an MPC architecture to optimize for the control inputs. 
% The proposed discrete-time model with residual dynamics can be characterized as follows:
% \begin{equation}\label{eq:discrete_learned_model}
%     \bfx_{k+1} = \bff\left(\bfx_k, \bfu_k, \bfr_{k} \right) + \bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k} \right),
% \end{equation}
The residual term $\delta\bff_{\bftheta}\left(. \right)$ in (\ref{eq:discrete_learned_model}) is\redst{defined as}
%
\begin{equation}\label{eq:discrete_learned_res_model}
\delta\bff_{\bftheta}\left(. \right) = 
 \bfh_{\bftheta}(\bfx_k, \bfr_{k}) \Delta t_k  + \bfG_{\bftheta}(\bfx_k, \bfr_{k}) \Delta t_k \bfu_k,
\end{equation}
%
where $\bfh_{\bftheta}(\bfx_k, \bfr_{k})$ and $\bfG_{\bftheta}(\bfx_k, \bfr_{k})$ are represented by neural networks with learning parameters $\bftheta$.
% We aim to learn $\bfh_{\bftheta}$ and $\bfG_{\bftheta}$ with parameters $\bftheta$ that approximate the residual dynamics on the dataset $\mathcal{D}$ of state and control trajectories. 
Since $\bfu_k=\bf0$ during the flight phase, $\bfG_{\bftheta}\bfu_k=\bf0$. We have two separate models for the contact ($\calC$) and flight phase ($\calF$):
% \begin{subequations}\label{eq:res_dynamics_each_phase}
%     \begin{align}
%        &(\calC):
%        ~&\bfx_{k+1}&= \bfA_{\calC,k} \bfx_{k} + \bfB_k \bfu_{k} \nonumber \\ 
%        &&&~~~ + \bfh_{\bftheta_1}(\bfx_{k}, \bfr_{k})  + \bfG_{\bftheta_1}(\bfx_{k}, \bfr_{k}) \bfu_{k}, \\
%        &(\calF):
%        ~&\bfx_{k+1}& = \bfA_{\calF,k}  \bfx_{k} + \bfh_{\bftheta_2}( \bfx_{k}, \bfr_k),
%      \end{align}
% \end{subequations}
\begin{subequations}\label{eq:res_dynamics_each_phase}
    \begin{align}
     & (\calC):  ~ \bfx_{k+1} = \bfA_{\calC}\bfx_k + \bfB_{\calC}(\bfr_k) \bfu_k \nonumber \\
     & ~~~~~~~~~ + \bfh_{\bftheta_1}(\bfx_k, \bfr_{k})  \Delta t_{\calC} + \bfG_{\bftheta_1}(\bfx_k, \bfr_{k})\Delta t_{\calC} \bfu_k, \\ 
     &(\calF):  ~~~ \bfx_{k+1} = \bfA_{\calF}\bfx_k + \bfh_{\bftheta_2}(\bfx_k, \bfr_{k})\Delta t_{\calF}
     \end{align}
\end{subequations}
% \Abdullah{I think both $\bfh_{\bftheta_1}(\bfx_{k}, \bfr_{k})$ and $\bfG_{\bftheta_1}(\bfx_{k}, \bfr_{k})$ should be multiplied with $\Delta t$, right?}
% \begin{equation}
% \label{eq:ode_solver}
% \{\tilde{\bfx}_1^{(i)}, \ldots, \tilde{\bfx}_N^{(i)}\} = \text{EI}(\bfx_0^{(i)}, \bff_{no}+\tilde{\bff}_{\bftheta}, u_0^{(i)}, \ldots, u_{N-1}^{(i)}),
% \end{equation}
where $\bfA_{\calC} = \bfI_7 + \bfA_{ct} \Delta t_{\calC}$, $\bfB_{\calC}(\bfr_k)=\bfB_{ct}(\bfr_k) \Delta t_{\calC}$, and $\bfA_{\calF} = \bfI_7 + \bfA_{ct} \Delta t_{\calF}$.
% \subsection{Training with Adaptive Frequency} \label{sec:training}
% We aim to learn a residual model that can provide accurate prediction of the robot state trajectory during different phases of a jump. Therefore, we propose to train the model with the same adaptive-frequency scheme and horizons as MPC, instead of training separately for each phase. The state prediction for each sequence can leverage the contact transition and the entire flight phase.
%To train the neural networks, we minimize the discrepancy between the predicted state sequence $\tilde{\bfx}_{1:K}$ and the true state sequence $\bfx_{1:K}$ (i.e. labels) from $\calD$, as described in Problem \ref{problem:dynamics_learning}. 
% ) along $K$ horizons with adaptive sampling time as MPC
%  described in Sec. \ref{sec:sys_overview}
%  from the learned model
We roll out the dynamics based on \eqref{eq:res_dynamics_each_phase}, starting from initial state $\bfx_0$ with given control input sequence $\bfu_{0:K-1}$ to obtain a predicted state sequence $\tilde{\bfx}_{1:K}$. Using the \rebut{variable-frequency}\redst{adaptive-frequency} scheme, the state prediction accounts for contact transitions (feet taking off the ground), a long flight phase, and the final robot state upon landing. We define the loss functions in Problem \ref{problem:dynamics_learning} as follows:
%
\begin{equation}
\begin{aligned}
\mathcal{L} (\bfx,\tilde{\bfx}) & = \| \boldsymbol{\mathfrak{q}} - \tilde{\boldsymbol{\mathfrak{q}}}\|^2_2 + \| \bfzeta - \tilde{\bfzeta}\|^2_2\\
\mathcal{L}_{reg} (\bftheta) & = \alpha_1 \Vert  \bfh_{\bftheta} \Vert + \alpha_2 \Vert  \bfG_{\bftheta}  \Vert.
\end{aligned}
\end{equation}
%
The parameters $\bftheta = [\bftheta_1, \bftheta_2]$ for each phase are updated by gradient descent to minimize the total loss.
%$\mathcal{L} (\bfx,\tilde{\bfx}) + \mathcal{L}_{reg} (\bftheta)$.

% \NA{This sentence is unclear. We have not defined what the adaptive frequency scheme for MPC is and it is indeed too early for this perhaps.}. 
% This also allows us to learn the discretization errors for state prediction.
% We denote the dataset as $\calD = \{t_{k:k+K}^{(i)}, \bfx^{(i)}_{k:k+K}, \bfr^{(i)}_{k:k+K}, \bfu^{(i)}_{k:k+K}\}_{i=1}^D$ consisting of $D$ state sequences $\bfx^{(i)}_{k:k+K}$, obtained by applying control inputs $\bfu^{(i)}_{k:k+K}$ to the system, and $\bfr^{(i)}_{k:k+K}$ represents the foot position w.r.t the body's CoM in the world frame\NA{This information was already provided in the problem statement. It is not necessary to repeat it here. You may refer to Problem 1 if necessary.}.
% Let $\tilde{\bfx}^{(i)}_{k+1} \in \bbR^{7}$ denote the state trajectory predicted with control input $\bfu^{(i)}_k$ by the approximate dynamics $\tilde{\bfx}^{(i)}_{k+1} = \bff\left(\bfx^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k \right) + \bff_{\bftheta}\left(\bfx^{(i)}_k, \bfu^{(i)}_k , \bfr^{(i)}_k\right)$\NA{Should we have tilde for the arguments of the functions?}. The state prediction for each sequence can leverage the contact transition and the entire flight phase.
% The robot state in the contact and flight phase can be predicted as follows
% \begin{subequations}\label{eq:res_dynamics}
%     \begin{align}
%        & (\calC):
%        % \tilde{\bfx}_{k+1}^{(i)}&= \bfA_{\calC,k} \bfx_k^{(i)} + \bfB_k \bfu_k^{(i)} \\  & + \bfh_{\bftheta_1}(\bfx_k^{(i)}, \bfr_k^{(i)})  + \bfG_{\bftheta_1}(\bfx_k^{(i)}, \bfr_{k}^{(i)}) \bfu_k^{(i)}, \\
%        % \vdots \\
%        ~\tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calC,k} \tilde{\bfx}_{k}^{(i)} + \bfB_k \bfu_{k}^{(i)} \nonumber \\ 
%        & ~~~~~~~~~~~~~~~ + \bfh_{\bftheta_1}(\tilde{\bfx}_{k}^{(i)}, \bfr_{k}^{(i)})  + \bfG_{\bftheta_1}(\tilde{\bfx}_{k}^{(i)}, \bfr_{k}^{(i)}) \bfu_{k}^{(i)}, \\
%        & (\calF):
%        ~~\tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calF,k} \tilde{\bfx}_k^{(i)} + \bfh_{\bftheta_2}(\tilde{\bfx}_k^{(i)}, \bfr_k^{(i)}),
%      \end{align}
% \end{subequations}

% To optimize the parameters $\bftheta$, we roll out the dynamics with initial state $\bfx_k^{(i)}$ and control $\bfu^{(i)}_{k:k+K}$ and minimize the discrepancy between the computed state sequence $\tilde{\bfx}^{(i)}_{k:k+K}$ and the true state sequence $\bfx^{(i)}_{k:k+K}$ from $\calD$. 
% Given an initial state $\bfx_k^{(i)}$ at time $t_k^{(i)}$\NA{There is no notion of time since we are already working in discrete time.} and control input $\bfu_k^{(i)}, \ldots, \bfu_{k+K-1}^{(i)}$ from the dataset, a forward pass returns predicted states for $K$ steps $t_{k+1}^{(i)}, \ldots, t_{k+K}^{(i)}$ as $\lbrace \tilde{\bfx}_{k+1}^{(i)}, \tilde{\bfx}_{k+2}^{(i)}, ..., \tilde{\bfx}_{k+K}^{(i)} \rbrace $, where state trajectory prediction 
% $\tilde{\bfx}_{k+j}^{(i)} = [\tilde{\mathbf\frakq}_{k+j}^{(i)\top} \quad \tilde{\bfzeta}_{k+j}^{(i)\top} \quad g]^\top$, where $\tilde{\mathbf\frakq}_{k+j}^{(i)\top} = [\tilde{\bfp}_{k+j}^{(i)\top} \quad \tilde{\phi}_{k+j}^{(i)\top} ]^\top$, $\tilde{\bfzeta}_{k+j}^{(i)\top} = [\tilde{\bfv}_k^{(i)\top} \quad \tilde{\omega}_{k+j}^{(i)\top}]^\top$, $j = 1,...,K$\NA{A lot of information in this sentence is redundant. We already defined the states and explained that we do prediction by rolling out the dynamics.}.
% Our objective is to learn the parameters $\bftheta$ that minimize the loss function in (\ref{eq:problem_formulation_unknown_env_equation}) with state predictions\NA{It is also not necessary to repeat this. Just refer to the model in \eqref{eq:res_dynamics}. I think it is already clear from the problem statement and the discussion above that we use the dynamics to predict $\tilde{\bfx}_k$.}: 
% \Abdullah{I think the last line in (6) should be $\tilde{\bfx}^{(i)}(t_0) = \bfx_{0}^{(i)}, \quad \tilde{\bfx}_{k}^{(i)} =  \tilde{\bfx}^{(i)}(t_k), \quad \forall k = 0, \ldots, K, \quad \forall i = 1, \ldots, D$},
% \begin{subequations}
%     \begin{align}
%        &(\calC):
%        \tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calC,k}  \tilde{\bfx}_k^{(i)} + \bfB_{k}(\bfr_{k}^{(i)}) \bfu_k^{(i)} \nonumber \\ 
%        & ~~~~~~~~~~~~~~~ + \bfh_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}) + \bfG_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}^{(i)}) \bfu_k^{(i)}, \\
%        &(\calF):
%        ~~ \tilde{\bfx}_{k+1}^{(i)} = \bfA_{\calF,k} \tilde{\bfx}_k^{(i)} + \bfh_{\bftheta_2}(\tilde{\bfx}_k^{(i)}, \bfr_k^{(i)}),
%      \end{align}
% \end{subequations}
% \begin{equation}
% \begin{aligned}
% & \underset{\bftheta}{\text{min}}
% & & \sum_{i=1}^{D} \sum_{k=1}^{K}  \mathcal{L}_{\bftheta} (\bfx^{(i)}_k,\tilde{\bfx}^{(i)}_k)\\
% & \text{s.t.}
% & & \begin{aligned}[t]
%  (\calC): \tilde{\bfx}_{k+1}^{(i)} = &\ \bfA_{\calC,k}  \tilde{\bfx}_k^{(i)} + \bfB_{k}(\bfr_{k}^{(i)}) \bfu_k^{(i)} \\ 
% &+ \bfh_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}) + \bfG_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}^{(i)}) \bfu_k^{(i)} \\
% \end{aligned} \\
% & & & (\calF): \tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calF,k} \tilde{\bfx}_k^{(i)} + \bfh_{\bftheta_2}(\tilde{\bfx}_k^{(i)}, \bfr_k^{(i)}), \\
% & & &  \tilde{\bfx}_{0}^{(i)} =  \tilde{\bfx}^{(i)}(t_k), \quad \forall k = 0, \ldots, K, \quad \forall i = 1, \ldots, D, 
% \end{aligned}
% \end{equation}
% where $\mathcal{L}$ is a distance metric on the state space.
% We train separate models for the contact and flight phase, i.e. $\bfh_{\bftheta_1}$ and $\bfG_{\bftheta_1}$ for contact phase, and $\bfh_{\bftheta_2}$ and $\bfG_{\bftheta_2}$ for flight phase. The learning model represents the relationship between robot states and force control, instead of actual ground contact force which is hard to estimate accurately or not available when force sensors are not available. 
% We aim to learn the model, which will then be utilized to obtain predictions in MPC. For this purpose, we propose to train the model with adaptive frequency as MPC. This also allows us to learn the discretization errors for state prediction.
% The nominal dynamics at each time step $t_k^{(i)}$ above is defined as
% \begin{equation}
%     f_{no}\left(\bfx_k, \bfu_k, \bfr_k  \right) = \bfA \bfx_k + \bfB_k(\bfr_k ) \bfu_k
% \end{equation}
% and the residual dynamics:
% \begin{equation}
%     \tilde{f}_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k} \right) = 
%  h_{\bftheta}(\bfx_k, \bfr_{k})  + g_{\bftheta}(\bfx_k, \bfr_{k}) \bfu_k
% \end{equation}
% The predicted rotation matrix $\tilde{\bfR}_n^{(i)} = [\tilde{\bfr}_{1n}^{(i)} \quad \tilde{\bfr}_{2n}^{(i)} \quad \tilde{\bfr}_{3n}^{(i)}]^\top$ and the ground-truth one $\bfR_n^{(i)} = [\tilde{\bfr}_{1n}^{(i)} \quad \tilde{\bfr}_{2n}^{(i)} \quad \tilde{\bfr}_{3n}^{(i)}]^\top$ are used to calculate an orientation loss:
% %
% \begin{equation}
% \mathcal{L}_{\bfR}(\bftheta) = \sum_{i = 1}^D \sum_{n = 1}^N \left\|\left(\log (\tilde{\bfR}_n^{(i)} \bfR_n^{(i)\top})\right)^{\vee} \right\|_2^2,
% \end{equation}
% 
% We aim to minimize the loss which represents the discrepancy between prediction state $\lbrace \tilde{\bfx}_{k+1}^{(i)}, \tilde{\bfx}_{k+2}^{(i)}, ..., \tilde{\bfx}_{k+K}^{(i)} \rbrace $ and the label from dataset $\lbrace \bfx_{k+1}^{(i)}, \bfx_{k+2}^{(i)}, ..., \bfx_{k+K}^{(i)} \rbrace $. 
% Refer to  We use the squared Euclidean norm to calculate losses for the position and generalized velocity terms:\NA{The notation below is strange because it is not clear what $\bfp$ and $\bfzeta$ are on the left-hand-side of the equations. To be consistent with \eqref{problem:dynamics_learning}, we should define $\mathcal{L} (\bfx,\tilde{\bfx}) = \| \mathbf\frakq - \tilde{\mathbf\frakq}\|^2_2 + \| \bfzeta - \tilde{\bfzeta}\|^2_2$. We should also introduce the regularization term $\calL_{\text{reg}}(\bftheta)$ in \eqref{problem:dynamics_learning} and define it here as $\calL_{\text{reg}}(\bftheta) = \alpha_1 \|  \bfh_{\bftheta} \| + \alpha_2 \| \bfG_{\bftheta}  \|$.} 
%\begin{equation}
%\mathcal{L}_{\bfp}(\bftheta) = \sum_{i = 1}^D \sum_{n = 1}^N \Vert \bfp_n^{(i)} - \tilde{\bfp}_n^{(i)} \Vert^2_2, \mathcal{L}_{\bfzeta}(\bftheta) = \sum_{i = 1}^D \sum_{n = 1}^N \Vert \bfzeta_n^{(i)} - \tilde{\bfzeta}_n^{(i)} \Vert^2_2.
%\end{equation}
%

% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{\bftheta}(\bfp) &= \sum_{i = 1}^D \sum_{k = 1}^K \Vert \mathbf\frakq_k^{(i)} - \tilde{\mathbf\frakq}_k^{(i)} \Vert^2_2,\\
% \mathcal{L}_{\bftheta}(\bfzeta) &= \sum_{i = 1}^D \sum_{k = 1}^K \Vert \bfzeta_k^{(i)} - \tilde{\bfzeta}_k^{(i)} \Vert^2_2 \\
% \mathcal{L}_{reg} (\bftheta) &= \sum_{i = 1}^D \sum_{k = 1}^K \alpha_1 \Vert  \bfh_{\bftheta} \Vert + \alpha_2 \Vert  \bfG_{\bftheta}  \Vert.
% \end{aligned}
% \end{equation}
%
% The total loss $\calL_{\bftheta}$ is defined as:
% \begin{equation}
% \calL_{\bftheta}= \mathcal{L}_{\bftheta}(\bfp) + \mathcal{L}_{\bftheta}(\bfzeta) + \mathcal{L}_{reg} (\bftheta).
% \end{equation}
% The total loss $\calL_{\bftheta}$ is defined as:
% \begin{equation}
% \calL_{\bftheta}= \mathcal{L} (\bfx,\tilde{\bfx}) + \mathcal{L}_{reg} (\bftheta).
% \end{equation}
% The gradient of the total loss function $\calL(\bftheta)$ is back-propagated by solving an ODE with adjoint states \cite{chen2018neural}. Specifically, let $\bfa = \frac{\partial \calL}{\partial \tilde{\bfx}}$ be the adjoint state and $\bfs = (\tilde{\bfx}, \bfa, \frac{\partial \calL}{\partial \bftheta})$ be the augmented state. The augmented state dynamics are \cite{chen2018neural}:
% %
% \begin{equation}
% \dot{\bfs} = \tilde{\bff}_{\bfs} = (\tilde{\bff}_{\bftheta}, -\bfa^\top\frac{\partial \tilde{\bff}_{\bftheta}}{\partial \tilde{\bfx}}, -\bfa^\top\frac{\partial \tilde{\bff}_{\bftheta}}{\partial \bftheta}).
% \end{equation}
% %
% The predicted state $\tilde{\bfx}$, the adjoint state $\bfa$, and the derivatives $\frac{\partial \calL}{\partial \bftheta}$ can be obtained by a single call to a reverse-time ODE solver starting from $\bfs_N = \bfs({t_N})$:
% %
% \begin{equation}
% \bfs_0 = \left(\tilde{\bfx}_0, \bfa_0, \frac{\partial \calL}{\partial \bftheta}\right) = \text{ODESolver}(\bfs_N, \tilde{\bff}_\bfs, t_N),
% \end{equation}
% %
% where at each time $t_k, k = 1, \ldots, N$, the adjoint state $\bfa_{k}$ at time $t_k$ is reset to $ \frac{\partial \calL}{\partial \tilde{\bfx}_{k}}$. The resulting derivative $ \frac{\partial \calL}{\partial \bftheta}$ is used to update the parameters $\bftheta$ using gradient descent.

\subsection{Data Collection}
\label{subsec:data_gen}
% \subsubsection{Nominal Dynamic Model}

\rebut{For model learning, we directly collect state-control trajectories from hardware experiments by implementing}\redst{To collect state-control trajectories for residual dynamics learning, we implemented} an MPC controller with the nominal dynamics model \eqref{eq:discrete_nominal_model} and a reference body trajectory $\bfx^*$ obtained from full-body TO.
% To collect state-control trajectories for residual dynamics learning, we implemented an MPC controller with the nominal dynamics model \eqref{eq:discrete_nominal_model} and a reference body trajectory $\bfx^*$ obtained from full-body trajectory optimization. 
The TO assumes jumping from flat and hard ground with point foot contact. We generated various jumps \redst{trajectories} to different targets under different \redst{ground}disturbances (e.g., blocks under the robot feet with random height) to obtain a diverse dataset. 


% The trajectory optimization provides a reference state trajectory $\bfx_{0:K}^*$ and ground contact forces $\bfu_{0:K}^*$.



% While MPC aims to track body trajectory $\bfx^*$, an additional joint PD controller is adopted to track the joint trajectory reference from trajectory optimization. This yields the total torque applied to the robot motors as:
% \begin{align} \label{eq:applied_torque}
%     \bftau= \bftau_{mpc} + \bftau_{pd},
% \end{align} 
% where $\bm{\tau}_{mpc}=\mathbf{J}(\bfq_{j})^\top \bfR(\phi)^\top \bfu_{mpc}$ converts the MPC force $\bfu_{mpc}$ to joint torque, $\bfR(\phi) = \begin{bmatrix}
%     \text{cos}(\phi) & -\text{sin}(\phi); \text{sin}(\phi) & \text{cos}(\phi)
% \end{bmatrix} \in \mathbb{R}^{2\times 2}$ is a rotation matrix,
% % \NA{How is this rotation matrix obtained? Is it related to $\phi_k$?}, 
% $\mathbf{J}(\bfq_{j})$ is the foot Jacobian at the current joint configuration $\bfq_{j}$ \NA{This may be confused with $\frakq$. Should we explain that the full-body model is defined in terms of joint angles $\bfq_{j}$?}. A joint PD controller $\bftau_{pd} = \bfK_{p,j}(\bfq_{j}^*-\bfq_j)+\bfK_{d,j}(\mathbf{\dot q}_{j}^*-\mathbf{\dot q}_j)$ is adopted for joint tracking reference.


% Since the evolution of robot states is in fact governed by the combination of MPC and the joint PD controller, we collect the trajectory dataset $\calD$ with the \rep{stored inputs as}: 
% % \NA{When collecting trajectories we are not applying anything to the learned model. Do you mean that this is the reference input stored in $\calD$?}
% \begin{equation}
%     \bfu = \left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1}  \bftau =  \bfu_{mpc} + \bfu_{pd},
% \end{equation}
% where $\bfu_{pd} =\left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1} \bftau_{pd}$\NA{Define this earlier, when you define $\bftau_{mpc}$.} converting the joint torque data to its corresponding force in the world frame. 

While the MPC aims to track the body reference trajectory $\bfx_{0:K}^*$, a joint PD controller is used to track the joint reference trajectory $(\bfq_{\mathbf{J}}^*, \mathbf{\dot q}_{\mathbf{J}}^*)$ from the full-body TO via  $\bftau_{pd,setpoint} = \bfK_{p}(\bfq_{\mathbf{J}}^*-\bfq_{\mathbf{J}})+\bfK_{d}(\mathbf{\dot q}_{\mathbf{J}}^*-\mathbf{\dot q}_{\mathbf{J}})$. Thus, the evolution of the robot states is governed by the combination of MPC and the joint PD controller. We collected the trajectory dataset $\calD$ with inputs $\bfu =  \bfu_{mpc} + \bfu_{pd},$
% \begin{equation}
%     \bfu =  \bfu_{mpc} + \bfu_{pd},
% \end{equation}
where $\bfu_{pd} =\left(\mathbf{\mathbf{J}}(\bfq_{\mathbf{J}})^{\top} \bfR^{\top}\right)^{-1} \bftau_{pd,setpoint}$, \redst{with rotation matrix $\bfR(\phi) = \begin{bmatrix}
    \text{cos}(\phi) & -\text{sin}(\phi); \text{sin}(\phi) & \text{cos}(\phi)
\end{bmatrix} \in \mathbb{R}^{2\times 2}$ and }$\mathbf{J}(\bfq_{\mathbf{J}})$ is the foot Jacobian.\redst{at joint configuration $\bfq_{\mathbf{J}}$}. 
% \NA{This may be confused with $\frakq$. Should we explain that the full-body model is defined in terms of joint angles $\bfq_{\mathbf{J}}$?}, \CN{}.



% \todo{Explain how data is chunked and collected in more detail}
The dataset is collected at the different time steps for the contact and flight phases, i.e., $\Delta t_{\calC}$ and $\Delta t_{\calF}$, respectively. \rebut{The data for each jump is then chunked by shifting a sliding window, size of $K$ by 1 timesteps}. Let $N$ be the number of collected state-control data points for each jump and $H$ be the number of jumps. We then obtain $D = H\times(N-K+1)$ state-control trajectories in total.

% The dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consists of state sequences $\bfx^{(i)}_{0:K}$, where $\bfx_k^{(i)}~=~[\mathbf\frakq_n^{(i)\top} \quad \bfzeta_k^{(i)\top}]^\top$, $\mathbf\frakq_k^{(i)}~=~[\bfp_k^{(i)\top} \quad \phi_{k}^{(i)\top}]^\top~\in~\mathbb{R}^{3}$, $\bfzeta_k^{(i)}~=~[\bfv_k^{(i)\top} \quad \omega_k^{(i)\top}]^\top \in \mathbb{R}^3$ for $k = 0, \ldots, K$\NA{This last sentence is not necessary. It was defined before and besides it is too late for this information as the last sentence of the section.}.



% Since jumping is a highly complex motion, it requires a real-time feedback control policy and whole-body coordination to enable successful jumps. In addition, we are only able to rely on force control during the contact phase to achieve safe and accurate jumping. In hardware, without appropriate control, the robot is unable to jump or make the jumping fail badly, which could lead to a hardware break. Therefore, we are unable to apply a constant or random control input $\bfu^{(i)}$ during contact phases to the system to collect the data.
% Jumping is a highly complex motion and requires efficient real-time feedback control policy and whole-body coordination. 



% \subsubsection{MPC for nominal dynamics}


% %Full-body TO is utilized to solve for reference body trajectory $\bfx^*$, joint profiles $ \{\bfq_{j}^*, \bm{\dot q}_{j}^*\}$, and ground contact force $\bfu^*$ given different targets, assuming the jumping from flat ground \cite{QuannICRA19}. It is noted that the full-body TO assumes constant calf lengths, point foot contact, and hard ground.
% % We then adopt the MPC controller in our prior work \cite{continuous_jump} to execute various jumps under a variety of disturbances. 
% % \note{The offline reference torque $\bm{\tau}_d$ generates the main force contribution for the whole body motion. In case of model uncertainties (e.g. box under feet), our idea is to adjust this reference torque $\bm{\tau}_d$ by the online offset $\Delta \bm{\tau}_{mpc}$ from MPC controller as proposed in our prior work \cite{continuous_jump}}.
% % The MPC is then designed based on SRB dynamics, i.e., nominal dynamics (\ref{eq:nominal_dynamics}). 

% % The baseline MPC is formulated as a quadratic programming (QP) with moving horizons to solve for optimal force control, which minimizes the weighted tracking errors of reference from trajectory optimization:
% % %
% % \begin{subequations} \label{eq:MPC_jumping}
% % \begin{align}
% %  \textrm{min} \textrm{ } & \sum_{k=t}^{t+K-1} \| \bfx_k-\bfx_{k}^* \|_{P_k} + \| \bfu_k - \bfu_{k}^* \|_{Q_k},\\
% % % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% % \text{s.t. }
% %              & \bfx_{k+1}=\bfA_k\bfx_k+ \bfB_k \bfu_k, \forall k=t, ..., t+K-1, \label{eq:MPC_jumping_c1} \\
% %              & \bfc_k^{min} \leq \bfC_k \bfu_k \leq \bfc_k^{max}, \forall k=t, ..., t+K-1, \label{eq:MPC_jumping_c2} \\ 
% %              & \bfD_k \bfu_k =\bm{0}, \label{eq:MPC_jumping_c3} \forall k=t, ..., t+K-1,
% % \end{align}
% % \end{subequations}
% % where E.q (\ref{eq:MPC_jumping_c2}) captures constraints related to friction cone and force limits, while E.q (\ref{eq:MPC_jumping_c3}) represents the shifting contact schedule that nullifies the force control in flight phase. 
% While MPC aims to track body trajectory $\bfx^*$, an additional joint PD controller is adopted to track the joint trajectory reference from trajectory optimization. This yields the total torque applied to the robot motors as:
% \begin{align} \label{eq:applied_torque}
%     \bftau= \bftau_{mpc} + \bftau_{pd},
% \end{align} 
% where $\bm{\tau}_{mpc}=\mathbf{J}(\bfq_{j})^\top \bfR^\top \bfu_{mpc}$ converts the MPC force to joint torque, $\bfR$ is a rotation matrix, $\mathbf{J}(\bfq_{j})$ is the foot Jacobian at the current joint configuration $\bfq_{j}$. 
% % \begin{align} \label{eq:delta_MPC}
% %     \Delta \bm{\tau}_{mpc}=\bm{J}(\bfq_{j})^\top \bfr^\top[\bfu_{mpc}^* - \bfu_{d}],
% % \end{align} 
% % \begin{align} \label{eq:delta_MPC}
% %     \bm{\tau}_{mpc}=\bm{J}(\bfq_{j})^\top \bfR^\top \bfu_{mpc},
% % \end{align} 
% % where $\bfR$ is a rotation matrix, $\bm{J}(\bfq_{j})$ is the foot Jacobian at the current joint configuration $\bfq_{j}$. 
% The joint PD controller $\bftau_{pd} = \bfK_{p,j}(\bfq_{j}^*-\bfq_j)+\bfK_{d,j}(\mathbf{\dot q}_{j}^*-\mathbf{\dot q}_j)$ is adopted for joint tracking reference.
% % \begin{align} \label{eq:applied_torque}
% %     \bm{\tau}_{t}= \bm{\tau}_{mpc} + \bm{\tau}_{pd,j},
% % \end{align} 
% % where
% % \begin{align}
% % % \bm{\tau}_{a}  &= \bm{\tau}_d + \Delta \bm{\tau}_{mpc}  \\
% % \bm{\tau}_{pd} & = \bm{K}_{p,j}(\bfq_{j,d}-\bfq_j)+\bm{K}_{d,j}(\bm{\dot q}_{j,d}-\bm{\dot q}_j)
% % \end{align} \label{eq:jointPDController}

% % \begin{align}
% % % \bm{\tau}_{a}  &= \bm{\tau}_d + \Delta \bm{\tau}_{mpc}  \\
% % \bm{\tau}_{pd} & = \bm{K}_{p,j}(\bfq_{j}^*-\bfq_j)+\bm{K}_{d,j}(\bm{\dot q}_{j}^*-\bm{\dot q}_j)
% % \end{align} \label{eq:jointPDController}

% % where the torque $\bm{\tau}_d$ and joint profiles $ \{\bfq_{J,d}, \bm{\dot q}_{J,d} \}$ obtained from the trajectory optimization for the full nonlinear dynamics.

% % \note{Another idea is to directly apply the solution MPC from (\ref{eq:MPC_jumping}) instead of using the offset MPC. In other words, we combine:
% % \begin{align} \label{eq:mpc_pd}
% %     \bm{\tau}_{t}= \bm{\tau}_{mpc}^b + \bm{\tau}_{pd,j},
% % \end{align}
% % where $\bm{\tau}_{mpc}^b =(\bfq_{j})^\top \bfr^\top\bm{f}_{mpc}^*$.
% % However, I have observed that it has not worked well in hardware. That's why we combine the reference torque with offset torque from MPC for data collection in experiments.}
% % We can have several options to select the force control for our learned model (\ref{eq:discrete_learned_model})
% % \begin{itemize}
% %     \item Option 1: Torque $\bm{\tau}_d + \Delta \bm{\tau}_{mpc}$ will then converted to the force control via
% % \begin{equation}
% %     \bfu = (\bm{J}(\bfq_j)^T \bfr^T)^{-1} (\bm{\tau}_d + \Delta \bm{\tau}_{mpc}) \nonumber
% % \end{equation}
% %     \item Option 2: Directly use $\bfu_{mpc}^*$
% %     % \item Option 2: Total torque $\bm{\tau}_{t} = \bm{\tau}_d + \Delta \bm{\tau}_{mpc}^b + \bm{\tau}_{pd,j} $
% % \end{itemize}
% % which will then be converted to generalized force control in the world frame
% % \begin{equation}
% %     \bfu = (\bm{J}(\bfq_j)^T \bfr^T)^{-1} \bm{\tau}
% % \end{equation}
% % }.
% % We then convert the total torque to force $\bfu =\bm{J}(\bfq_j)^T \bfr^T)^{-1} \bm{\tau}_t$, which then be used for the learned model.
%  Since the evolution of robot states is in fact governed by the combination of MPC and the joint PD controller, we collect the $\calD$ state-control trajectories with the following total control force applying for the learned model:
% \begin{equation}
%     \bfu = \left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1}  \bftau =  \bfu_{mpc} + \bfu_{pd},
% \end{equation}
% where $\bfu_{pd} =\left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1} \bftau_{pd}$ converting the joint torque data to its corresponding force in the world frame. 

% % \todo{Explain how data is chunked and collected in more detail}
% The dataset is collected at the different sampling time steps for the contact and flight phases, denoted as $\Delta t_{\calC}$ and $\Delta t_{\calF}$. Denote $N$ as a number of collected state-control data points for each jump, and $H$ as a number of jumps. Given $K$ as a horizon, we then obtain
% $D = H\times(N-K+1)$ state-control trajectories in total.
% The dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consists of state sequences $\bfx^{(i)}_{0:K}$, where $\bfx_k^{(i)}~=~[\mathbf\frakq_n^{(i)\top} \quad \bfzeta_k^{(i)\top}]^\top$, $\mathbf\frakq_k^{(i)}~=~[\bfp_k^{(i)\top} \quad \theta_{k}^{(i)\top}]^\top~\in~\mathbb{R}^{3}$, $\bfzeta_k^{(i)}~=~[\bfv_k^{(i)\top} \quad \omega_k^{(i)\top}]^\top \in \mathbb{R}^3$ for $k = 0, \ldots, K$.
% % Such data are generated by applying a constant control input $\bfu^{(i)}$ to the system and sampling the state $\bfx_{n}^{(i)} = \bfx^{(i)}(t_n^{(i)})$ at times $t_n^{(i)}$ for $n = 0, \ldots, N$.


% % The coordinates $\mathbf\frakq$ and velocity $\bfzeta$ may be obtained from the robot's IMU, or from a motion capture system. 

% % In physics-based simulation the data can be generated by applying random control inputs $\bfu^{(i)}$. In real-world applications, where safety is a concern, data may be collected by a human operator manually controlling the robot.


\section{\rebut{Variable-Frequency}\redst{Adaptive-Frequency} MPC with Learned Dynamics} \label{sec:adaptive-MPC}

% \subsubsection{Model Prediction with Learned Residual Dynamics} 
In this section, we design \rebut{a variable-frequency}\redst{an adaptive-frequency} MPC controller for the learned dynamics \eqref{eq:res_dynamics_each_phase} to track a desired jumping reference trajectory obtained from full-body TO. \rebut{For a given robot state $\bfx_0$,} we formulate MPC as:
%  \redst{optimization problem}
%
\begin{subequations} \label{eq:MPC_learned}
\begin{align}
 \min_{\bfu_{0:K-1}} & \; \sum_{k=1}^{K} \| \bfx_k-\bfx_{k}^* \|_{\bfQ_k} + \| \bfu_{k-1}-\bfu_{k-1}^* \|_{\bfR_k},\\
% & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
\text{s.t. }
     & (\calC):  ~~ \bfx_{k+1} = \bfA_{\calC}\bfx_k + \bfB_{\calC}(\bfr_k) \bfu_k \nonumber  \\ 
     & ~~~~~+ \bfh_{\bftheta_1}(\bfx_k, \bfr_{k})  \Delta t_{\calC} + \bfG_{\bftheta_1}(\bfx_k, \bfr_{k})\Delta t_{\calC} \bfu_k, \\ 
     &(\calF):  ~~ \bfx_{k+1} = \bfA_{\calF}\bfx_k + \bfh_{\bftheta_2}(\bfx_k, \bfr_{k})\Delta t_{\calF}, \\
     & \underline{\bfc}_k \leq \bfC_k \bfu_k \leq \bar{\bfc}_k, \; \forall k=0, ..., K-1, \label{eq:learn_MPC_ineq} \\ 
     & \bfD_k \bfu_k =\bm{0}, \qquad\quad \forall k=0, ..., K-1, \label{eq:learn_MPC_eq} 
\end{align}
\end{subequations}
where \eqref{eq:learn_MPC_ineq} represents input constraints related to friction cone and force limits and \eqref{eq:learn_MPC_eq} aims to nullify the force on the swing legs based on the contact schedule.


%TO and achieve both accurate and robust target jumping.
% For the first horizon prediction, we utilize the current robot state to compute the forward pass of the neural networks. From the second prediction, we utilize the reference trajectory to compute the output of the neural network. In particular, we predict the future robot states as follows:
% % The residual dynamics $g_{\bftheta,t+i}$,  $h_{\bftheta,t+i}$
% and the mapping function $\bm{m}_{t+i}$ with $i\in [0, N-1]$,
% are computed at future time step $t+i$. 
% At the current time $t$, these functions are evaluated with current robot states and foot positions. For a future time, we rely on reference trajectory to estimate these functions.
% \begin{subequations}\label{eq:res_dynamics}
%     \begin{align}
%         \tilde{\bfx}_{t+1}&= \bfA \bfx_t + \bfB_t \bfu_t + \left( f_{res,t} + h_{res,t} \bm{m}_t \bfu_t \right) \delta t, \nonumber\\
%         \tilde{\bfx}_{t+2}&= \bfA  \tilde{\bfx}_{t+1} + \bfB_{t+1} \bfu_{t+1} \nonumber \\  & + \left( f_{res,t+1} + h_{res,t+1} \bm{m}_{t+1} \bfu_{t+1} \right) \delta t,\nonumber \\
%         \vdots \nonumber \\
%         \tilde{\bfx}_{t+N}&= \bfA  \tilde{\bfx}_{t+N-1} + \bfB_{t+N-1} \bfu_{t+N-1} \nonumber \\ & + \left( f_{res,t+N-1} + h_{res,t+N-1} \bm{m}_{t+N-1} \bfu_{t+N-1} \right) \delta t,\nonumber
%      \end{align}
% \end{subequations}
% \begin{subequations}\label{eq:res_dynamics}
%     \begin{align}
%         \tilde{\bfx}_{k+1}&= \bfA_k \bfx_k + \bfB_k \bfu_k + \bfh_{\bftheta}(\bfx_k, \bfr_{k})  + \bfG_{\bftheta}(\bfx_k, \bfr_{k}) \bfu_k, \nonumber\\
%         \tilde{\bfx}_{k+2}&= \bfA_k  \tilde{\bfx}_{k+1} + \bfB_{k+1} \bfu_{k+1} \nonumber \\  & + \bfh_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*)  + \bfG_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*) \bfu_k,\nonumber \\
%         \vdots \nonumber \\
%         \tilde{\bfx}_{k+K}&= \bfA_k  \tilde{\bfx}_{k+K-1} + \bfB_{k+K-1} \bfu_{k+K-1} \nonumber \\ & + \bfh_{\bftheta}(\bfx_{k+K-1}^*, \bfr_{k}^*)  + \bfG_{\bftheta}(\bfx_{k+K-1}^*, \bfr_{k+K-1}^*) \bfu_k,\nonumber
%      \end{align}
% \end{subequations}
% as the shifting-horizon 


% \begin{subequations} \label{eq:MPC_learned}
% \begin{align}
%  \min & \sum_{k=0}^{K} \| \bfx_k-\bfx_{k}^* \|_{P_k} + \| \bfu_k-\bfu_{k}^* \|_{Q_k},\\
% % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% \text{s.t. }
%      & (\calC):  ~ \bfx_{k+1} = \bfA_{\calC,k}\bfx_k + \bfB_{\calC,k} \bfu_k \\ \nonumber 
%      & ~~~~~~~~~~~~ ~~~~~ + \bfh_{\bftheta_1}(\bfx_k, \bfr_{k})  \Delta t_{\calC} + \bfG_{\bftheta_1}(\bfx_k, \bfr_{k}) \bfu_k \\ 
%      &(\calF):  ~~~ \bfx_{k+1} = \bfA_{\calF,k}\bfx_k + \bfh_{\bftheta_2}(\bfx_k, \bfr_{k}) \\
%      & \bfc_k^{min} \leq \bfC_k \bfu_k \leq \bfc_k^{max}, \forall k=0, ..., K-1 \label{eq:learn_MPC_ineq} \\ 
%      & \bfD_k \bfu_k =\bm{0}, \label{eq:learn_MPC_eq} \forall k=0, ..., K-1
% \end{align}
% \end{subequations}



% \underline{Contact Prediction Mode}:  in this mode, the whole predicted horizons are in scheduled contact phase
% % \begin{equation}\label{eq:learK_contact_prediction}
% %      \tilde{\bfX}_{\calC,k}= \bfA_{\calC} \bfx_k + \bfB_{\calC} \tilde{\bfU} + \bm{\psi}_{\calC,\bftheta} + \bm{\phi}_{\calC,\bftheta} 
% % \end{equation}
% \begin{equation}\label{eq:learK_contact_prediction}
%      \tilde{\bfX}_{\calC,k}= \bfA_{\calC} \bfx_k + (\bfB_{\calC} + \bfB_{\calC,\bftheta})  \tilde{\bfU} + \bm{\psi}_{\calC,\bftheta}, 
% \end{equation}
% where the predicted states $\tilde{\bfX}_{\calC,k} = [\tilde{\bfx}_{k+1}^T, \tilde{\bfx}_{k+2}^T ..., \tilde{\bfx}_{k+K}^T]^T $ concatenate the predicted states from $k+1$ to $k+K$. The prediction is governed by control input $\tilde{\bfU} = [\tilde{\bfu}_k^T, \tilde{\bfu}_{k+1}^T, ..., \tilde{\bfu}_{k+K-1}^T]^T \in \mathbb{R}^{K \times n_x}$
% $\bfA_{\mathcal{C}}= \begin{bmatrix}
% (\bfA_{\calC,k})^\top
% (\bfA_{\calC,k}^2)^\top
% \ldots 
% (\bfA_{\calC,k}^{K})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK \times n_x}$, 
% % $\bfA_k = \bfI+ \bfA \delta t$.
% % $\bfB_{\calC}= \begin{bmatrix}
% % \bfB_k & \bm{0} & \ldots & \bm{0}\\
% % \bfA \bfB_k & \bfB_{k+1} & \ldots & \bm{0} & \\
% % \vdots \\
% % \bfA^{K-1} \bfB_k & \bfA^{K-2} \bfB_{k+1} & \ldots & \bfB_{k+K-1}
% % \end{bmatrix}
% % $
% \[[\bfB_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} \bfB_{k+n-1} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% % $\bfB_{\calC,\bftheta}= \begin{bmatrix}
% % \bfB_{\bftheta,k} & \bm{0} & \ldots & \bm{0}\\
% % \bfA_k \bfB_{\bftheta,k} & \bfB_{\bftheta,k+1} & \ldots & \bm{0} & \\
% % \vdots \\
% % \bfA_k^{N-1} \bfB_{\bftheta,k} & \bfA_k^{N-2} \bfB_{\bftheta,k+1} & \ldots & \bfB_{\bftheta,k+N-1}
% % \end{bmatrix}$
% \[[\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} \bfB_{\bftheta,k+n-1} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% % Let $\bfB_{t}^{res} = g_{res,t} \bm{m}_t $, and we define
% Let $\bfB_{\bftheta,k} = \bfG_{\bftheta}(\bfx_k, \bfr_{k}) $ obtained at the current time, and predictions are computed as
% $\bfB_{\bftheta,k+j} = \bfG_{\bftheta}(\bfx_{k+j}^*, \bfr_{k+j}^*)$, $j = 1,..., K-1$, we define:
% % \[[\bfB_{\calC}+\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
% %   \begin{array}{lr}
% %     \bfA_k^{m-n} (\bfB_{k+n-1}+ \bfB_{\bftheta,k+n-1}) : & \textit{if} ~ m \geq n \\
% %     \bm{0}  & \textit{otherwise}
% %   \end{array}
% % \right.
% % \]
% % and residual matrix 
% % \begin{equation}
% %     \bm{\phi}_{c,\bftheta} = \bfB_{c,\bftheta}^{qp} \tilde{\bfu}
% % \end{equation}
% \begin{equation}
%     \bm{\psi}_{c,\bftheta} = \begin{bmatrix}
% \bfI & \bm{0} & \ldots & \bm{0}\\
% \bfA_k & \bfI & \ldots & \bm{0} \\
% \vdots \\
% \bfA_k^{N-1} & \bfA_k^{N-2} & \ldots & \bfI
% \end{bmatrix} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_k, \bfr_{k})\\
% \bfh_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{k+N-1}^*, \bfr_{k+N-1}^*)
% \end{bmatrix}
% \end{equation}
% \\
% \\
% \underline{Adaptive Prediction Mode}: in this mode, predicted horizons are in both contact phases and flight phases. We present our proposed MPC for the learning hybrid contact model. 



%  $0\leq K_{\calC} \leq K$
% We use a greater time step for state prediction in flight phase to capture the whole flight phase (i.e. $dt_f > dt_c$). We define 
% From current time step $k$, with ($T_c-N < t <T_c$), we define
% During the flight phase, the force control output from MPC is unavailable.
% Given the current time $k$, the number of horizons for predicted contact phase $K_c$ satisfies $K_c = T_c -k$. Here, $T_c$ is a predefined schedule time at the end of the contact phase. 
% During the flight phase, there is no control input applied to the system. 
% The remaining prediction horizons $N_f = K - K_c$ are in flight phase.
% $\bfA_{\mathcal{C}}= \begin{bmatrix}
% (\bfA_{\calC,k})^\top
% (\bfA_{\calC,k}^2)^\top
% \ldots 
% (\bfA_{\calC,k}^{K_c})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x}$,  $\bfA_{\mathcal{F}}= \begin{bmatrix}
% (\bfA_{\calF,k})^\top
% (\bfA_{\calF,k}^2)^\top
% \ldots 
% (\bfA_{\calF,k}^{K_{\calF}})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_{\calF} \times n_x}$, 

% $\bfA_t = \bfI+ \bfA_c \delta t_c$.

% $\bfB_{c}^{qp}= \begin{bmatrix}
% \bfB_k & \bm{0} & \ldots & \bm{0}\\
% \bfA_k \bfB_t & \bfB_{t+k} & \ldots & \bm{0} & \\
% \vdots \\
% \bfA_k^{K_c-1} \bfB_t & \bfA_k^{K_c-2} \bfB_{k+1} & \ldots & \bfB_{k+K_c-1}
% \end{bmatrix}
% $


With the MPC horizon including $K_{\calC}$ steps in the contact phase and $K_{\calF} = K-K_{\calC}$ steps in the flight phase, we define \rebut{$\tilde{\bfU}_{\calC} = [\tilde{\bfu}_0^{\top}, \tilde{\bfu}_{1}^{\top}, ..., \tilde{\bfu}_{K_{\calC} - 1}^{\top}]^{\top} \in \mathbb{R}^{K_{\calC} \times 4}$}
%
% \begin{equation}
%     \tilde{\bfU}_{\calC} = [\tilde{\bfu}_0^{\top}, \tilde{\bfu}_{1}^{\top}, ..., \tilde{\bfu}_{K_{\calC} - 1}^{\top}]^{\top} \in \mathbb{R}^{K_c \times n_x}
% \end{equation}
% \rebut{\begin{equation}
%     \tilde{\bfU}_{\calC} = [\tilde{\bfu}_0^{\top}, \tilde{\bfu}_{1}^{\top}, ..., \tilde{\bfu}_{K_{\calC} - 1}^{\top}]^{\top} \in \mathbb{R}^{K_{\calC} \times 4}
% \end{equation}}
%
as a concatenation of the control inputs in the contact phase. With this notation, the predicted trajectory is:
% \NA{We should change the notation below because I removed the subscript $k$ from $\bfA_{\calC}$. One option is to use $\calA_\calC = \begin{bmatrix}
% (\bfA_{\calC})^\top
% (\bfA_{\calC}^2)^\top
% \ldots 
% (\bfA_{\calC}^{K_c})^\top
% \end{bmatrix}$}
%
\begin{subequations}\label{eq:adaptive_prediction}
    \begin{align}
        (\calC): ~ \tilde{\bfX}_{\calC}&= \calA_\calC \bfx_0 + (\calB_{\calC} + \calB_{\calC, \bftheta} ) \tilde{\bfU}_{\calC} + \bfH_{\calC, \bftheta}\label{eq:predict_phase1}\\
        (\calF): ~ \tilde{\bfX}_{\calF}&= \calA_{\calF} \tilde{\bfx}_{K_c}+ \bfH_{\calF, \bftheta} \label{eq:predict_phase2}
     \end{align}
\end{subequations}
% \begin{subequations}\label{eq:whole_state_prediction}
%     \begin{align}
%         \textrm{(contact)} \tilde{\bfx}_{c}&= \bfA_{c}^{qp} \bfx_t + \left( \bfB_{c}^{qp} + \bfB_{c, res}^{qp} \right) \tilde{\bfu}_c + \bm{H}_{c, res} \quad \label{eq:predict_phase1}\\
%         \textrm{(flight)} \tilde{\bfx}_{f}&= \bfA_{f}^{qp} \tilde{\bfx}_{t+K_c}+ \bm{H}_{f, res}^{} \quad , \label{eq:predict_phase2}
%      \end{align}
% \end{subequations}
%
where
$\tilde{\bfX}_{\calC} = [\tilde{\bfx}_{1}^{\top}, \tilde{\bfx}_{2}^{\top}, ..., \tilde{\bfx}_{K_c}^{\top}]^{\top} $ and 
$\tilde{\bfX}_{\calF} = [\tilde{\bfx}_{K_c+1}^{\top}, \tilde{\bfx}_{K_c+2}^{\top}, ..., \tilde{\bfx}_{K}^{\top}]^{\top} $ denote the concatenation of predicted states belonging to the contact and flight phase, respectively. The matrices $\calA_{\calC}$ and $\calA_{\calF}$ are computed as
% $\bfA_{\calC}= \begin{bmatrix}
% \bfA_k^1\\
% \bfA_k^2\\
% \vdots \\
% \bfA_k^{K_c}
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x}$, 
%
% \[\left\{
%   \begin{array}{lr}
%     \calA_{\calC}= \begin{bmatrix}
% (\bfA_{\calC})^\top
% (\bfA_{\calC}^2)^\top
% \ldots 
% (\bfA_{\calC}^{K_c})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x},  \\
% \calA_{\calF}= \begin{bmatrix}
% (\bfA_{\calF})^\top
% (\bfA_{\calF}^2)^\top
% \ldots 
% (\bfA_{\calF}^{K_{\calF}})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_{\calF} \times n_x}.
% \end{array}
% \right.
% \]
\rebut{
\[\left\{
  \begin{array}{lr}
    \calA_{\calC}= \begin{bmatrix}
(\bfA_{\calC})^\top
(\bfA_{\calC}^2)^\top
\ldots 
(\bfA_{\calC}^{K_c})^\top
\end{bmatrix} \in \mathbb{R}^{7 K_c \times 7},  \\
\calA_{\calF}= \begin{bmatrix}
(\bfA_{\calF})^\top
(\bfA_{\calF}^2)^\top
\ldots 
(\bfA_{\calF}^{K_{\calF}})^\top
\end{bmatrix} \in \mathbb{R}^{7 K_{\calF} \times 7}.
\end{array}
\right.
\]
}
%
\rebut{While we use the current robot state for training the neural networks $\lbrace \bfG_{\bftheta}$, $\bfh_{\bftheta}\rbrace$ as presented in Sec. \ref{sec:adaptive-frequency-learning}, we utilize the reference trajectory ($\bfx_{k}^*, \bfr_{k}^* $) in future MPC horizons for guiding the MPC since the future robot states are not available at each MPC update (\cite{continuous_jump_bipedal,YanranDingTRO, GabrielICRA2021,ZhitaoIROS22, park2017high}). 
% we utilize the reference trajectory ($\bfx_{k}^*, \bfr_{k}^* $) in future horizons for guiding MPC to track reference. 
The reference will be used to compute the output of the neural networks $\bfG_{\bftheta}$ and $\bfh_{\bftheta}$ in future horizons. }
\rebut{In particular, we still use the current robot state and foot position $(\bfx_0, \bfr_{0})$ to evaluate the residual term $\bfB_{\bftheta,0} = \bfG_{\bftheta}(\bfx_0, \bfr_{0}) \Delta t_0 $ for each MPC update, then define 
$\bfB_{\bftheta,k} = \bfG_{\bftheta}(\bfx_{k}^*, \bfr_{k}^*) \Delta t_k$, $k = 1,..., K_{\calC}$. }\redst{We estimate the residual terms via where $\bfx_{k}^*, \bfr_{k}^* $ are the reference states and foot positions, }
% \NA{I think we should explain the use of the reference trajectory here, rather than at the end of this section.}. 
\rebut{In (\ref{eq:predict_phase1}), we obtain $[\calB_{\calC}]_{\lbrace m,n \rbrace} =   \bfA_{\calC}^{m-n} \bfB_{n-1}$ and its residual $\left[\calB_{\calC, \bftheta}\right]_{\lbrace m,n \rbrace} = \bfA_{\calC}^{m-n} \bfB_{\bftheta,n-1} ~ \textit{if} ~ m \geq n, \textit{and} ~ \bm{0} ~ \textit{otherwise}.$}
\redst{\begin{equation}
     \begin{array}{lr}
    [\calB_{\calC}]_{\lbrace m,n \rbrace} ~~=   \bfA_{\calC}^{m-n} \bfB_{n-1}  ~~~ \textit{if} ~ m \geq n, \textit{and} ~ \bm{0} ~ \textit{otherwise}  \\
   \left[\calB_{\calC, \bftheta}\right]_{\lbrace m,n \rbrace} = \bfA_{\calC}^{m-n} \bfB_{\bftheta,n-1} ~ \textit{if} ~ m \geq n, \textit{and} ~ \bm{0} ~ \textit{otherwise}
     \end{array}  \nonumber
\end{equation}}

% \[[\bfB_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{k+n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise},
%   \end{array}
% \right.
% \]
% \[[\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{\bftheta,k+n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise}.
%   \end{array}
% \right.
% \]
% \[[\bfB_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise},
%   \end{array}
% \right.
% \]
% \[[\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{\bftheta,n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise}.
%   \end{array}
% \right.
% \]
% with $m,n$ from 1 to $K_c$
% and 
% $\bfA_{f}^{qp}= \begin{bmatrix}
% \bfA_k^1\\
% \bfA_k^2\\
% \vdots \\
% \bfA_k^{N_f}
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x}$, 
% % $\bfA_t = \bfI+ \bfA_c \delta t_f$
%
%
% $\bfA_{\mathcal{F}}= \begin{bmatrix}
% (\bfA_{\calF,k})^\top
% (\bfA_{\calF,k}^2)^\top
% \ldots 
% (\bfA_{\calF,k}^{K_{\calF}})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_{\calF} \times n_x}$, 
%
% and residual matrix 
% \begin{equation}
%     \bm{\phi}_{c, res} = \bfB_{c,res}^{qp} \tilde{\bfu}_c
% \end{equation}
% \begin{equation*}
%     \bm{\psi}_{\calC,\bftheta} = \begin{bmatrix}
% \bfI & \bm{0} & \ldots & \bm{0}\\
% \bfA_{c,k} & \bfI & \ldots & \bm{0} \\
% \vdots \\
% \bfA_{c,k}^{K_c-1} & \bfA_{c,k}^{K_c-2} & \ldots & \bfI
% \end{bmatrix} \begin{bmatrix}
% h_{\bftheta}(\bfx_k, \bfr_{k})\\
% h_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*)\\
% \vdots \\
% h_{\bftheta}(\bfx_{k+K_c-1}^*, \bfr_{k+K_c-1}^*)
% \end{bmatrix} 
% \end{equation*}
%
%
%
\rebut{For the sake of notation, we define $\chi_k =(\bfx_k, \bfr_k)$, $\chi_k^* =(\bfx_k^*, \bfr_k^*)$ as the actual and reference robot state and foot trajectory. The residual matrix $\bfH_{\calC, \bftheta}$ in (\ref{eq:adaptive_prediction}) is $\bfH_{\calC,\bftheta} =  \Delta t_{\calC}$ $\mathbf{S}_{\calC} \left[
\bfh_{\bftheta}(\chi_0)^{\top}~
\bfh_{\bftheta}(\chi_1^*)^{\top}~...~
\bfh_{\bftheta}(\chi_{K_c-1}^*)^{\top}
\right]^{\top}$,} 
\redst{The residual matrix $\bfH_{\calC, \bftheta}$ in (\ref{eq:adaptive_prediction}) is $\bfH_{\calC,\bftheta} =  \Delta t_{\calC}$ $\mathbf{S}_{\calC} \left[
\bfh_{\bftheta}(\bfx_0, \bfr_{0})^{\top}~
\bfh_{\bftheta}(\bfx_{1}^*, \bfr_{1}^*)^{\top}~...~
\bfh_{\bftheta}(\bfx_{K_c-1}^*, \bfr_{K_c-1}^*)^{\top}
\right]^{\top}$,} 
\rebut{where $\bfS_{\calC}$ is lower triangular matrix with each entry $[\bfS_{\calC}]_{\lbrace m,n \rbrace} = \bfA_{\calC}^{m-n} \in \mathbb{R}^{7 \times 7}$, $m \geq n$. }\rebut{The residual matrix 
$\bfH_{\calF,\bftheta} = \Delta t_{\calF} \bfS_{\calF} \left[
\bfh_{\bftheta}(\chi_{K_c}^{*})^{\top} \quad
\ldots \quad 
\bfh_{\bftheta}(\chi_{K}^*)^{\top}
\right]^{\top}$}
\redst{$\bfH_{\calF,\bftheta} = \Delta t_{\calF} \bfS_{\calF} \left[
\bfh_{\bftheta}(\bfx_{K_c}^{*}, \bfr_{K_c}^*)^{\top}~...~ 
\bfh_{\bftheta}(\bfx_{K}^*, \bfr_{K}^*)^{\top}
\right]^{\top}$}
% where $m,n$ from 1 to $K_{\calF}$
% \begin{subequations}
% \begin{align}
%     \bfH_{\calC,\bftheta}  &= \mathbf{S}_{\calC} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_0, \bfr_{0})\\
% \bfh_{\bftheta}(\bfx_{1}^*, \bfr_{1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{K_c-1}^*, \bfr_{K_c-1}^*)
% \end{bmatrix}, \\
%     \bfH_{\calF,\bftheta} & = \bfS_{\calF} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_{K_c}^*, \bfr_{K_c}^*)\\
% \bfh_{\bftheta}(\bfx_{K_c+1}^*, \bfr_{K_c+1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{K}^*, \bfr_{K}^*)
% \end{bmatrix},
% \end{align}
% \end{subequations}
\rebut{where $\bfS_{\calF}$ is lower triangular matrix with each entry defined $[\bfS_{\calF}]_{\lbrace m,n \rbrace} = \bfA_{\calF}^{m-n} \in \mathbb{R}^{7 \times 7}$, $m \geq n$.} 
% \[[\bfS_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% \begin{equation}
%     \bm{\psi}_{\calF,\bftheta} = \begin{bmatrix}
% \bfI & \bm{0} & \ldots & \bm{0}\\
% \bfA_{f,k} & \bfI & \ldots & \bm{0} \\
% \vdots \\
% \bfA_{f,k}^{N_f} & \bfA_{f,k}^{N_f-1} & \ldots & \bfI
% \end{bmatrix} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_{k+K_c}^*, \bfr_{k+K_c}^*)\\
% \bfh_{\bftheta}(\bfx_{k+K_c+1}^*, \bfr_{k+K_c+1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{k+N}^*, \bfr_{k+N}^*)
% \end{bmatrix}
% \end{equation}
% where $m,n$ from 1 to $K-K_c$
% \[[\bfS_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% \begin{align}
% \tilde{\bfx}_{k+K_c}= & \bfA_{\calC,k}^{K_c} \bfx_k + \sum_{i=0}^{K_c-1} \bfA_{\calC,k}^{K_c-1-i} \left (\bfB_{k+i} + \bfB_{\bftheta, k+i} \right) \tilde{\bfu}_{k+i}, \nonumber
% \end{align}
The state prediction at the end of $K_{\calC}$ steps can be computed as
%
\begin{equation}\label{eq:x_kNc}
    \tilde{\bfx}_{K_c}= \bfA_{\calC}^{K_c} \bfx_0 + (\bfS + \bfS_{\theta}) \tilde{\bfU}_{\calC} + \bm{\phi}_{\bftheta}, 
\end{equation}
%
where $\bfS = \left[\bfA_{\calC}^{K_c-1}\bfB_0 \quad \bfA_{\calC}^{K_c-2}\bfB_{1} \quad ... \quad \bfB_{K_c-1}  \right] $, $\bfS_{\bftheta} = \left[\bfA_{\calC}^{K_c-1}\bfB_{\bftheta,0} \quad \bfA_{\calC}^{K_c-2}\bfB_{\bftheta,1} \quad ... \quad \bfB_{\bftheta,K_c-1}  \right] $,  and $\bm{\phi}_{\bftheta} = \left[\bfA_{\calC}^{K_c-1}\bfh_{\bftheta,0} \quad \bfA_{\calC}^{K_c-2}\bfh_{\bftheta,1} \quad ...\quad \bfh_{\bftheta,K_c-1}  \right]$.\redst{Substituting \eqref{eq:x_kNc} into \eqref{eq:predict_phase2} yields:} \rebut{Substituting \eqref{eq:x_kNc} into \eqref{eq:adaptive_prediction} yields the state prediction as}
\begin{equation} \label{eq:state_prediction2}
    \tilde{\bfX}_{\calF}= \bfA_{\calF} \bfA_{\calC}^{K_c} \bfx_0+ \bfA_{\calF} (\bfS + \bfS_{\theta}) \tilde{\bfU}_{\calC}  + \bfA_{\calF} \bm{\phi}_{\bftheta} +  \bfH_{\calF, \bftheta}.
\end{equation}
% Then, the state predictions for $K$ steps becomes:
\begin{equation}
    \tilde{\bfX} = \begin{bmatrix}
        \tilde{\bfX}_{\calC} \\ \tilde{\bfX}_{\calF}
    \end{bmatrix} = \bfA_{\text{qp}} + \left(\bfB_{\text{qp}} + \bfB_{\bftheta,\text{qp}}\right) \tilde{\bfU} + \bfH_{\bftheta}
\end{equation}
% $\bfS , \bfS_{\bftheta} \in \mathbb{R}^{n_{\bfx} \times (n_{\bfu} \times K_c)}$. 
% Substituting $\tilde{\bfx}_{k+K_c}$ to equation (\ref{eq:predict_phase2}), we obtain $\tilde{\bfx}_{f,k}$.
% \subsection{Training}
% - data collection (hybrid) \\
% - data augmentation (duplicate data) \\
% - neural network architecture  \\
% - loss function \\
% - gradient descent \\
% The solution $\bm{f}_{MPC}^*$ that takes the value at the first horizon of solution $\bm{F}_t$ will be utilized to compensate for the errors between actual and reference jumping:
% \begin{align} \label{eq:delta_MPC}
%     \Delta \bm{\tau}_{MPC}=\bm{J}(\bfq_{j})^\top \bfr^\top[\bm{f}_{MPC}^* - \bm{f}_{d}],
% \end{align} 
% where $\bm{J}(\bfq_{j})$ is the foot Jacobian at the configuration $\bfq_{j}$; $\bfr$ is the rotation matrix which transforms from body
% to world frame. The compensation $\Delta \bm{\tau}_{MPC}$ will be combined with the high frequency joint PD controller, leveraging the reference of the torque $\bm{\tau}_d$ and joint profiles $ \{\bfq_{J,d}, \bm{\dot q}_{J,d} \}$ obtained from the trajectory optimization. This results in a feed forward torque applying to the robot actuators:
% \begin{align} \label{eq:MPC_feedforward_torque}
%     \bm{\tau}_{ff}= \bm{\tau}_d + \bm{\tau}_{PD}^{joint} + \Delta \bm{\tau}_{MPC},
% \end{align} 
% \begin{align}
% \bm{\tau}_{PD}^{joint} = \bm{K}_{p,j}(\bfq_{J,d}-\bfq_J)+\bm{K}_{d,J}(\bm{\dot q}_{J,d}-\bm{\dot q}_J)
% \end{align} \label{eq:jointPDController}


% \begin{subequations} \label{eq:MPC_jumping}
% \begin{align}
%  \textrm{min} \textrm{ } & \sum_{k=t}^{t+N-1} \| \bfx_k-\bfx_{d,k} \|_{P_k} + \| \bm{f}_k-\bm{f}_{d,k} \|_{Q_k},\\
% % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% \text{s.t. }
%              & \bfx_{k+t}=\Psi_k (\bfx_k)+ \phi_k (\bm{f}_k), \label{eq:MPC_jumping_c1} \\
%              & \bm{c}_k^{min} \leq \bm{C}_k \bm{f}_k \leq \bm{c}_k^{max}, \label{eq:MPC_jumping_c2} \textrm{(friction cone)}  \\ 
%              & \bm{D}_k \bm{f}_k =\bm{0} ~\label{eq:MPC_jumping_c3} \textrm{(contact phases)}
% \end{align}
% \end{subequations}
% where a contact force reference $\bm{f}_d$ and body trajectory reference $\bfx_d$ are obtained from trajectory optimization; $P_k$ and $Q_k$ are the weighted diagonal matrices at step $k$; $N$ is a number of predicted horizon. The equation (\ref{eq:MPC_jumping_c2}) captures constraints related to friction cone and force limits, while the equation (\ref{eq:MPC_jumping_c3}) is represented for the shifting contact schedule.


% \subsection{Approach}
% \begin{itemize}
%     \item Nonlinear functions $\Psi_k$ and $\phi_k$ in (\ref{eq:MPC_jumping}) are learned from data, either using Eq. \eqref{eq:var_int_Rn} for 2D jumping or Eq. \eqref{eq:_var_int_SE3} for 3D jumping.
%     \item The long-term prediction of Eq. \eqref{eq:var_int_Rn} and Eq. \eqref{eq:_var_int_SE3} will benefit MPC.
%     \item Linearization would be required and have to handle neural networks, and hopefully we are able to reformulate the MPC problem as QP problem for fast solving.
% \end{itemize}

% \begin{figure*}[!t]
% 	\centering
% 	\resizebox{0.9\linewidth}{!}{\includegraphics[trim={0cm 6cm 0cm 0cm},clip]{Figures/framework.pdf}}
% 	\caption{Block diagram for the proposed framework.} 
% 	\label{fig:framework}
% \end{figure*}

% \begin{figure}[!t]
% 	\centering
% 	{\centering
% 		\resizebox{0.9\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{Figures/framework.pdf}}
% 	}
% 	\caption{\textbf{Periodic jumping phases}. Each periodic jumping motion consists of four phases}
% 	\label{fig:contact_schedule}
% \end{figure}

% \section{Setting Discussion}

% \begin{itemize}
%     \item To enable fast computation, we prefer to implement to MPC in C++. The learned model by Pytorch will be use to predict states in MPC formulation in ROS. However, we currently do not have a interface for Pytorch-learned-model with MPC in ROS.
%     \item We currently have MPC for jumping in C++ (ROS and hardware experiments), which is based on single rigid body dynamics represented via Euler angles. Thus, to implement 3D juming, additional implementation work is required to use rotation matrix instead of Euler angles. 
% \end{itemize}
% \subsubsection{\textcolor{blue}{Real-time Optimization}}

where, $\bfA_{\text{qp}} = \begin{bmatrix}
    \calA_{\calC} \\ \calA_{\calF} \bfA_{\calC}^{K_c}
\end{bmatrix}$, $\bfB_{\text{qp}} = \begin{bmatrix}
    \calB_{\calC} & \bf0 \\
    \calA_{\calF} \bfS & \bf0
\end{bmatrix}$, $\bfB_{\bftheta,\text{qp}} = \begin{bmatrix}
    \calB_{\calC,\bftheta} & \bf0 \\
    \calA_{\calF} \bfS_{\bftheta} & \bf0
\end{bmatrix}$, $\bfH_{\bftheta} = \begin{bmatrix}
    \bfH_{\calC, \bftheta} \\
    \bfH_{\calF, \bftheta} + \calA_{\calF} \bm{\phi}_{\bftheta}
\end{bmatrix}$, and $\tilde{\bfU} = \begin{bmatrix}
    \tilde{\bfU}_{\calC} \\
    \tilde{\bfU}_{\calF}
\end{bmatrix} $.
% \NA{Use comments before and after equations to avoid new lines being produced by latex.} 
% \NA{Why do we distinguish the contact prediction mode and the adaptive prediction mode? Should we describe only one of these?}

% \begin{subequations} \label{eq:MPC_learned_QPcompact}
% \begin{align}
%  \textrm{min} \textrm{ } &  \| \tilde{\bfX}_k-\bfX_{k}^* \|_{\bfP_k} + \| \tilde{\bfU}_k-\bfU_{k}^* \|_{\bfQ_k},\\
% % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% \text{s.t. }
%              & \tilde{\bfX}_{k} = \bfA_{qp} + \left(\bfB_{qp} + \bfB_{\bftheta,qp}\right) \tilde{\bfU}_k + \bfH_{\bftheta} \\
%              & \bm{c}_{\Sigma,k}^{min} \leq \bm{C}_{\Sigma,k} \tilde{\bfU}_k \leq \bm{c}_{\Sigma,k}^{max}, \label{eq:MPC_jumping_c2_learn} \\ 
%              & \bm{D}_{\Sigma,k} \tilde{\bfU}_k =\bm{0}, \label{eq:MPC_jumping_c3_learn} \forall k=t, ..., t+N-1
% \end{align}
% \end{subequations}
The objective of the MPC in \eqref{eq:MPC_learned} can be rewritten as:
\begin{equation}
    J(\bfU) = \| \tilde{\bfX}-\bfX^* \|_{\bfP}^2 + \| \tilde{\bfU}-\bfU^* \|_{\bfQ}^2,
\end{equation}
leading to a quadratic program (QP):
%formulation of the MPC 
%\eqref{eq:MPC_learned}
%Then, the MPC formulation (\ref{eq:MPC_learned}) can be formulated as the Quadratic Programming for solving in real-time as follows:
\begin{equation}\label{eq:MPC_learned_QPcompact}
\begin{aligned}
& \underset{\bfU}{\text{min}}
& & \bfU^{\top} \bfalpha \bfU + \bfbeta^\top \bfU  \quad \text{s.t.} \;\;\bfU_k \in \calU_k,
\end{aligned}
\end{equation}
where 
% \NA{It would be nice to use capital letters for $\bfalpha$ and $\bfbeta$}
\begin{equation*}
    \begin{aligned}
        \bfalpha &= (\bfB_{\text{qp}}+ \bfB_{\bftheta,\text{qp}}) 
 ^{\top} \bfQ (\bfB_{\text{qp}}+ \bfB_{\bftheta,\text{qp}}) + \bfR, \\ 
        \bfbeta &= 2 (\bfB_{\text{qp}}+ \bfB_{\bftheta,\text{qp}}) 
 ^{\top} \bfQ \left( \bfA_{\text{qp}} \bfx_{k} + \bfH_{\bftheta}- \bfX^* \right) -\bfR \bfU^*,\\
        \calU_k &= \{ \bfu \in \bbR^4 \mid \underline{\bfc}_k \leq \bfC_k \bfu_k \leq \bar{\bfc}_k, \bfD_k \bfu_k =\bm{0}\}.
    \end{aligned}
\end{equation*}

%Since the future robot states are not available at each MPC update, we utilize the reference trajectory to compute the output of the neural networks
% \NA{Which neural networks? We should be more precise.}. 
\rebut{
% This QP formulation of the learning-based MPC enables real-time execution of jumping maneuvers. In addition, as we only learn the residual dynamics, i.e. still keeping the nominal dynamics into account, we still provide a degree of stability and robustness while we expect the actual trajectory to be close to the reference trajectory. 
% By contrast, learning the dynamics from scratch normally requires a large dataset, and heavyweight neural networks, and the neural networks may output bad predictions when the model is not learned well.
}

% \todo{Mention the QP solving explicitly}

% \note{To execute the jumping, we apply the same control structure as data collection described in Sec. \ref{subsec:data_gen}}. The solution obtained from the MPC $\bfu_{mpc}$ will be offset with the reference force $\bfu_d$, which then be combined with reference torque $\bm{\tau}_d$ and low-level feedback joint torque $\bm{\tau}_{pd,j}$ to apply to the robot motor as



% \begin{align} \label{eq:applied_torque}
%     \bm{\tau}_{t}= \bm{\tau}_{d} + \bm{\tau}_{pd,j} + \Delta \bm{\tau}_{mpc}
% \end{align} 
% where
% \begin{align}
%  \Delta \bm{\tau}_{mpc}  &=  \bm{J}(\bfq_{j})^\top \bfR^\top[\bfu_{mpc}^* - \bfu_{d}],  \\
% \bm{\tau}_{pd,j} & = \bm{K}_{p,j}(\bfq_{j,d}-\bfq_j)+\bm{K}_{d,j}(\bm{\dot q}_{j,d}-\bm{\dot q}_j)
% \end{align} \label{eq:jointPDController}	
	
% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-026.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-030.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-067.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ fixed frequency}: Motion snapshots from a jump forward $60~cm$ under unknown ground perturbation. This jumping is executed by MPC with fixed time step $\delta t = 25ms$ for nominal model.} 
% 	\label{fig:ros-mpc-fixfreq-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-001.png}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-012.png}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-014.png}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-034.png}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ adaptive frequency}: Motion snapshots from a jump forward $60~cm$ under unknown ground perturbation. This jumping is executed by MPC with adaptive frequency update $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms $ for nominal model.} 
% 	\label{fig:ros-mpc-adaptfreq-nominal-snapshots}
% \end{figure*}
% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-028.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-034.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-048.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ adaptive frequency}:Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms $ for learned model.} 
% 	\label{fig:ros-mpc-adaptfreq-learn-snapshots}
% \end{figure*}






\section{Evaluation}
\label{sec:results}

% We verify the effectiveness of our model learning and real-time control techniques for quadruped jumping tasks.



% \begin{table}[t!]
% %	\hspace{0.2cm}
% 	\centering
% 	\caption{A1 Robot Parameters}
% 	\label{tab:PRP}
% 	\begin{tabular}{cccc}
% 		\hline
% 		Parameter & Symbol & Value & Units\\
% 		\hline
% 		Trunk dimension & $l,w,h$ & 0.361, 0.194, 0.114 & $\unit{m}$ \\[.5ex]
% 		Trunk Inertia  & $I_{xx},I_{yy},I_{zz}$  & 0.017, 0.056, 0.065 & $\unit{kg}.\unit{m}^2$ \\[.5ex]
% 		Leg Link Lengths & $l_{1}, l_{2}$ & 0.2 & $\unit{m}$ \\[.5ex]
% 		\hline 
% 	\end{tabular}
% \end{table}







% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0139.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0172.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0201.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ fix frequency}: Motion snapshots from a failure to jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC 5fix frequency for nominal model.} 
% 	\label{fig:mpc-fixfreq-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0141.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0172.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0189.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ adaptive frequency}: Motion snapshots from a failure to jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency for nominal model.} 
% 	\label{fig:mpc-adaptive-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0141.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0194.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0210.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ adaptive frequency}: Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency for learning adaptive model.} 
% 	\label{fig:mpc-adaptive-learn-snapshots}
% \end{figure*}
% \begin{figure*}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/fcmd_new/separate/contact/roll_out.eps}}}\\
%     \caption{\textbf{Rolling out state prediction during $K=10$ horizons that belongs to scheduled contact phase:} The figures show comparisons between the prediction of learned model (blue lines), the nominal model (green lines), and the ground-truth trajectory (black lines).} 
%     \label{fig:roll_out_contact}
% \end{figure*} 
% \begin{figure*}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/fcmd_new/hybrid/roll_out.eps}}}\\
%     \caption{\textbf{Rolling out prediction for contact and flight phase with adaptive frequency} Comparison between the prediction of our neural network, the nominal model, and the ground-truth trajectory. \textcolor{blue}{PENDING: Abdullah will add a prediction with fixed frequency}} 
%     \label{fig:roll_out_hybrid}
% \end{figure*} 
% \begin{figure*}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/rollouts/rollout_2.pdf}}}\\
%     \caption{\textbf{Rolling out predictions for contact and flight phase on a random dataset.} Comparison between the prediction of our neural networks for learned model with adaptive frequency, learned model with fixed frequency, nominal model with adaptive frequency, and the ground-truth trajectories (labels).} 
%     \label{fig:roll_out_hybrid}
% \end{figure*} 
% \Abdullah{Chuong, the prediction plots have been added.}




% \begin{figure}[t]
%     \centering
%     \begin{minipage}[b]{1.0\linewidth} 
%         \centering
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\textwidth]{figures/Training/ftotal_mpc_pd/loss.eps}
%         \caption{\textbf{Training loss and testing loss (Log scale).}}
%         \label{fig:loss}
%     \end{minipage}
%     \vspace{2em}
%     \begin{minipage}[b]{0.9\linewidth} 
%         \centering
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\textwidth]{figures/Training/rollouts/rollout_5.pdf}
%         \caption{\textbf{State prediction comparison on a random testing dataset} among the learned model with adaptive frequency (our method), learned model with a fixed frequency, nominal model with adaptive frequency, and the ground-truth trajectories.}
%         \label{fig:roll_out_hybrid}
%     \end{minipage}
% \end{figure}

% with parameters and actuation capabilities summarized in Table \ref{tab:motor_batterry}.


\subsection{Experiment Setup}

We evaluated our approach using a A1 robot. \rebut{To get data for real-time control, we utilized a motion capture system}\redst{we utilized an Optitrack motion capture system with five Optitrack Prime $13W$ cameras} for estimating the position and orientation of the robot trunk at $1$ kHz with position errors of $1$ mm. \rebut{We obtain velocity data from position data using forward finite-difference method.}
%We validate our approach using a Unitree A1 robot. To collect real-world data, we utilized an Optitrack motion capture (MoCap) system to estimate the position and orientation of the robot trunk, instead of relying on the robot's IMU, which normally provides inaccurate estimates during the flight phase. The MoCap system consists of five Optitrack Prime $13W$ cameras, providing tracking at a frequency of $1$ kHz with position errors of at most $1$ mm.
%

We used \textit{Pytorch} to implement and train the residual dynamics model. The trained \textit{Pytorch} model was converted to a torch script trace, which in turn, was loaded in our MPC implementation in C++. \rebut{The MPC is solved by a QP solver (qpOASES)}.
We utilized the optimization toolbox 
\rebut{\textit{CasADi}} \cite{casadi} to set up and solve the full-body TO for various jumping targets within $[0.3, 0.8]$ m on a flat ground. We considered jumping motions with contact phase (C) consisting of an all-leg contact period (e.g., $500$ ms) and a rear-leg contact period (e.g., $300$ ms). With the flight phase (F) scheduled for $400$ ms, the front legs and rear legs become swing legs (SW) up to $58\%$ and $33\%$ of the entire jumping period, respectively. Jumping maneuvers feature long flight phases, i.e., the robot can jump up to $4$ times its normal standing height during the mid-air period. \rebut{All jumping experiments are executed with sufficient battery level ($>90\%$)}

% For all jumps, we consider the contact schedule for the contact and flight phase as $cs = \lbrace 800, 400\rbrace $ (ms). The contact phase consists of the all-leg contact period for the first $500~ms$ and the rear-leg contact period for $300~ms$. Thus, the front and rear legs are supposed to be the swing leg (SW) for $700~ms$ and $400~ms$, which is up to $58\%$ and $33\%$ period of the total jump.

% The reference from trajectory optimization will then be tracked by the proposed MPC under unknown disturbance (e.g. box under feet).

% \begin{figure}
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/ftotal_mpc_pd/loss.eps}}}\\
%     \caption{\textbf{Training loss and testing loss (Log scale).}} 
%     \label{fig:loss}
% \end{figure} 

% In the neural network architechture, we select


% \begin{figure*}[!t]
% 	\centering
% 	{\centering
% 		\resizebox{\linewidth}{!}{\includegraphics[trim={0cm 4.5cm 0cm 7cm},clip]{figures/Exp/v2/Comparison_Exp_onbox.pdf}}
% 	}
% 	\caption{
% 	\textbf{Jumping on a box:} Comparison among full-body TO, nominal-model MPC with fixed and adaptive frequency, and learned-model MPC with fixed and adaptive frequency. All MPC problems were solved with horizon $K=10$.} 
%  % The actual trajectories are recorded in Fig. \ref{fig:traj_compare_box_jumping}}
% 	\label{fig:box_jumping}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	{\centering
% 		\resizebox{\linewidth}{!}{\includegraphics[trim={0cm 4.5cm 0cm 7.5cm},clip]{figures/Exp/v2/Comparison_Exp_d60.pdf}}
% 	}
% 	\caption{
% 	\textbf{Forward jumping from uneven terrain:} Comparison among full-body TO, nominal-model MPC and learned-model MPC with fixed and adaptive frequency. All MPC problems were solved with horizon $K=10$. A $5$ cm block ($30\%$ of the robot's initial height) was introduced under the robot's front feet. With adaptive-frequency learned-model MPC (our method), the robot is able to compensate for the disturbance and jump over the block successfully.}
% 	\label{fig:forward_60cm}
% \end{figure*}



\subsection{Data Collection and Training}
\begin{table}[t]
	\centering
	\caption{Training Parameters}
	\begin{tabular}{ccc}
		\hline
		Parameter & Symbol & Value\\
		\hline
        \rebut{Variable time steps} & $\Delta t _{\calC}, \Delta t _{\calF} $ & $\lbrace 25, 100 \rbrace (ms)$ \\[.5ex]
        Prediction steps & $K$ & $10$ \\[.5ex]
		NN architecture & $\bfh_{\bftheta_1}(\mathbf\frakq, \bfr)$ & $7$ - $400$ Tanh - $400$ Tanh - $3$ \\[.5ex]
  		 & $\bfG_{\bftheta_1}(\mathbf\frakq, \bfr)$ & $7$ - $1000$ Tanh - $1000$ Tanh - $12$ \\[.5ex]
              & $\bfh_{\bftheta_2}(\mathbf\frakq, \bfr)$ & $7$ - $400$ Tanh - $400$ Tanh - $3$ \\[.5ex]
        Learning rate & $\gamma$ & $2.10^{-4}$ \\[.5ex]
        Regulation weights & $\alpha_1, \alpha_2$ & $10^{-3},10^{-3}$ \\[.5ex]
        % Learning rate & $\gamma$ & $2.10^{-4}$ \\[.5ex]
        Total training steps & $N_{train}$ & $2.10^{4}$ \\[.5ex]
		\hline 
		\label{tab:training_params}
	\end{tabular}
  \vspace{-2.2em}
\end{table}

\begin{figure}
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.45\textwidth]{figures/Training/ftotal_mpc_pd/loss_log.pdf}
\caption{\textbf{Training loss and testing loss (Log scale).}}
\label{fig:loss}
\vspace{-0.7cm} 
\end{figure}



% The jumping includes contact and flight phase, with a contact schedule $cs = \lbrace 800, 400\rbrace $ (ms) respectively.
% \todo{Explain how we train model with Pytorch, and how we load the model in C++}
% Baseline MPC based on the nominal model, as described in Section \ref{subsec:data_gen}), is implemented for tracking a set of jumping references from the full-body TO under a variety of unknown disturbances (i.e. box under feet with random height within $[0, 8]cm$).
\textcolor{black}{We aim to learn a residual dynamics model that is not trajectory-specific and can generalize to a whole family of forward jumps. To collect a sufficient dataset for training, we utilized a baseline MPC controller with a nominal model (Sec. \ref{subsec:data_gen}) to generate diverse trajectories under a variety of unknown disturbances (box under the front feet with random height within $[0, 8]$ cm) and zero-height jumping targets.}
% A baseline MPC controller using the nominal model, described in Sec. \ref{subsec:data_gen}, was implemented to generate jumping trajectories under a variety of unknown disturbances (i.e. box under feet with random height within $[0, 8]$ cm) and \rebut{zero-height targets}.
% \cite{continuous_jump}. 
% The MPC is adopted from our prior work \cite{continuous_jump}, which lumps the robot dynamics as a single rigid body model (i.e. nominal model). 
We collected data from $H=20$ jumps with $80\%$ for training and $20\%$ for testing. The data points were sampled with variable sampling time  $\Delta t _{\calC} = 25$ ms, $\Delta t_{\calF} = 100$ ms, and horizon length of $K=10$. 
\redst{The dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consisted of $D = 20\times 28$ state-control sequences for training. }
% of $\bfx^{(i)}_{0:K}$, foot position $\bfr^{(i)}_{0:K}$, and control input $\bfu^{(i)}_{0:K}$.
% Each subset consists of robot states and controls for $K$ horizon. 
% It is noted that these sequences do not necessarily have the same length of time due to the adaptive-frequency sampling policy.
% As the robot dynamics in our settings are translation-invariant, e.g., the dynamics do not depend on the robot position, we offset the data sequences to start from the origin and train the dynamics model around the origin.


% has a dimension of $7$ that 


The training parameters are listed in Table \ref{tab:training_params}. We used fully-connected neural networks with architectures listed in Table \ref{tab:training_params}: the first number is the input dimension, the last number is the output dimension, and the numbers in between are the hidden layers' dimensions and activation functions. 
\redst{For all networks, the input consists of body position, body orientation, and foot position w.r.t the body's CoM in the world frame. }\redst{Note that }The output of $\bfG_{\bftheta_1}$ is then converted to a $3\times4$ matrix. The training and testing losses are illustrated in Fig. \ref{fig:loss}. 
% \begin{enumerate}
% 	\item Contact phase:
% 		\begin{itemize}
% 		\item $\bfh_{\bftheta_1}(\mathbf\frakq, \bfr)$ : $7$ - $400$ Tanh - $400$ Tanh - $3$.
% 		\item $\bfG_{\bftheta_1}(\mathbf\frakq, \bfr)$ $7$: - $400$ Tanh - $400$ Tanh - $12$. The output of $\bfG_{\bftheta_1}$ is then converted as a matrix of size $(3,4)$
% 	\end{itemize}

% 	\item Flight phase:
% 	\begin{itemize}
% 	\item $\bfh_{\bftheta_2}(\mathbf\frakq, \bfr)$ : $7$ - $400$ Tanh - $400$ Tanh - $3$.
% 	\end{itemize} 
% \end{enumerate}
% The training takes approximately $10 mins$ on GPU

% \subsection{Testing}



% \begin{figure}
%     \centering
%     {\centering
%         % \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/time.eps}}}\\
%         \resizebox{1.1\linewidth}{!}{\includegraphics[trim={1cm 0cm 0cm 0.cm},clip]{figures/ROS/compare_horizon/time.pdf}}}\\
%     \caption{Solving time for MPC ($t_{MPC}$) with different horizons $K=10$ and $K=22$, respectively. The red dashed line denotes the sampling time of $25$ ms to execute MPC. Real-time performance is achieved if $t_{MPC}$ is much less than the sampling time.} 
%     \label{fig:computational_time}
% \end{figure} 


\begin{figure}
\centering
    \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.48\textwidth]{figures/Training/rollouts/rollout_12x8.pdf}
    \caption{\textbf{State prediction comparison on a random testing dataset}.  \rebut{It starts at $650$ ms, consisting of $K_c = 6$ steps in the contact phase and $K_f = 4$ steps covering the flight period of $400$ ms. The blue and yellow areas represent the contact and flight periods, respectively. We compare variable-frequency learned model (our method), fixed-frequency learned model, variable-frequency nominal model, and the ground-truth trajectories. The ground-truth data is directly obtained from hardware experiments.}}
    \label{fig:roll_out_hybrid}
    \vspace{-0.3cm} 
\end{figure}
\begin{figure} % left, down, right, up
    \centering
    {\centering
        % \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/time.eps}}}\\
        \resizebox{1.1\linewidth}{!}{\includegraphics[trim={2.5cm 11.8cm 1cm 11.8cm},clip]{figures/ROS/compare_horizon/time1.pdf}}}\\
    \caption{\rebut{MPC solving time ($t_{MPC}^{sol}$) with various horizons $K=10$ and $K=22$. The red dashed line denotes the MPC update time ($1/f_{MPC}^{upd}$) of $25$ ms. Real-time performance is achieved if $t_{MPC}^{sol}<<1/f_{MPC}^{upd}$.}}
    \label{fig:computational_time}
    \vspace{-0.2cm} 
\end{figure} 

\begin{figure}[!ht]
\centering
\includegraphics[trim={0.6cm 0cm 0.4cm 0cm},clip,width=0.5\textwidth]{figures/Exp/compare_mpc_tasks2.eps}
    \caption{\rebut{Comparison of error of final target jumping (in cm) for four real-time MPC setups with different models and timesteps resolutions in a total of $92$ jumps with robot hardware. Positive values indicate that the jumps fall short of the target. The cross (\textcolor{red}{$\times$}) denotes failure to jump on the box. Supplemental video: \url{https://youtu.be/2QjZkARs1mU}.}}
	\label{fig:compare_approach}
     \vspace{-0.5cm} 
\end{figure}

\begin{figure*}[!t]
	\centering
	{\centering
		\resizebox{\linewidth}{!}{\includegraphics[trim={0cm 0.3cm 0cm 0cm},clip]{figures/Exp/v2/Comparison_Exp_rebut.pdf}}
	}
	\caption{
	\textbf{Jumping from uneven terrain and Jumping on a box:} \rebut{Comparison among full-body TO, nominal-model MPC with fixed and variable frequency, and learned-model MPC with fixed and variable frequency. All MPCs have a horizon length of $K=10$. An unknown $5$ cm block ($30\%$ of the robot's initial height) was introduced under the robot's front feet (upper figures). With variable-frequency learned-model MPC (our method), the robot is able to compensate for the disturbance and perform successful jumps. Supplemental video:} \url{https://youtu.be/yUqI_MBOC6Q}.} 
 % The actual trajectories are recorded in Fig. \ref{fig:traj_compare_box_jumping}}
\label{fig:box_jumping_and_forward60_dis}
    \vspace{-0.4cm} 
\end{figure*}





\subsection{Comparative Analysis}

% We validate our proposed adaptive-frequency MPC for learned model, and make comprehensive comparisons with the utilization of nominal model and fixed MPC frequency update.
% \begin{itemize}
%     \item \textit{MPC with fixed frequency for nominal model }
%     \item \textit{MPC with adaptive frequency for nominal model }

%     \item \textit{MPC with fixed frequency for learned model}

%     \item \textit{MPC with adaptive frequency for learned model}
% \end{itemize}


% Given the accurate state prediction of learned model, we then verify the effectiveness of real-time MPC to achieve both robust and target jumping accuracy. We consider a jumping forward to the target location at $60cm$. We consider a perturbation to the initial configuration (e.g. a box under the front feet), which is unknown to controllers. 

\subsubsection{Evaluation on testing dataset}
% We validate the efficiency of neural network architecture for prediction on the test dataset. 
% The fig. 
We rolled out the learned dynamics with \rebut{variable frequency}\redst{adaptive frequency} to predict the future state trajectories and compared with \textit{(i)} those of \rebut{the variable-frequency nominal model}\redst{the nominal model with adaptive frequency}, \textit{(ii)} those of \rebut{the fixed-frequency learned model}\redst{the learned model with fixed frequency}, and \textit{(iii)} the ground-truth states in Fig. \ref{fig:roll_out_hybrid}. 
\redst{We select two \textit{random} subsets of testing data. The first starts at $525 (ms)$, leveraging a timing window of $K\Delta t_{\calC}$. This subset is within the scheduled contact phase as shown in Figure \ref{fig:roll_out_contact}. The second starts at $650 (ms)$, leveraging $K = 10$ horizons that consist of $K_c = 6$ horizon for contact phase and $K_f = 4$ horizon for flight phase, as depicted in Fig. \ref{fig:roll_out_hybrid}.} The fixed-frequency learned model is trained with $K=10$ and $\Delta t=25$ ms. The figure shows that our proposed learned model (red lines) outperforms variable-frequency nominal model (green lines) and fixed-frequency learned model (blue lines). 
% It shows that the predicted state trajectory from the learned model with \rebut{variable}\redst{adaptive} frequency (red lines) outperforms the prediction by the nominal model with \rebut{variable}\redst{adaptive} frequency (green lines) and learned model with fixed frequency (blue lines).
\rebut{We highlight a large deviation in trajectory prediction of variable-frequency nominal model with the others. This inaccuracy can be explained by the use of conventional SRBD for the entire prediction horizon and the coarse Euler integration for the flight phase. Our variable-frequency learned model helps address the inaccuracies introduced by the nominal model and keeps sufficient accuracy of trajectory prediction while allowing real-time MPC by keeping a small number of decision variables.
% For example, during contact and take-off, since the simplified dynamics ignore the significant leg movements and uncertainties in contact and hardware, the error prediction for $w$ is accumulated and can be large at the time of take-off. The error for body angle $\phi$ is then accumulated with coarse integration during the long flight phase, as can be seen in Fig. \ref{fig:roll_out_hybrid}.
}
% This covers the entire flight period of $400 ms$.
% This covers the long timing window of $K_c \Delta t_{\calC} + K_f \Delta t_{\calF}$, covering the entire flight phase of $400 ms$.
% For instance, comparing Adaptive-frequency nominal model to Adaptive-frequency learned model suggests that the learned model helps mitigate the inaccuracies introduced by using a coarse integration timestep. This allows to solve the MPC faster by keeping the number of decision variables small, while keeping prediction accuracy sufficiently accurate thanks to the learned model.


% Figure \ref{fig:roll_out_hybrid} shows that the predicted state trajectory from the learned model with \rebut{variable}\redst{adaptive} frequency (red lines) outperforms the prediction by the nominal model with \rebut{variable}\redst{adaptive} frequency (green lines) and learned model with fixed frequency (blue lines). For example, our approach reduces the prediction error in the $x$ coordinate by 8 and 5 times, respectively.




\subsubsection{Effect of prediction horizon}
Fig. \ref{fig:computational_time} compares the solving time for MPC with different horizons. With our \rebut{variable-frequency scheme}\redst{adaptive-frequency scheme}, we can use a few prediction horizons, e.g., $K=10$ ($6$ for contact and $4$ for the flight phase), allowing QP solving time for each MPC update (\eqref{eq:MPC_learned_QPcompact}) to be $2$ ms only on average. This efficient computation enables real-time performance for MPC. Using a fixed-frequency scheme with sample time of $25$ ms requires MPC to use a large number of steps, e.g. $K=22$ ($6$ for contact and $16$ for the whole flight phase). \rebut{This long horizon yields a large optimization problem, which takes $\sim$$30$ ms for each MPC update and deteriorates the real-time performance.}
\redst{This long horizon yields a large optimization problem, causing significant computational costs. It takes an average of $30$ ms for each MPC update, thus deteriorating the real-time performance.}

\subsubsection{Execution}
We verified that our proposed approach enables both robust and accurate target jumping to various targets. We compared \textit{(a)} nominal model $\&$ fixed-frequency MPC, \textit{(b)} nominal model $\&$ \redst{adaptive-frequency}\rebut{variable-frequency} MPC, \textit{(c)} fixed-frequency learned model $\&$ fixed-frequency MPC, and \textit{(d)} \redst{adaptive-frequency}\rebut{variable-frequency} learned model $\&$ \redst{adaptive-frequency}\rebut{variable-frequency} MPC (\textit{our approach}). \rebut{The fixed-frequency scheme uses $(\Delta t _{\calC}, \Delta t _{\calF}) =(25, 25) ms$ and variable-frequency one utilizes $(\Delta t _{\calC}, \Delta t _{\calF}) =(25, 100) ms$. All MPCs use the prediction horizon $K=10$, thus the fixed-frequency MPC does not cover the entire flight phase. 

For each combination, we perform $23$ jumps consisting of (i) 3 single jumps for each of five targets: $x=40$ cm, $x = 50$ cm, $x = 60$ cm, $(x,z) = (60, 20)$ cm for jump on box, and $x = 70$ cm, and (ii) $8$ continuous jumps of $60$ cm. This yields a total of $92$ jumps for comparison. Fig.~\ref{fig:compare_approach} shows the average final jump target errors of four different MPC combinations across different jumping tasks.}
% These errors are computed via $\bm{e} = \bar{e} \pm \frac{1}{N} \sqrt{\sum_{i=1}^{N} (e_i - \bar{e})^2} $, where $\bar{e} = \frac{1}{N} \sum_{i=1}^{N} e_i$, $e_i = x_i - d_i$, $d_i$ is the target for each jump.
Our approach outperforms the methods that adopt fixed-frequency or nominal models, reducing the jumping distance error up to $8$ times.
\rebut{Our method demonstrates successful jumping on a box with \redst{an error of only $1-2$ cm in distance and} landing angle errors $<15^\circ$, while the fixed-frequency MPC or nominal model MPC fail, as shown in Fig.~\ref{fig:box_jumping_and_forward60_dis}. Note that the box-jumping task is not executed during data collection, verifying the scalability of our method to generalize to unseen reference trajectories and unseen tasks. With our method, the robot also successfully jumps under model uncertainty, e.g, an unknown $5cm$ block ($30\%$ robot standing height) placed under the front feet (Fig. \ref{fig:box_jumping_and_forward60_dis}). This task uses a reference trajectory designed for flat ground and demonstrates an example where the robot significantly deviates from the reference trajectory.}
\redst{Due to space limitation, we discuss two jumping tasks \textit{(i)} box jumping with the target at $(x,z)=(60,20)$ cm, and \textit{(ii)} forward jumping $60$ cm with an unknown disturbance (i.e., a block of $5$ cm under the robot's feet). The results are shown in Fig. \ref{fig:box_jumping_and_forward60_dis}} 
\redst{All MPC methods use prediction horizon $K=10$. The fixed-frequency scheme used a time step of $25$ ms for all jumping phases, so the MPC prediction does not cover the entire flight phase.}
% We consider two jumping tasks: \textit{(a)} box jumping with target at $(x,z)=(60,20)$ cm, and \textit{(b)} forward jumping $60$ cm with an unknown disturbance (i.e., a block disturbance of $5$ cm under the robot's feet). 
% For each jumping task, we make comparisons of variations of MPC, including combinations of the nominal model, learned model, and different sampling time resolutions. 
% The experiment results are shown in Fig. \ref{fig:box_jumping} and Fig. \ref{fig:forward_60cm}, which compare \textit{(a)} nominal model $\&$ fixed-frequency MPC, \textit{(b)} nominal model $\&$ adaptive-frequency MPC, \textit{(c)} fixed-frequency learned model $\&$ fixed-frequency MPC, and \textit{(d)} adaptive-frequency learned model $\&$ adaptive-frequency MPC (\textit{our approach}). 
% Among the evaluated methods, ours outperforms other MPC setups that adopt fixed frequency or nominal models. With our method, the robot is able to jump to target location with an error of only $1-2$ cm and a landing angle error $<15^\circ$, while fixed-frequency MPC or nominal model use cause the robot to land far short of the target. 
% \rebut{Note that the box-jumping task is not executed during data collection, verifying the scalability of our method to execute unseen tasks during training.}


% \begin{table*}[t]
%     \centering
%     \caption{\rebut{Hardware experiments. Comparison of error of final target jumping (in cm) for four real-time MPC setups with different models and timesteps resolutions. Supplemental video: \url{https://youtu.be/KhjUFMdm5-w}.}}
%     %\textcolor{red}{Explain what this link is.}\url{https://www.youtube.com/watch?v=KhjUFMdm5-w}}
%     \label{tab:compare_approach}
%     %\scriptsize % Reduce font size
%     \setlength{\tabcolsep}{4pt} % Reduce column padding
%     \renewcommand{\arraystretch}{0.9} % Reduce row padding
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ *{5}{c} }
%       \toprule
%       \makecell{\textit{Jumping}\\\textit{Task}} & \makecell{Fixed-Frequency \\ (Nominal Model + MPC)} & \makecell{Variable-frequency \\ (Nominal Model + MPC)} & \makecell{Fixed-Frequency\\ (Learned Model + MPC)} & \makecell{\textbf{Variable-Frequency} \\ \textbf{(Learned Model + MPC)}} \\
%       \midrule
%      \textit{Single 40 cm} & 11.67 $\pm$ 1.53 & 7.67 $\pm$ 0.58 & 6.35 $\pm$ 0.68 & \textbf{1.67} $\pm$ \textbf{0.83} \\
%      \textit{Single 50 cm} & -12.67 $\pm$ 2.85 & -8.10 $\pm$ 0.61 & -9.67 $\pm$ 0.88 & \textbf{2.12} $\pm$ \textbf{1.35} \\
%      \textit{Single 60 cm} & -13.27 $\pm$ 2.18 & -8.51 $\pm$ 3.34 & -10.73 $\pm$ 2.54 & \textbf{3.53} $\pm$ \textbf{1.22} \\
%      \textit{Single 70 cm} & -14.65 $\pm$ 1.76 & -9.20 $\pm$ 0.81 & -9.32 $\pm$ 1.73 & \textbf{-3.16} $\pm$ \textbf{0.98} \\
%      \textit{On box (60, 20) cm} & -18.33 $\pm$ 4.41 & -8.39 $\pm$ 0.78 & -10.62 $\pm$ 2.19 & \textbf{4.10} $\pm$ \textbf{0.55} \\
%      \textit{Continuous Jump} & -16.5 $\pm$ 4.62 & -7.52 $\pm$ 3.58 & -12.5 $\pm$ 2.89 & \textbf{1.75} $\pm$ \textbf{1.22} \\
%       \bottomrule
%     \end{tabular}}
%     \vspace{-0.5cm} % Reduce space after the table
% \end{table*}



% as shown in Fig. \ref{fig:box_jumping} and \ref{fig:forward_60cm} for the two jumping tasks.

We also studied the effect of uncertainty in the model by evaluating the jumping performance if we only utilize a joint PD controller to track the joint reference from full-body TO \cite{QuannICRA19}, via \rebut{ $\bftau_{pd} = \bftau_{ff} + \bfK_{p}(\bfq_{\mathbf{J}}^*-\bfq_{\mathbf{J}})+\bfK_{d}(\mathbf{\dot q}_{\mathbf{J}}^*-\mathbf{\dot q}_{\mathbf{J}})$}. The full-order model can be conservative by assuming hard feet, point-to-surface contact, and hard ground. These assumptions, however, are not valid for the Unitree A1 robot equipped with deformable feet \cite{Zachary_RAL_online_calibration_2022}.
% which likely leads to model mismatch (variable calf lengths), unknown ground stiffness and damping, and surface-to-surface contact, when the contact force significantly changes during contact. 
Uncertainties due to DC motors working at extreme conditions or motor deficiency are difficult to model and are normally ignored in the full-body model. These factors affect the model accuracy and prevent the robot from reaching the jumping target if we solely rely on the joint PD, as can be seen in Fig. \ref{fig:box_jumping_and_forward60_dis}. 
% Our learned model captures unknown dynamics and model mismatch from the real robot hardware, which enables the learned-model MPC to achieve accurate jumping.

% verified by following controllers in order:
% % \subsubsection{Pybullet}
% \begin{itemize}
%     \item \textit{Feed-forward control}: We adopt a joint PD controller as the feed-forward controller to track the joint reference profile obtained from full-body TO (e.g.\cite{QuannICRA19}).
%     \item \textit{Fixed-frequency MPC for nominal model:}  We use fixed time step of $25~ms$ for the state prediction. With the horizon windows of $K=10$, the prediction does not leverage the entire flight phase of $400ms$.
%     % The hardware experiments are shown in Fig. \ref{fig:exp-mpc-fixfreq-nominal-snapshots}, respectively.
%     \item \textit{Adaptive-frequency MPC for nominal model:} We use adaptive frequency for prediction (e.g. $\Delta t_{\calC} = 25~ms$ and $\Delta t_{\calF} = 100~ms$). This allows us to leverage the whole flight phase when MPC is executed.
%     % The jumping results are reported in Fig. \ref{fig:exp-mpc-adaptfreq-nominal-snapshots} for simulation and experiments.

%     \item \textit{Fixed-frequency MPC + fixed-frequency learned model:} The sampling time of MPC's prediction and the learned model are set identically as $ 25~ms$. 
%     % The hardware experiment is illustrated in Fig. \ref{fig:exp-mpc-adaptfreq-learn-snapshots}.
    
%     \item \textit{Adaptive-frequency MPC + adaptive-frequency learned model:} In this setup, the prediction of MPC based on the learned model is able to leverage the whole flight phase.
% \end{itemize}
% In all experiments with MPC, the weights in cost functions are identical as $ Q[12] = {0.25, 50, 0.25, 2.5, 2.5, 30, 0, 10, 0, 0.2, 0.2, 0.2}$;


% Some uncertainties, for example, inaccurate leg length due to deformable feet or unknown ground stiffness and damping, are hard to estimate correctly during jumping and these factors can significantly affect the model accuracy as discussed in \cite{Zachary_RAL_online_calibration_2022} for Unitree A1 robot. 
% Our prior work \cite{QuannICRA19} also shows that the landing error 


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/Exp-results-rebut.pdf}
    \caption{\textbf{Hardware experiments:} \rebut{We conduct $2$ rounds with $4$ jumps in each round for each method. The figures (a)-(d) select snapshots of the first and the last jumps when the robot executes four consecutive jumps with different MPC approaches. The target for each jump is $0.6$ m.}} \label{fig:compare_all_mpcs_hardware}
    %
    \includegraphics[width=\linewidth,trim={0.6cm 0.6cm 0.4cm 0.2cm},clip]{figures/Exp/continuous/obstacle/2/fmpc_and_joint.eps}
    \caption{\textbf{Continuous jumping on uneven terrain with A1 robot, shown in Fig. \ref{fig:introduction}:} control forces on the front (a) and rear (b) legs, where the forces are $0$ for swing legs;
    % $L$ denotes the landing phase, which aims to handle hard impact and makes transitions between two consecutive jumps. 
    % The red circles denote the corresponding three targets; 
    and (c) accurate joint tracking of thigh and calf of rear legs. \rebut{Plots (a) and (b) show the force outputs satisfy $|F_z| \leq F_{max} = 350$ N and the friction cone $|F_x/F_z| \leq \mu = 0.6$ during all phases.}}
    \label{fig:uneven-terrain-mpc-hardware}
    % The force controls on both legs satisfy limits $|F_z| \leq F_{max} = 400(N)$ and the friction cone constraint is enforced as $|F_x/F_z| \leq \mu = 0.6$ .
\vspace{-0.5cm} 
\end{figure}

 %    {\centering
	% 	\resizebox{1.1\linewidth}{!}{\includegraphics[trim={1.5cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/traj_x.pdf}}
	% }
 % MPC horizon is all set as $K = 10$.
 % Figure (e) records the actual body's CoM trajectories in the $x$ coordinate.
 


% achieving an accurate full-body model remains challenging, particularly for agile jumping maneuvers that introduce significant uncertainties and unmodeled dynamics. For example, the interaction between foot and ground introduces various uncertainties, such as varied friction or unknown ground stiffness and damping. Additionally, parameter variations, such as inaccurate kinematic parameters, also affect model accuracy. For instance, the authors in \cite{Zachary_RAL_online_calibration_2022} show that the actual leg length of the robot with deformable feet is likely difficult to measure due to dynamic deformation effects and rolling contacts. \NEW{These uncertainties and unmodelled dynamics, unfortunately, are normally simplified or ignored in trajectory optimization framework and real-time execution 

% Using MPC as a feedback control from body trajectory is verified to improve robustness and target accuracy. 


% While full-body TO can plan complex motions, we verify that solely relying on joint PD controller to track the optimal joint reference from full-body TO does guarantee accurate target jumping. We select the experiments of jumping on the box from flat ground to make it match with the initial configuration as TO, as can be seen in Fig. \ref{fig:box_jumping}. The model of full-body dynamics is normally conservative as it assumes constant calf lengths, point-to-surface foot contact, and hard ground, and also ignores other unknown dynamics in hardware and contact. Unlike MIT Cheetah 3 \cite{QuannICRA19}, these assumptions however, are not valid for the Unitree A1 robot equipped with deformable feet, which likely leads to model mismatch (variable calf lengths), unknown ground stiffness and damping, and surface-to-surface contact, when the contact force significantly changes during the entire motion as discussed in \cite{Zachary_RAL_online_calibration_2022}. These factors are also hard to estimate correctly during jumping and can significantly affect the model accuracy. 

% Fig. \ref{fig:traj_compare_box_jumping} compares actual jumping trajectories in hardware under various MPC setups, associated with Fig. \ref{fig:box_jumping}. 
%With our method, the robot jumps to the target accurately with an error of $1-2$ cm and a landing angle error $<15^0$. 

\redst{For further evaluation of target accuracy and robustness,  we performed 4 consecutive jumps (targeting $0.6$ m per jump), repeated 2 times, on flat ground for each of four MPC setups} 
We \redst{further}evaluate the target accuracy and robustness with our method for continuous jumps on flat ground.
The results are presented in Fig. \ref{fig:compare_all_mpcs_hardware}, showing some selected snapshots of the first and the last jump to the final target $2.4$ m. Our method achieves the highest target accuracy, allowing the robot to traverse $2.47$ m with an average distance error of only $1.75$ cm per jump.
During flight periods, the robot can jump up to $4\times$ its standing height.
% Our method with adaptive-frequency learned model and adaptive-frequency MPC allows the robot to traverse $2.47$ m with an average distance error of only $1.75$ cm per jump.



% \note{talk more about learn uncertainties in leg length,...}

% To reduce the computational time of neural network, we combine the
% , which might affect the real-time performance

Note that computing residual matrices $\bfG_{\calC,\bftheta}, \bfH_{\calC,\bftheta}, \bfH_{\calF,\bftheta}$ can consume significant time if we feed the neural network with $(\bfx_0, \bfu_0), (\bfx_{1}^*, \bfu_{1}^*), ..., (\bfx_{K}^*, \bfu_{K}^*)$ sequentially. To improve computational efficiency, we combined the current state and reference as a batch, then feed-forward the entire batch to the learned neural networks all at once, reducing the neural network query time to less than $1$ ms. 




% While full-body TO can plan complex motions, we verify that solely relying on joint PD controller to track the optimal joint reference from full-body TO does not guarantee accurate target jumping. 
% We also verify that solely relying on joint PD controller to track the optimal joint reference from full-body TO does not guarantee accurate target jumping. 
% We select the experiments of jumping on the box from flat ground to make it match with the initial configuration as TO, as can be seen in Fig. \ref{fig:box_jumping}. 

% These factors are also hard to estimate correctly during jumping and can significantly affect the model accuracy. 

% With a sizable prediction horizon (e.g., $K=10$), the solving time for $QP$ of each MPC update (\ref{eq:MPC_learned_QPcompact}) takes an average $2$ ms. This efficient computational time in total enables real-time performance for MPC with learned models. We also verify that if we use a large number of MPC horizons, i.e. $K=22$ when we use a fixed-frequency prediction scheme to cover the entire flight phase. This long horizon yields a big optimization size, causing significant computational costs. It takes an average of $30ms$ for each MPC update, which deteriorates the real-time performance, as shown in Fig. \ref{fig:computational_time}.
% \todo{How to convert batches data}

% 

% \subsection{Continuous Jumping}
% % The figure below shows the snapshot of continuous jumping that uses a feedforward PD controller to track reference from full-body trajectory optimization \cite{QuannICRA19}. We execute three jumps consecutively, with a desired distance of $60cm$ for each jump. However, the robot can leap only about $1.2m$ for all three jumps in total, which is only $67\%$ of the total desired distance.

% For further evaluation, we conduct 4 consecutive jumps on hardware with all MPC methods for the jumping target $60cm$ on flat ground. The experimental results are illustrated in Fig. \ref{fig:compare_all_mpcs_hardware}, showing some selected snapshots of the first and the last jump of four sequential jumps to the final target of $2.4m$. Our method with adaptive-frequency learned model and adaptive-frequency MPC can make the robot traverse $2.45m$, which yields an average distance error of only $1.25cm$ for each jump \TD{(Nitpicking) This actually doesn't mean the average error per jump will be small. E.g., the sum of 4 jumps could be 2.45m but it could be 0.1m + 1m + 0.45m + 0.9m, leading to an average error of 0.33m per jump. It's more precise to say that we calculate the errors for each jump and average them out}.

% \begin{figure}[!t]
%     % \setlength{\belowcaptionskip}{-1pt}
% 	\centering
% 	% {\centering
% 	% 	\resizebox{1.1\linewidth}{!}{\includegraphics[trim={0.9cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/obstacle/1/traj.pdf}}
% 	% }
%     {\centering
% 		\resizebox{1.1\linewidth}{!}{\includegraphics[trim={3.5cm 10cm 2.6cm 11cm},clip]{figures/Exp/continuous/obstacle/2/fmpc_rebut.pdf}}
% 	}
%     {\centering
% 		\resizebox{1.1\linewidth}{!}{\includegraphics[trim={3.5cm 12cm 2.6cm 12cm},clip]{figures/Exp/continuous/obstacle/2/compare_joint_rebut.pdf}}
% 	}
% 	\caption{\textbf{Continuous jumping performance on uneven terrain with A1 hardware, shown in  Fig. \ref{fig:introduction}:} control forces on the front (a) and rear (b) legs, where the forces are $0$ when they are swing legs;
%  % $L$ denotes the landing phase, which aims to handle hard impact and makes transitions between two consecutive jumps. 
%  % The red circles denote the corresponding three targets; 
%  and (c) accurate joint tracking of thigh and calf of rear legs.
%  % The force controls on both legs satisfy limits $|F_z| \leq F_{max} = 400(N)$ and the friction cone constraint is enforced as $|F_x/F_z| \leq \mu = 0.6$ .
%  }
% 	\label{fig:uneven-terrain-mpc-hardware}
%      \vspace{-0.8cm} 
% \end{figure}



% \begin{figure}
% \centering
% \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.45\textwidth]{figures/Training/ftotal_mpc_pd/loss_log.pdf}
% \caption{\textbf{Training loss and testing loss (Log scale).}}
% \label{fig:loss}
% \vspace{-0.7cm} 
% \end{figure}

% \subsection{\rebut{Effect of variable-frequency timesteps}}
\rebut{
We further evaluate MPC with different models learned with other timing choices of $(\Delta t_c, \Delta t_f)= \lbrace (50,50), (25, 80)\rbrace$ ms, in addition to the two timesteps $(\Delta t_c, \Delta t_f)= \lbrace (25, 25), (25, 100) \rbrace$ we already discussed above.
% The supplemental video is here: \footnote{\url{https://www.youtube.com/watch?v=KhjUFMdm5-w}}
}
\begin{table}[t]
	\centering
	\caption{Distance errors (cm) when varying coarseness of timesteps $(\Delta t _{\calC}, \Delta t _{\calF})$ ms. Red colors indicate jumping failure as robot falls short of the box (positive values). The distance errors are measured by the motion capture system at the end of the predefined flight period ($1200$ms). Supplemental video: \url{https://youtu.be/2QjZkARs1mU}.}
	\begin{tabular}{ccccc}
		\hline
		Task & $(25,25)$ & $(50,50)$ & $(25,80)$ & $(25,100)$ \\[.5ex]
		\hline
        Box-Jump & \textcolor{red}{$18.3 \pm 3.7$} & \textcolor{red}{$10.8 \pm 2.1$} & $-1.8 \pm 0.9$ & $-2.0 \pm 1.3$ \\[.5ex]
        % 1 & 1 & 1 & 1 \\[.5ex]
		\hline 
		\label{tab:vary_timestep}
	\end{tabular}
  \vspace{-3.6em}
\end{table}
\rebut{Three jumps are conducted separately for each timing choice of jumping on box task, and the experiments are summarized in Tab. \ref{tab:vary_timestep}. We also achieved successful jumps using the variable-frequency scheme $(25, 80)$ ms. We also observed that using higher timestep in contact to cover the whole flight phase even with fixed-frequency scheme, e.g.,$( 50, 50)$ ms does not guarantee successful jumps.
% For this second set, the time step for prediction in contact is set higher to cover the whole flight phase\NA{I do not understand this sentence. Aren't the time steps equal at 50-50 ms?}. 
% These results validate that, unlike the flight phase, the contact phase has more model complexity due to contact. Thus, using fine time-step discretization to enhance trajectory prediction accuracy in contact is important. 
This confirms our rationale that due to the higher complexity of the robot dynamics during the contact phase, a
coarse time step during this phase leads to higher accumulated prediction errors, even in the flight phase, causing task
failures.


% These experimental results evidence our choice of using fine time-step discretization for contact and coarse time-step for the flight phase.
}


\subsection{Continuous Jumping on Uneven Terrain}
% \rebut{Compared to a single jump, continuous jumping for long-flight maneuvers adds a significant challenge to handling the hard impact and smooth transitions, given the significant linear and angular velocity upon landing and the mismatch timings between predefined schedule and actual contact states (i.e., the robot can transition to a new mode early or late)} 
We tested the robustness and target accuracy of our learning-based MPC for continuous jumping on uneven terrains with a target of $60$ cm for each jump, as illustrated in Fig. \ref{fig:introduction} and Fig. \ref{fig:uneven-terrain-mpc-hardware}. The terrain consisted of multiple blocks with random heights between $2-4$ cm, randomly placed on the ground. 
% We utilized MPC for the landing phase (L) to handle the hard impact and make a transition between two consecutive jumps. Each jump started with an all-leg contact period.
% For execution, when the robot is in the air and about to land, the jumping MPC still outputs zero force control until all legs impact the ground. Thus, it’s not necessary to consider the landing phase
% in the planning horizons when the robot is still in the air. 
\rebut{Since the robot legs can impact the ground early or late on the real robot, there is usually a mismatch between scheduled contact and actual contact states. Whenever both contacts happen (i.e., the landing phase $L$ starts), we activate a separate landing MPC to make a transition between two jumps in a short period of $\sim$$200$ ms \cite{continuous_jump}. The landing MPC is designed with simplified dynamics, $K=10$, and $\Delta t=25$ ms. This aims to track the body reference trajectory from TO for continuous jumping \cite{continuous_jump} and connects two jumps seamlessly.}
% \TD{Does this use the learned model or not?} to handle the hard impact and make a transition between two consecutive jumps. 
% For landing (L), we design MPC 
% \TD{Does this use the learned model or not?} to handle the hard impact and make a transition between two consecutive jumps.
\redst{Fig. \ref{fig:uneven-terrain-mpc-hardware}(a)}\rebut{Figure \ref{fig:introduction}} shows the actual trajectory of three continuous jumps, leaping around $175$ cm in total that yields only $1.67$ cm distance error ($<3\%$) for each jump on the uneven terrain. \rebut{Compared to our prior work \cite{continuous_jump}, we successfully achieve continuous jumping in hardware in this work.}
\redst{Fig. \ref{fig:uneven-terrain-mpc-hardware}(b) and (c) show the force outputs \redst{from adaptive-frequency MPC for the learned model. The force controls} on both legs satisfy $|F_z| \leq F_{max} = 350$ N and the friction cone $|F_x/F_z| \leq \mu = 0.6$ during all phases.} 
With our framework, we also achieve a target jumping error of less than $2$ cm ($3.5\%$) on $34$ single and continuous jumps with different targets and uneven terrain.

% \note{More results with MPC will come here}



% These properties of our learning MPC framework 


 % \subsubsection{ROS}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/60cm_compare_f_fpd/use_f/contact/rollout.png}}
% 	} \\
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/60cm_compare_f_fpd/use_fpd/contact/rollout.png}}
% 	}\\
% 	\caption{\textbf{Control input for neural network}. Comparison between the prediction of neural network for different selection of control inputs. The upper figures using control force, and the lower figures using the combination of control force + joint torque PD (Eq.\ref{eq:f_pd})}
% 	\label{fig:hardware_training_prediction_contact}
% \end{figure*}





% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-026.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-030.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-067.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ fixed frequency}: Motion snapshots from a jump forward $60~cm$ under unknown ground perturbation. This jumping is executed by MPC with fixed time step $\delta t = 25ms$ for learned model.} 
% 	\label{fig:ros-mpc-adaptive-learn-snapshots}
% \end{figure*}

% \begin{figure}[!t]
%     \centering
%     {\centering
%         \resizebox{1.1\linewidth}{!}{\includegraphics[trim={1cm 0cm 0cm 0cm},clip]{figures/Exp/v2/jump_on_box/compare_traj.eps}}}\\
%     \caption{\textbf{Box jumping task (hardware):} Comparison between different MPC implementations with (nominal/learn) model and (fixed/ adapt) frequency. All MPCs have the same $K=10$ prediction horizons. The red circle denotes the jumping target.} 
%     \label{fig:traj_compare_box_jumping}
% \end{figure} 




% \begin{figure}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/traj.eps}}}\\
%     \caption{\textbf{Forward jumping $60cm$:} Comparison between actual and reference trajectory when adaptive-frequency MPC for adaptive-frequency learned dynamics is utilized.} 
%     \label{fig:traj_mpc-adaptive-learn}
% \end{figure}  




% \begin{figure}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/GRF.eps}}}\\
%     \caption{\textbf{Output force from MPC for learned dynamics (hardware).} The force controls on both legs satisfy limits $|F_z| \leq F_{max} = 350(N)$ and the friction cone constraint is enforced as $|F_x/F_z| \leq \mu = 0.6$} 
%     \label{fig:force_mpc-adaptive-learn}
% \end{figure} 



% \begin{figure}
%     \centering
%     {\centering
%         % \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/time.eps}}}\\
%         \resizebox{1.0\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/adapt-learn/learn-adapt.pdf}}}\\
%     \caption{Perform 4 successive jumps with adaptive-frequency learning-based MPC} 
%     \label{fig:learn_adaptive_continuous}
% \end{figure} 


% \section{Hardware Experiments} \label{sec:hardware}
% \subsection{Setup and Training}

% MPC for nominal model is updated every $\delta_t = 25ms$, with number of horizon $N=10$.
% We use adaptive frequency for training. The Fig. 




% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mix/training/flight/rollout.png}}
% 	} \\
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mix/training/flight/rollout_vel.png}}
% 	}\\
% 	\caption{\textbf{Hardware experiments}: Comparison between the prediction of our neural network and the ground-truth trajectory of body position and orientation for flight phase.} 
% 	\label{fig:hardware_training_prediction_contact}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/training/contact/rollout_pos.png}}
% 	} \\
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/training/contact/rollout_vel.png}}
% 	}\\
% 	\caption{Comparison between the prediction of our neural network and the ground-truth trajectory of body position and orientation for flight phase.} 
% 	\label{fig:mpc-adaptive-learn-snapshots}
% \end{figure*}

% \subsection{Experiments}
% We validate our proposed MPC with adaptive frequency for learned model, and make comprehensive comparisons with the utilization of nominal model and fixed MPC frequency update.
% \begin{itemize}
%     \item \textit{MPC with fixed frequency for nominal model }
%     \item \textit{MPC with adaptive frequency for nominal model }

%     \item \textit{MPC with fixed frequency for learned model}

%     \item \textit{MPC with adaptive frequency for learned model}
% \end{itemize}



% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-094.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-120.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-160.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ fixed frequency}: Motion snapshots from a jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC fix frequency $\delta t_{ct} = 25ms$ for nominal model.} 
% 	\label{fig:exp-mpc-fixfreq-nominal-snapshots}
% \end{figure*}


% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-026.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-029.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-037.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ adaptive frequency}: Motion snapshots from a jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms$ for a nominal model .} 
% 	\label{fig:exp-mpc-adaptfreq-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-011.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-014.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-019.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ fix frequency}: Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC fix frequency $\delta t_{ct} = \delta t_{fl} = 100ms $ for learned model.} 
% 	\label{fig:exp-mpc-fixfreq-learn-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-021.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-024.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-028.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ adaptive frequency}: Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms $ for learned model.} 
% 	\label{fig:exp-mpc-adaptfreq-learn-snapshots}
% \end{figure*}





% \begin{figure}[!t]
% \centering
% {\centering
% \resizebox{\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/obstacle/1/traj.eps}}
% }
% \caption{\textbf{Hardware:} The figures show the trajectory of three consecutive jumps on uneven terrain with our MPC approach. MPC horizon is all set as $K=10$. It is associated with Fig. The red circles denote the corresponding three targets. \ref{fig:jump_on_uneven_terrain} }
% \label{fig:compare-mpc-hardware}
% \end{figure}







\section{Discussion and Conclusion} \label{sec:conclusion}
% In this letter, we developed a learned-model MPC approach that enables both target accuracy and robustness for aggressive jumping motions. We learned a residual model from a limited amount of data collected on a real robot to account for the effect of leg dynamics and the mismatch between the nominal model and hardware. Given the learned model, we designed a learning-based \rebut{MPC controller with multiple-timesteps}\redst{an adaptive-frequency MPC controller} that considers the jumping transition, the entire flight phase, and the jumping target during the optimization process.
In this letter, we developed a learned-model MPC approach that enables both target accuracy and robustness for aggressive \rebut{planar} jumping motions. We learned a residual model from a limited dataset to account for the effect of leg dynamics and model mismatch with real hardware. Given the learned model, we designed \rebut{a learning-based variable-frequency MPC that considers the jumping transitions, the entire flight phase, and the jumping target} during the optimization process. 
% Our future work will focus on aggressive maneuvers in 3D, incorporating line-foot and rolling contact.
We demonstrated the scalability of our approach to handle new jumping targets with unseen reference trajectories. %or unseen jumping tasks \textcolor{blue}{in a whole family of motions (e.g. forward jumps)}.
\textcolor{black}{While allowing real-time computation, our approach uses the reference trajectory to evaluate the neural network residual model and ensure a linear model for MPC, which sacrifices a certain degree of accuracy if the system does not operate around the reference under substantial disturbances.} 
\textcolor{black}{To overcome this limitation, our future work will explore the use of nonlinear MPC and address its associated higher computational cost}. \textcolor{black}{We will also generalize the model learning and control framework with varying contact schedules.} Further, we will incorporate line-foot, rolling, and soft contact in learning aggressive legged locomotion maneuvers.

% While offering real-time computational efficiency, l
% , e.g., heavy loads

% \rebut{Addressing the scalability to a new generalized target is an open challenge for learning, especially,
% when a new task is completely different or its distribution is out of training data. It is even more challenging for jumping as different tasks (e.g., backflips, barrel rolls, forward, backward) will normally depend on different contact schedules, constraints, and the unpredicted nature of hardware in extreme conditions. Our future work will improve the scalability to generalize the framework to different jumping tasks. One possible idea is to learn error dynamics, which can reduce the training of trajectory space into a smaller error space and possibly efficiently
% scale up in testing. Also, we will incorporate line-foot, rolling and soft contact in future work.}

% \rebut{Since we aim to use a limited dataset to learn the model and use reference trajectory for future horizons of MPC, we may need
% to collect more data and retrain a new neural network if a new jumping reference is quite significantly different
% from the training set. Our future work is to enhance the scalability of our approach. A possible idea is to learn error dynamics. Then, even with a significantly different reference trajectory, we still can use the error model with MPC. Basically, we reduce the space of all trajectories to the error space, which is smaller and easier to scale}
% \TD{This paragraph is a bit wordy and redundant. Perhaps we can add a couple of sentences discussing this issue before the ``Our future work..." sentence of the previous paragraph and mention scalability as one of our future direction as well.}

% \rebut{It is possible to learn residual dynamics to reason about the hard impact during landing, which, however, may require further study to represent the hybrid dynamics and account for the sudden change of body linear and angular velocity efficiently. Thus, we would like to leave it for future work. In this paper, we find it is still efficient to use nominal SRBD for landing MPC to handle the hard impact and make an efficient transition between two jumps in hardware}

%to realize accurate and robust continuous 3D jumping as well as consider line-foot and rolling contact.


%tailored for both robustness and target jumping accuracy by covering the prediction of the entire flight phase and the target. 
% Via extensive experiments in hardware, we validate that our method outperforms baseline MPC controllers that adopts a nominal model and fixed frequency.

% \begin{figure}[!t]
% 	\centering
% 	{\centering
% 		\resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 1cm 0cm 5cm},clip]{figures/Exp/continuous/TO/TO_continuous.png}}
% 	}
% 	\caption{
% 	\textbf{Continuous jumping} with Full-body TO + feed-forward PD controller}
% 	\label{fig:TO_continuous}
% \end{figure}

==> Sections/version1.tex <==
\section{Introduction}
Aggressive maneuvers with legged robots, such as jumping \cite{QuannICRA19,RL_jump_bipedal}, back-flipping \cite{unitreeH1}, and barrel rolls \cite{chuongjump3D}, have received significant attention recently, and have been successfully demonstrated using trajectory optimization \cite{QuannICRA19,chuongjump3D,matthew_mit2021_1,ChignoliICRA2021}, model-based control \cite{YanranDingTRO,continuous_jump_bipedal,GabrielICRA2021,park2017high, ZhitaoIROS22,fullbody_MPC}, and learning-based control \cite{zhuang2023robot, RL_jump_bipedal,yang2023cajun,vassil_drl,jumpingrl,lokesh_ogmp}. Unlike walking or running, aggressive motions are particularly challenging due to \textit{(1)} the extreme underactuation in the mid-air phase (the robot mainly relies on the force control during contact to regulate its global position and orientation), \textit{(2)} significant dynamics model error and uncertainty that are inherently hard to model accurately, especially with contact and hardware load during extreme motions, and \textit{(3)} the trade-off between model accuracy and efficient computation for real-time execution. Achieving both target accuracy and robustness for long-flight maneuvers, such as high or long jumps, therefore still presents an open challenge. 
In this work, we address this challenge by developing a real-time MPC for quadruped jumping using a robot dynamics model learned from experiments.
% In this work, we address this challenge by developing a
% real-time MPC with dynamics model learned from experiments, demonstrated via an example of quadruped jumping.

%developing a real-time model predictive control policy with adaptive frequency and accurate learned robot dynamics from data.

% Recent advancements in model-based approaches, notably MPC, have proven effective in realizing robust acrobatic motions \cite{GabrielICRA2021,park2017high, YanranDingTRO,continuous_jump}. 

% In the realm of model-based control and optimization, the main challenge of modeling choice to realize jumping tasks is how to compromise between model accuracy and online control. 
%a varied selection of models
% \rep{Many advanced control and optimization frameworks with different dynamics formulations have been proposed to realize jumping maneuvers}.

% \TD{What does it mean to be full-nonlinear dynamics? Does that mean it accounts for the leg dynamics? This is because we just mentioned in the previous paragraph that some parts of the dynamics are hard to model but here, it might make an impression to readers that full dynamics are available to use.} 


Various dynamics models have been proposed for control and optimization of aggressive robot maneuvers. Full-body nonlinear dynamics are normally utilized to generate complex trajectories with long flight phases, but are often used for offline planning only due to high model complexity (e.g., \cite{QuannICRA19,chuongjump3D}).
% However, since the optimization is very high dimensional and objectives are highly nonlinear, solutions are normally obtained offline. 
% For efficient computation, many offline trajectory optimization frameworks adopt reduced-order models such as spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid} or standard single-rigid-body dynamic (SRBD) \cite{ChignoliICRA2021, ZhitaoIROS22}.
% Many frameworks sacrifice model accuracy for very efficient computation by using simplified models such as spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid} or single-rigid-body dynamic (SRBD) \cite{NMPC_3D_hopping, ZhitaoIROS22,GabrielICRA2021, park2017high,YanranDingTRO} that lumps the trunk and legs into a unified body. 
Many methods sacrifice model accuracy for real-time performance by using simplified models such as nominal single-rigid-body dynamics (SRBD) \cite{NMPC_3D_hopping,ZhitaoIROS22,GabrielICRA2021, park2017high,YanranDingTRO} that combine the trunk and legs as a unified body. 
% To consider the effect of leg dynamics, Zhou \textit{et al.} \cite{ZiyiZhouRAL} recently propose a linearized variant of the full centroidal dynamics, incorporating joint information to centroidal model of quadruped jumping \cite{ZiyiZhouRAL}; He \textit{et al.} \cite{He2024} exploit centroidal inertia decomposition model to regulate angular momentum during flight phase of bipedal jumping. In most existing works, the effects of model mismatch or unknown dynamics in hardware and contact on the accuracy of aggressive maneuvers, however, have not been well explored and modeled effectively. 
Recently, designing models that both consider leg dynamics and enable real-time execution has gained considerable attention. Zhou \textit{et al.} \cite{ZiyiZhouRAL} propose a linearized variant of the full centroidal dynamics, incorporating joint information in a centroidal model of quadruped jumping. He \textit{et al.} \cite{He2024} exploit a centroidal inertia decomposition model to regulate angular momentum during the flight phase of bipedal jumping. However, developing an approach that can account for model mismatch with hardware and dynamics uncertainty as well as effectively predict long flight phases, which is important for control policies to enhance both target accuracy and jumping robustness, is still an open challenge.

% that combines the trunk and legs into a unified body. 
% which usually ignores the change in the centroidal inertia due to the limb movements. 
% To reason the effect of leg dynamics, the authors in \cite{KeMechatronics23} abstract the legged robots as a standard SRBD for the base and point masses for the legs. This choice reduces a certain complexity to the model for offline planning, compared to the full-order model resolution.
% , or centroidal dynamics with kinematic constraints \cite{matthew_mit2021_1, ChignoliICRA2022}. 
% To reason the effect of leg dynamics, recent work \cite{KeMechatronics23} abstracts the legged robots as a standard SRB for the base and point masses for the legs.
% These reduced-order models are utilized for offline planning to generate reference trajectories for long-flight maneuvers, which then be tracked by additional real-time control.
% However, incorporating joint information to reason about the centroidal inertia is non-trivial with these models, which limits their ability to generate angular-momentum-rich motions using limb movements such as jumping.
% The lumped-leg SRBM attempted to augment the standard SRBM
% by approximating the time-varying inertia tensor; however, neither use the full capabilities of the joint motions.
% Many optimization frameworks sacrifice model accuracy for very efficient computation by assuming the robot dynamics as a single rigid body (SRB) dynamics (\cite{ChignoliICRA2021, ZhitaoIROS22}), or centroidal dynamics with kinematic constraints (\cite{matthew_mit2021_1, ChignoliICRA2022}), which ignore the dynamic effect of all legs in the whole-body jumping motions.
% To leverage the limb movement, the authors in \cite{KeMechatronics23} abstract the legged robots as a SRB for the base and point masses for the legs. However, leveraging leg motions typically adds a certain complexity to the model, thus this is mainly utilized for offline planning. 
% Recently, there have been increasing efforts to achieve real-time control with models that account for non-constant leg inertia.
% These simplified models have also been widely adopted for online control pipelines for jumping \cite{GabrielICRA2021,park2017high, YanranDingTRO}. 
% However, incorporating leg configuration to reason about the centroidal inertia is non-trivial with these models. 

% These simplifications consider the effect of leg dynamics partially or ignore it in the whole-body linear and angular momentum. 
% Thus, it may compromise target jumping accuracy for real-time control.
% However, since these simplifications ignore the dynamic effect of all legs in the whole-body linear and angular momentum, adopting these models may compromise target accuracy as well as success rates when translating highly agile motions to hardware.
% To enable real-time execution, the complexity of the dynamics has been simplified and led to the introduction of various models. Single rigid body model (SRBM) ....(\cite{NMPC_3D_hopping, YanranDingTRO, GabrielICRA2021}), spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid}, . Such simplification normally ignores the dynamic effects of legs.
% In summary, the main challenge of modeling choice is how to compromise between model accuracy and online control.
% In this work, we attempt to address this problem by proposing a well-balanced middle-ground model that is able to leverage the effect of legged dynamics, but can be efficiently utilized for real-time control and optimization.
% Difference from previous work, we develop
% a learning-base model that can represent the effect of leg
% dynamics in the whole-body linear and angular momentum
% of the robot trajectories, while it is efficiently utilized for
% real-time control and optimization

% In this work, we propose a dynamics model learned from data, which considers not only the effects of leg dynamics but also model mismatch with the real robot hardware.

\begin{figure}[!t]
    \centering
\includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{figures/Introduction/Introduction-v5.pdf}	
 % The Unitree A1 robot is able to jump on box with target error of $1~cm$ and orientation error less than $10^0$ degree upon landing.
 \caption{A Unitree A1 robot performs continuous jumps on unknown uneven terrain, achieving both target accuracy and robustness. The flight phase covers a vertical height of up to $4 \times$ the robot's normal height. Supplemental video: \url{https://youtu.be/qaXPPGrvVr4}.}
    \label{fig:introduction}
\end{figure}

% \note{Dynamic learning}
Learning robot models from experiments to capture complex dynamics effects and account for model errors with real hardware has become a popular approach \cite{nguyen2011model, greydanus2019hamiltonian, lutter2019deeplagrangian, sanchez2018graph, bauersfeld2021neurobem,hewing2019cautious,saviolo2022physics,duong23porthamiltonian}.
% A recent line of work aims to learn dynamic models entirely from real-world data, with a primary investigation of dynamical systems without contact \cite{salzmann2023real, bauersfeld2021neurobem,hewing2019cautious,saviolo2022physics}. 
% Compared to Deep Reinforcement Learning which often requires millions of timesteps of simulation interactions and bridging sim-to-real gaps \cite{jumpingrl,yang2023cajun, RL_jump_bipedal,zhang2024wococo,unitreeH1}, directly learning real-world models via residual dynamics can require a smaller number of data points \cite{bauersfeld2021neurobem, salzmann2023real}
% directly learning real-world models for control is able to address these challenges. In addition, by exploiting the residual dynamics of a nominal model, it can even require a smaller number of data points to effectively learn the model \cite{bauersfeld2021neurobem, salzmann2023real}
% Compared to learning the full model, learning the residual dynamics of a nominal model simplifies the learning tasks and allows describing the model augmentation using only a smaller number of data points. 
Many frameworks learn residual dynamics using neural networks \cite{bauersfeld2021neurobem, salzmann2023real} or Gaussian processes \cite{hewing2019cautious, cao2017gaussian} and use model predictive control (MPC) to control the learned systems \cite{salzmann2023real, pohlodek2022hilompc} to improve tracking errors.
Most existing works, however, primarily investigate dynamical systems without contact. Recently, Sun et al. \cite{sun2021online} proposed a notable method to learn a linear residual model, addressing unknown dynamics during legged locomotion. Nevertheless, the method is designed for walking stabilization specifically and does not leverage the effect of leg dynamics. Compared to existing works, learning dynamics for aggressive maneuvers with long-flight periods on legged robots presents some challenges, such as \textit{(1)} the switching between multiple dynamic models due to contact, including flight phase where control action has very little effect on the body dynamics, \textit{(2)} disturbances and uncertainty in dynamic modeling due to hard impact in jumping, and \textit{(3)} the effect of intermittent control at contact transitions on state predictions. 


% \TD{We haven't defined adaptive frequency until the next paragraph. Also, I don't think that adaptive frequency affects the comparison of our approach with others here. So maybe we can omit it.}

% enhancing target jumping accuracy for dynamic maneuvers with extended flight phases.

% \rep{ Compared to the abundance of work that exists for learning the dynamics, the literature for learning the dynamic maneuvers of systems with contact, such as jumping on legged robots, is comparatively sparse and consists of unique challenges such as \textit{(1)}  the period of extreme underactuation, \textit{(2)} complex contact dynamics, and \textit{(3)} the effect of intermittent control at contact transitions to state predictions. To address these challenges, we propose a residual learning model for legged robots and design the learning in an adaptive frequency scheme to realize the model for enhancing target jumping accuracy for dynamic maneuvers with extended flight phases.}
% Most of the work, however, mainly focuses on learning systems without contact such as aerial robots \cite{bauersfeld2021neurobem, salzmann2023real,duong23porthamiltonian}.
% Several works augment a nominal model with a learned residual to account for uncertainties or to capture complex dynamic effects. 
% One approach is to complement a nominal model with a Gaussian process \cite{kabzan2019learning, torrente2021data, khadivar2023self}, but a key drawback is a computational complexity due to its nonparametric nature. Another approach is to use neural networks for the residual term \cite{salzmann2023real, saviolo2022physics}. 
% Khadivar et al. \cite{khadivar2023self} learn a residual inverse dynamics model for a quadratic programming-based controller to account for model uncertainties using a Gaussian process.
% Existing works discussed above, however, aims to learn the dynamics systems without contact dynamics. 
% For learning systems with contact, Sun et al. \cite{sun2021online} recently propose a notable framework to learn a time-varying linear residual model for a quadruped robot to compensate for the unmodeled dynamics online, which however mainly focuses on the walking stabilization.
% The work \cite{sun2021online} shows impressive robustness of walking motion under model uncertainties; however, leveraging the effect of leg dynamics on the model is not demonstrated.
% \note{To our knowledge, such approaches have not yet been demonstrated for modeling the legged robots.}



%MPC has recently been brought into the realm of real-time dynamic jumping control due to its ability to optimize control actions during the contact phase based on predictions of where the robot in mid-air periods

In this letter, we propose a residual learning model using an adaptive-frequency scheme to tackle the aforementioned challenges and enhance long-term trajectory predictions over different jumping phases. MPC has been commonly used for jumping by optimizing the control inputs during the contact phase based on future state prediction during the flight phase (e.g.,\cite{GabrielICRA2021, fullbody_MPC, park2017high, YanranDingTRO,  continuous_jump}). 
% When it comes to model selection, there is typically an inherent trade-off between model accuracy and computational efficiency.
% A full-body nonlinear dynamics model can leverage the whole effect of leg dynamics on the robot trajectory; however, it normally poses a challenge to utilize this model for real-time performance due to its high nonlinearity. Therefore, it is mainly utilized for offline planning to generate complex motions with long flight phases to consider all feasible nonlinear constraints (e.g., \cite{QuannICRA19,chuongjump3D}).
% ; nevertheless, it can take a significant amount of time to converge to the optimal solution due to the model's complexity.
%\rep{When designing MPC for long flight maneuvers, a major challenge is how to utilize a limited number of the prediction horizons but still effectively cover the entire flight phase and especially the final target in the horizons, as it is the most important goal for jumping. Another challenge is to obtain an accurate model to leverage complex dynamic maneuvers, unknown dynamics, and model mismatch with real hardware in order to improve jumping accuracy, while still ensuring real-time performance.}
%in the horizons, as it is the most important goal 
A major challenge in MPC for long flight maneuvers is to utilize a limited number of prediction steps yet still effectively cover the entire flight phase and especially the final jumping target. Another challenge is to obtain an accurate model for complex dynamic maneuvers, unknown dynamics, and model mismatch with the real hardware to improve the jumping accuracy, while still ensuring real-time performance. Related works have address these challenges partially.
% how to achieve accurate trajectory prediction for the entire flight phase
% To facilitate real-time computation, 
%  to sacrifice model accuracy for 
% , as demonstrated via robust jumping tasks (e.g. 
For example, many MPC methods utilize conventional SRBD models, ignoring the leg dynamics, to achieve real-time execution \cite{GabrielICRA2021,continuous_jump_bipedal,YanranDingTRO}. Some recent methods account for leg inertia \cite{ZiyiZhouRAL,He2024,fullbody_MPC}, however, disturbance and uncertainty in dynamic modeling have not been considered. These frameworks also focus on jumping robustness rather than accurate target jumping. 
% \rep{In this work, we aim to address these challenges altogether by \textit{(1)} designing and learning a dynamics model for dynamic maneuvers directly from experimental data, \textit{(2)} learning with an adaptive-frequency scheme that utilizes a fine time step for contact phases and coarse time step for flight phase, allowing the coverage of the entire flight phase, the jumping target, and the contact transitions, thereby significantly enhancing long-term trajectory predictions, and \textit{(3)} designing an MPC with the learned dynamics for dynamics maneuvers, using the same adaptive frequency technique from dynamic learning.}
% , which plays a key factor in achieving accurate target jumping in hardware.
% While using SRBD expedites computations, these simplifications in the robot model may compromise both accuracy and success rates when translating highly agile motions to hardware.
% Many model-based control and optimization frameworks are designed to address
% these challenges partially.
% % In the realm of model-based control and optimization, the main challenge of modeling choice to realize jumping tasks is how to compromise between model accuracy and online control. 
% Trajectory optimization, which adopts a full-body nonlinear dynamics model leveraging the whole effect of leg dynamics on the robot trajectory can effectively generate complex quadruped jumping trajectory with nonlinear constraints and long flight phases (e.g., \cite{QuannICRA19,chuongjump3D}); nevertheless, it can take a significant amount of time to converge to the optimal solution due to the model's complexity.
% However, since the optimization is very high dimensional and objectives are highly nonlinear, solutions are normally obtained offline. 
% For efficient computation, many offline trajectory optimization frameworks adopt reduced-order models such as spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid} or standard single-rigid-body dynamic (SRBD) \cite{ChignoliICRA2021, ZhitaoIROS22}.
% On the other hand, many optimization frameworks sacrifice model accuracy for very efficient computation by using simplified models such as spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid} or conventional single-rigid-body dynamic (SRBD) \cite{ChignoliICRA2021, ZhitaoIROS22}, which normally ignore the change the centroidal inertia due to the limb movements. 
% To reason the effect of leg dynamics, the authors in \cite{KeMechatronics23} abstract the legged robots as a standard SRBD for the base and point masses for the legs. This choice reduces a certain complexity to the model for offline planning, compared to the full-order model resolution.
% , or centroidal dynamics with kinematic constraints \cite{matthew_mit2021_1, ChignoliICRA2022}. 
% To reason the effect of leg dynamics, recent work \cite{KeMechatronics23} abstracts the legged robots as a standard SRB for the base and point masses for the legs.
% These reduced-order models are utilized for offline planning to generate reference trajectories for long-flight maneuvers, which then be tracked by additional real-time control.
% However, incorporating joint information to reason about the centroidal inertia is non-trivial with these models, which limits their ability to generate angular-momentum-rich motions using limb movements such as jumping.
% The lumped-leg SRBM attempted to augment the standard SRBM
% by approximating the time-varying inertia tensor; however, neither use the full capabilities of the joint motions.
% Many optimization frameworks sacrifice model accuracy for very efficient computation by assuming the robot dynamics as a single rigid body (SRB) dynamics (\cite{ChignoliICRA2021, ZhitaoIROS22}), or centroidal dynamics with kinematic constraints (\cite{matthew_mit2021_1, ChignoliICRA2022}), which ignore the dynamic effect of all legs in the whole-body jumping motions.
% To leverage the limb movement, the authors in \cite{KeMechatronics23} abstract the legged robots as a SRB for the base and point masses for the legs. However, leveraging leg motions typically adds a certain complexity to the model, thus this is mainly utilized for offline planning. 
% Recently, there have been increasing efforts to achieve real-time MPC with models that account for non-constant leg inertia.
% These simplified models have also been widely adopted for online control pipelines for jumping \cite{GabrielICRA2021,park2017high, YanranDingTRO}. 
% However, incorporating leg configuration to reason about the centroidal inertia is non-trivial with these models. 
% Zhou et al. propose a linearized variant of the full centroidal dynamics, incorporating joint information in the robot model to reason about the centroidal inertia \cite{ZiyiZhouRAL} of quadruped robots; He et al. exploit centroidal inertia decomposition model to regulate angular momentum during flight phase and track landing pose target for bipedal jumping \cite{He2024}. 
% These simplifications consider the effect of leg dynamics partially or ignore it in the whole-body linear and angular momentum. 
% Thus, it may compromise target jumping accuracy for real-time control.
% However, since these simplifications ignore the dynamic effect of all legs in the whole-body linear and angular momentum, adopting these models may compromise target accuracy as well as success rates when translating highly agile motions to hardware.
% To enable real-time execution, the complexity of the dynamics has been simplified and led to the introduction of various models. Single rigid body model (SRBM) ....(\cite{NMPC_3D_hopping, YanranDingTRO, GabrielICRA2021}), spring-loaded inverted pendulum \cite{Patrick14_jump_humanoid}, . Such simplification normally ignores the dynamic effects of legs.
% In summary, the main challenge of modeling choice is how to compromise between model accuracy and online control.
% In this work, we attempt to address this problem by proposing a well-balanced middle-ground model that is able to leverage the effect of legged dynamics, but can be efficiently utilized for real-time control and optimization.
% In contrast with previous legged-jumping MPC frameworks, we develop a model with neural networks and experimental datasets, which can fully represent the nonlinear effects of leg dynamics in the whole-body linear and angular momentum of the robot trajectories, while the model is efficiently utilized for real-time control for jumping.
% \rep{In this paper, we aims to learn .....}
% %
% Much progress has been made in realizing aggressive maneuvers on legged robotics in recent years. Successful hardware demonstrations include trajectory optimization \cite{QuannICRA19,chuongjump3D,matthew_mit2021_1,ChignoliICRA2021}, model-based control \cite{YanranDingTRO,continuous_jump_bipedal,GabrielICRA2021,park2017high, ZhitaoIROS22,fullbody_MPC}, and learning-based control \cite{zhuang2023robot, RL_jump_bipedal,yang2023cajun,jumping_inpixel,jumpingrl,lokesh_ogmp}, just to name a few. 
% Despite these successes and progresses, achieving both target accuracy and robustness for long-flight maneuvers still presents an open but challenging problem. The goal of this work is to provide a feasible solution by combining the novelty of dynamic learning and real-time MPC in an adaptive frequency scheme, demonstrated through an example of quadruped jumping.
% For jumping tasks with long flight phase, 

% A long-standing challenge for jumping maneuvers is how to enable both accurate target jumping and robust to uncertainties. while , characterized by a long aerial phase with control only applied during a short contact phase.  During the aerial phase, control inputs have little impact on the robot trajectory. Therefore, trajectory errors may be accumulated and may prevent the robot from reaching desired targets. In addition, control during the contact phase needs to predict any uncertainty and unknown dynamics involved in the complex contact dynamics and hardware model during the whole jump. This challenge has been motivated extensively research to realize these jumping motion in hardware \cite{AtlasBackflip2023, fullbody_MPC, katz2019mini, QuannICRA19, ZhitaoIROS22}.

% \note{Model-based Control and Optimization:}
% Explain simplified dynamics --> robustness but not target accuracy
% TO for full-body dynamics --> too complex --> not suitable for real-time
% Model-based optimization and control are extensively investigated to realize the jumping in legged robots.
% Recent advancements in model-based approaches have proven effective in realizing jumping motions.
% In the realm of model-based control and optimization, the selection of model complexity is typically tailored to the specific purpose at hand. 

%Unlike walking or running gaits, the unique challenge of achieving both target accuracy and robustness for jumping originated from typical reasons such as \textit{(1)} the periods of extreme underactuation in the mid-air phase, thus the robot mainly relies on the force control during the contact phase to regulate its global position and orientation, \textit{(2)} model mismatch, uncertainties, and unknown dynamics inherently exist and hard to model accurately in contact and hardware for this extreme motion, and \textit{(3)} the trade-off between model accuracy and efficient computation for real-time execution. 
% When designing MPC for target jumping tasks, a major challenge is how to achieve accurate trajectory prediction for the entire flight phase during the execution of MPC in the contact phase. To enable real-time performance, the control pipelines with simplified dynamics are  favorable designs. MPC based on conventional SRBD has been extensively studied by many research groups to realize robust quadruped jumping \cite{GabrielICRA2021, park2017high}. However, their selections of simplified model may affect the accuracy of trajectory prediction for the long flight phase, which plays a key factor in achieving accurate target jumping.
% In this work, we leverage the advantages of dynamic learning and MPC to enhance both robust and accurate target jumping on legged robots. 
% In the past few years, MPC has been extensively studied by many research groups to realize robust jumping \cite{GabrielICRA2021,park2017high,YanranDingTRO}. 
% To enable real-time performance, the control pipelines with simplified dynamics and limited prediction horizons are favorable designs. These selections may affect the accuracy of trajectory prediction for the long flight phase, which plays a key factor in achieving accurate target jumping. 




% Compared to existing models, we develop a model that can leverage the legged dynamics but can efficiently used for real-time optimization for jumping.




% It is also noticed that even with the full-order nonlinear model, there always exits some mismatch between the model for optimization and hardware to model uncertainties from hardware,
% In our prior work on quadruped jumping, observe some error at pitch around 
%  significant pitch angle error with a magnitude of more
%  than $30^0-45^0$ upon landing.
%  Our model can learn some uncertainties in hardware ....

% They aims to generate the motion offline, then tracked by various controller such as joint PD \cite{ZhitaoIROS22}, variational-based control \cite{ChignoliICRA2021}, or whole-body control \cite{cite}
% To reduce solving time, centroidal dynamics with kinematic constraints can be adopted in the TO \cite{ZhitaoIROS22} to generate reference, which then be tracked by joint PD controller/ whole body controller, \cite{citeMIT paper}.
% Full-body trajectory
% optimization has very high dimensional and objectives are
% highly nonlinear, which often leads optimization procedures
% into bad local minima. However, the trajectory optimization
% can be slow, especially when a good initial guess is not
% available. Therefore, solutions are normally obtained offline
% with trajectory optimization
% These approaches rely on the accuracy of model of the dynamical system to generate optimal control inputs \cite{fullbody_MPC, NMPC_3D_hopping}. 


% However, relying on model simplification may compromise for target position \& orientation accuracy, and the success rate of transferring highly agile motions to hardware.

% For highly dynamic jumping, the unknown dynamics related to complex contact model and hardware at the extreme conditions are normally simplified or ignored to reduce the computational resources. Full-body dynamics has proven to be effective to generate motions with long flight phase \cite{chuongjump3D,matthew_mit2021_1}; however, this normally requires offline computation due to complexity of the dynamics. On the other hand, a widely-used single rigid body dynamics allows real-time control but may compromise for target jumping accuracy when transferring to hardware \cite{GabrielICRA2021, YanranDingTRO}.

% \note{Learning-based control}
% Most of the work focuses on robustness


% In this work, we propose an approach that allows learning dynamics from a limited dataset, thus alleviating the need to use extensive data from hardware experiments. 
% A real-time control is then developed based on the learning model to achieve both jumping accuracy and robustness.


% On the other hand, using data from hardware allows us to learn a more accurate model and reduce the sim-to-real gap. However, performing jumping tasks in hardware to collect data for DRL can be risky, expensive, and inefficient. 

% To enable learning efficiency, DRL typically requires large amounts of diverse data. This often necessitates extensive and time-consuming setup and calibration, and many motions are not safe to practice in hardware. Therefore, it can pose a challenge for DRL approaches to learn efficiently while only using a limited dataset collected from real hardware. 
% Due to the inherent complexity and
% time-consuming hardware experiments of jumping tasks,
% DRL frameworks normally rely on simulation to collect extensive training data, which normally requires bridging the sim-
% to-real gap.


% Difference than normal locomotion such as walking or running, perform jumping tasks in hardware to collect data for DRL can be risky, expensive, and inefficient. To enable learning efficiency, DRL normally require large amounts of diverse data. It often requires extensive setup and calibration, and many motions however are not safe to practice in hardware. Therefore, it can pose a challenge to DRL approaches to use a limited dataset collection from hardware.  Therefore, collecting data on simulation is more safer, efficient, and scalable. Nevertheless, due to the unpredictable nature of hardware that hardly modeled accurately in the simulation environment, there can exist a sim-to-real gap transfer \cite{RL_jump_bipedal,jumping_inpixel,jump_mentor}. 


% Difference from DRL, our approach for jumping tasks requires less training data and can efficiently solve for the optimal control inputs within a second in a standard computer. Additionally, our method enables robots to learn the model directly in hardware instead of heavily relying on simulation for hardware transfer as DRL.
% DRL also normally relies on random exploration of the control actions with extensive trials and errors until it converges to an optimal policy. Our proposed method, on the other hand, enforces control actions into an optimization framework instead of random exploration. Thus, it only requires a small number of trials to accomplish desired tasks, which are mostly unattainable through DRL.
% \cite{sun2021online} propose a data-driven approach for walking. In contrast our work is for jumping

% \TD{I think jumping straight to DRL might be a bit abrupt.}To enhance jumping robustness, many learning-based control frameworks rely on deep reinforcement learning (DRL) with terrain and dynamic randomization, demonstrated via many impressive experiments, such as quadruped jumping \cite{jumping_inpixel,jumpingrl,yang2023cajun}, bipedal/humanoid jumping \cite{RL_jump_bipedal,zhang2024wococo,unitreeH1}.
% To enable learning efficiency, DRL for jumping often requires extensive training data and millions of timesteps of simulation interactions.
% % In this light, collecting data in simulation is more efficient and safer. 
% However, the jumping task usually involves the motor operating under extreme conditions, making it challenging to accurately model the unpredictable nature of hardware in the simulation environment. Therefore, it normally requires bridging the sim-to-real gap to enhance target jumping accuracy and robustness. 
% % \cite{RL_jump_bipedal,jumping_inpixel}. 
% It is worth noticing that in order to achieve accurate jumping, it is necessary to not only rely on an accurate model but also have the capability to cover the entire flight phase in the limited prediction horizon used for control synthesis. 
% In contrast with conventional MPC frameworks, we design an adaptive-frequency scheme that utilizes a fine sampling time step in near MPC horizons and a relaxed time step in far prediction horizons. Importantly, the adaptive frequency is also utilized and synchronized with the learning of the model. This allows us to significantly enhance the accuracy of the body trajectory prediction in the long term, covering the entire flight phase, the jumping target, and the transitions between contact and flight.
% \note{Mention about uncertainties--> learning model}
% \note{Contributions}
% Jumping stands out as a notable advantage that legged robots possess over their wheeled or tracked counterparts. This distinctive capability empowers legged robots to adeptly traverse rough terrain, high obstacles, and large gaps, with speed and efficiency. 
% In the last decades, this notable advantage has inspired various studies to realize these acrobatic motions on the robot hardware \cite{AtlasBackflip2023, katz2019mini, QuannICRA19, fullbody_MPC, ZhitaoIROS22}. 
% Jumping typically require long aerial period. During this aerial period, the system becomes
% under-actuated systems and the control has little impact on
% the robot trajectory during this period.
% We aim to tackle these problems by \textit{(i)} designing a learning model of residual dynamics that represents the effect of legged dynamics and other model uncertainties, and \textit{(ii)} designing an adaptive frequency scheme that considers a larger sampling time for flight phase prediction to leverage the whole flight trajectory, given a limited prediction horizons, and \textit{(iii)} the proposed data-driven model expresses the direct relationship between robot states and force control, allowing us to incorporate the learned model with the MPC architecture to optimize for the control actions.
% The adaptive scheme is supported by the data-driven model to enhance the accuracy of trajectory prediction for the whole flight phase.
% for the  That ignore the full capability of leg movements on the robot model. Using this simplified dynamics may compromise accurate long-horizon prediction. 
% In addition, the existing simplified dynamics has not represent well the affect of contact dynamics to the system. 
% Having high prediction accuracy and leveraging the effect of contact dynamics and hardware models are necessary for MPC to generate optimal control, which enables trajectory tracking and compensates for uncertainties.
% \note{Motivation to use adaptive frequency?}



In this work, we address these challenges by learning a dynamics model from hardware date and designing an adaptive-frequency MPC capturing both the contact and entire flight phase in the optimization process. The contributions of this letter are summarized as follows.

% The highly dynamic jump typically requires the robot to reach its hardware limits. In these extreme condition, the accurate model is hard to achieve.
% Our work proposes a solution to tackle this problem by leveraging the advantage of supervised learning and real-time model predictive control.
% Contributions:
\begin{itemize}
  % \item We learn a \emph{residual dynamics model} directly from a small real experiment dataset. The model accounts for nonlinear leg dynamics, hardware modeling errors, and model mismatch during contact.
  \item We learn a \emph{residual dynamics model} directly from a small real experiment dataset. The model accounts for nonlinear leg dynamics, modeling errors, and unknown dynamics mismatch in hardware and during contact.
  
  % \item \rep{A residual adaptive-frequency learning model that aims not only to learn the nonlinear leg dynamics, unknown dynamics, and model mismatch from real robot hardware but also enhance long-term state predictions over different jumping phases} 
  
  % \item We introduce an \emph{adaptive-frequency scheme} that leverages different time resolution to capture the entire flight phase, the jumping target, and the contact transitions over a few-step horizon, thereby significantly improving the accuracy of long-term trajectory prediction.

    \item We propose learning the model in an \emph{adaptive-frequency scheme} that leverages different time resolutions to capture the entire flight phase, the jumping target, and the contact transitions over a few-step horizon, thereby significantly improving the accuracy of long-term trajectory prediction.
    
  % \item \rep{A residual model learning approach that learns the effect of unknown nonlinear dynamics, e.g., leg dynamics, and model mismatch from real robot hardware from real-world data in an adaptive-frequency scheme.} 
%   We propose to learn a residual model from real-world
% data and in an adaptive-frequency scheme to leverage
% the effect of leg dynamics, unknown dynamics, and
% model mismatch with the real robot hardware, as well
% as enhance target jumping accuracy.

  % The model can be efficiently utilized for real-time control and optimization of highly dynamic jumping.
  \item We develop \emph{adaptive-frequency MPC using the learned model} to synthesize controls that improve both target accuracy and robustness in dynamic robot maneuvers.
  
  \item \emph{Extensive hardware experiments} validate the effectiveness and robustness of our approach with single and consecutive jumps on uneven terrains. Comparisons with other MPC techniques using a nominal model or fixed frequency are also provided.
  % \item \rep{ We also validate the framework on robust and consecutive jumping on uneven terrain consisting of perturbation of random heights ($13-27\%$ of the robot's standing height), achieving an average distance error of $1.67~cm$.}
  % \item We conduct 48 dynamic jumps .
\end{itemize}

% Our approach outperforms other MPC settings, achieving a jumping distance error of less than $3\%$ compared to the target, based on the overall performance of 20 jumps with different target locations and ground uncertainties.
Our approach outperforms other MPC settings, reducing the jumping distance error up to $8$ times. We demonstrate robust and consecutive jumping on uneven terrain with height perturbations ($13-27\%$ of the robot's standing height), achieving a distance error of $1.67$ cm on average. Testing on $34$ single and continuous jumps, our approach achieves target jumping error of less than $2$ cm ($3.5\%$) for different targets and uneven terrain.

% This letter is organized as follows. Section \ref{sec:overview} presents the overview of the proposed system architecture. In more detail, Section \ref{sec:proposed_approach} introduces the proposed learned residual model, followed by adaptive-frequency model training and MPC execution for learned dynamics. The results of hardware experiments are reported in Section \ref{sec:results}. Finally, we summarize our conclusions and discuss directions for future research in Section \ref{sec:conclusion} .
 
% Using simplified model is evidenced to enable real-time computation; However, it normally sacrifices the target jumping accuracy. On the other hand, full-body dynamic model typically enables accurate jumping with further requirement on off-line solving
% Our work towards that goal by bringing the 
% Numerous recent advancements in robotics draw inspiration from nature, emphasizing the refinement of efficiency and precision in highly dynamic jumping maneuvers targeted at a specific point within real-world applications.

% \section{Related Work} \label{sec:related_work}

% \subsection{Model-based Control and Optimization} Recent advancements in model-based approaches, notably Model Predictive Control (MPC), have proven effective in realizing diverse acrobatic motions \cite{GabrielICRA2021,park2017high,YanranDingTRO,continuous_jump, Quad-SDK}. To facilitate real-time computation, MPC often builds up on simplified dynamics models that combine the body and legs into a unified rigid body. While this approach expedites computations, these simplifications in the robot model may compromise both accuracy and success rates when translating highly agile motions to hardware. At the other end, trajectory optimization (TO) has shown as an effective solution for improving accuracy by considering a full-body dynamics model, making it well-suited for planning acrobatic motions with long flight times \cite{QuannICRA19, matthew_mit2021_1,chuongjump3D}. Full-body trajectory optimization has very high dimensional and objectives are highly nonlinear, which often leads optimization procedures into bad local minima. However, the trajectory optimization can be slow, especially when a good initial guess is not available. Therefore, solutions are normally obtained offline with trajectory optimization.


% In the context of conventional locomotion
% strategies like walking and running, such initial guesses can
% be generated by simplified models [15], but such templates are
% not readily available for tasks that require whole-body shape
% changes like in mid-air acrobatics.

% Although both MPC and trajectory optimization offer promising solutions for dynamic jumping, they typically rely on the accuracy of the model. Nevertheless, an accurate model may hardly be achieved due to uncertainties and unmodelled dynamics involved in jumping motion. 
% For example, the interaction between foot and ground introduces various uncertainties, such as varied friction or unknown ground stiffness and damping. In addition, parameter variations (i.e. inaccurate kinematic parameters) contribute to the model accuracy as well. The authors in \cite{Zachary_RAL_online_calibration_2022} show that the actual leg length of a robot with deformable feet is likely difficult to measure due to dynamic deformation effects and rolling contacts. These problems are likely to cause inaccuracy in hardware transfer. 
% Last but not least, the jumping motion typically involves long flight maneuvers. During this aerial period, the system becomes under-actuated systems and the control has little impact on the robot trajectory during this period \cite{falling_cat}. Therefore, the trajectory errors are normally accumulated and prevent the robot from reaching desired targets at high accuracy. 


% In our prior work \cite{continuous_jump}, we combine real-time MPC
% and joint PD controller to track the reference motion from
% the trajectory optimization under unknown disturbance. The MPC is also designed based on single rigid body dynamics. However, since the predicted horizon of MPC in our prior work is limited, it would not efficient to deal with jumping with long flight time.

% \subsection{Learning-based approaches} 


% \subsection{Dynamics learning.} 

% Saviolo et al. \cite{saviolo2022physics} relax the nominal model's strict physical constraints, guiding the neural network to learn the true system dynamics from data by using soft constraints to guide the training. 










% \textbf{Variational Integrator Networks}
% MPC controllers rely on long-term predictions of the robot states given a control policy, by using an ODE solver to integrate the continuous-time dynamics over time, such as Euler approximation or Runge-Kutta methods. While such solvers are universal, they do not account for the structure or symmetry of a physical system, e.g. respecting the law of energy conservation, leading to poor long-term predictions. Instead,  variational integrators \cite{marsden2001discrete} have been used to predict the future states of a physical system by discretizing Langrange-d'Alembert principle instead of Euler-Lagrange equations, e.g. in astronomy (\todo{cite}) (\todo{search for papers in robotics as well?}). This leads to an integration rule that respects the law of energy conservation and accurately predicts the future trajectory.

% Let $\frakq$ and $\dot{\frakq}$ be the generalized coordinates and velocity. The Lagrangian of the system is defined as the difference between the kinetic energy and the potential energy:
% \begin{equation}
%     \calL(\frakq, \dot{\frakq}) = \frac{1}{2}\dot{\frakq}^\top \bfM \dot{\frakq} - V(\frakq),
% \end{equation}
% where $\bfM$ is the generalized mass, e.g. mass for linear velocity and inertia matrix for angular velocity, and $V(\frakq)$ is the potential energy. The Lagrange-d'Alembert principle states that:
% \begin{equation}
% \label{eq:Lagrange-dAlembert}
%     \delta  \int_0^T \calL(\frakq(t), \dot{\frakq}(t))dt + \int_0^T\bff(\frakq(t), \dot{\frakq}(t), \bfu(t))\delta \frakq(t)dt = 0.
% \end{equation}
% This leads to the standard Euler-Lagrange equations:
% \begin{equation}
% \label{eq:Euler-Lagrange}
%     \frac{\partial \calL(\frakq(t), \dot{\frakq}(t))}{\partial\frakq} - \frac{d}{dt}\left(\frac{\partial \calL(\frakq(t), \dot{\frakq}(t))}{\partial\dot{\frakq}}\right) + \bff(\frakq(t), \dot{\frakq}(t), \bfu(t)) = 0.
% \end{equation}
% While normal integrators discretize Eq. \eqref{eq:Euler-Lagrange}, variational integrators discretize Eq. \eqref{eq:Lagrange-dAlembert} and yield the following integration rules for $\frakq$ in $\bbR^n$:
% \begin{equation}
% \label{eq:var_int_Rn}
%     \begin{aligned}
%         \frakq_{k+1} &= \frakq_k + h\dot{\frakq}_k + \frac{h^2}{2}\bfM^{-1}(F(\frakq_k, \bfu_k) - \nabla V(\frakq_k)) \\
%         \dot{\frakq}_{k+1} &= \dot{\frakq}_k + h\bfM^{-1}(F(\frakq_k, \bfu_k) - \frac{\nabla V(\frakq_k) + \nabla V(\frakq_{k+1})}{2}),
%     \end{aligned}
% \end{equation}
% where $F(\frakq_k, \bfu_k)$ represents the average external force over the time step $h$. Havens et al. \cite{havens2021forced} model $\bfM, F$ and $V$ in Eq. \eqref{eq:var_int_Rn} by neural networks and learn them from data. Please refer to \cite{havens2021forced} and references therein for more details.

% When the coordinates $\frakq$ evolves on the $SE(3)$ manifold, the integration rules are derived to respect both the law of energy conservation and the manifold constraints as follows.
% \begin{equation}
% \label{eq:_var_int_SE3}
%     \begin{aligned}
%    & h\hat{\pi}_k   +   h \hat{\bff}_{d_k}^{R-} + (1-\alpha)h^2 \hat{\xi}_k  =  Z_k J_d - J_d Z_k^\top , \\ &
%     R_{k+1}  = R_k Z_k , \\
%     & \pi_{k+1}  = Z_k^\top \pi_k + (1-\alpha)h Z_k^\top \xi_k+ \alpha h \xi_{k+1}   + Z_k^\top \bff_{d_k}^{R-}+ \bff_{d_k}^{R+}   , \\ &
%       x_{k+1}  =  x_{k} + \frac{h}{m} \gamma_k - (1-\alpha)\frac{h^2}{m} \frac{\partial U_k}{\partial x_k} -  \frac{h}{m} R_k \bff_{d_k}^{x-}  , \\ &
%         \gamma_{k+1}  = \gamma_k - (1-\alpha)h    \frac{\partial U_k}{\partial x_k} - \alpha h \frac{\partial U_{k+1}}{\partial x_{k+1}} +  R_k \bff_{d_k}^{x-} \\ & \qquad \qquad + R_{k+1} \bff_{d_k}^{x+},
% \end{aligned}
% \end{equation}
% where $\pi_{k} = m\bfv_k$ is the linear momentum, $\gamma_k = \mathbf{J}\Omega$ is the angular momentum, and $\hat{\xi}_k = \frac{\partial  V_{k}}{\partial R_{k}}^\top R_{k} - R_{k}^\top \frac{\partial V_{k}}{\partial R_{k}}$. Our previous paper \cite{duruisseaux2022lie} model the mass $(m,\mathbf{J})$, the potential energy $V$ and the generalized force $\bff_d$ by neural networks, trained from data. Please refer to \cite{lee2008computational, duruisseaux2022lie} for more details. (\todo{Unify notations in Eq. \eqref{eq:var_int_Rn} and Eq. \eqref{eq:_var_int_SE3}}).

% \textbf{Energy-based control for jumping.} \todo{Questions}: Can we design an energy-based controller for jumping? The control input is only applied during contact phase, which is different from the setting from our previous paper \cite{Duong-RSS-21}. It is perhaps related to event-triggered control?




% \section{Problem Formulation}
% \label{sec:Method}
% % We separate as two problems: Jumping in 2D and Jumping in 3D



%  to capture the whole-body coordination

% \section{Preliminaries} \label{sec:Preliminaries}
% % We first revisit two fundamental models for quadruped locomotion.

% % \subsection{Full-body dynamics}
% % Jumping is a highly complex motion for a legged robots, requiring coordination of the whole body while respecting all physical constraints of the robots' actuators. To achieve highly accurate jumping, a full-body dynamics model is usually utilized. For quadrupedal animals, high jumping is normally restricted to a sagittal plane. Therefore, this paper will also focus on 2D motion of the robot\NA{This sentence can be moved before the subsubsection as part of the brief overview.}. The robot model thus can be considered as a rigid-body system consisting of $5$ links in the 2D plane\NA{Explain that the 5 links are the 4 legs and the body}. A jumping task is modeled as a sequence of three contact phases: double contact (all legs have contact), single contact (rear legs have contact), and flight (no legs have contact). The equations of motion can be formulated as follows \cite{QuannICRA19}:  
% % %
% % \begin{equation}\label{eq:full_dynamics_2D}
% % \begin{bmatrix}\bm{H} & -(\bm{J}_c^f)^\top \\ -(\bm{J}_c^f)^\top & \mathbf{0} \end{bmatrix} \begin{bmatrix}
% % \bm{\ddot{q}} \\ \bm{f}
% % \end{bmatrix}= \begin{bmatrix}-\bm{C}\bm{\dot q}-\bm{G} + \bm{S}\bm{\tau}+\bm{S}_{f}\bm{\tau}_{f} \\ \bm{\dot J}_{c}^f\bm{\dot q}\end{bmatrix}
% % \end{equation}
% % %
% % % \begin{subequations}\label{eq:gait_1}
% % %     \begin{align}
% % %     \bm{M} \bm{\ddot{q}}+\bm{C}\bm{\dot q}+\bm{g} &= \bm{J}_c^T \bm{f}_c +\bm{S}\bm{\tau}+\bm{S}_{f}\bm{\tau}_{f} \\
% % %     \bm{J}_c^T \bm{\ddot{q}} + \bm{\dot J}_{c}(\bfq)\bm{\dot q} &=0
% % %     \end{align}
% % % \end{subequations}
% % %
% % where $\bfq:=\left[\bfq_b;~\bfq_{j}\right]$ is a vector of generalized coordinates, in which $\bfq_b = [ x,z,q_{pitch}]$ is the body coordinates including CoM\NA{This abbreviation has not been introduced} position and body's pitch angles respectively, and $\bfq_j$\NA{Specify the dimension} is a vector of joint angles.\NA{The sentence should not end here} $\bm{H}$ is the mass matrix, $\bm{C}$ is represented for Coriolis  and centrifugal terms, $\bfA_g$\NA{This is denoted by $\bm{g}$ above} denotes gravity vector. $\bm{J}_c^f(\bfq)$\NA{It may be good to make the dependence on $\bfq$ explicit in the model above} is the spatial Jacobian respectively with the generalized coordinate $\bfq$ and expressed at the contact foot. $\bm{S}$ and $\bm{S}_{fric}$ \NA{This is denoted by $\bm{S}_{f}$ above} are distribution matrices of actuator torques $\bm{\tau}$ and the joint friction torques $\bm{\tau}_{fric}$\NA{This is denoted by $\bm{\tau}_{f}$ above}, $\bm{f}$ is the spatial contact force at the feet. The dimensions of $\bm{J}_c$ and $\bm{f}$ depend on the phase of the gait and the number of legs in contact with the ground.
% \subsection{Single rigid body dynamics}
%  This simplification considers the whole trunk and legs as a unified single rigid body subject to forces at the contact patches (e.g. \cite{park2017high,YanranDingTRO,ParkRSS15}). 
%  % which finds highly efficient to real-time control. 
%  % Although ignoring leg dynamics is a major simplification, the controller
%  % is still able to stabilize a high-DoF system and is robust
%  % to these multi-body effects.
%  % Consider a robot modeled as a single rigid body with position $\bfp \in \bbR^2$, orientation $\theta \in \mathbb{R}$. 
%  We denote the robot's generalized coordinates as $\boldsymbol{\mathfrak{q}} = \begin{bmatrix} \bfp^{\top} & \theta \end{bmatrix}^{\top} \in \mathbb{R}^{3}$, where $\bfp \in \bbR^2$ is the position of center of mass (CoM) of the body, and $\theta \in \mathbb{R}$ is the body orientation. We define the generalized velocity of the robot by $\bfzeta = \begin{bmatrix} \bfv^{\top} & \omega \end{bmatrix}^{\top} \in \mathbb{R}^3$, where $\bfv \in \mathbb{R}^2$ is the linear velocity and $\omega \in \mathbb{R}$ is the angular velocity. Both $\mathfrak{q}$ and $\bfzeta$ are expressed in the world frame. Under the control input $\bfu = \begin{bmatrix} \bff_1^{\top} & \bff_2^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{n_u}$,  robot state $\bfx = \begin{bmatrix} \boldsymbol{\mathfrak{q}}^{\top} & \bfzeta^{\top} & g\end{bmatrix}^{\top} \in \mathbb{R}^{n_x}$ is evolved by the following continuous-time state-space model:
% %
% \begin{equation} \label{eq:nominal_continuous_dynamics}
% 	\dot{\bfx}(t) = \bfA_{ct} \bfx(t) + \bfB_{ct}(\bfr) \bfu(t),
% \end{equation}
% %
% with 
% \begin{equation}
% \begin{aligned}
%     \bfA_{ct} &= 
%     \begin{bmatrix}
%         \bf0_{3} & \bfI_{3} & \bf0 \\ 
%         \bf0_{3} & \bf0_{3} & -\bfe_{3} \\ 
%         \bf0^{\top} & \bf0^{\top} & 0
%     \end{bmatrix}, 
%     \bfB_{ct}(\bfr) = 
%     \begin{bmatrix}
%         \bf0_{3\times2} & \bf0_{3\times2} \\ 
%         \bfI_{2} / m & \bfI_{2} / m \\ 
%         [\bfr_1]_{\times}/J & [\bfr_2]_{\times}/J \\ 
%         \bf0^{\top} & \bf0^{\top}
%     \end{bmatrix},
% \end{aligned}
% \end{equation}
% where $\bfA_{ct}\in \mathbb{R}^{n_x\times n_x}$, $\bfB_{ct} \in \mathbb{R}^{n_x\times n_u}$, $\bfe_3= \begin{bmatrix} 0 & -1 & 0
% \end{bmatrix}^\top$, $m$ is the body mass, $J$ is the moment inertia of the body, $\bfr_i$ is the foot $i = \{1, 2\}$ position relative to the CoM in the world frame and $[\bfr_i]_{\times}^{\top} = \begin{bmatrix} r_{iz} & -r_{ix} \end{bmatrix}^{\top} \in \mathbb{R}^2$. These relative position vectors $\bfr_i$ are combined as $\bfr$ for the sake of notation. The gravity term $g$ is added to the robot state to obtain the convenient state-space form (\ref{eq:nominal_continuous_dynamics}).
% The discrete dynamics is then propagated using the Euler forward scheme as
% \begin{equation} \label{eq:nominal_dynamics}
% 	\bfx_{k+1} = \bfA_k \bfx_{k} + \bfB_k(\bfr_k) \bfu_k,
% \end{equation}
% where $\bfA_k = \bfI_{n_x} + \bfA_{ct} \Delta t$, $\bfB_k= \bfB_{ct} \Delta t$, $\Delta t$ is sampling step.
% \begin{remark}
%     The full-body dynamic model \eqref{eq:full_dynamics_2D} is complex and, normally, not favorable for real-time control\NA{Explain more precisely what makes the model complex and unfavorable for real-time control. Is it the fact that the model is nonlinear due to the term $\bm{J}_c^f(\bfq)$ and its time derivative? Is it the fact that linearizaiton as part of MPC is not accurate?}. In addition, with even higher accuracy, this model still ignores the uncertainties and unknown dynamics. Unlike normal operations, dynamic jumping poses a unique challenge as it rapidly reaches hardware limits. In these extreme conditions, accurately modeling the hardware is challenging. On the other hand, the SRB model (E.q. \ref{eq:simplified dynamics}) is favorable for real-time control. However, this model neglects the leg dynamics, which are important to achieve accurate jumping. 
% \end{remark}
% \subsubsection{Single Rigid Body Dynamics}Another widely used model of robot dynamics is a single rigid body \cite{park2017high,YanranDingTRO,ParkRSS15}. This model treats the whole robot as a single rigid body, neglecting the leg dynamics  which finds highly efficient to real-time control.\NA{An equation should be part of a sentence.}\NA{We had denoted gravity as $\bm{g}$ before.}\NA{Why is the second equation below using $\frac{\mathrm{d}}{\mathrm{d} t}(I_b {\bm{\omega}})$ on the right-hand side? Is $I_b$ a function of the state?}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{subequations}\label{eq:simplified dynamics}
%     \begin{align} \label{eq:simplified dynamics}
%     \ddot{\bm{p}} =\frac{\sum_{i=1}^{2}\bm{f}_{i}}{m}-\bfA_g, ~~~ \frac{\mathrm{d}}{\mathrm{d} t}(I_b {\bm{\omega}}) =\sum_{i=1}^{2} \mathbf{r}_{i} \times \bm{f}_{i},
%     \end{align}
% % \end{subequations}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% where $\bm{p} =[p_x; p_z] \in \mathbb{R}^2$ is the CoM position in the world frame; $\bfr_i=[r_{ix};r_{iz}]$ and $\bm{f}_i=[f_{ix};f_{iz}]$ denotes the position of contact point relatively to CoM, and contact force at foot $i^{th}$ respectively in the world frame; $\bm{\omega}=\dot{\theta} \vec{k}$ is angular velocity of the body; $\theta$ is a pitch angle. \NA{What is $\vec{k}$? What is $I_b$?}


% We define $\bfx^s=[\bm{p};\theta;\dot{\bm{p}};\dot{\theta},a_g]$\NA{Why is gravity part of the state?} as the state of a simplified dynamics, $a_g$ is gravity, $\bfu^s=[\bm{f}_1^\top; \bm{f}_2^\top]$\NA{The notation here is weird. Why do we have ";" to separate the variables and why do we have transpose on the entries but not on the overall vector. Are we trying to obtain a column vector?}. Then, the simplified dynamics in continuous time can be rewritten as:\NA{Should we have $\bfB_{ct}$ instead of $\bfB_{ct}$?}
% \begin{equation}\label{eq:simplified_dynamics}
% \dot{\bfx}^s=\bfA_{ct}\bfx^s+\bfB_{ct}(\bfr) \bfu^s,
% \end{equation}
% where
% \\
% $\bfA_{ct}= \begin{bmatrix}
% \bm{0} & \bfI & \bm{0}\\
% \bm{0} & \bm{0} & \bm{e}_g\\
% \bm{0} & \bm{0} & \bm{0}
% \end{bmatrix}$, $\bfB_{ct}(\bfr)= \begin{bmatrix}
% \bm{0} & \bm{0}\\
% \bfI/m & \bfI/m \\
%  [\bfr_1]_{\times}/I_b &  [\bfr_2]_{\times}/I_b \\
% \bm{0} & \bm{0}
% \end{bmatrix}$, $\bm{e}_g= \begin{bmatrix} 0 & -1 & 0
% \end{bmatrix}^\top$ \\
% % $\bm{\sigma}_i= I_b^{-1} \begin{bmatrix} -r_{iz} & r_{ix}
% In discrete time, 
% \begin{equation}\label{eq:dis_simplified_dynamics}
% \bfx_{k+1}^s=\bfA\bfx_k^s+\bfB(\bfr_k) \bfu_k^s,
% \end{equation}

% \begin{remark}
%     The full-body dynamic model \eqref{eq:full_dynamics_2D} is complex and, normally, not favorable for real-time control\NA{Explain more precisely what makes the model complex and unfavorable for real-time control. Is it the fact that the model is nonlinear due to the term $\bm{J}_c^f(\bfq)$ and its time derivative? Is it the fact that linearizaiton as part of MPC is not accurate?}. In addition, with even higher accuracy, this model still ignores the uncertainties and unknown dynamics. Unlike normal operations, dynamic jumping poses a unique challenge as it rapidly reaches hardware limits. In these extreme conditions, accurately modeling the hardware is challenging. On the other hand, the SRB model (E.q. \ref{eq:simplified dynamics}) is favorable for real-time control. However, this model neglects the leg dynamics, which are important to achieve accurate jumping. 
% \end{remark}

% This motivates us to use propose Neural Network:
% \begin{itemize}
%     \item learn residual dynamics to compensate for model uncertainties and unknown dynamics.
%     \item choose to learn residual dynamics for single rigid body to enable real-time control with MPC
% \end{itemize}

% \begin{figure}[!tpb]
%       \centering
%       % \vspace{.06in}
%       % \vspace{-1em}
%       \includegraphics[width=2.7in,trim={0cm 0cm 0cm 0.5cm},clip]{figures/jumping_phases.png} \\
%       \vspace{-0.6em}
%       \caption{A generalized jumping motion in 2D. }
%       \label{fig:jumping_phases}
%       \vspace{-1.5em}
% \end{figure}
% \begin{figure}[!tpb]
%       \centering
%       % \vspace{.06in}
%       % \vspace{-1em}
%       \includegraphics[width=2in,trim={0cm 1.7cm 0cm 0cm},clip]{figures/2D_rigid.png} \\
%       \vspace{-0.em}
%       \caption{A rigid body in 2D. }
%       \label{fig:2D_rigid_body}
%       \vspace{-0.5em}
% \end{figure}
% \subsection{3D jumping}

% The single rigid body dynamics in SE(3) has a form
% \begin{subequations}\label{eq:SRB_dynamics}
%     \begin{align}
%         \ddot{\bm{p}}&=\sum_{s=1}^{n_s} \bm{f}^{s}/m-\bm{g}, \label{eq:SRB_dynamics1}\\
%         \bm{I_b} \dot{\bm{\Omega}} + \bm{\Omega} \times \bm{I_b} \bm{\Omega} &= \bfr^{-1} \sum_{s=1}^{n_s} \bm{f}^s \times (\bm{p} - \bm{p}_f^s) ,\label{eq:SRB_dynamics2}\\
%         \dot{\bfr} &= \bfr\widehat{\mathbf{\Omega}}\label{eq:SRB_dynamics3}
%     \end{align}
% \end{subequations}

% where $n_s$ is number of feet, m is the robot's mass, $\bm{\Omega} \in \mathbb{R}^3$ is angular velocity expressed in the body frame, $\bfr$ is rotation matrix of the body frame, $\bm{g}$ is the gravity acceleration; $\bm{p}, \dot{\bm{p}}, \ddot{\bm{p}} \in \mathbb{R}^3$ is the CoM position, velocity, acceleration of the body in the world frame; $\bm{f}^s \in \mathbb{R}^3$ is GRF on foot $s^{th}$;   $\bm{p}_f^s \in \mathbb{R}^3$ is $s^{th}$ foot position in the world frame. The hat map $(\hat{.}):\mathbb{R}^3  \rightarrow so(3) $ converts any vector in $\mathbb{R}^3$ to the space of skew-symmetric matrices. For the sake of notation, we define the robot's state as
% $\bfx:=\left[\bm{p}; \dot{\bm{p}}; \bm{\Omega}; \dot{\bm{\Omega}}; \bfr\right]$. 

% \section{Problem Statement}
% \label{sec:problem_statement}



% Further, we aim to design a model predictive controller that attempts to track a desired state trajectory $\bfx^*(t)$, $t \geq t_0$, for any learned realization $\tilde{\bff}_{\bftheta}$ of the robot dynamics and unknown disturbance and uncertainties\NA{We keep mentioning disturbance and uncertainty but I am not sure what this is referring to. Where in the models do we have uncertainty and disturbances?}.

% \begin{problem}
% \label{problem:setpoint_reg}
% Given an initial condition $\bfx_0$ at time $t_0$, desired state trajectory $\bfx^*(t)$, $t \geq t_0$, and learned dynamics $\tilde{\bff}_{\bftheta}$, design a model predictive control law $\bfu = \bfpi(\bfx, \bftheta, \bfx^*(t))$ for contact phases to track the whole jumping reference that involves long acrobatic period.
% \end{problem}

% In our setting, the robot kinematics need to evolve over the $SE(3)$ manifold and the dynamics $\bff(\bfx, \bfu)$ respect the law of energy conservation, when there is no control input, $\bfu = \bf0$. We embed these constraints in the structure of the parametric function $\tilde{\bff}_{\bftheta}$. We review the $SE(3)$ kinematics and Hamiltonian dynamics equations next.


% \section{Problem Statement} \label{sec:statement}
% In the following, we present the learning model with adaptive frequency and model predictive control for the learned dynamics.



% \subsection{Residual Dynamics}

% - \note{use u as control input --> uncertainties in contact, motor dynamics, hardware model --> }
% - \note{problem statement}


% \note{We consider \ref{eq:nominal_continuous_dynamics} as nominal model , then develop residual dynamics}


% Our main objective is to formulate a real-time executable MPC scheme for controlling
% quadruped robotics to perform a variety of dynamic motions. To meet the real-time require-
% ment, the optimization problem posed by the MPC has to be solved robustly at a high rate
% on the mobile embedded computer, which has limited computational resources. Hence, a
% simplified model is adopted to reduce the dimensionality of the optimization problem. Since
% the mass of all legs combined is less than 10% of the total body mass, a single rigid body
% model serves as a reasonable approximation.
\begin{figure*}
      \centering
      \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=\linewidth]{figures/framework-v5.pdf}
      \caption{\textbf{System Architecture}. The learning procedure and MPC execution are paired with the same adaptive frequency $\lbrace \Delta t_{\calC}, \Delta t_{\calF} \rbrace$, prediction horizon $K$, and contact schedule ($cs$). The MPC and low-level joint PD controllers are updated at $40Hz$ and $1kHz$, respectively. 
      % The MPC aim to track the jumping reference $\bfx^*$ from full-body trajectory optimization \cite{QuannICRA19}.      
      % The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $
      }
      \label{fig:overview_framework}
      %\vspace{-0.5em}
\end{figure*}

\section{Problem Statement} \label{sec:problem_statement}

% \NA{I think we should have a problem statement section that explains what we are trying to do before we have an overview of how we are doing it.}

Consider a legged robot modelled by state $\bfx_k$, consisting of the pose and velocity of the body's center of mass (CoM), foot positions $\bfr_k$ relative to the body's CoM, and ground force control input $\bfu_k$ at the legs, sampled at time $t_k$. We  augment the nominal SRBD model (e.g., \cite{GabrielICRA2021, park2017high,YanranDingTRO}) with a learned residual term to account for leg dynamics, model mismatch with the real robot hardware, as well as capture complex dynamic effects in contact and hardware:
%
\begin{equation}\label{eq:discrete_learned_model}
    \bfx_{k+1} = \bff\left(\bfx_k, \bfu_k, \bfr_{k}, \Delta t_k \right) + \delta\bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k},\Delta t_k \right),
\end{equation}
%
where $\bff$ represents the nominal SRBD model, $\delta\bff_{\bftheta}$ with parameters $\bftheta$ approximates the residual dynamics, and $\Delta t_k$ is the sampling interval. Our first objective is to learn the residual dynamics $\bff_{\bftheta}$ using a dataset of jumping trajectories.


%on the dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consisting of $D$ state sequences $\bfx^{(i)}_{0:K}$, obtained by applying control inputs $\bfu^{(i)}_{0:K}$ to the system, and $\bfr^{(i)}_{0:K}$ represents the foot positions.
% $\bff_{\bftheta}$ with state $\bfx_{0:K-1}^{(i)}$ and control $\bfu^{(i)}_{0:K-1}$ 
% \tilde{\bfx}^{(i)}_k = \tilde{\bfx}^{(i)}(t_k), \quad 
%  of $K+1$ collocation points}
% indexed by $t_{0:K}$

\begin{problem} \label{problem:dynamics_learning}
Given a set $\calD \!=\! \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ of $D$ sequences of states, foot positions, and control inputs,
% \NA{Do we need the time indices $t_{0:K}$?},
find the parameters $\bftheta$ of the residual dynamics $\delta \bff_{\bftheta}$ in \eqref{eq:discrete_learned_model} by rolling out the dynamics model and minimizing the discrepancy between the predicted state sequence $\tilde{\bfx}^{(i)}_{1:K}$ and the true state sequence $\bfx^{(i)}_{1:K}$ in $\calD$:
%
\begin{align}
\min_{\bftheta} \;&\sum_{i = 1}^D \sum_{k = 1}^K \mathcal{L} (\bfx^{(i)}_k,\tilde{\bfx}^{(i)}_k) + \calL_{\text{reg}}(\bftheta) \notag\\
\text{s.t.} \;\; & \tilde{\bfx}^{(i)}_{k+1} = \bff \left(\tilde{\bfx}^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k, \Delta t_k\right)\notag\\ 
&\qquad \qquad\qquad + \delta \bff_{\bftheta}\left(\tilde{\bfx}^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k, \Delta t_k \right), \notag\\
& \tilde{\bfx}^{(i)}_0 = \bfx_{0}^{(i)}, \quad \forall k=0,...,K-1, \label{eq:problem_formulation_unknown_env_equation}
\end{align}
%
where $\mathcal{L}$ is an error function in the state space, and $\calL_{\text{reg}}(\bftheta)$ is a regularization term to avoid overfitting. Note that it is not necessary for $\Delta t_k = t_{k+1}-t_{k}$ to be fixed.
\end{problem}

After learning to improve the accuracy of model prediction, our second objective is to use the learned model \eqref{eq:discrete_learned_model} for MPC to track a desired state trajectory $\bfx_{0:K}^*$.

\begin{problem} \label{problem:mpc_learn}
Given the dynamics model \eqref{eq:discrete_learned_model}, a current robot state $\bfx_0$ and foot positions $\bfr_0$, a desired trajectory of states $\bfx^*_{0:K}$, foot positions $\bfr^*_{0:K}$, and control $\bfu^*_{0:K}$,
% \NA{Do we need the time indices $t_{0:K}$?},
design a control law $\bfu_0 = \bfpi(\bfx_0, \bfr_0, \bfx^*_{0:K}, \bfr^*_{0:K},\bfu^*_{0:K}; \bftheta)$ to achieve accurate and robust tracking of the desired state trajectory via shifting-horizon optimization:
%
\begin{align}
\min_{\bfu_{0:K-1}} \;& \sum_{k = 1}^K \| \bfx_k-\bfx_{k}^* \|_{\bfQ_k} + \| \bfu_{k-1}-\bfu_{k-1}^* \|_{\bfR_k} \notag\\
\text{s.t.} \;\; & \bfx_{k+1} = \bff\left(\bfx_k, \bfu_k, \bfr_{k}, \Delta t_k \right) + \delta \bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k}, \Delta t_k \right), \notag\\
& \bfu_k \in \calU_k, \quad \forall k=0,...,K-1, \label{eq:mpc_formulation}
\end{align}
%
where $\bfQ_k$ and $\bfR_k$ are positive definite weight matrices,
% weight matrices, i.e., diagonal matrices with positive diagonal entries,
% \NA{Do we need $\bfP_k$ to be positive semidefinite and $\bfQ_k$ to be positive definite? The usual notation is to use $\bfQ_k$ for $\bfx_k$ and $\bfR_k$ for $\bfu_k$. We should define what we mean by $\|\cdot\|_{\bfQ}$. Do we need to select $\bfu_K$? Seems that it will always be equal to $\bfu_K^*$ in the above optimization.}, 
and $\calU_{0:K-1}$ represents an input constraint set. 
% \CN{I just corrected the equation (3)}
\end{problem}

% Achieving accurate target jumping with MPC requires not only an accurate model but also consideration of the desired trajectory $\bfx_{0:K}^*,\bfr_{0:K}^*,\bfu_{0:K}^*$, including the final state upon landing. 
Achieving accurate target jumping with MPC requires not only an accurate model but also the coverage of the final state upon landing, which represents the accuracy of the jumping target. Using a fixed-frequency has shown to be efficient for locomotion tasks with limited aerial phases; however, this can face two challenges in long-flight maneuvers. On the one hand, using a fine time-step dirscretization enhances the model prediction accuracy but requires a large number of steps to capture the entire flight phase, thereby increasing the optimization size and computational cost. On the other hand, using a coarse time-step discretization allows capturing the entire flight phase efficiently but can sacrifice model prediction accuracy. For jumping tasks, different phases may require different model resolutions, e.g., fine time resolution during the contact phase but coarser time resolution during the flight phase as the model complexity is reduced due to unavailable force control and contact. Therefore, we propose to learn a model for dynamic maneuvers (Problem \ref{problem:dynamics_learning}) with an adaptive-frequency scheme that uses a coarse time discretization in the flight phase and a fine time discretization in the contact phase. Importantly, this adaptive-frequency scheme is also synchronized with the MPC control of the learned model (Problem \ref{problem:mpc_learn}) to leverage the same discretization errors when using the model for MPC predictions. Thus, in our formulation $t_{0:K}$ does not have equal time steps and is a mixture of fine and coarse discretization capturing the contact and flight phases of a jumping motion.



% Given the dynamics model in \eqref{eq:discrete_learned_model}, design a control law \rep{$\bfu_k = \bfpi(\bfx_k, \bfr_k, \bftheta, \bfx^*_{0:K}, \bfr^*_{0:K},\bfu^*_{0:K})$} 
% % \NA{Should this depend on $\bfr_k$ as well?}\NA{Should the policy depend on a reference control input $\bfu^*_{0:K}$ as well? It seems that trajectory optimization provides this as well.} 
% to achieve accurate and robust tracking of a desired state trajectory $\bfx_{0:K}^*$.
% %target jumping, which involves flight phase (i.e. extreme underactuated systems).
% % that involves long acrobatic period.


% \rep{Explain Adaptive frequency here}
% Jumping and Flight phase --> use adaptive frequency -->  Define of time step $t_{0:K}$, sample with different freq
% The MPC design tailor for jumping motions consisting of two distinguish phases: contact and flight phase. 



% \CN{I added this paragraph to explain the adaptive frequency; it seems a little bit long and replicates some information from the introduction. \textcolor{red}{ Please let me know if you have any suggestions}} 

%the coverage of the final state upon landing, which represents the accuracy of the jumping target. 

%for discretization normally enhances the dynamic representation, but it also requires a  large number of prediction steps to leverage the entire flight maneuvers, thereby increasing the optimization size and computational cost.

%On the other hand, adopting relaxed time steps leverage the whole flight prediction with computational efficiency but can sacrifice model accuracy\NA{I am not sure what this sentence means}.
% Using fine time-step discretization normally enhances the prediction accuracy, but it also requires a large number of prediction steps to leverage the entire light phase. This likely increases the optimization size and computational cost that can ruin the real-time performance. 





% The adaptive-frequency protocol relaxes the time steps for the discretization of flight-phase dynamics while still keeping a fine sampling time for robot dynamics in the contact phase. 

%In our formulation, $t_{0:K}$ does not necessarily have equal time intervals. It can be a mixture of fine and relaxed time steps if the horizon involves different phases. 
% Therefore, $t_{0:K}$ do not necessarily have the same length of time due to the adaptive-frequency sampling policy.


% For example, the time sequence is not sampled
% \CN{I rewrite this section to describe system overview}

\section{System Overview}
\label{sec:sys_overview}

Fig. \ref{fig:overview_framework} presents an overview of our system architecture. Our approach consists of two stages: adaptive-frequency model learning (Sec. \ref{sec:adaptive-frequency-learning}) and adaptive-frequency MPC (Sec. \ref{sec:adaptive-MPC}), which solve Problem~\ref{problem:dynamics_learning} and Problem~\ref{problem:mpc_learn}, respectively.
% Our approach for quadruped jumping consists of three stages
% \NA{We should give the three stages good names and use them consistently in the figures and section captions.}: data collection, adaptive-frequency model learning (Problem~\ref{problem:dynamics_learning}), and adaptive-frequency MPC (Problem~\ref{problem:mpc_learn})
% \NA{The caption of Fig.~\ref{fig:overview_framework} is not very well organized. The second sentence is already discussing paring adaptive frequencies but we have not even explained what adaptive frequency means yet. We should first provide an overview of the 3 stages: data collection, model learning, and MPC before delving into the details.}. 
% In the data collection stage (Sec. \ref{subsec:data_gen})\NA{Should we discuss only 2 stages and merge the data collection with the model learning stage? This will be better aligned both with the two problems above and with the two sections (3 and 4) that follow.}, we combine nominal MPC using a conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD\NA{Has this acronym been defined?} controller to generate diverse motions with different jumping references and disturbance. 

We synchronize the adaptive-frequency scheme for both model learning and MPC execution with the same \textit{(1)} adaptive sampling time $\Delta t_{\calC}$ and $\Delta t_{\calF}$ for contact and flight phase, respectively, \textit{(2)} the same horizon length $K$ for all data collection, training, and MPC, and \textit{(3)} the same contact schedule.
% \NA{What is a contact schedule?}. 
Full-body trajectory optimization (TO) \cite{QuannICRA19} is utilized to generate jumping references for various targets, including body states $\bfx^*$, joint states $\lbrace \bfq_{\mathbf{J}}^*, \dot{\bfq}_{\mathbf{J}}^* \rbrace$, ground contact force $\bfu^*$, and foot positions $\bfr^*$. 
For data collection, we combine a baseline MPC using a nominal SRBD model and joint PD 
% \TD{Have we defined PD before using this abbreviation?}
controller, generating diverse motions under disturbances. For training, we design a neural network to learn the discretized residual model $\delta \bff_{\bftheta}$ with adaptive sampling time via supervised learning. For control, we design an adaptive-frequency MPC using the learned dynamics to track a desired reference trajectory obtained from full-body TO. 
% It works together with a high-frequency joint tracking PD controller to execute jumping motions. 
% \NA{I don't think this sentence is adding much.}. 
The feedback states from the robot include global body's CoM $\bfx$, and joint states $\bfq_{\mathbf{J}}, \dot{\bfq}_{\mathbf{J}} \in \mathbb{R}^4 $, and foot positions $\bfr \in \mathbb{R}^4$.
% \NA{The sentence is out of place here. This information should be presented earlier.}. 



% These models aim
% to predict robot states for the upcoming $K$ horizons as MPC
% schedule, which can cover contact transitions and the entire
% flight phase
% In contrast with existing methods, we use adaptive sampling time in the learning process to cover both the contact transitions and the entire flight phase within the MPC planning horizon\NA{Currently we are highlighting the adaptive frequency twice. Once during model-learning and once during MPC. It may be confusing. Should we highlight it once, e.g., just for the MPC to keep it clear in the reader's mind what the key ideas in the three stages are?}.


% Using adaptive sampling time enables MPC to cover the entire flight phase and the transition between jumping phases within planning horizons}
% \NA{Currently we are highlighting the adaptive frequency twice. Once during model-learning and once during MPC. It may be confusing. Should we highlight it once, e.g., just for the MPC to keep it clear in the reader's mind what the key ideas in the three stages are?}.
% It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. 
% The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $\NA{The information in this and the previous sentence should be moved later. They read like low-level details rather than the key novelty of the adaptive MPC}
% \todo{Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness. We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. 
% \NA{This information needs more context. What does adaptive-frequency mean? Why is it useful? Are we the first to propose it?}
% \NA{Are we the first to propose it?}

%To tackle these problems, we propose the following system architecture as depicted in Fig. \ref{fig:overview_framework}, which includes the baseline MPC with nominal SRBD for collecting data for training, the Adaptive-frequency learning (Sec. \ref{sec:adaptive_learn_model}, \ref{sec:training}), and the Adaptive-frequency MPC for the learned dynamics (Sec. \ref{sec:adaptive-MPC}). 


%Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness. We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. For data collection, we combine nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD controller, generating diverse motions with different jumping references and disturbance, as presented in Sec. \ref{subsec:data_gen}. For adaptive-frequency learning, we design neural networks to learn the discretized models for contact and flight phases with adaptive sampling time via the supervised learning, aiming to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover contact transitions and the entire flight phase. Finally, adaptive-frequency MPC is designed to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 


% % The proposed learning-based MPC framework comprises of
% % two primary parts, the Adaptive-frequency model training and the Adaptive-frequency MPC execution for the learned dynamics, which are presented in Sec. \ref{sec:training} and \ref{sec:adaptive-MPC} respectively.

% % Conventional MPC usually either adopt fixed frequency in state prediction or has not leverage of legged dynamics in dynamic model, which may limits accurate trajectory prediction for whole long flight phase. 
% Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness.
% % Unlike conventional MPC, we design a learning residual model and adaptive-frequency to leverage the effect of complex leg dynamics, unknown dynamics in contact and hardware, as well as compensate for model mismatch, which will then followed by adaptive prediction frequency design to leverage the whole flight phase inside MPC predictions. 
% % Both factors are combined as a unified model, allowing us to enhance the accuracy of trajectory prediction for long flight phase within a limited MPC horizon. 
% We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. 
% % We denote the synchronized sampling time $\Delta t_{\calC}$ and $\Delta t_{\calF}$ for contact and flight phase, $\Delta t_{\calF} > \Delta t_{\calC}$, respectively. 
% % This synchronization aims to avoid conflict in discretization. 
% % \textcolor{red}{We use the same contact schedule}
% For data collection, we combine nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD controller, generating diverse motions with different jumping references and disturbance, as presented in Sec. \ref{subsec:data_gen}. 
% % For data collection for jumping, we combine both nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) for high-level body trajectory tracking and joint PD controller for low-level joint profile tracking, generating a diverse motions with different jumping references and disturbance. 
% % presented in Sec. \ref{subsec:data_gen}. 
% For adaptive-frequency learning, we design neural networks to learn the discretized models for contact and flight phases with adaptive sampling time via the supervised learning, aiming to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover contact transitions and the entire flight phase.
% % For adaptive-frequency learning, we design neural networks with Pytorch to learn the discretized models for contact and flight phases with adaptive sampling time. The training is based on supervised learning and we aim to learn the model to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover the contact transition and the entire flight phase.
% Finally, adaptive-frequency MPC is designed to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 





%for contact and flight phase $\calD$, the nominal dynamics $\bff$, and  function $\bff_{\bftheta}$ representing residual dynamics,
% $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$, 
% a function $\bff$ representing nominal SRBD (e.g. \cite{GabrielICRA2021, park2017high,YanranDingTRO}), and a function $\bff_{\bftheta}$ representing residual dynamics, 
%we aim to optimize the parameters $\bftheta$ 



%system and unknown dynamics in the contact and hardware, which yields the discrete-time model:
% Importantly, we also aim to design model predictive control using the learned model to achieve accurate jumping under uncertainty.
% We utilize the simplified dynamics to enable real-time control but propose to learn a residual term to account for legged dynamics and other model uncertainties in contact dynamics or hardware. 
% The proposed discrete-time model with residual dynamics can be characterized as follows

% where the nominal and residual dynamics are defined as
% \begin{equation}\label{eq:discrete_learned_model}
% \begin{aligned}
%     \bff\left(\bfx_k, \bfu_k, \bfr_{k} \right) = & \bfA_k \bfx_{k} + \bfB_k(\bfr_k) \bfu_k,\\ 
%     \bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k} \right) = & 
%  \bfh_{\bftheta}(\bfx_k, \bfr_{k})  + \bfG_{\bftheta}(\bfx_k, \bfr_{k}) \bfu_k.
% \end{aligned}
% \end{equation}


% Consider a robot with state $\bfx$ consisting of its position $\bfp \in \mathbb{R}^3$, orientation $\bfR\in SO(3)$, body-frame linear velocity $\bfv \in \bbR^3$, and body-frame angular velocity $\bfomega\in \mathbb{R}^3$. 

% Let $\bfx_{k+1} = \bff(\bfx_{k}, \bfu_k)$\NA{This is a sudden jump since in the previous section we specified continuous-time models}\NA{I see that there is a cleaner formulation in green in the appendix.} characterize the robot dynamics with control input $\bfu$. We assume that the function $\bff$ represented the unknown robot dynamics in discrete time, for which we aim to approximate it using a dataset $\mathcal{D}$ of state and control trajectories\NA{Use present tense. The second part of this sentence is awkward. Rewrite.}. Specifically, let $\calD = \{t_{0:N}^{(i)}, \bfx^{(i)}_{0:N}, \bfr^{(i)}_{0:N}, \bfu^{(i)}_{0:N}\}_{i=1}^D$ consist of $D$ state sequences $\bfx^{(i)}_{0:N}$, obtained by applying appropriate\NA{What does appropriate mean?} control inputs $\bfu^{(i)}_{0:N}$ to the system, and $\bfr^{(i)}_{0:N}$ represents the foot position.
% with initial condition $\bfx^{(i)}_0$ at time $t_0^{(i)}$ and sampling its state $\bfx^{(i)}(t_n^{(i)}) =: \bfx^{(i)}_n$ at times $t_0^{(i)} < t_1^{(i)} < \ldots < t_N^{(i)}$. 
% We aim to find a function $\tilde{\bff}_{\bfbeta}$ with parameters $\bfbeta$ that approximates the residual\NA{Why residual? This idea has not been introduced.} dynamics $\bff$ on the dataset $\mathcal{D}$. To optimize the parameters $\bfbeta$, we roll out the approximate dynamics $\tilde{\bff}_{\bfbeta}$ with initial state $\bfx_0^{(i)}$ and control $\bfu^{(i)}_{0:N}$ and minimize the discrepancy between the computed state sequence $\tilde{\bfx}^{(i)}_{1:N}$ and the true state sequence $\bfx^{(i)}_{1:N}$ in $\calD$. The dynamics learning problem is summarized below.
%where a function $\bff$ representing nominal SRBD, and $\bff_{\bftheta}$ with parameters $\bftheta$ approximates the residual dynamics on the dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consisting of $D$ state sequences $\bfx^{(i)}_{0:K}$, obtained by applying control inputs $\bfu^{(i)}_{0:K}$ to the system, and $\bfr^{(i)}_{0:K}$ represents the foot positions.
% To optimize the parameters $\bftheta$, we roll out the approximate dynamics $\bff_{\bftheta}$ with initial state $\bfx_0^{(i)}$ and control $\bfu^{(i)}_{0:K}$ and minimize the discrepancy between the computed state sequence $\tilde{\bfx}^{(i)}_{1:K}$ and the true state sequence $\bfx^{(i)}_{1:K}$ in $\calD$. 
% The dynamics learning problem is stated below.

% \begin{problem}
% \label{problem:dynamics_learning}
% Given a dataset for contact and flight phase $\calD$, the nominal dynamics $\bff$, and  function $\bff_{\bftheta}$ representing residual dynamics,
% % $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$, 
% % a function $\bff$ representing nominal SRBD (e.g. \cite{GabrielICRA2021, park2017high,YanranDingTRO}), and a function $\bff_{\bftheta}$ representing residual dynamics, 
% we aim to optimize the parameters $\bftheta$ by rolling out the approximate dynamics $\bff_{\bftheta}$ with state $\bfx_{0:K-1}^{(i)}$ and control $\bfu^{(i)}_{0:K-1}$ and minimizing the discrepancy between the predicted state sequence $\tilde{\bfx}^{(i)}_{1:K}$ and the true state sequence $\bfx^{(i)}_{1:K}$ in $\calD$:
% %
% \begin{equation}
% \label{eq:problem_formulation_unknown_env_equation}
% \begin{aligned}
% \min_{\bftheta} \;&\sum_{i = 1}^D \sum_{k = 1}^K \mathcal{L} (\bfx^{(i)}_k,\tilde{\bfx}^{(i)}_k)\\
% \text{s.t.} \;\; & \tilde{\bfx}^{(i)}_{k+1} = \bff \left(\bfx^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k \right) + \bff_{\bftheta}\left(\bfx^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k \right), \\
% & \tilde{\bfx}^{(i)}_k = \tilde{\bfx}^{(i)}(t_k), \quad \tilde{\bfx}^{(i)}_0 = \bfx_{0}^{(i)}, \quad \forall k=0,...,K-1,
% \end{aligned}
% \end{equation}
% %
% where $\mathcal{L}$ is a distance metric on the state space.
% \end{problem}



%that tracks a desired state trajectory $\bfx^*(t)$, $t \geq t_0$, for the learned realization of the robot dynamics with unknown dynamics and model mismatches (\ref{eq:discrete_learned_model}).

% \begin{problem}
% \label{problem:setpoint_reg}
% Given an initial condition $\bfx_0$ at time $t_0$, desired state trajectory $\bfx^*(t)$, $t \geq t_0$, and learned realization (\ref{eq:discrete_learned_model}), design a model predictive control law $\bfu = \bfpi(\bfx, \bftheta, \bfx^*(t))$ to achieve both accurate and robust target jumping, which involves flight phase (i.e. extreme underactuated systems).
% % that involves long acrobatic period.
% \end{problem}

% To tackle these problems, we propose the following system architecture as depicted in Fig. \ref{fig:overview_framework}, which includes the baseline MPC with nominal SRBD for collecting data for training, the Adaptive-frequency learning (Sec. \ref{sec:adaptive_learn_model}, \ref{sec:training}), and the Adaptive-frequency MPC for the learned dynamics (Sec. \ref{sec:adaptive-MPC}). 

% % The proposed learning-based MPC framework comprises of
% % two primary parts, the Adaptive-frequency model training and the Adaptive-frequency MPC execution for the learned dynamics, which are presented in Sec. \ref{sec:training} and \ref{sec:adaptive-MPC} respectively.

% % Conventional MPC usually either adopt fixed frequency in state prediction or has not leverage of legged dynamics in dynamic model, which may limits accurate trajectory prediction for whole long flight phase. 
% Unlike conventional MPC, we design a learning residual model and learning-based MPC with adaptive-frequency scheme to enhance both target accuracy and robustness.
% % Unlike conventional MPC, we design a learning residual model and adaptive-frequency to leverage the effect of complex leg dynamics, unknown dynamics in contact and hardware, as well as compensate for model mismatch, which will then followed by adaptive prediction frequency design to leverage the whole flight phase inside MPC predictions. 
% % Both factors are combined as a unified model, allowing us to enhance the accuracy of trajectory prediction for long flight phase within a limited MPC horizon. 
% We synchronize the adaptive-frequency scheme for all data collection, model learning, and MPC execution. 
% % We denote the synchronized sampling time $\Delta t_{\calC}$ and $\Delta t_{\calF}$ for contact and flight phase, $\Delta t_{\calF} > \Delta t_{\calC}$, respectively. 
% % This synchronization aims to avoid conflict in discretization. 
% % \textcolor{red}{We use the same contact schedule}
% For data collection, we combine nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) and joint PD controller, generating diverse motions with different jumping references and disturbance, as presented in Sec. \ref{subsec:data_gen}. 
% % For data collection for jumping, we combine both nominal MPC using conventional SRBD model (e.g. \cite{YanranDingTRO,ChignoliICRA2022}) for high-level body trajectory tracking and joint PD controller for low-level joint profile tracking, generating a diverse motions with different jumping references and disturbance. 
% % presented in Sec. \ref{subsec:data_gen}. 
% For adaptive-frequency learning, we design neural networks to learn the discretized models for contact and flight phases with adaptive sampling time via the supervised learning, aiming to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover contact transitions and the entire flight phase.
% % For adaptive-frequency learning, we design neural networks with Pytorch to learn the discretized models for contact and flight phases with adaptive sampling time. The training is based on supervised learning and we aim to learn the model to predict robot states for the upcoming $K$ horizons as MPC schedule, which can cover the contact transition and the entire flight phase.
% Finally, adaptive-frequency MPC is designed to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. It works together with a high-frequency joint tracking PD controller to execute dynamic jumping motions. The feedback states from robot includes global body's CoM $\bfx $, and the joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 
% With the constructed adaptive residual learning model, the MPC is formulated with adaptive frequency in prediction in order to track the adaptive sampling body's reference trajectory $\bfx^*$ from full-body TO. The real-time MPC works together with high-frequency joint tracking PD controller to execute entire dynamic jumping motion. The feedback states from robot includes global body's CoM $\bfx $, and the local joint profile $\bfq_j, \dot{\bfq}_j \in \mathbb{R}^4 $. 
% The transformation $\mathbf{J}^T \bfR^T$ converts the output of MPC controller in world frame to joint torque in the robot frame, where $\mathbf{J} (\bfq_j)^T$ is leg Jacobian and $\bfR$ is rotation matrix. 
% The references for MPC and joint PD controller are obtained from full-body TO (e.g. \cite{QuannICRA19}). 

% We implement MPC for the nominal dynamics model (\ref{eq:nominal_dynamics}) to track reference from full-body TO \cite{QuannICRA19}, generating various jumping motions to different targets. The ground disturbances (i.e. blocks under feet with random height) are added to obtain a variety set of data for training.



\section{Adaptive-Frequency Model Learning}
\label{sec:adaptive-frequency-learning}

In this section, we describe how to learn the residual dynamics $\delta \bff_{\bftheta}$ from data with an adaptive-frequency scheme that can cover the entire flight phase, the final state upon landing, and the contact transitions between jumping phases.


% \subsection{Overview framework}
% \NA{We should use the title of this section as an opportunity to highlight our method. We should have a better title that highlights the novelty or the name of our approach.}

% \subsection{Model Learning with Adaptive Frequency}
% - Adaptive Frequency to contact phase and flight phases
% - Neural Network, Euler integration, 
% \label{sec:training}

\subsection{Learning Residual Dynamics with Adaptive Frequency}  \label{sec:adaptive_learn_model}

% In contrast with many legged-jumping MPC frameworks using SRBD (e.g.\cite{YanranDingTRO, GabrielICRA2021,park2017high,continuous_jump_bipedal}), we propose to add learned residual terms to account for leg dynamics, model mismatch, and unknown dynamics in the contact model or hardware \NA{This sentence could be moved to the intro/related work}. 
% This model also leverage the state transition between contact and flight phase, aiming to achieve accurate trajectory prediction for real-time control and optimization.
% We utilize the simplified dynamics to enable real-time control but propose to learn a residual term to account for legged dynamics, model mismatch (e.g. kinematic parameters, or unknown dynamics in contact model or hardware. 


% We aim to develop a learned model for quadruped jumping that is able to represent the complexity of whole-body dynamics and capture the robot model uncertainties, while it is necessary compact and lightweight to be utilized for real-time feedback control\NA{I suggest toning down this sentence and making it more specific. We introduced the full-body and single-rigid-body models in the previous section. We can build on these, i.e., explain that we focus on the SRB model due to its simplicity (linearity?) for online control but aim to learn residual terms the account for the leg dynamics.}. Importantly, we also aim to design model predictive control using the learned model to achieve accurate jumping under uncertainty.

% Consider a robot with state $\bfx$ consisting of its position $\bfp \in \mathbb{R}^3$, orientation $\bfR\in SO(3)$, body-frame linear velocity $\bfv \in \bbR^3$, and body-frame angular velocity $\bfomega\in \mathbb{R}^3$. 

% Let $\bfx_{k+1} = \bff(\bfx_{k}, \bfu_k)$ characterize the robot dynamics with control input $\bfu$.
% We aim to approximate the residual dynamics using a dataset $\mathcal{D}$ of state and control trajectories. 

 % This simplifies the whole trunk and legs as a unified single rigid body subject to forces at the contact patches (e.g. \cite{park2017high,YanranDingTRO,ParkRSS15}). 
 % which finds highly efficient to real-time control. 
 % Although ignoring leg dynamics is a major simplification, the controller
 % is still able to stabilize a high-DoF system and is robust
 % to these multi-body effects.
 % Consider a robot modeled as a single rigid body with position $\bfp \in \bbR^2$, orientation $\theta \in \mathbb{R}$. 
 % \TD{I think before this sentence, we should clarify that in this paper, we only consider 2D jumping, leading to the generalized coordinates that follow. Up to this point, the state $\bfx$ is general.} 

 
We consider a 2D jumping motion on a legged robot with point foot contact, e.g., quadruped robot, with generalized coordinates $\boldsymbol{\mathfrak{q}} = \begin{bmatrix} \bfp^{\top} & \phi \end{bmatrix}^{\top} \!\in \mathbb{R}^{3}$, where $\bfp \in \bbR^2$ is the CoM's position, and $\phi \in \mathbb{R}$ is the body pitch angle. We define the generalized robot's velocity as $\bfzeta = \begin{bmatrix} \bfv^{\top} & \omega \end{bmatrix}^{\top} \in \mathbb{R}^3$, where $\bfv \in \mathbb{R}^2$ and $\omega \in \mathbb{R}$ are the linear and angular velocity. Both $\mathfrak{q}$ and $\bfzeta$ are expressed in world-frame coordinates. The robot state is $\bfx = \begin{bmatrix} \boldsymbol{\mathfrak{q}}^{\top} & \bfzeta^{\top} & g\end{bmatrix}^{\top} \in \mathbb{R}^{7}$, where the (constant) gravity acceleration $g$ is added to obtain a convenient state-space form \cite{Carlo2018}.
 % \TD{This is a bit vague. Why is it convenient?}.
% Under the control input $\bfu = \begin{bmatrix} \bff_1^{\top} & \bff_2^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{n_u}$,  robot state $\bfx = \begin{bmatrix} \boldsymbol{\mathfrak{q}}^{\top} & \bfzeta^{\top} & g\end{bmatrix}^{\top} \in \mathbb{R}^{n_x}$.
Denote $\bfr = \begin{bmatrix} \bfr_1^{\top} & \bfr_2^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{4}$, where $\bfr_i$ as the foot $i \in \{1, 2\}$ position relative to the body's CoM in the world frame. With the force control input for the front and rear legs as $\bfu = \begin{bmatrix} \bfu_f^{\top} & \bfu_r^{\top} \end{bmatrix} ^{\top}\in \mathbb{R}^{4}$, the nominal discrete-time SRBD model can be written as:
% \NA{What is the control input? What is its dimension?}
% We use discrete-time SRBD as the nominal dynamics model:
% \NA{Is it necessary for $\bfB$ to depend on $k$? Is it because we will be changing $\Delta t$? Then, perhaps, it is better to use $\Delta t_k$.}
\begin{equation}\label{eq:discrete_nominal_model}
    \bff\left(\bfx_k, \bfu_k, \bfr_{k},\Delta t_k \right)  = \bfA_k\bfx_{k} + \bfB_k(\bfr_k) \bfu_k,
\end{equation}
where $\bfA_k = \bfI_{7} + \bfA_{ct} \Delta t_k$, $\bfB_k(\bfr_k)= \bfB_{ct}(\bfr_k) \Delta t_k$, $\Delta t_k$ is the adaptive sampling time (e.g., $\Delta t_{\calC}$ or $\Delta t_{\calF}$ for the contact phase of flight phase, respectively), and $\bfA_{ct}$ and $\bfB_{ct}$ are obtained from the continuous-time robot dynamics:
% \NA{Also, should we call the vector $\bfe_2$?}
%
\begin{equation}
    \bfA_{ct} = 
    \begin{bmatrix}
        \bf0 & \bfI_{3} & \bf0 \\ 
        \bf0 & \bf0 & \bfe_{3} \\ 
        \bf0 & \bf0 & 0
    \end{bmatrix}, 
    \bfB_{ct}(\bfr) = 
    \begin{bmatrix}
        \bf0 & \bf0 \\ 
        \bfI_{2} / m & \bfI_{2} / m \\ 
        [\bfr_1]_{\times}^{\top}/J & [\bfr_2]_{\times}^{\top}/J \\ 
        \bf0 & \bf0
    \end{bmatrix}, \nonumber
\end{equation}
where $\bfA_{ct}\in \mathbb{R}^{7\times 7}$, $\bfB_{ct}(\bfr) \in \mathbb{R}^{7\times 4}$, $\bfe_3= \begin{bmatrix} 0 & -1 & 0
\end{bmatrix}^\top$, $m$ is the body mass, $J$ is the moment inertia of the body, $[\bfr_i]_{\times} = \begin{bmatrix} r_{iz} & -r_{ix} \end{bmatrix}^{\top} \in \mathbb{R}^2$.
% $\bfr$\NA{Perhaps this should be introduced earlier, e.g., before eq. (3) where we define the state and input}.  
% for the sake of notation. 
% The discrete dynamics is then propagated using the Euler forward scheme as
% \begin{equation} \label{eq:nominal_dynamics}
% 	\bfx_{k+1} = \bfA_k \bfx_{k} + \bfB_k(\bfr_k) \bfu_k,
% \end{equation}
% We choose to learn a model that represents the relationship between the robot states and force control, rather than actual ground contact force which is hard to estimate accurately \cite{Zachary_RAL_online_calibration_2022} or when force sensors are not equipped, which is the case for many quadruped robots (e.g. \cite{QuannICRA19,YanranDingTRO,ChignoliICRA2022})\NA{Should this information be moved earlier where we define $\bfx_k$ and $\bfu_k$?}. In addition, this representation allows us to directly incorporate the learned model with an MPC architecture to optimize for the control inputs. 
% The proposed discrete-time model with residual dynamics can be characterized as follows:
% \begin{equation}\label{eq:discrete_learned_model}
%     \bfx_{k+1} = \bff\left(\bfx_k, \bfu_k, \bfr_{k} \right) + \bff_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k} \right),
% \end{equation}
The residual term $\delta\bff_{\bftheta}\left(. \right)$ in (\ref{eq:discrete_learned_model}) is defined as
%
\begin{equation}\label{eq:discrete_learned_res_model}
\delta\bff_{\bftheta}\left(. \right) = 
 \bfh_{\bftheta}(\bfx_k, \bfr_{k}) \Delta t_k  + \bfG_{\bftheta}(\bfx_k, \bfr_{k}) \Delta t_k \bfu_k,
\end{equation}
%
where $\bfh_{\bftheta}(\bfx_k, \bfr_{k})$ and $\bfG_{\bftheta}(\bfx_k, \bfr_{k})$ are represented by neural networks with learning parameters $\bftheta$.
% We aim to learn $\bfh_{\bftheta}$ and $\bfG_{\bftheta}$ with parameters $\bftheta$ that approximate the residual dynamics on the dataset $\mathcal{D}$ of state and control trajectories. 
Since $\bfu_k=\bf0$ during the flight phase, $\bfG_{\bftheta}\bfu_k=\bf0$. We have two separate models for the contact ($\calC$) and flight phase ($\calF$):
% \begin{subequations}\label{eq:res_dynamics_each_phase}
%     \begin{align}
%        &(\calC):
%        ~&\bfx_{k+1}&= \bfA_{\calC,k} \bfx_{k} + \bfB_k \bfu_{k} \nonumber \\ 
%        &&&~~~ + \bfh_{\bftheta_1}(\bfx_{k}, \bfr_{k})  + \bfG_{\bftheta_1}(\bfx_{k}, \bfr_{k}) \bfu_{k}, \\
%        &(\calF):
%        ~&\bfx_{k+1}& = \bfA_{\calF,k}  \bfx_{k} + \bfh_{\bftheta_2}( \bfx_{k}, \bfr_k),
%      \end{align}
% \end{subequations}
\begin{subequations}\label{eq:res_dynamics_each_phase}
    \begin{align}
     & (\calC):  ~ \bfx_{k+1} = \bfA_{\calC}\bfx_k + \bfB_{\calC}(\bfr_k) \bfu_k \nonumber \\
     & ~~~~~~~~~ + \bfh_{\bftheta_1}(\bfx_k, \bfr_{k})  \Delta t_{\calC} + \bfG_{\bftheta_1}(\bfx_k, \bfr_{k})\Delta t_{\calC} \bfu_k, \\ 
     &(\calF):  ~~~ \bfx_{k+1} = \bfA_{\calF}\bfx_k + \bfh_{\bftheta_2}(\bfx_k, \bfr_{k})\Delta t_{\calF}
     \end{align}
\end{subequations}
% \Abdullah{I think both $\bfh_{\bftheta_1}(\bfx_{k}, \bfr_{k})$ and $\bfG_{\bftheta_1}(\bfx_{k}, \bfr_{k})$ should be multiplied with $\Delta t$, right?}
% \begin{equation}
% \label{eq:ode_solver}
% \{\tilde{\bfx}_1^{(i)}, \ldots, \tilde{\bfx}_N^{(i)}\} = \text{EI}(\bfx_0^{(i)}, \bff_{no}+\tilde{\bff}_{\bftheta}, u_0^{(i)}, \ldots, u_{N-1}^{(i)}),
% \end{equation}
where $\bfA_{\calC} = \bfI_7 + \bfA_{ct} \Delta t_{\calC}$, $\bfB_{\calC}(\bfr_k)=\bfB_{ct}(\bfr_k) \Delta t_{\calC}$, and $\bfA_{\calF} = \bfI_7 + \bfA_{ct} \Delta t_{\calF}$.

% \subsection{Training with Adaptive Frequency} \label{sec:training}

% We aim to learn a residual model that can provide accurate prediction of the robot state trajectory during different phases of a jump. Therefore, we propose to train the model with the same adaptive-frequency scheme and horizons as MPC, instead of training separately for each phase. The state prediction for each sequence can leverage the contact transition and the entire flight phase.

%To train the neural networks, we minimize the discrepancy between the predicted state sequence $\tilde{\bfx}_{1:K}$ and the true state sequence $\bfx_{1:K}$ (i.e. labels) from $\calD$, as described in Problem \ref{problem:dynamics_learning}. 
% ) along $K$ horizons with adaptive sampling time as MPC
%  described in Sec. \ref{sec:sys_overview}
%  from the learned model

We roll out the dynamics based on \eqref{eq:res_dynamics_each_phase}, starting from initial state $\bfx_0$ with given control input sequence $\bfu_{0:K-1}$ to obtain a predicted state sequence $\tilde{\bfx}_{1:K}$. Using the adaptive-frequency scheme, the state prediction accounts for contact transitions (feet taking off the ground), a long flight phase, and the final robot state upon landing. We define the loss functions in Problem \ref{problem:dynamics_learning} as follows:
%
\begin{equation}
\begin{aligned}
\mathcal{L} (\bfx,\tilde{\bfx}) & = \| \boldsymbol{\mathfrak{q}} - \tilde{\boldsymbol{\mathfrak{q}}}\|^2_2 + \| \bfzeta - \tilde{\bfzeta}\|^2_2\\
\mathcal{L}_{reg} (\bftheta) & = \alpha_1 \Vert  \bfh_{\bftheta} \Vert + \alpha_2 \Vert  \bfG_{\bftheta}  \Vert.
\end{aligned}
\end{equation}
%
The parameters $\bftheta = [\bftheta_1, \bftheta_2]$ for each phase are updated by gradient descent to minimize the total loss.
%$\mathcal{L} (\bfx,\tilde{\bfx}) + \mathcal{L}_{reg} (\bftheta)$.

% \NA{This sentence is unclear. We have not defined what the adaptive frequency scheme for MPC is and it is indeed too early for this perhaps.}. 
% This also allows us to learn the discretization errors for state prediction.
% We denote the dataset as $\calD = \{t_{k:k+K}^{(i)}, \bfx^{(i)}_{k:k+K}, \bfr^{(i)}_{k:k+K}, \bfu^{(i)}_{k:k+K}\}_{i=1}^D$ consisting of $D$ state sequences $\bfx^{(i)}_{k:k+K}$, obtained by applying control inputs $\bfu^{(i)}_{k:k+K}$ to the system, and $\bfr^{(i)}_{k:k+K}$ represents the foot position w.r.t the body's CoM in the world frame\NA{This information was already provided in the problem statement. It is not necessary to repeat it here. You may refer to Problem 1 if necessary.}.
% Let $\tilde{\bfx}^{(i)}_{k+1} \in \bbR^{7}$ denote the state trajectory predicted with control input $\bfu^{(i)}_k$ by the approximate dynamics $\tilde{\bfx}^{(i)}_{k+1} = \bff\left(\bfx^{(i)}_k, \bfu^{(i)}_k, \bfr^{(i)}_k \right) + \bff_{\bftheta}\left(\bfx^{(i)}_k, \bfu^{(i)}_k , \bfr^{(i)}_k\right)$\NA{Should we have tilde for the arguments of the functions?}. The state prediction for each sequence can leverage the contact transition and the entire flight phase.
% The robot state in the contact and flight phase can be predicted as follows
% \begin{subequations}\label{eq:res_dynamics}
%     \begin{align}
%        & (\calC):
%        % \tilde{\bfx}_{k+1}^{(i)}&= \bfA_{\calC,k} \bfx_k^{(i)} + \bfB_k \bfu_k^{(i)} \\  & + \bfh_{\bftheta_1}(\bfx_k^{(i)}, \bfr_k^{(i)})  + \bfG_{\bftheta_1}(\bfx_k^{(i)}, \bfr_{k}^{(i)}) \bfu_k^{(i)}, \\
%        % \vdots \\
%        ~\tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calC,k} \tilde{\bfx}_{k}^{(i)} + \bfB_k \bfu_{k}^{(i)} \nonumber \\ 
%        & ~~~~~~~~~~~~~~~ + \bfh_{\bftheta_1}(\tilde{\bfx}_{k}^{(i)}, \bfr_{k}^{(i)})  + \bfG_{\bftheta_1}(\tilde{\bfx}_{k}^{(i)}, \bfr_{k}^{(i)}) \bfu_{k}^{(i)}, \\
%        & (\calF):
%        ~~\tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calF,k} \tilde{\bfx}_k^{(i)} + \bfh_{\bftheta_2}(\tilde{\bfx}_k^{(i)}, \bfr_k^{(i)}),
%      \end{align}
% \end{subequations}

% To optimize the parameters $\bftheta$, we roll out the dynamics with initial state $\bfx_k^{(i)}$ and control $\bfu^{(i)}_{k:k+K}$ and minimize the discrepancy between the computed state sequence $\tilde{\bfx}^{(i)}_{k:k+K}$ and the true state sequence $\bfx^{(i)}_{k:k+K}$ from $\calD$. 
% Given an initial state $\bfx_k^{(i)}$ at time $t_k^{(i)}$\NA{There is no notion of time since we are already working in discrete time.} and control input $\bfu_k^{(i)}, \ldots, \bfu_{k+K-1}^{(i)}$ from the dataset, a forward pass returns predicted states for $K$ steps $t_{k+1}^{(i)}, \ldots, t_{k+K}^{(i)}$ as $\lbrace \tilde{\bfx}_{k+1}^{(i)}, \tilde{\bfx}_{k+2}^{(i)}, ..., \tilde{\bfx}_{k+K}^{(i)} \rbrace $, where state trajectory prediction 
% $\tilde{\bfx}_{k+j}^{(i)} = [\tilde{\mathbf\frakq}_{k+j}^{(i)\top} \quad \tilde{\bfzeta}_{k+j}^{(i)\top} \quad g]^\top$, where $\tilde{\mathbf\frakq}_{k+j}^{(i)\top} = [\tilde{\bfp}_{k+j}^{(i)\top} \quad \tilde{\phi}_{k+j}^{(i)\top} ]^\top$, $\tilde{\bfzeta}_{k+j}^{(i)\top} = [\tilde{\bfv}_k^{(i)\top} \quad \tilde{\omega}_{k+j}^{(i)\top}]^\top$, $j = 1,...,K$\NA{A lot of information in this sentence is redundant. We already defined the states and explained that we do prediction by rolling out the dynamics.}.
% Our objective is to learn the parameters $\bftheta$ that minimize the loss function in (\ref{eq:problem_formulation_unknown_env_equation}) with state predictions\NA{It is also not necessary to repeat this. Just refer to the model in \eqref{eq:res_dynamics}. I think it is already clear from the problem statement and the discussion above that we use the dynamics to predict $\tilde{\bfx}_k$.}: 
% \Abdullah{I think the last line in (6) should be $\tilde{\bfx}^{(i)}(t_0) = \bfx_{0}^{(i)}, \quad \tilde{\bfx}_{k}^{(i)} =  \tilde{\bfx}^{(i)}(t_k), \quad \forall k = 0, \ldots, K, \quad \forall i = 1, \ldots, D$},
% \begin{subequations}
%     \begin{align}
%        &(\calC):
%        \tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calC,k}  \tilde{\bfx}_k^{(i)} + \bfB_{k}(\bfr_{k}^{(i)}) \bfu_k^{(i)} \nonumber \\ 
%        & ~~~~~~~~~~~~~~~ + \bfh_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}) + \bfG_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}^{(i)}) \bfu_k^{(i)}, \\
%        &(\calF):
%        ~~ \tilde{\bfx}_{k+1}^{(i)} = \bfA_{\calF,k} \tilde{\bfx}_k^{(i)} + \bfh_{\bftheta_2}(\tilde{\bfx}_k^{(i)}, \bfr_k^{(i)}),
%      \end{align}
% \end{subequations}
% \begin{equation}
% \begin{aligned}
% & \underset{\bftheta}{\text{min}}
% & & \sum_{i=1}^{D} \sum_{k=1}^{K}  \mathcal{L}_{\bftheta} (\bfx^{(i)}_k,\tilde{\bfx}^{(i)}_k)\\
% & \text{s.t.}
% & & \begin{aligned}[t]
%  (\calC): \tilde{\bfx}_{k+1}^{(i)} = &\ \bfA_{\calC,k}  \tilde{\bfx}_k^{(i)} + \bfB_{k}(\bfr_{k}^{(i)}) \bfu_k^{(i)} \\ 
% &+ \bfh_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}) + \bfG_{\bftheta_1}( \tilde{\bfx}_k^{(i)}, \bfr_{k}^{(i)}) \bfu_k^{(i)} \\
% \end{aligned} \\
% & & & (\calF): \tilde{\bfx}_{k+1}^{(i)}= \bfA_{\calF,k} \tilde{\bfx}_k^{(i)} + \bfh_{\bftheta_2}(\tilde{\bfx}_k^{(i)}, \bfr_k^{(i)}), \\
% & & &  \tilde{\bfx}_{0}^{(i)} =  \tilde{\bfx}^{(i)}(t_k), \quad \forall k = 0, \ldots, K, \quad \forall i = 1, \ldots, D, 
% \end{aligned}
% \end{equation}
% where $\mathcal{L}$ is a distance metric on the state space.
% We train separate models for the contact and flight phase, i.e. $\bfh_{\bftheta_1}$ and $\bfG_{\bftheta_1}$ for contact phase, and $\bfh_{\bftheta_2}$ and $\bfG_{\bftheta_2}$ for flight phase. The learning model represents the relationship between robot states and force control, instead of actual ground contact force which is hard to estimate accurately or not available when force sensors are not available. 
% We aim to learn the model, which will then be utilized to obtain predictions in MPC. For this purpose, we propose to train the model with adaptive frequency as MPC. This also allows us to learn the discretization errors for state prediction.
% The nominal dynamics at each time step $t_k^{(i)}$ above is defined as
% \begin{equation}
%     f_{no}\left(\bfx_k, \bfu_k, \bfr_k  \right) = \bfA \bfx_k + \bfB_k(\bfr_k ) \bfu_k
% \end{equation}
% and the residual dynamics:
% \begin{equation}
%     \tilde{f}_{\bftheta}\left(\bfx_k, \bfu_k, \bfr_{k} \right) = 
%  h_{\bftheta}(\bfx_k, \bfr_{k})  + g_{\bftheta}(\bfx_k, \bfr_{k}) \bfu_k
% \end{equation}
% The predicted rotation matrix $\tilde{\bfR}_n^{(i)} = [\tilde{\bfr}_{1n}^{(i)} \quad \tilde{\bfr}_{2n}^{(i)} \quad \tilde{\bfr}_{3n}^{(i)}]^\top$ and the ground-truth one $\bfR_n^{(i)} = [\tilde{\bfr}_{1n}^{(i)} \quad \tilde{\bfr}_{2n}^{(i)} \quad \tilde{\bfr}_{3n}^{(i)}]^\top$ are used to calculate an orientation loss:
% %
% \begin{equation}
% \mathcal{L}_{\bfR}(\bftheta) = \sum_{i = 1}^D \sum_{n = 1}^N \left\|\left(\log (\tilde{\bfR}_n^{(i)} \bfR_n^{(i)\top})\right)^{\vee} \right\|_2^2,
% \end{equation}
% 
% We aim to minimize the loss which represents the discrepancy between prediction state $\lbrace \tilde{\bfx}_{k+1}^{(i)}, \tilde{\bfx}_{k+2}^{(i)}, ..., \tilde{\bfx}_{k+K}^{(i)} \rbrace $ and the label from dataset $\lbrace \bfx_{k+1}^{(i)}, \bfx_{k+2}^{(i)}, ..., \bfx_{k+K}^{(i)} \rbrace $. 
% Refer to  We use the squared Euclidean norm to calculate losses for the position and generalized velocity terms:\NA{The notation below is strange because it is not clear what $\bfp$ and $\bfzeta$ are on the left-hand-side of the equations. To be consistent with \eqref{problem:dynamics_learning}, we should define $\mathcal{L} (\bfx,\tilde{\bfx}) = \| \mathbf\frakq - \tilde{\mathbf\frakq}\|^2_2 + \| \bfzeta - \tilde{\bfzeta}\|^2_2$. We should also introduce the regularization term $\calL_{\text{reg}}(\bftheta)$ in \eqref{problem:dynamics_learning} and define it here as $\calL_{\text{reg}}(\bftheta) = \alpha_1 \|  \bfh_{\bftheta} \| + \alpha_2 \| \bfG_{\bftheta}  \|$.} 
%\begin{equation}
%\mathcal{L}_{\bfp}(\bftheta) = \sum_{i = 1}^D \sum_{n = 1}^N \Vert \bfp_n^{(i)} - \tilde{\bfp}_n^{(i)} \Vert^2_2, \mathcal{L}_{\bfzeta}(\bftheta) = \sum_{i = 1}^D \sum_{n = 1}^N \Vert \bfzeta_n^{(i)} - \tilde{\bfzeta}_n^{(i)} \Vert^2_2.
%\end{equation}
%

% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{\bftheta}(\bfp) &= \sum_{i = 1}^D \sum_{k = 1}^K \Vert \mathbf\frakq_k^{(i)} - \tilde{\mathbf\frakq}_k^{(i)} \Vert^2_2,\\
% \mathcal{L}_{\bftheta}(\bfzeta) &= \sum_{i = 1}^D \sum_{k = 1}^K \Vert \bfzeta_k^{(i)} - \tilde{\bfzeta}_k^{(i)} \Vert^2_2 \\
% \mathcal{L}_{reg} (\bftheta) &= \sum_{i = 1}^D \sum_{k = 1}^K \alpha_1 \Vert  \bfh_{\bftheta} \Vert + \alpha_2 \Vert  \bfG_{\bftheta}  \Vert.
% \end{aligned}
% \end{equation}
%
% The total loss $\calL_{\bftheta}$ is defined as:
% \begin{equation}
% \calL_{\bftheta}= \mathcal{L}_{\bftheta}(\bfp) + \mathcal{L}_{\bftheta}(\bfzeta) + \mathcal{L}_{reg} (\bftheta).
% \end{equation}
% The total loss $\calL_{\bftheta}$ is defined as:
% \begin{equation}
% \calL_{\bftheta}= \mathcal{L} (\bfx,\tilde{\bfx}) + \mathcal{L}_{reg} (\bftheta).
% \end{equation}
% The gradient of the total loss function $\calL(\bftheta)$ is back-propagated by solving an ODE with adjoint states \cite{chen2018neural}. Specifically, let $\bfa = \frac{\partial \calL}{\partial \tilde{\bfx}}$ be the adjoint state and $\bfs = (\tilde{\bfx}, \bfa, \frac{\partial \calL}{\partial \bftheta})$ be the augmented state. The augmented state dynamics are \cite{chen2018neural}:
% %
% \begin{equation}
% \dot{\bfs} = \tilde{\bff}_{\bfs} = (\tilde{\bff}_{\bftheta}, -\bfa^\top\frac{\partial \tilde{\bff}_{\bftheta}}{\partial \tilde{\bfx}}, -\bfa^\top\frac{\partial \tilde{\bff}_{\bftheta}}{\partial \bftheta}).
% \end{equation}
% %
% The predicted state $\tilde{\bfx}$, the adjoint state $\bfa$, and the derivatives $\frac{\partial \calL}{\partial \bftheta}$ can be obtained by a single call to a reverse-time ODE solver starting from $\bfs_N = \bfs({t_N})$:
% %
% \begin{equation}
% \bfs_0 = \left(\tilde{\bfx}_0, \bfa_0, \frac{\partial \calL}{\partial \bftheta}\right) = \text{ODESolver}(\bfs_N, \tilde{\bff}_\bfs, t_N),
% \end{equation}
% %
% where at each time $t_k, k = 1, \ldots, N$, the adjoint state $\bfa_{k}$ at time $t_k$ is reset to $ \frac{\partial \calL}{\partial \tilde{\bfx}_{k}}$. The resulting derivative $ \frac{\partial \calL}{\partial \bftheta}$ is used to update the parameters $\bftheta$ using gradient descent.

\subsection{Data Collection}
\label{subsec:data_gen}
% \subsubsection{Nominal Dynamic Model}

To collect state-control trajectories for residual dynamics learning, we implemented an MPC controller with the nominal dynamics model \eqref{eq:discrete_nominal_model} and a reference body trajectory $\bfx^*$ obtained from full-body trajectory optimization. The trajectory optimization assumes jumping from flat and hard ground with point foot contact. We generated various jumping trajectories to different targets under different ground disturbances (e.g., blocks under the robot feet with random height) to obtain a diverse dataset for training. 


% The trajectory optimization provides a reference state trajectory $\bfx_{0:K}^*$ and ground contact forces $\bfu_{0:K}^*$.



% While MPC aims to track body trajectory $\bfx^*$, an additional joint PD controller is adopted to track the joint trajectory reference from trajectory optimization. This yields the total torque applied to the robot motors as:
% \begin{align} \label{eq:applied_torque}
%     \bftau= \bftau_{mpc} + \bftau_{pd},
% \end{align} 
% where $\bm{\tau}_{mpc}=\mathbf{J}(\bfq_{j})^\top \bfR(\phi)^\top \bfu_{mpc}$ converts the MPC force $\bfu_{mpc}$ to joint torque, $\bfR(\phi) = \begin{bmatrix}
%     \text{cos}(\phi) & -\text{sin}(\phi); \text{sin}(\phi) & \text{cos}(\phi)
% \end{bmatrix} \in \mathbb{R}^{2\times 2}$ is a rotation matrix,
% % \NA{How is this rotation matrix obtained? Is it related to $\phi_k$?}, 
% $\mathbf{J}(\bfq_{j})$ is the foot Jacobian at the current joint configuration $\bfq_{j}$ \NA{This may be confused with $\frakq$. Should we explain that the full-body model is defined in terms of joint angles $\bfq_{j}$?}. A joint PD controller $\bftau_{pd} = \bfK_{p,j}(\bfq_{j}^*-\bfq_j)+\bfK_{d,j}(\mathbf{\dot q}_{j}^*-\mathbf{\dot q}_j)$ is adopted for joint tracking reference.


% Since the evolution of robot states is in fact governed by the combination of MPC and the joint PD controller, we collect the trajectory dataset $\calD$ with the \rep{stored inputs as}: 
% % \NA{When collecting trajectories we are not applying anything to the learned model. Do you mean that this is the reference input stored in $\calD$?}
% \begin{equation}
%     \bfu = \left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1}  \bftau =  \bfu_{mpc} + \bfu_{pd},
% \end{equation}
% where $\bfu_{pd} =\left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1} \bftau_{pd}$\NA{Define this earlier, when you define $\bftau_{mpc}$.} converting the joint torque data to its corresponding force in the world frame. 

While the MPC controller aims to track the body reference trajectory $\bfx_{0:K}^*$, an additional joint PD controller is used to track the joint reference trajectory $(\bfq_{\mathbf{J}}^*, \mathbf{\dot q}_{\mathbf{J}}^*)$ from the full-body trajectory optimization via  $\bftau_{pd} = \bfK_{p}(\bfq_{\mathbf{J}}^*-\bfq_{\mathbf{J}})+\bfK_{d}(\mathbf{\dot q}_{\mathbf{J}}^*-\mathbf{\dot q}_{\mathbf{J}})$. Thus, the evolution of the robot states is governed by the combination of MPC and the joint PD controller. We collected the trajectory dataset $\calD$ with inputs:
\begin{equation}
    \bfu =  \bfu_{mpc} + \bfu_{pd},
\end{equation}
where $\bfu_{pd} =\left(\mathbf{\mathbf{J}}(\bfq_{\mathbf{J}})^{\top} \bfR^{\top}\right)^{-1} \bftau_{pd}$ with rotation matrix $\bfR(\phi) = \begin{bmatrix}
    \text{cos}(\phi) & -\text{sin}(\phi); \text{sin}(\phi) & \text{cos}(\phi)
\end{bmatrix} \in \mathbb{R}^{2\times 2}$ and $\mathbf{J}(\bfq_{\mathbf{J}})$ is the foot Jacobian at joint configuration $\bfq_{\mathbf{J}}$. 
% \NA{This may be confused with $\frakq$. Should we explain that the full-body model is defined in terms of joint angles $\bfq_{\mathbf{J}}$?}, \CN{}.



% \todo{Explain how data is chunked and collected in more detail}
The dataset is collected at the different sampling time steps for the contact and flight phases, i.e., $\Delta t_{\calC}$ and $\Delta t_{\calF}$, respectively. The data for each jump is then chunked by a shifting window size of $K$ with a slicing step of $1$. Let $N$ be the number of collected state-control data points for each jump and $H$ be the number of jumps. We then obtain $D = H\times(N-K+1)$ state-control trajectories in total.

% The dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consists of state sequences $\bfx^{(i)}_{0:K}$, where $\bfx_k^{(i)}~=~[\mathbf\frakq_n^{(i)\top} \quad \bfzeta_k^{(i)\top}]^\top$, $\mathbf\frakq_k^{(i)}~=~[\bfp_k^{(i)\top} \quad \phi_{k}^{(i)\top}]^\top~\in~\mathbb{R}^{3}$, $\bfzeta_k^{(i)}~=~[\bfv_k^{(i)\top} \quad \omega_k^{(i)\top}]^\top \in \mathbb{R}^3$ for $k = 0, \ldots, K$\NA{This last sentence is not necessary. It was defined before and besides it is too late for this information as the last sentence of the section.}.



% Since jumping is a highly complex motion, it requires a real-time feedback control policy and whole-body coordination to enable successful jumps. In addition, we are only able to rely on force control during the contact phase to achieve safe and accurate jumping. In hardware, without appropriate control, the robot is unable to jump or make the jumping fail badly, which could lead to a hardware break. Therefore, we are unable to apply a constant or random control input $\bfu^{(i)}$ during contact phases to the system to collect the data.
% Jumping is a highly complex motion and requires efficient real-time feedback control policy and whole-body coordination. 



% \subsubsection{MPC for nominal dynamics}


% %Full-body TO is utilized to solve for reference body trajectory $\bfx^*$, joint profiles $ \{\bfq_{j}^*, \bm{\dot q}_{j}^*\}$, and ground contact force $\bfu^*$ given different targets, assuming the jumping from flat ground \cite{QuannICRA19}. It is noted that the full-body TO assumes constant calf lengths, point foot contact, and hard ground.
% % We then adopt the MPC controller in our prior work \cite{continuous_jump} to execute various jumps under a variety of disturbances. 
% % \note{The offline reference torque $\bm{\tau}_d$ generates the main force contribution for the whole body motion. In case of model uncertainties (e.g. box under feet), our idea is to adjust this reference torque $\bm{\tau}_d$ by the online offset $\Delta \bm{\tau}_{mpc}$ from MPC controller as proposed in our prior work \cite{continuous_jump}}.
% % The MPC is then designed based on SRB dynamics, i.e., nominal dynamics (\ref{eq:nominal_dynamics}). 

% % The baseline MPC is formulated as a quadratic programming (QP) with moving horizons to solve for optimal force control, which minimizes the weighted tracking errors of reference from trajectory optimization:
% % %
% % \begin{subequations} \label{eq:MPC_jumping}
% % \begin{align}
% %  \textrm{min} \textrm{ } & \sum_{k=t}^{t+K-1} \| \bfx_k-\bfx_{k}^* \|_{P_k} + \| \bfu_k - \bfu_{k}^* \|_{Q_k},\\
% % % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% % \text{s.t. }
% %              & \bfx_{k+1}=\bfA_k\bfx_k+ \bfB_k \bfu_k, \forall k=t, ..., t+K-1, \label{eq:MPC_jumping_c1} \\
% %              & \bfc_k^{min} \leq \bfC_k \bfu_k \leq \bfc_k^{max}, \forall k=t, ..., t+K-1, \label{eq:MPC_jumping_c2} \\ 
% %              & \bfD_k \bfu_k =\bm{0}, \label{eq:MPC_jumping_c3} \forall k=t, ..., t+K-1,
% % \end{align}
% % \end{subequations}
% % where E.q (\ref{eq:MPC_jumping_c2}) captures constraints related to friction cone and force limits, while E.q (\ref{eq:MPC_jumping_c3}) represents the shifting contact schedule that nullifies the force control in flight phase. 
% While MPC aims to track body trajectory $\bfx^*$, an additional joint PD controller is adopted to track the joint trajectory reference from trajectory optimization. This yields the total torque applied to the robot motors as:
% \begin{align} \label{eq:applied_torque}
%     \bftau= \bftau_{mpc} + \bftau_{pd},
% \end{align} 
% where $\bm{\tau}_{mpc}=\mathbf{J}(\bfq_{j})^\top \bfR^\top \bfu_{mpc}$ converts the MPC force to joint torque, $\bfR$ is a rotation matrix, $\mathbf{J}(\bfq_{j})$ is the foot Jacobian at the current joint configuration $\bfq_{j}$. 
% % \begin{align} \label{eq:delta_MPC}
% %     \Delta \bm{\tau}_{mpc}=\bm{J}(\bfq_{j})^\top \bfr^\top[\bfu_{mpc}^* - \bfu_{d}],
% % \end{align} 
% % \begin{align} \label{eq:delta_MPC}
% %     \bm{\tau}_{mpc}=\bm{J}(\bfq_{j})^\top \bfR^\top \bfu_{mpc},
% % \end{align} 
% % where $\bfR$ is a rotation matrix, $\bm{J}(\bfq_{j})$ is the foot Jacobian at the current joint configuration $\bfq_{j}$. 
% The joint PD controller $\bftau_{pd} = \bfK_{p,j}(\bfq_{j}^*-\bfq_j)+\bfK_{d,j}(\mathbf{\dot q}_{j}^*-\mathbf{\dot q}_j)$ is adopted for joint tracking reference.
% % \begin{align} \label{eq:applied_torque}
% %     \bm{\tau}_{t}= \bm{\tau}_{mpc} + \bm{\tau}_{pd,j},
% % \end{align} 
% % where
% % \begin{align}
% % % \bm{\tau}_{a}  &= \bm{\tau}_d + \Delta \bm{\tau}_{mpc}  \\
% % \bm{\tau}_{pd} & = \bm{K}_{p,j}(\bfq_{j,d}-\bfq_j)+\bm{K}_{d,j}(\bm{\dot q}_{j,d}-\bm{\dot q}_j)
% % \end{align} \label{eq:jointPDController}

% % \begin{align}
% % % \bm{\tau}_{a}  &= \bm{\tau}_d + \Delta \bm{\tau}_{mpc}  \\
% % \bm{\tau}_{pd} & = \bm{K}_{p,j}(\bfq_{j}^*-\bfq_j)+\bm{K}_{d,j}(\bm{\dot q}_{j}^*-\bm{\dot q}_j)
% % \end{align} \label{eq:jointPDController}

% % where the torque $\bm{\tau}_d$ and joint profiles $ \{\bfq_{J,d}, \bm{\dot q}_{J,d} \}$ obtained from the trajectory optimization for the full nonlinear dynamics.

% % \note{Another idea is to directly apply the solution MPC from (\ref{eq:MPC_jumping}) instead of using the offset MPC. In other words, we combine:
% % \begin{align} \label{eq:mpc_pd}
% %     \bm{\tau}_{t}= \bm{\tau}_{mpc}^b + \bm{\tau}_{pd,j},
% % \end{align}
% % where $\bm{\tau}_{mpc}^b =(\bfq_{j})^\top \bfr^\top\bm{f}_{mpc}^*$.
% % However, I have observed that it has not worked well in hardware. That's why we combine the reference torque with offset torque from MPC for data collection in experiments.}
% % We can have several options to select the force control for our learned model (\ref{eq:discrete_learned_model})
% % \begin{itemize}
% %     \item Option 1: Torque $\bm{\tau}_d + \Delta \bm{\tau}_{mpc}$ will then converted to the force control via
% % \begin{equation}
% %     \bfu = (\bm{J}(\bfq_j)^T \bfr^T)^{-1} (\bm{\tau}_d + \Delta \bm{\tau}_{mpc}) \nonumber
% % \end{equation}
% %     \item Option 2: Directly use $\bfu_{mpc}^*$
% %     % \item Option 2: Total torque $\bm{\tau}_{t} = \bm{\tau}_d + \Delta \bm{\tau}_{mpc}^b + \bm{\tau}_{pd,j} $
% % \end{itemize}
% % which will then be converted to generalized force control in the world frame
% % \begin{equation}
% %     \bfu = (\bm{J}(\bfq_j)^T \bfr^T)^{-1} \bm{\tau}
% % \end{equation}
% % }.
% % We then convert the total torque to force $\bfu =\bm{J}(\bfq_j)^T \bfr^T)^{-1} \bm{\tau}_t$, which then be used for the learned model.
%  Since the evolution of robot states is in fact governed by the combination of MPC and the joint PD controller, we collect the $\calD$ state-control trajectories with the following total control force applying for the learned model:
% \begin{equation}
%     \bfu = \left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1}  \bftau =  \bfu_{mpc} + \bfu_{pd},
% \end{equation}
% where $\bfu_{pd} =\left(\mathbf{J}(\bfq_j)^T \bfR^T\right)^{-1} \bftau_{pd}$ converting the joint torque data to its corresponding force in the world frame. 

% % \todo{Explain how data is chunked and collected in more detail}
% The dataset is collected at the different sampling time steps for the contact and flight phases, denoted as $\Delta t_{\calC}$ and $\Delta t_{\calF}$. Denote $N$ as a number of collected state-control data points for each jump, and $H$ as a number of jumps. Given $K$ as a horizon, we then obtain
% $D = H\times(N-K+1)$ state-control trajectories in total.
% The dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consists of state sequences $\bfx^{(i)}_{0:K}$, where $\bfx_k^{(i)}~=~[\mathbf\frakq_n^{(i)\top} \quad \bfzeta_k^{(i)\top}]^\top$, $\mathbf\frakq_k^{(i)}~=~[\bfp_k^{(i)\top} \quad \theta_{k}^{(i)\top}]^\top~\in~\mathbb{R}^{3}$, $\bfzeta_k^{(i)}~=~[\bfv_k^{(i)\top} \quad \omega_k^{(i)\top}]^\top \in \mathbb{R}^3$ for $k = 0, \ldots, K$.
% % Such data are generated by applying a constant control input $\bfu^{(i)}$ to the system and sampling the state $\bfx_{n}^{(i)} = \bfx^{(i)}(t_n^{(i)})$ at times $t_n^{(i)}$ for $n = 0, \ldots, N$.


% % The coordinates $\mathbf\frakq$ and velocity $\bfzeta$ may be obtained from the robot's IMU, or from a motion capture system. 

% % In physics-based simulation the data can be generated by applying random control inputs $\bfu^{(i)}$. In real-world applications, where safety is a concern, data may be collected by a human operator manually controlling the robot.


\section{Adaptive-Frequency MPC with Learned Dynamics} \label{sec:adaptive-MPC}

% \subsubsection{Model Prediction with Learned Residual Dynamics} 
In this section, we design an adaptive-frequency MPC controller for the learned dynamics \eqref{eq:res_dynamics_each_phase} to track a desired jumping reference trajectory obtained from full-body TO. We formulate the MPC optimization problem as follows:
%
\begin{subequations} \label{eq:MPC_learned}
\begin{align}
 \min_{\bfu_{0:K-1}} & \; \sum_{k=1}^{K} \| \bfx_k-\bfx_{k}^* \|_{\bfQ_k} + \| \bfu_{k-1}-\bfu_{k-1}^* \|_{\bfR_k},\\
% & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
\text{s.t. }
     & (\calC):  ~ \bfx_{k+1} = \bfA_{\calC}\bfx_k + \bfB_{\calC}(\bfr_k) \bfu_k \nonumber  \\ 
     & ~~~~~+ \bfh_{\bftheta_1}(\bfx_k, \bfr_{k})  \Delta t_{\calC} + \bfG_{\bftheta_1}(\bfx_k, \bfr_{k})\Delta t_{\calC} \bfu_k, \\ 
     &(\calF):  ~~~ \bfx_{k+1} = \bfA_{\calF}\bfx_k + \bfh_{\bftheta_2}(\bfx_k, \bfr_{k})\Delta t_{\calF}, \\
     & \underline{\bfc}_k \leq \bfC_k \bfu_k \leq \bar{\bfc}_k, \; \forall k=0, ..., K-1, \label{eq:learn_MPC_ineq} \\ 
     & \bfD_k \bfu_k =\bm{0}, \qquad\quad \forall k=0, ..., K-1, \label{eq:learn_MPC_eq} 
\end{align}
\end{subequations}
where \eqref{eq:learn_MPC_ineq} represents input constraints related to friction cone and force limits and \eqref{eq:learn_MPC_eq} aims to nullify the force on the swing legs based on the contact schedule.


%TO and achieve both accurate and robust target jumping.
% For the first horizon prediction, we utilize the current robot state to compute the forward pass of the neural networks. From the second prediction, we utilize the reference trajectory to compute the output of the neural network. In particular, we predict the future robot states as follows:
% % The residual dynamics $g_{\bftheta,t+i}$,  $h_{\bftheta,t+i}$
% and the mapping function $\bm{m}_{t+i}$ with $i\in [0, N-1]$,
% are computed at future time step $t+i$. 
% At the current time $t$, these functions are evaluated with current robot states and foot positions. For a future time, we rely on reference trajectory to estimate these functions.
% \begin{subequations}\label{eq:res_dynamics}
%     \begin{align}
%         \tilde{\bfx}_{t+1}&= \bfA \bfx_t + \bfB_t \bfu_t + \left( f_{res,t} + h_{res,t} \bm{m}_t \bfu_t \right) \delta t, \nonumber\\
%         \tilde{\bfx}_{t+2}&= \bfA  \tilde{\bfx}_{t+1} + \bfB_{t+1} \bfu_{t+1} \nonumber \\  & + \left( f_{res,t+1} + h_{res,t+1} \bm{m}_{t+1} \bfu_{t+1} \right) \delta t,\nonumber \\
%         \vdots \nonumber \\
%         \tilde{\bfx}_{t+N}&= \bfA  \tilde{\bfx}_{t+N-1} + \bfB_{t+N-1} \bfu_{t+N-1} \nonumber \\ & + \left( f_{res,t+N-1} + h_{res,t+N-1} \bm{m}_{t+N-1} \bfu_{t+N-1} \right) \delta t,\nonumber
%      \end{align}
% \end{subequations}
% \begin{subequations}\label{eq:res_dynamics}
%     \begin{align}
%         \tilde{\bfx}_{k+1}&= \bfA_k \bfx_k + \bfB_k \bfu_k + \bfh_{\bftheta}(\bfx_k, \bfr_{k})  + \bfG_{\bftheta}(\bfx_k, \bfr_{k}) \bfu_k, \nonumber\\
%         \tilde{\bfx}_{k+2}&= \bfA_k  \tilde{\bfx}_{k+1} + \bfB_{k+1} \bfu_{k+1} \nonumber \\  & + \bfh_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*)  + \bfG_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*) \bfu_k,\nonumber \\
%         \vdots \nonumber \\
%         \tilde{\bfx}_{k+K}&= \bfA_k  \tilde{\bfx}_{k+K-1} + \bfB_{k+K-1} \bfu_{k+K-1} \nonumber \\ & + \bfh_{\bftheta}(\bfx_{k+K-1}^*, \bfr_{k}^*)  + \bfG_{\bftheta}(\bfx_{k+K-1}^*, \bfr_{k+K-1}^*) \bfu_k,\nonumber
%      \end{align}
% \end{subequations}
% as the shifting-horizon 


% \begin{subequations} \label{eq:MPC_learned}
% \begin{align}
%  \min & \sum_{k=0}^{K} \| \bfx_k-\bfx_{k}^* \|_{P_k} + \| \bfu_k-\bfu_{k}^* \|_{Q_k},\\
% % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% \text{s.t. }
%      & (\calC):  ~ \bfx_{k+1} = \bfA_{\calC,k}\bfx_k + \bfB_{\calC,k} \bfu_k \\ \nonumber 
%      & ~~~~~~~~~~~~ ~~~~~ + \bfh_{\bftheta_1}(\bfx_k, \bfr_{k})  \Delta t_{\calC} + \bfG_{\bftheta_1}(\bfx_k, \bfr_{k}) \bfu_k \\ 
%      &(\calF):  ~~~ \bfx_{k+1} = \bfA_{\calF,k}\bfx_k + \bfh_{\bftheta_2}(\bfx_k, \bfr_{k}) \\
%      & \bfc_k^{min} \leq \bfC_k \bfu_k \leq \bfc_k^{max}, \forall k=0, ..., K-1 \label{eq:learn_MPC_ineq} \\ 
%      & \bfD_k \bfu_k =\bm{0}, \label{eq:learn_MPC_eq} \forall k=0, ..., K-1
% \end{align}
% \end{subequations}



% \underline{Contact Prediction Mode}:  in this mode, the whole predicted horizons are in scheduled contact phase
% % \begin{equation}\label{eq:learK_contact_prediction}
% %      \tilde{\bfX}_{\calC,k}= \bfA_{\calC} \bfx_k + \bfB_{\calC} \tilde{\bfU} + \bm{\psi}_{\calC,\bftheta} + \bm{\phi}_{\calC,\bftheta} 
% % \end{equation}
% \begin{equation}\label{eq:learK_contact_prediction}
%      \tilde{\bfX}_{\calC,k}= \bfA_{\calC} \bfx_k + (\bfB_{\calC} + \bfB_{\calC,\bftheta})  \tilde{\bfU} + \bm{\psi}_{\calC,\bftheta}, 
% \end{equation}
% where the predicted states $\tilde{\bfX}_{\calC,k} = [\tilde{\bfx}_{k+1}^T, \tilde{\bfx}_{k+2}^T ..., \tilde{\bfx}_{k+K}^T]^T $ concatenate the predicted states from $k+1$ to $k+K$. The prediction is governed by control input $\tilde{\bfU} = [\tilde{\bfu}_k^T, \tilde{\bfu}_{k+1}^T, ..., \tilde{\bfu}_{k+K-1}^T]^T \in \mathbb{R}^{K \times n_x}$
% $\bfA_{\mathcal{C}}= \begin{bmatrix}
% (\bfA_{\calC,k})^\top
% (\bfA_{\calC,k}^2)^\top
% \ldots 
% (\bfA_{\calC,k}^{K})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK \times n_x}$, 
% % $\bfA_k = \bfI+ \bfA \delta t$.
% % $\bfB_{\calC}= \begin{bmatrix}
% % \bfB_k & \bm{0} & \ldots & \bm{0}\\
% % \bfA \bfB_k & \bfB_{k+1} & \ldots & \bm{0} & \\
% % \vdots \\
% % \bfA^{K-1} \bfB_k & \bfA^{K-2} \bfB_{k+1} & \ldots & \bfB_{k+K-1}
% % \end{bmatrix}
% % $
% \[[\bfB_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} \bfB_{k+n-1} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% % $\bfB_{\calC,\bftheta}= \begin{bmatrix}
% % \bfB_{\bftheta,k} & \bm{0} & \ldots & \bm{0}\\
% % \bfA_k \bfB_{\bftheta,k} & \bfB_{\bftheta,k+1} & \ldots & \bm{0} & \\
% % \vdots \\
% % \bfA_k^{N-1} \bfB_{\bftheta,k} & \bfA_k^{N-2} \bfB_{\bftheta,k+1} & \ldots & \bfB_{\bftheta,k+N-1}
% % \end{bmatrix}$
% \[[\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} \bfB_{\bftheta,k+n-1} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% % Let $\bfB_{t}^{res} = g_{res,t} \bm{m}_t $, and we define
% Let $\bfB_{\bftheta,k} = \bfG_{\bftheta}(\bfx_k, \bfr_{k}) $ obtained at the current time, and predictions are computed as
% $\bfB_{\bftheta,k+j} = \bfG_{\bftheta}(\bfx_{k+j}^*, \bfr_{k+j}^*)$, $j = 1,..., K-1$, we define:
% % \[[\bfB_{\calC}+\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
% %   \begin{array}{lr}
% %     \bfA_k^{m-n} (\bfB_{k+n-1}+ \bfB_{\bftheta,k+n-1}) : & \textit{if} ~ m \geq n \\
% %     \bm{0}  & \textit{otherwise}
% %   \end{array}
% % \right.
% % \]
% % and residual matrix 
% % \begin{equation}
% %     \bm{\phi}_{c,\bftheta} = \bfB_{c,\bftheta}^{qp} \tilde{\bfu}
% % \end{equation}
% \begin{equation}
%     \bm{\psi}_{c,\bftheta} = \begin{bmatrix}
% \bfI & \bm{0} & \ldots & \bm{0}\\
% \bfA_k & \bfI & \ldots & \bm{0} \\
% \vdots \\
% \bfA_k^{N-1} & \bfA_k^{N-2} & \ldots & \bfI
% \end{bmatrix} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_k, \bfr_{k})\\
% \bfh_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{k+N-1}^*, \bfr_{k+N-1}^*)
% \end{bmatrix}
% \end{equation}
% \\
% \\
% \underline{Adaptive Prediction Mode}: in this mode, predicted horizons are in both contact phases and flight phases. We present our proposed MPC for the learning hybrid contact model. 



%  $0\leq K_{\calC} \leq K$
% We use a greater time step for state prediction in flight phase to capture the whole flight phase (i.e. $dt_f > dt_c$). We define 
% From current time step $k$, with ($T_c-N < t <T_c$), we define
% During the flight phase, the force control output from MPC is unavailable.
% Given the current time $k$, the number of horizons for predicted contact phase $K_c$ satisfies $K_c = T_c -k$. Here, $T_c$ is a predefined schedule time at the end of the contact phase. 
% During the flight phase, there is no control input applied to the system. 
% The remaining prediction horizons $N_f = K - K_c$ are in flight phase.
% $\bfA_{\mathcal{C}}= \begin{bmatrix}
% (\bfA_{\calC,k})^\top
% (\bfA_{\calC,k}^2)^\top
% \ldots 
% (\bfA_{\calC,k}^{K_c})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x}$,  $\bfA_{\mathcal{F}}= \begin{bmatrix}
% (\bfA_{\calF,k})^\top
% (\bfA_{\calF,k}^2)^\top
% \ldots 
% (\bfA_{\calF,k}^{K_{\calF}})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_{\calF} \times n_x}$, 

% $\bfA_t = \bfI+ \bfA_c \delta t_c$.

% $\bfB_{c}^{qp}= \begin{bmatrix}
% \bfB_k & \bm{0} & \ldots & \bm{0}\\
% \bfA_k \bfB_t & \bfB_{t+k} & \ldots & \bm{0} & \\
% \vdots \\
% \bfA_k^{K_c-1} \bfB_t & \bfA_k^{K_c-2} \bfB_{k+1} & \ldots & \bfB_{k+K_c-1}
% \end{bmatrix}
% $


With the MPC horizons including $K_{\calC}$ steps in the contact phase and $K_{\calF} = K-K_{\calC}$ steps in the flight phase, we define
%
\begin{equation}
    \tilde{\bfU}_{\calC} = [\tilde{\bfu}_0^{\top}, \tilde{\bfu}_{1}^{\top}, ..., \tilde{\bfu}_{K_{\calC} - 1}^{\top}]^{\top} \in \mathbb{R}^{K_c \times n_x}
\end{equation}
as a concatenation of the control inputs in the contact phase. With this notation, the predicted trajectory is:
% \NA{We should change the notation below because I removed the subscript $k$ from $\bfA_{\calC}$. One option is to use $\calA_\calC = \begin{bmatrix}
% (\bfA_{\calC})^\top
% (\bfA_{\calC}^2)^\top
% \ldots 
% (\bfA_{\calC}^{K_c})^\top
% \end{bmatrix}$}
%
\begin{subequations}\label{eq:adaptive_prediction}
    \begin{align}
        (\calC): ~ \tilde{\bfX}_{\calC}&= \calA_\calC \bfx_0 + (\calB_{\calC} + \calB_{\calC, \bftheta} ) \tilde{\bfU}_{\calC} + \bfH_{\calC, \bftheta}\label{eq:predict_phase1}\\
        (\calF): ~ \tilde{\bfX}_{\calF}&= \calA_{\calF} \tilde{\bfx}_{K_c}+ \bfH_{\calF, \bftheta} \label{eq:predict_phase2}
     \end{align}
\end{subequations}
% \begin{subequations}\label{eq:whole_state_prediction}
%     \begin{align}
%         \textrm{(contact)} \tilde{\bfx}_{c}&= \bfA_{c}^{qp} \bfx_t + \left( \bfB_{c}^{qp} + \bfB_{c, res}^{qp} \right) \tilde{\bfu}_c + \bm{H}_{c, res} \quad \label{eq:predict_phase1}\\
%         \textrm{(flight)} \tilde{\bfx}_{f}&= \bfA_{f}^{qp} \tilde{\bfx}_{t+K_c}+ \bm{H}_{f, res}^{} \quad , \label{eq:predict_phase2}
%      \end{align}
% \end{subequations}
%
where
$\tilde{\bfX}_{\calC} = [\tilde{\bfx}_{1}^{\top}, \tilde{\bfx}_{2}^{\top}, ..., \tilde{\bfx}_{K_c}^{\top}]^{\top} $ and 
$\tilde{\bfX}_{\calF} = [\tilde{\bfx}_{K_c+1}^{\top}, \tilde{\bfx}_{K_c+2}^{\top}, ..., \tilde{\bfx}_{K}^{\top}]^{\top} $ denote the concatenation of predicted states belonging to the contact and flight phase, respectively. The matrices $\calA_{\calC}$ and $\calA_{\calF}$ are computed as
% $\bfA_{\calC}= \begin{bmatrix}
% \bfA_k^1\\
% \bfA_k^2\\
% \vdots \\
% \bfA_k^{K_c}
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x}$, 
%
\[\left\{
  \begin{array}{lr}
    \calA_{\calC}= \begin{bmatrix}
(\bfA_{\calC})^\top
(\bfA_{\calC}^2)^\top
\ldots 
(\bfA_{\calC}^{K_c})^\top
\end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x},  \\
\calA_{\calF}= \begin{bmatrix}
(\bfA_{\calF})^\top
(\bfA_{\calF}^2)^\top
\ldots 
(\bfA_{\calF}^{K_{\calF}})^\top
\end{bmatrix} \in \mathbb{R}^{n_xK_{\calF} \times n_x}.
\end{array}
\right.
\]
%
The residual term $\bfB_{\bftheta,0} = \bfG_{\bftheta}(\bfx_0, \bfr_{0}) \Delta t_0 $ is evaluated at the current state, and the other residual terms are estimated via
$\bfB_{\bftheta,k} = \bfG_{\bftheta}(\bfx_{k}^*, \bfr_{k}^*) \Delta t_k$, where $\bfx_{k}^*, \bfr_{k}^* $ are the reference states and foot positions, $k = 1,..., K_{\calC}$. Thus, we have
\begin{equation}
     \begin{array}{lr}
    [\calB_{\calC}]_{\lbrace m,n \rbrace} ~~=   \bfA_{\calC}^{m-n} \bfB_{n-1}  ~~~ \textit{if} ~ m \geq n, \textit{and} ~ \bm{0} ~ \textit{otherwise}  \\
   \left[\calB_{\calC, \bftheta}\right]_{\lbrace m,n \rbrace} = \bfA_{\calC}^{m-n} \bfB_{\bftheta,n-1} ~ \textit{if} ~ m \geq n, \textit{and} ~ \bm{0} ~ \textit{otherwise}
     \end{array}  \nonumber
\end{equation}

% \[[\bfB_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{k+n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise},
%   \end{array}
% \right.
% \]
% \[[\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{\bftheta,k+n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise}.
%   \end{array}
% \right.
% \]
% \[[\bfB_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise},
%   \end{array}
% \right.
% \]
% \[[\bfB_{\calC, \bftheta}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC}^{m-n} \bfB_{\bftheta,n-1},  & \textit{if} ~ m \geq n, \\
%     \bm{0}  & \textit{otherwise}.
%   \end{array}
% \right.
% \]
% with $m,n$ from 1 to $K_c$
% and 
% $\bfA_{f}^{qp}= \begin{bmatrix}
% \bfA_k^1\\
% \bfA_k^2\\
% \vdots \\
% \bfA_k^{N_f}
% \end{bmatrix} \in \mathbb{R}^{n_xK_c \times n_x}$, 
% % $\bfA_t = \bfI+ \bfA_c \delta t_f$
%
%
% $\bfA_{\mathcal{F}}= \begin{bmatrix}
% (\bfA_{\calF,k})^\top
% (\bfA_{\calF,k}^2)^\top
% \ldots 
% (\bfA_{\calF,k}^{K_{\calF}})^\top
% \end{bmatrix} \in \mathbb{R}^{n_xK_{\calF} \times n_x}$, 
%
% and residual matrix 
% \begin{equation}
%     \bm{\phi}_{c, res} = \bfB_{c,res}^{qp} \tilde{\bfu}_c
% \end{equation}
% \begin{equation*}
%     \bm{\psi}_{\calC,\bftheta} = \begin{bmatrix}
% \bfI & \bm{0} & \ldots & \bm{0}\\
% \bfA_{c,k} & \bfI & \ldots & \bm{0} \\
% \vdots \\
% \bfA_{c,k}^{K_c-1} & \bfA_{c,k}^{K_c-2} & \ldots & \bfI
% \end{bmatrix} \begin{bmatrix}
% h_{\bftheta}(\bfx_k, \bfr_{k})\\
% h_{\bftheta}(\bfx_{k+1}^*, \bfr_{k+1}^*)\\
% \vdots \\
% h_{\bftheta}(\bfx_{k+K_c-1}^*, \bfr_{k+K_c-1}^*)
% \end{bmatrix} 
% \end{equation*}
%
The residual matrix $\bfH_{\calC, \bftheta}$ in (\ref{eq:adaptive_prediction}) is $\bfH_{\calC,\bftheta} =  \Delta t_{\calC}$ $\mathbf{S}_{\calC} \left[
\bfh_{\bftheta}(\bfx_0, \bfr_{0})^{\top} \quad
\bfh_{\bftheta}(\bfx_{1}^*, \bfr_{1}^*)^{\top} 
\ldots \quad
\bfh_{\bftheta}(\bfx_{K_c-1}^*, \bfr_{K_c-1}^*)^{\top}
\right]^{\top}$, where $\bfS_{\calC}$ is lower triangular matrix with entries $[\bfS_{\calC}]_{\lbrace m,n \rbrace} = \bfA_{\calC}^{m-n} \in \mathbb{R}^{n_x \times n_x}$, $m \geq n$. The residual matrix $\bfH_{\calF,\bftheta} = \Delta t_{\calF} \bfS_{\calF} \left[
\bfh_{\bftheta}(\bfx_{K_c}^{*}, \bfr_{K_c}^*)^{\top} \quad
\ldots \quad 
\bfh_{\bftheta}(\bfx_{K}^*, \bfr_{K}^*)^{\top}
\right]^{\top}$
% where $m,n$ from 1 to $K_{\calF}$
% \begin{subequations}
% \begin{align}
%     \bfH_{\calC,\bftheta}  &= \mathbf{S}_{\calC} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_0, \bfr_{0})\\
% \bfh_{\bftheta}(\bfx_{1}^*, \bfr_{1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{K_c-1}^*, \bfr_{K_c-1}^*)
% \end{bmatrix}, \\
%     \bfH_{\calF,\bftheta} & = \bfS_{\calF} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_{K_c}^*, \bfr_{K_c}^*)\\
% \bfh_{\bftheta}(\bfx_{K_c+1}^*, \bfr_{K_c+1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{K}^*, \bfr_{K}^*)
% \end{bmatrix},
% \end{align}
% \end{subequations}
where $\bfS_{\calF}$ is lower triangular matrix with entries $[\bfS_{\calF}]_{\lbrace m,n \rbrace} = \bfA_{\calF}^{m-n} \in \mathbb{R}^{n_x \times n_x}$, $m \geq n$. 
% \[[\bfS_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% \begin{equation}
%     \bm{\psi}_{\calF,\bftheta} = \begin{bmatrix}
% \bfI & \bm{0} & \ldots & \bm{0}\\
% \bfA_{f,k} & \bfI & \ldots & \bm{0} \\
% \vdots \\
% \bfA_{f,k}^{N_f} & \bfA_{f,k}^{N_f-1} & \ldots & \bfI
% \end{bmatrix} \begin{bmatrix}
% \bfh_{\bftheta}(\bfx_{k+K_c}^*, \bfr_{k+K_c}^*)\\
% \bfh_{\bftheta}(\bfx_{k+K_c+1}^*, \bfr_{k+K_c+1}^*)\\
% \vdots \\
% \bfh_{\bftheta}(\bfx_{k+N}^*, \bfr_{k+N}^*)
% \end{bmatrix}
% \end{equation}
% where $m,n$ from 1 to $K-K_c$
% \[[\bfS_{\calC}]_{\lbrace m,n \rbrace} = \left\{
%   \begin{array}{lr}
%     \bfA_{\calC,k}^{m-n} : & \textit{if} ~ m \geq n \\
%     \bm{0}  & \textit{otherwise}
%   \end{array}
% \right.
% \]
% \begin{align}
% \tilde{\bfx}_{k+K_c}= & \bfA_{\calC,k}^{K_c} \bfx_k + \sum_{i=0}^{K_c-1} \bfA_{\calC,k}^{K_c-1-i} \left (\bfB_{k+i} + \bfB_{\bftheta, k+i} \right) \tilde{\bfu}_{k+i}, \nonumber
% \end{align}
The state prediction at the end of $K_{\calC}$ steps can be computed as
%
\begin{equation}\label{eq:x_kNc}
    \tilde{\bfx}_{K_c}= \bfA_{\calC}^{K_c} \bfx_0 + (\bfS + \bfS_{\theta}) \tilde{\bfU}_{\calC} + \bm{\phi}_{\bftheta}, 
\end{equation}
%
where $\bfS = \left[\bfA_{\calC}^{K_c-1}\bfB_0 \quad \bfA_{\calC}^{K_c-2}\bfB_{1} \quad ... \quad \bfB_{K_c-1}  \right] $, $\bfS_{\bftheta} = \left[\bfA_{\calC}^{K_c-1}\bfB_{\bftheta,0} \quad \bfA_{\calC}^{K_c-2}\bfB_{\bftheta,1} \quad ... \quad \bfB_{\bftheta,K_c-1}  \right] $,  and $\bm{\phi}_{\bftheta} = \left[\bfA_{\calC}^{K_c-1}\bfh_{\bftheta,0} \quad \bfA_{\calC}^{K_c-2}\bfh_{\bftheta,1} \quad ...\quad \bfh_{\bftheta,K_c-1}  \right]$. Substituting (\ref{eq:x_kNc}) into (\ref{eq:predict_phase2}) yields:
\begin{equation} \label{eq:state_prediction2}
    \tilde{\bfX}_{\calF}= \bfA_{\calF} \bfA_{\calC}^{K_c} \bfx_0+ \bfA_{\calF} (\bfS + \bfS_{\theta}) \tilde{\bfU}_{\calC}  + \bfA_{\calF} \bm{\phi}_{\bftheta} +  \bfH_{\calF, \bftheta}.
\end{equation}
% $\bfS , \bfS_{\bftheta} \in \mathbb{R}^{n_{\bfx} \times (n_{\bfu} \times K_c)}$. 
% Substituting $\tilde{\bfx}_{k+K_c}$ to equation (\ref{eq:predict_phase2}), we obtain $\tilde{\bfx}_{f,k}$.
% \subsection{Training}
% - data collection (hybrid) \\
% - data augmentation (duplicate data) \\
% - neural network architecture  \\
% - loss function \\
% - gradient descent \\
% The solution $\bm{f}_{MPC}^*$ that takes the value at the first horizon of solution $\bm{F}_t$ will be utilized to compensate for the errors between actual and reference jumping:
% \begin{align} \label{eq:delta_MPC}
%     \Delta \bm{\tau}_{MPC}=\bm{J}(\bfq_{j})^\top \bfr^\top[\bm{f}_{MPC}^* - \bm{f}_{d}],
% \end{align} 
% where $\bm{J}(\bfq_{j})$ is the foot Jacobian at the configuration $\bfq_{j}$; $\bfr$ is the rotation matrix which transforms from body
% to world frame. The compensation $\Delta \bm{\tau}_{MPC}$ will be combined with the high frequency joint PD controller, leveraging the reference of the torque $\bm{\tau}_d$ and joint profiles $ \{\bfq_{J,d}, \bm{\dot q}_{J,d} \}$ obtained from the trajectory optimization. This results in a feed forward torque applying to the robot actuators:
% \begin{align} \label{eq:MPC_feedforward_torque}
%     \bm{\tau}_{ff}= \bm{\tau}_d + \bm{\tau}_{PD}^{joint} + \Delta \bm{\tau}_{MPC},
% \end{align} 
% \begin{align}
% \bm{\tau}_{PD}^{joint} = \bm{K}_{p,j}(\bfq_{J,d}-\bfq_J)+\bm{K}_{d,J}(\bm{\dot q}_{J,d}-\bm{\dot q}_J)
% \end{align} \label{eq:jointPDController}


% \begin{subequations} \label{eq:MPC_jumping}
% \begin{align}
%  \textrm{min} \textrm{ } & \sum_{k=t}^{t+N-1} \| \bfx_k-\bfx_{d,k} \|_{P_k} + \| \bm{f}_k-\bm{f}_{d,k} \|_{Q_k},\\
% % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% \text{s.t. }
%              & \bfx_{k+t}=\Psi_k (\bfx_k)+ \phi_k (\bm{f}_k), \label{eq:MPC_jumping_c1} \\
%              & \bm{c}_k^{min} \leq \bm{C}_k \bm{f}_k \leq \bm{c}_k^{max}, \label{eq:MPC_jumping_c2} \textrm{(friction cone)}  \\ 
%              & \bm{D}_k \bm{f}_k =\bm{0} ~\label{eq:MPC_jumping_c3} \textrm{(contact phases)}
% \end{align}
% \end{subequations}
% where a contact force reference $\bm{f}_d$ and body trajectory reference $\bfx_d$ are obtained from trajectory optimization; $P_k$ and $Q_k$ are the weighted diagonal matrices at step $k$; $N$ is a number of predicted horizon. The equation (\ref{eq:MPC_jumping_c2}) captures constraints related to friction cone and force limits, while the equation (\ref{eq:MPC_jumping_c3}) is represented for the shifting contact schedule.


% \subsection{Approach}
% \begin{itemize}
%     \item Nonlinear functions $\Psi_k$ and $\phi_k$ in (\ref{eq:MPC_jumping}) are learned from data, either using Eq. \eqref{eq:var_int_Rn} for 2D jumping or Eq. \eqref{eq:_var_int_SE3} for 3D jumping.
%     \item The long-term prediction of Eq. \eqref{eq:var_int_Rn} and Eq. \eqref{eq:_var_int_SE3} will benefit MPC.
%     \item Linearization would be required and have to handle neural networks, and hopefully we are able to reformulate the MPC problem as QP problem for fast solving.
% \end{itemize}

% \begin{figure*}[!t]
% 	\centering
% 	\resizebox{0.9\linewidth}{!}{\includegraphics[trim={0cm 6cm 0cm 0cm},clip]{Figures/framework.pdf}}
% 	\caption{Block diagram for the proposed framework.} 
% 	\label{fig:framework}
% \end{figure*}

% \begin{figure}[!t]
% 	\centering
% 	{\centering
% 		\resizebox{0.9\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{Figures/framework.pdf}}
% 	}
% 	\caption{\textbf{Periodic jumping phases}. Each periodic jumping motion consists of four phases}
% 	\label{fig:contact_schedule}
% \end{figure}

% \section{Setting Discussion}

% \begin{itemize}
%     \item To enable fast computation, we prefer to implement to MPC in C++. The learned model by Pytorch will be use to predict states in MPC formulation in ROS. However, we currently do not have a interface for Pytorch-learned-model with MPC in ROS.
%     \item We currently have MPC for jumping in C++ (ROS and hardware experiments), which is based on single rigid body dynamics represented via Euler angles. Thus, to implement 3D juming, additional implementation work is required to use rotation matrix instead of Euler angles. 
% \end{itemize}
% \subsubsection{\textcolor{blue}{Real-time Optimization}}
Then, the state predictions for $K$ steps becomes:
\begin{equation}
    \tilde{\bfX} = \begin{bmatrix}
        \tilde{\bfX}_{\calC} \\ \tilde{\bfX}_{\calF}
    \end{bmatrix} = \bfA_{\text{qp}} + \left(\bfB_{\text{qp}} + \bfB_{\bftheta,\text{qp}}\right) \tilde{\bfU} + \bfH_{\bftheta}
\end{equation}
where, $\bfA_{\text{qp}} = \begin{bmatrix}
    \calA_{\calC} \\ \calA_{\calF} \bfA_{\calC}^{K_c}
\end{bmatrix}$, $\bfB_{\text{qp}} = \begin{bmatrix}
    \calB_{\calC} & \bf0 \\
    \calA_{\calF} \bfS & \bf0
\end{bmatrix}$, $\bfB_{\bftheta,\text{qp}} = \begin{bmatrix}
    \calB_{\calC,\bftheta} & \bf0 \\
    \calA_{\calF} \bfS_{\bftheta} & \bf0
\end{bmatrix}$, $\bfH_{\bftheta} = \begin{bmatrix}
    \bfH_{\calC, \bftheta} \\
    \bfH_{\calF, \bftheta} + \calA_{\calF} \bm{\phi}_{\bftheta}
\end{bmatrix}$, and $\tilde{\bfU} = \begin{bmatrix}
    \tilde{\bfU}_{\calC} \\
    \tilde{\bfU}_{\calF}
\end{bmatrix} $.
% \NA{Use comments before and after equations to avoid new lines being produced by latex.} 
% \NA{Why do we distinguish the contact prediction mode and the adaptive prediction mode? Should we describe only one of these?}

% \begin{subequations} \label{eq:MPC_learned_QPcompact}
% \begin{align}
%  \textrm{min} \textrm{ } &  \| \tilde{\bfX}_k-\bfX_{k}^* \|_{\bfP_k} + \| \tilde{\bfU}_k-\bfU_{k}^* \|_{\bfQ_k},\\
% % & \textrm{ } \textrm{ }  +  \| \bfx_{h}-\bfx_{h,d} \|_{P_h}+ \| \bm{f}_h-\bm{f}_{h,d} \|_{Q_h} \nonumber\\
% \text{s.t. }
%              & \tilde{\bfX}_{k} = \bfA_{qp} + \left(\bfB_{qp} + \bfB_{\bftheta,qp}\right) \tilde{\bfU}_k + \bfH_{\bftheta} \\
%              & \bm{c}_{\Sigma,k}^{min} \leq \bm{C}_{\Sigma,k} \tilde{\bfU}_k \leq \bm{c}_{\Sigma,k}^{max}, \label{eq:MPC_jumping_c2_learn} \\ 
%              & \bm{D}_{\Sigma,k} \tilde{\bfU}_k =\bm{0}, \label{eq:MPC_jumping_c3_learn} \forall k=t, ..., t+N-1
% \end{align}
% \end{subequations}
The objective of the MPC in \eqref{eq:MPC_learned} can be rewritten as:
\begin{equation}
    J(\bfU) = \| \tilde{\bfX}-\bfX^* \|_{\bfP}^2 + \| \tilde{\bfU}-\bfU^* \|_{\bfQ}^2,
\end{equation}
leading to a quadratic program:
%formulation of the MPC 
%\eqref{eq:MPC_learned}
%Then, the MPC formulation (\ref{eq:MPC_learned}) can be formulated as the Quadratic Programming for solving in real-time as follows:
\begin{equation}\label{eq:MPC_learned_QPcompact}
\begin{aligned}
& \underset{\bfU}{\text{min}}
& & \bfU^{\top} \bfalpha \bfU + \bfbeta^\top \bfU  \quad \text{s.t.} \;\;\bfU_k \in \calU_k,
\end{aligned}
\end{equation}
where 
% \NA{It would be nice to use capital letters for $\bfalpha$ and $\bfbeta$}
\begin{equation*}
    \begin{aligned}
        \bfalpha &= (\bfB_{\text{qp}}+ \bfB_{\bftheta,\text{qp}}) 
 ^{\top} \bfQ (\bfB_{\text{qp}}+ \bfB_{\bftheta,\text{qp}}) + \bfR, \\ 
        \bfbeta &= 2 (\bfB_{\text{qp}}+ \bfB_{\bftheta,\text{qp}}) 
 ^{\top} \bfQ \left( \bfA_{\text{qp}} \bfx_{k} + \bfH_{\bftheta}- \bfX^* \right) -\bfR \bfU^*,\\
        \calU_k &= \{ \bfu \in \bbR^4 \mid \underline{\bfc}_k \leq \bfC_k \bfu_k \leq \bar{\bfc}_k, \bfD_k \bfu_k =\bm{0}\}.
    \end{aligned}
\end{equation*}

% \todo{Mention the QP solving explicitly}

% \note{To execute the jumping, we apply the same control structure as data collection described in Sec. \ref{subsec:data_gen}}. The solution obtained from the MPC $\bfu_{mpc}$ will be offset with the reference force $\bfu_d$, which then be combined with reference torque $\bm{\tau}_d$ and low-level feedback joint torque $\bm{\tau}_{pd,j}$ to apply to the robot motor as



% \begin{align} \label{eq:applied_torque}
%     \bm{\tau}_{t}= \bm{\tau}_{d} + \bm{\tau}_{pd,j} + \Delta \bm{\tau}_{mpc}
% \end{align} 
% where
% \begin{align}
%  \Delta \bm{\tau}_{mpc}  &=  \bm{J}(\bfq_{j})^\top \bfR^\top[\bfu_{mpc}^* - \bfu_{d}],  \\
% \bm{\tau}_{pd,j} & = \bm{K}_{p,j}(\bfq_{j,d}-\bfq_j)+\bm{K}_{d,j}(\bm{\dot q}_{j,d}-\bm{\dot q}_j)
% \end{align} \label{eq:jointPDController}	
	
% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-026.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-030.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-067.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ fixed frequency}: Motion snapshots from a jump forward $60~cm$ under unknown ground perturbation. This jumping is executed by MPC with fixed time step $\delta t = 25ms$ for nominal model.} 
% 	\label{fig:ros-mpc-fixfreq-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-001.png}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-012.png}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-014.png}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-norminal-adaptive/ezgif-frame-034.png}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ adaptive frequency}: Motion snapshots from a jump forward $60~cm$ under unknown ground perturbation. This jumping is executed by MPC with adaptive frequency update $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms $ for nominal model.} 
% 	\label{fig:ros-mpc-adaptfreq-nominal-snapshots}
% \end{figure*}
% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-028.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-034.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/ezgif-frame-048.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ adaptive frequency}:Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms $ for learned model.} 
% 	\label{fig:ros-mpc-adaptfreq-learn-snapshots}
% \end{figure*}






\section{Evaluation}
\label{sec:results}

% We verify the effectiveness of our model learning and real-time control techniques for quadruped jumping tasks.



% \begin{table}[t!]
% %	\hspace{0.2cm}
% 	\centering
% 	\caption{A1 Robot Parameters}
% 	\label{tab:PRP}
% 	\begin{tabular}{cccc}
% 		\hline
% 		Parameter & Symbol & Value & Units\\
% 		\hline
% 		Trunk dimension & $l,w,h$ & 0.361, 0.194, 0.114 & $\unit{m}$ \\[.5ex]
% 		Trunk Inertia  & $I_{xx},I_{yy},I_{zz}$  & 0.017, 0.056, 0.065 & $\unit{kg}.\unit{m}^2$ \\[.5ex]
% 		Leg Link Lengths & $l_{1}, l_{2}$ & 0.2 & $\unit{m}$ \\[.5ex]
% 		\hline 
% 	\end{tabular}
% \end{table}







% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0139.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0172.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-fix-nominal/0201.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ fix frequency}: Motion snapshots from a failure to jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC 5fix frequency for nominal model.} 
% 	\label{fig:mpc-fixfreq-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0141.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0172.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-nominal/0189.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ adaptive frequency}: Motion snapshots from a failure to jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency for nominal model.} 
% 	\label{fig:mpc-adaptive-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0141.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0194.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={10cm 5cm 5cm 5cm},clip]{figures/Pybullet/mpc-adaptive-learn/0210.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ adaptive frequency}: Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency for learning adaptive model.} 
% 	\label{fig:mpc-adaptive-learn-snapshots}
% \end{figure*}
% \begin{figure*}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/fcmd_new/separate/contact/roll_out.eps}}}\\
%     \caption{\textbf{Rolling out state prediction during $K=10$ horizons that belongs to scheduled contact phase:} The figures show comparisons between the prediction of learned model (blue lines), the nominal model (green lines), and the ground-truth trajectory (black lines).} 
%     \label{fig:roll_out_contact}
% \end{figure*} 
% \begin{figure*}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/fcmd_new/hybrid/roll_out.eps}}}\\
%     \caption{\textbf{Rolling out prediction for contact and flight phase with adaptive frequency} Comparison between the prediction of our neural network, the nominal model, and the ground-truth trajectory. \textcolor{blue}{PENDING: Abdullah will add a prediction with fixed frequency}} 
%     \label{fig:roll_out_hybrid}
% \end{figure*} 
% \begin{figure*}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/rollouts/rollout_2.pdf}}}\\
%     \caption{\textbf{Rolling out predictions for contact and flight phase on a random dataset.} Comparison between the prediction of our neural networks for learned model with adaptive frequency, learned model with fixed frequency, nominal model with adaptive frequency, and the ground-truth trajectories (labels).} 
%     \label{fig:roll_out_hybrid}
% \end{figure*} 
% \Abdullah{Chuong, the prediction plots have been added.}




% \begin{figure}[t]
%     \centering
%     \begin{minipage}[b]{1.0\linewidth} 
%         \centering
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\textwidth]{figures/Training/ftotal_mpc_pd/loss.eps}
%         \caption{\textbf{Training loss and testing loss (Log scale).}}
%         \label{fig:loss}
%     \end{minipage}
%     \vspace{2em}
%     \begin{minipage}[b]{0.9\linewidth} 
%         \centering
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\textwidth]{figures/Training/rollouts/rollout_5.pdf}
%         \caption{\textbf{State prediction comparison on a random testing dataset} among the learned model with adaptive frequency (our method), learned model with a fixed frequency, nominal model with adaptive frequency, and the ground-truth trajectories.}
%         \label{fig:roll_out_hybrid}
%     \end{minipage}
% \end{figure}

% with parameters and actuation capabilities summarized in Table \ref{tab:motor_batterry}.


\subsection{Experiment Setup}

We evaluated our approach using a Unitree A1 robot. To collect real-world data, we utilized an Optitrack motion capture (MoCap) system, consisting of five Optitrack Prime $13W$ cameras, to estimate the position and orientation of the robot trunk at $1$ kHz with position errors of at most $1$ mm.


%We validate our approach using a Unitree A1 robot. To collect real-world data, we utilized an Optitrack motion capture (MoCap) system to estimate the position and orientation of the robot trunk, instead of relying on the robot's IMU, which normally provides inaccurate estimates during the flight phase. The MoCap system consists of five Optitrack Prime $13W$ cameras, providing tracking at a frequency of $1$ kHz with position errors of at most $1$ mm.

%

We used \textit{Pytorch} \cite{pytorch} to implement and train the residual dynamics model. The trained \textit{Pytorch} model was converted to a torch script trace, which in turn, was loaded in our MPC implementation in C++.
We utilized the optimization toolbox \textit{Casadi} \cite{casadi} to set up and solve the full-body TO for various jumping targets within $[0.3, 0.8]$ m on a flat ground. We considered jumping motions with contact phase (C) consisting of an all-leg contact period (e.g., $500$ ms) and a rear-leg contact period (e.g., $300$ ms). With the flight phase (F) scheduled for $400$ ms, the front legs and rear legs become swing legs (SW) up to $58\%$ and $33\%$ of the entire jumping period, respectively. Jumping maneuvers feature long flight phases, i.e., the robot can jump up to $4$ times its normal standing height during the mid-air period.

\begin{table}[t]
	\centering
	\caption{Training Parameters}
	\begin{tabular}{ccc}
		\hline
		Parameter & Symbol & Value\\
		\hline
        Adaptive sampling & $\Delta t _{\calC}, \Delta t _{\calF} $ & $\lbrace 25, 100 \rbrace (ms)$ \\[.5ex]
        Prediction steps & $K$ & $10$ \\[.5ex]
		NN architecture & $\bfh_{\bftheta_1}(\mathbf\frakq, \bfr)$ & $7$ - $400$ Tanh - $400$ Tanh - $3$ \\[.5ex]
  		 & $\bfG_{\bftheta_1}(\mathbf\frakq, \bfr)$ & $7$ - $1000$ Tanh - $1000$ Tanh - $12$ \\[.5ex]
              & $\bfh_{\bftheta_2}(\mathbf\frakq, \bfr)$ & $7$ - $400$ Tanh - $400$ Tanh - $3$ \\[.5ex]
        Learning rate & $\gamma$ & $2.10^{-4}$ \\[.5ex]
        Regulation weights & $\alpha_1, \alpha_2$ & $10^{-3},10^{-3}$ \\[.5ex]
        % Learning rate & $\gamma$ & $2.10^{-4}$ \\[.5ex]
        Total training steps & $N_{train}$ & $2.10^{4}$ \\[.5ex]
		\hline 
		\label{tab:training_params}
	\end{tabular}
  \vspace{-2.2em}
\end{table}

\begin{figure}
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.45\textwidth]{figures/Training/ftotal_mpc_pd/loss_log.pdf}
\caption{\textbf{Training loss and testing loss (Log scale).}}
\label{fig:loss}
\end{figure}





% For all jumps, we consider the contact schedule for the contact and flight phase as $cs = \lbrace 800, 400\rbrace $ (ms). The contact phase consists of the all-leg contact period for the first $500~ms$ and the rear-leg contact period for $300~ms$. Thus, the front and rear legs are supposed to be the swing leg (SW) for $700~ms$ and $400~ms$, which is up to $58\%$ and $33\%$ period of the total jump.

% The reference from trajectory optimization will then be tracked by the proposed MPC under unknown disturbance (e.g. box under feet).

% \begin{figure}
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Training/ftotal_mpc_pd/loss.eps}}}\\
%     \caption{\textbf{Training loss and testing loss (Log scale).}} 
%     \label{fig:loss}
% \end{figure} 

% In the neural network architechture, we select
\begin{figure*}[!t]
	\centering
	{\centering
		\resizebox{\linewidth}{!}{\includegraphics[trim={0cm 4.5cm 0cm 7cm},clip]{figures/Exp/v2/Comparison_Exp_onbox.pdf}}
	}
	\caption{
	\textbf{Jumping on a box:} Comparison among full-body TO, nominal-model MPC with fixed and adaptive frequency, and learned-model MPC with fixed and adaptive frequency. All MPC problems were solved with horizon $K=10$.} 
 % The actual trajectories are recorded in Fig. \ref{fig:traj_compare_box_jumping}}
	\label{fig:box_jumping}
\end{figure*}

\begin{figure*}[!t]
	\centering
	{\centering
		\resizebox{\linewidth}{!}{\includegraphics[trim={0cm 4.5cm 0cm 7.5cm},clip]{figures/Exp/v2/Comparison_Exp_d60.pdf}}
	}
	\caption{
	\textbf{Forward jumping from uneven terrain:} Comparison among full-body TO, nominal-model MPC and learned-model MPC with fixed and adaptive frequency. All MPC problems were solved with horizon $K=10$. A $5$ cm block ($30\%$ of the robot's initial height) was introduced under the robot's front feet. With adaptive-frequency learned-model MPC (our method), the robot is able to compensate for the disturbance and jump over the block successfully.}
	\label{fig:forward_60cm}
\end{figure*}





\subsection{Data Collection and Training}







% The jumping includes contact and flight phase, with a contact schedule $cs = \lbrace 800, 400\rbrace $ (ms) respectively.
% \todo{Explain how we train model with Pytorch, and how we load the model in C++}
% Baseline MPC based on the nominal model, as described in Section \ref{subsec:data_gen}), is implemented for tracking a set of jumping references from the full-body TO under a variety of unknown disturbances (i.e. box under feet with random height within $[0, 8]cm$).
A baseline MPC controller using the nominal model, described in Sec. \ref{subsec:data_gen}, was implemented to generate jumping trajectories under a variety of unknown disturbances (i.e. box under feet with random height within $[0, 8]$ cm).
% \cite{continuous_jump}. 
% The MPC is adopted from our prior work \cite{continuous_jump}, which lumps the robot dynamics as a single rigid body model (i.e. nominal model).  
We collected data from $H=20$ jumps with $80\%$ for training and $20\%$ for testing. The data points were sampled with adaptive sampling time  $\Delta t _{\calC} = 25$ ms, $\Delta t_{\calF} = 100$ ms, and horizon length of $K=10$. 
The dataset $\calD = \{t_{0:K}^{(i)}, \bfx^{(i)}_{0:K}, \bfr^{(i)}_{0:K}, \bfu^{(i)}_{0:K}\}_{i=1}^D$ consisted of $D = 20\times 28$ state-control sequences for training. 
% of $\bfx^{(i)}_{0:K}$, foot position $\bfr^{(i)}_{0:K}$, and control input $\bfu^{(i)}_{0:K}$.
% Each subset consists of robot states and controls for $K$ horizon. 
% It is noted that these sequences do not necessarily have the same length of time due to the adaptive-frequency sampling policy.
% As the robot dynamics in our settings are translation-invariant, e.g., the dynamics do not depend on the robot position, we offset the data sequences to start from the origin and train the dynamics model around the origin.


% has a dimension of $7$ that 

The training parameters are listed in Table \ref{tab:training_params}. We used fully-connected neural networks with architectures listed in Table \ref{tab:training_params}: the first number is the input dimension, the last number is the output dimension, and the numbers in between are the hidden layers' dimensions and activation functions. For all networks, the input consists of body position, body orientation, and foot position w.r.t the body's CoM in the world frame. Note that the output of $\bfG_{\bftheta_1}$ is then converted to a matrix of size $(3,4)$. The training and testing losses are illustrated in Fig. \ref{fig:loss}. 
% \begin{enumerate}
% 	\item Contact phase:
% 		\begin{itemize}
% 		\item $\bfh_{\bftheta_1}(\mathbf\frakq, \bfr)$ : $7$ - $400$ Tanh - $400$ Tanh - $3$.
% 		\item $\bfG_{\bftheta_1}(\mathbf\frakq, \bfr)$ $7$: - $400$ Tanh - $400$ Tanh - $12$. The output of $\bfG_{\bftheta_1}$ is then converted as a matrix of size $(3,4)$
% 	\end{itemize}

% 	\item Flight phase:
% 	\begin{itemize}
% 	\item $\bfh_{\bftheta_2}(\mathbf\frakq, \bfr)$ : $7$ - $400$ Tanh - $400$ Tanh - $3$.
% 	\end{itemize} 
% \end{enumerate}
% The training takes approximately $10 mins$ on GPU

% \subsection{Testing}




\begin{figure}
\centering
    \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.48\textwidth]{figures/Training/rollouts/rollout_5.pdf}
    \caption{\textbf{State prediction comparison on a random testing dataset} among adaptive-frequency learned model (our method), fixed-frequency learned model, adaptive-frequency nominal model, and the ground-truth trajectories.}
    \label{fig:roll_out_hybrid}
\end{figure}

\begin{figure}
    \centering
    {\centering
        % \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/time.eps}}}\\
        \resizebox{1.1\linewidth}{!}{\includegraphics[trim={1cm 0cm 0cm 0.cm},clip]{figures/ROS/compare_horizon/time.pdf}}}\\
    \caption{Solving time for MPC ($t_{MPC}$) with different horizons $K=10$ and $K=22$, respectively. The red dashed line denotes the sampling time of $25$ ms to execute MPC. Real-time performance is achieved if $t_{MPC}$ is much less than the sampling time.} 
    \label{fig:computational_time}
\end{figure} 

\subsection{Comparative Analysis}

% We validate our proposed adaptive-frequency MPC for learned model, and make comprehensive comparisons with the utilization of nominal model and fixed MPC frequency update.
% \begin{itemize}
%     \item \textit{MPC with fixed frequency for nominal model }
%     \item \textit{MPC with adaptive frequency for nominal model }

%     \item \textit{MPC with fixed frequency for learned model}

%     \item \textit{MPC with adaptive frequency for learned model}
% \end{itemize}


% Given the accurate state prediction of learned model, we then verify the effectiveness of real-time MPC to achieve both robust and target jumping accuracy. We consider a jumping forward to the target location at $60cm$. We consider a perturbation to the initial configuration (e.g. a box under the front feet), which is unknown to controllers. 

\subsubsection{Evaluation on testing dataset}
% We validate the efficiency of neural network architecture for prediction on the test dataset. 
% The fig. 
We rolled out the learned dynamics with adaptive frequency to predict the future state trajectories and compared with \textit{(i)} those of the nominal model with adaptive frequency, \textit{(ii)} those of the learned model with fixed frequency, and \textit{(iii)} the ground-truth states in Fig. \ref{fig:roll_out_hybrid}. 
% We select two \textit{random} subsets of testing data. The first starts at $525 (ms)$, leveraging a timing window of $K\Delta t_{\calC}$. This subset is within the scheduled contact phase as shown in Figure \ref{fig:roll_out_contact}. The second starts at $650 (ms)$, leveraging $K = 10$ horizons that consist of $K_c = 6$ horizon for contact phase and $K_f = 4$ horizon for flight phase, as depicted in Fig. \ref{fig:roll_out_hybrid}.
We selected a \textit{random} subset starting at $650$ ms, which consists of $K_c = 6$ steps in the contact phase and $K_f = 4$ stops covering the flight period of $400$ ms. 
% This covers the entire flight period of $400 ms$.
% This covers the long timing window of $K_c \Delta t_{\calC} + K_f \Delta t_{\calF}$, covering the entire flight phase of $400 ms$.
Fig. \ref{fig:roll_out_hybrid} shows that the predicted state trajectory from the learned model with adaptive frequency (blue lines) outperforms the prediction by the nominal model with adaptive frequency (green lines) and learned model with fixed frequency (red lines). For example, our approach reduces the prediction error in the $x$ coordinate by 8 and 5 times, respectively.

\subsubsection{Effect of prediction horizon}
Fig. \ref{fig:computational_time} compares the solving time for MPC with different horizons. With our adaptive-frequency scheme, we can use a long prediction horizon, e.g., $K=10$ ($6$ for contact and $4$ for the flight phase), allowing QP solving time for each MPC update (\eqref{eq:MPC_learned_QPcompact}) to be $2$ ms only on average. This efficient computation time enables real-time performance for MPC. Using a fixed-frequency scheme with sample time of $25$ ms requires MPC to use a large number of steps, e.g. $K=22$ ($6$ for contact and $16$ for the whole flight phase). This long horizon yields a large optimization problem, causing significant computational costs. It takes an average of $30$ ms for each MPC update, thus deteriorating the real-time performance.

\subsubsection{Execution}
We verified that our proposed approach enables both robust and accurate target jumping to various targets. We compared \textit{(a)} nominal model $\&$ fixed-frequency MPC, \textit{(b)} nominal model $\&$ adaptive-frequency MPC, \textit{(c)} fixed-frequency learned model $\&$ fixed-frequency MPC, and \textit{(d)} adaptive-frequency learned model $\&$ adaptive-frequency MPC (\textit{our approach}), on two jumping tasks \textit{(i)} box jumping with target at $(x,z)=(60,20)$ cm, and \textit{(ii)} forward jumping $60$ cm with an unknown disturbance (i.e., a block of $5$ cm under the robot's feet). The results are shown in Fig. \ref{fig:box_jumping} and Fig. \ref{fig:forward_60cm}. Note that all MPC problems used the same prediction horizon $K=10$. The fixed-frequency scheme used a time step of $25$ ms for all jumping phases, so the MPC prediction does not cover the entire flight phase.
% We consider two jumping tasks: \textit{(a)} box jumping with target at $(x,z)=(60,20)$ cm, and \textit{(b)} forward jumping $60$ cm with an unknown disturbance (i.e., a block disturbance of $5$ cm under the robot's feet). 
% For each jumping task, we make comparisons of variations of MPC, including combinations of the nominal model, learned model, and different sampling time resolutions. 
% The experiment results are shown in Fig. \ref{fig:box_jumping} and Fig. \ref{fig:forward_60cm}, which compare \textit{(a)} nominal model $\&$ fixed-frequency MPC, \textit{(b)} nominal model $\&$ adaptive-frequency MPC, \textit{(c)} fixed-frequency learned model $\&$ fixed-frequency MPC, and \textit{(d)} adaptive-frequency learned model $\&$ adaptive-frequency MPC (\textit{our approach}). 
Among the evaluated methods, ours outperforms other MPC setups that adopt fixed frequency or nominal models. \rep{With our method, the robot is able to jump to target location with an error of only $1-2$ cm and a landing angle error $<15^\circ$, while fixed-frequency MPC or nominal model use cause the robot to land far short of the target}.

% as shown in Fig. \ref{fig:box_jumping} and \ref{fig:forward_60cm} for the two jumping tasks.

We also studied the effect of uncertainty in the model by evaluating the jumping performance if we only utilize a joint PD controller to track the joint reference from full-body TO \cite{QuannICRA19}. The full-order model can be conservative by assuming hard feet, point-to-surface contact, and hard ground. These assumptions, however, are not valid for the Unitree A1 robot equipped with deformable feet \cite{Zachary_RAL_online_calibration_2022}.
% which likely leads to model mismatch (variable calf lengths), unknown ground stiffness and damping, and surface-to-surface contact, when the contact force significantly changes during contact. 
Uncertainties due to DC motors working at extreme conditions or motor deficiency are difficult to model and are normally ignored in the full-body model. These factors affect the model accuracy and prevent the robot from reaching the jumping target if we solely rely on the joint PD, as can be seen in Fig. \ref{fig:box_jumping}. Our learned model captures unknown dynamics and model mismatch from the real robot hardware, which enables the learned-model MPC to achieve accurate jumping.

% verified by following controllers in order:
% % \subsubsection{Pybullet}
% \begin{itemize}
%     \item \textit{Feed-forward control}: We adopt a joint PD controller as the feed-forward controller to track the joint reference profile obtained from full-body TO (e.g.\cite{QuannICRA19}).
%     \item \textit{Fixed-frequency MPC for nominal model:}  We use fixed time step of $25~ms$ for the state prediction. With the horizon windows of $K=10$, the prediction does not leverage the entire flight phase of $400ms$.
%     % The hardware experiments are shown in Fig. \ref{fig:exp-mpc-fixfreq-nominal-snapshots}, respectively.
%     \item \textit{Adaptive-frequency MPC for nominal model:} We use adaptive frequency for prediction (e.g. $\Delta t_{\calC} = 25~ms$ and $\Delta t_{\calF} = 100~ms$). This allows us to leverage the whole flight phase when MPC is executed.
%     % The jumping results are reported in Fig. \ref{fig:exp-mpc-adaptfreq-nominal-snapshots} for simulation and experiments.

%     \item \textit{Fixed-frequency MPC + fixed-frequency learned model:} The sampling time of MPC's prediction and the learned model are set identically as $ 25~ms$. 
%     % The hardware experiment is illustrated in Fig. \ref{fig:exp-mpc-adaptfreq-learn-snapshots}.
    
%     \item \textit{Adaptive-frequency MPC + adaptive-frequency learned model:} In this setup, the prediction of MPC based on the learned model is able to leverage the whole flight phase.
% \end{itemize}
% In all experiments with MPC, the weights in cost functions are identical as $ Q[12] = {0.25, 50, 0.25, 2.5, 2.5, 30, 0, 10, 0, 0.2, 0.2, 0.2}$;


% Some uncertainties, for example, inaccurate leg length due to deformable feet or unknown ground stiffness and damping, are hard to estimate correctly during jumping and these factors can significantly affect the model accuracy as discussed in \cite{Zachary_RAL_online_calibration_2022} for Unitree A1 robot. 
% Our prior work \cite{QuannICRA19} also shows that the landing error 


\begin{figure}[!t]
    \centering

    {\centering
        \resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/Exp-results-v4.pdf}}}\\
    {\centering
		\resizebox{1.1\linewidth}{!}{\includegraphics[trim={1.5cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/traj_x.pdf}}
	}
    \caption{\textbf{Hardware experiments:} The figure (a)-(d) show snapshots of the first and the last jumps when the robot executes four consecutive jumps with different MPC approaches. MPC horizon is all set as $K = 10$. Figure (e) records the actual body's CoM trajectories in the $x$ coordinate.} 
    \label{fig:compare_all_mpcs_hardware}
\end{figure} 



% achieving an accurate full-body model remains challenging, particularly for agile jumping maneuvers that introduce significant uncertainties and unmodeled dynamics. For example, the interaction between foot and ground introduces various uncertainties, such as varied friction or unknown ground stiffness and damping. Additionally, parameter variations, such as inaccurate kinematic parameters, also affect model accuracy. For instance, the authors in \cite{Zachary_RAL_online_calibration_2022} show that the actual leg length of the robot with deformable feet is likely difficult to measure due to dynamic deformation effects and rolling contacts. \NEW{These uncertainties and unmodelled dynamics, unfortunately, are normally simplified or ignored in trajectory optimization framework and real-time execution 

% Using MPC as a feedback control from body trajectory is verified to improve robustness and target accuracy. 


% While full-body TO can plan complex motions, we verify that solely relying on joint PD controller to track the optimal joint reference from full-body TO does guarantee accurate target jumping. We select the experiments of jumping on the box from flat ground to make it match with the initial configuration as TO, as can be seen in Fig. \ref{fig:box_jumping}. The model of full-body dynamics is normally conservative as it assumes constant calf lengths, point-to-surface foot contact, and hard ground, and also ignores other unknown dynamics in hardware and contact. Unlike MIT Cheetah 3 \cite{QuannICRA19}, these assumptions however, are not valid for the Unitree A1 robot equipped with deformable feet, which likely leads to model mismatch (variable calf lengths), unknown ground stiffness and damping, and surface-to-surface contact, when the contact force significantly changes during the entire motion as discussed in \cite{Zachary_RAL_online_calibration_2022}. These factors are also hard to estimate correctly during jumping and can significantly affect the model accuracy. 

% Fig. \ref{fig:traj_compare_box_jumping} compares actual jumping trajectories in hardware under various MPC setups, associated with Fig. \ref{fig:box_jumping}. 
%With our method, the robot jumps to the target accurately with an error of $1-2$ cm and a landing angle error $<15^0$. 

For further evaluation of target accuracy and robustness, we performed 4 consecutive jumps (targeting $0.6$ m per jump) on flat ground with all MPC methods. The results are presented in Fig. \ref{fig:compare_all_mpcs_hardware}, showing some selected snapshots of the first and the last jump to the final target $2.4$ m. Our method with adaptive-frequency learned model and adaptive-frequency MPC achieves the highest target accuracy, allowing the robot to traverse $2.47$ m with an average distance error of only $1.75$ cm per jump.
During flight periods, the robot can jump up to $4\times$ its normal height.
% Our method with adaptive-frequency learned model and adaptive-frequency MPC allows the robot to traverse $2.47$ m with an average distance error of only $1.75$ cm per jump.



% \note{talk more about learn uncertainties in leg length,...}

% To reduce the computational time of neural network, we combine the
% , which might affect the real-time performance

Note that computing residual matrices $\bfG_{\calC,\bftheta}, \bfH_{\calC,\bftheta}, \bfH_{\calF,\bftheta}$ can consume significant time if we feed the neural network with $(\bfx_0, \bfu_0), (\bfx_{1}^*, \bfu_{1}^*), ..., (\bfx_{K}^*, \bfu_{K}^*)$ sequentially. To improve computational efficiency, we combined the current state and reference as a batch, then feed-forward the entire batch to the learned neural networks all at once, reducing the neural network query time to less than $1$ ms. 

% While full-body TO can plan complex motions, we verify that solely relying on joint PD controller to track the optimal joint reference from full-body TO does not guarantee accurate target jumping. 
% We also verify that solely relying on joint PD controller to track the optimal joint reference from full-body TO does not guarantee accurate target jumping. 
% We select the experiments of jumping on the box from flat ground to make it match with the initial configuration as TO, as can be seen in Fig. \ref{fig:box_jumping}. 

% These factors are also hard to estimate correctly during jumping and can significantly affect the model accuracy. 

% With a sizable prediction horizon (e.g., $K=10$), the solving time for $QP$ of each MPC update (\ref{eq:MPC_learned_QPcompact}) takes an average $2$ ms. This efficient computational time in total enables real-time performance for MPC with learned models. We also verify that if we use a large number of MPC horizons, i.e. $K=22$ when we use a fixed-frequency prediction scheme to cover the entire flight phase. This long horizon yields a big optimization size, causing significant computational costs. It takes an average of $30ms$ for each MPC update, which deteriorates the real-time performance, as shown in Fig. \ref{fig:computational_time}.
% \todo{How to convert batches data}

% 

% \subsection{Continuous Jumping}
% % The figure below shows the snapshot of continuous jumping that uses a feedforward PD controller to track reference from full-body trajectory optimization \cite{QuannICRA19}. We execute three jumps consecutively, with a desired distance of $60cm$ for each jump. However, the robot can leap only about $1.2m$ for all three jumps in total, which is only $67\%$ of the total desired distance.

% For further evaluation, we conduct 4 consecutive jumps on hardware with all MPC methods for the jumping target $60cm$ on flat ground. The experimental results are illustrated in Fig. \ref{fig:compare_all_mpcs_hardware}, showing some selected snapshots of the first and the last jump of four sequential jumps to the final target of $2.4m$. Our method with adaptive-frequency learned model and adaptive-frequency MPC can make the robot traverse $2.45m$, which yields an average distance error of only $1.25cm$ for each jump \TD{(Nitpicking) This actually doesn't mean the average error per jump will be small. E.g., the sum of 4 jumps could be 2.45m but it could be 0.1m + 1m + 0.45m + 0.9m, leading to an average error of 0.33m per jump. It's more precise to say that we calculate the errors for each jump and average them out}.

\begin{figure}[!t]
	\centering
	{\centering
		\resizebox{1.1\linewidth}{!}{\includegraphics[trim={0.9cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/obstacle/1/traj.pdf}}
	}
    {\centering
		\resizebox{1.1\linewidth}{!}{\includegraphics[trim={0.8cm 0.1cm 0cm 0cm},clip]{figures/Exp/continuous/obstacle/2/fmpc.pdf}}
	}
    {\centering
		\resizebox{1.1\linewidth}{!}{\includegraphics[trim={0.7cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/obstacle/2/compare_joint.pdf}}
	}
	
	\caption{\textbf{Continuous jumping performance on uneven terrain with A1 hardware, shown in  Fig. \ref{fig:introduction}:} (a) the actual trajectory of three continuous jumps on uneven terrain with our MPC approach; control forces on the front (b) and rear (c) legs, where the forces are $0$ when they are swing legs;
 % $L$ denotes the landing phase, which aims to handle hard impact and makes transitions between two consecutive jumps. 
 % The red circles denote the corresponding three targets; 
 and (d) accurate joint tracking of thigh and calf of rear legs.
 % The force controls on both legs satisfy limits $|F_z| \leq F_{max} = 400(N)$ and the friction cone constraint is enforced as $|F_x/F_z| \leq \mu = 0.6$ .
 }
	\label{fig:uneven-terrain-mpc-hardware}
\end{figure}

\subsection{Continuous Jumping on Uneven Terrain}
We tested the robustness and target accuracy of our learning-based MPC for continuous jumping on uneven terrains with a target of $60$ cm for each jump, as illustrated in Fig. \ref{fig:introduction} and Fig. \ref{fig:uneven-terrain-mpc-hardware}. The terrain consisted of multiple blocks with random heights between $2-4$ cm, randomly placed on the ground. We utilized MPC for the landing phase (L) to handle the hard impact and make a transition between two consecutive jumps. Each jump started with an all-leg contact period.
% \TD{Does this use the learned model or not?} to handle the hard impact and make a transition between two consecutive jumps. 
% For landing (L), we design MPC 
% \TD{Does this use the learned model or not?} to handle the hard impact and make a transition between two consecutive jumps.
Fig. \ref{fig:uneven-terrain-mpc-hardware}(a) shows the actual trajectory of three continuous jumps, leaping around $175$ cm in total that yields only $1.67$ cm distance error ($<3\%$) for each jump on the uneven terrain.
Fig. \ref{fig:uneven-terrain-mpc-hardware}(b) and (c) show the force outputs from adaptive-frequency MPC for the learned model. The force controls on both legs satisfy limits $|F_z| \leq F_{max} = 350$ N and the friction cone $|F_x/F_z| \leq \mu = 0.6$ during all phases. With our proposed framework, we achieve a target jumping error of less than $2$ cm ($3.5\%$) on $34$ single and continuous jumps with different targets and uneven terrain.

% \note{More results with MPC will come here}



% These properties of our learning MPC framework 


 % \subsubsection{ROS}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/60cm_compare_f_fpd/use_f/contact/rollout.png}}
% 	} \\
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/60cm_compare_f_fpd/use_fpd/contact/rollout.png}}
% 	}\\
% 	\caption{\textbf{Control input for neural network}. Comparison between the prediction of neural network for different selection of control inputs. The upper figures using control force, and the lower figures using the combination of control force + joint torque PD (Eq.\ref{eq:f_pd})}
% 	\label{fig:hardware_training_prediction_contact}
% \end{figure*}





% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-026.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-030.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-fix-learn/ezgif-frame-067.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ fixed frequency}: Motion snapshots from a jump forward $60~cm$ under unknown ground perturbation. This jumping is executed by MPC with fixed time step $\delta t = 25ms$ for learned model.} 
% 	\label{fig:ros-mpc-adaptive-learn-snapshots}
% \end{figure*}

% \begin{figure}[!t]
%     \centering
%     {\centering
%         \resizebox{1.1\linewidth}{!}{\includegraphics[trim={1cm 0cm 0cm 0cm},clip]{figures/Exp/v2/jump_on_box/compare_traj.eps}}}\\
%     \caption{\textbf{Box jumping task (hardware):} Comparison between different MPC implementations with (nominal/learn) model and (fixed/ adapt) frequency. All MPCs have the same $K=10$ prediction horizons. The red circle denotes the jumping target.} 
%     \label{fig:traj_compare_box_jumping}
% \end{figure} 




% \begin{figure}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/traj.eps}}}\\
%     \caption{\textbf{Forward jumping $60cm$:} Comparison between actual and reference trajectory when adaptive-frequency MPC for adaptive-frequency learned dynamics is utilized.} 
%     \label{fig:traj_mpc-adaptive-learn}
% \end{figure}  




% \begin{figure}[!t]
%     \centering
%     {\centering
%         \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/GRF.eps}}}\\
%     \caption{\textbf{Output force from MPC for learned dynamics (hardware).} The force controls on both legs satisfy limits $|F_z| \leq F_{max} = 350(N)$ and the friction cone constraint is enforced as $|F_x/F_z| \leq \mu = 0.6$} 
%     \label{fig:force_mpc-adaptive-learn}
% \end{figure} 



% \begin{figure}
%     \centering
%     {\centering
%         % \resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/ROS/mpc-adaptive-learn/time.eps}}}\\
%         \resizebox{1.0\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/adapt-learn/learn-adapt.pdf}}}\\
%     \caption{Perform 4 successive jumps with adaptive-frequency learning-based MPC} 
%     \label{fig:learn_adaptive_continuous}
% \end{figure} 


% \section{Hardware Experiments} \label{sec:hardware}
% \subsection{Setup and Training}

% MPC for nominal model is updated every $\delta_t = 25ms$, with number of horizon $N=10$.
% We use adaptive frequency for training. The Fig. 




% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mix/training/flight/rollout.png}}
% 	} \\
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mix/training/flight/rollout_vel.png}}
% 	}\\
% 	\caption{\textbf{Hardware experiments}: Comparison between the prediction of our neural network and the ground-truth trajectory of body position and orientation for flight phase.} 
% 	\label{fig:hardware_training_prediction_contact}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/training/contact/rollout_pos.png}}
% 	} \\
% 	\subfloat{\centering
% 		\resizebox{1\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/training/contact/rollout_vel.png}}
% 	}\\
% 	\caption{Comparison between the prediction of our neural network and the ground-truth trajectory of body position and orientation for flight phase.} 
% 	\label{fig:mpc-adaptive-learn-snapshots}
% \end{figure*}

% \subsection{Experiments}
% We validate our proposed MPC with adaptive frequency for learned model, and make comprehensive comparisons with the utilization of nominal model and fixed MPC frequency update.
% \begin{itemize}
%     \item \textit{MPC with fixed frequency for nominal model }
%     \item \textit{MPC with adaptive frequency for nominal model }

%     \item \textit{MPC with fixed frequency for learned model}

%     \item \textit{MPC with adaptive frequency for learned model}
% \end{itemize}



% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-094.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-120.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-fix-nominal/ezgif-frame-160.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ fixed frequency}: Motion snapshots from a jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC fix frequency $\delta t_{ct} = 25ms$ for nominal model.} 
% 	\label{fig:exp-mpc-fixfreq-nominal-snapshots}
% \end{figure*}


% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-026.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-029.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/mpc-adaptive-nominal/ezgif-frame-037.jpg}}
% 	}\\
% 	\caption{\textbf{Nominal model $\&$ adaptive frequency}: Motion snapshots from a jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms$ for a nominal model .} 
% 	\label{fig:exp-mpc-adaptfreq-nominal-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-011.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-014.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-fix-learn/ezgif-frame-019.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ fix frequency}: Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC fix frequency $\delta t_{ct} = \delta t_{fl} = 100ms $ for learned model.} 
% 	\label{fig:exp-mpc-fixfreq-learn-snapshots}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-001.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-021.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-024.jpg}}
% 	}
% 	\subfloat{\centering
% 		\resizebox{0.24\linewidth}{!}{\includegraphics[trim={00cm 0cm 0cm 0cm},clip]{figures/Exp/v2/mpc-adaptive-learn/ezgif-frame-028.jpg}}
% 	}\\
% 	\caption{\textbf{Learned model $\&$ adaptive frequency}: Motion snapshots from a successful jump forward $60~cm$ under unknown perturbation. This jumping is executed with MPC adaptive frequency $\delta t_{ct} = 25ms, \delta t_{fl} = 100ms $ for learned model.} 
% 	\label{fig:exp-mpc-adaptfreq-learn-snapshots}
% \end{figure*}





% \begin{figure}[!t]
% \centering
% {\centering
% \resizebox{\linewidth}{!}{\includegraphics[trim={0cm 0cm 0cm 0cm},clip]{figures/Exp/continuous/obstacle/1/traj.eps}}
% }
% \caption{\textbf{Hardware:} The figures show the trajectory of three consecutive jumps on uneven terrain with our MPC approach. MPC horizon is all set as $K=10$. It is associated with Fig. The red circles denote the corresponding three targets. \ref{fig:jump_on_uneven_terrain} }
% \label{fig:compare-mpc-hardware}
% \end{figure}







\section{Conclusion} \label{sec:conclusion}
In this letter, we developed a learned-model MPC approach that enables both target accuracy and robustness for aggressive jumping motions. We learned a residual model from a limited amount of data collected on a real robot to account for the effect of leg dynamics and the mismatch between the nominal model and hardware. Given the learned model, we designed an adaptive-frequency MPC controller that enables considering the entire flight phase and the jumping target during the optimization process. Our future work will focus on aggressive maneuvers in 3D, incorporating line-foot and rolling contact.

%to realize accurate and robust continuous 3D jumping as well as consider line-foot and rolling contact.


%tailored for both robustness and target jumping accuracy by covering the prediction of the entire flight phase and the target. 
% Via extensive experiments in hardware, we validate that our method outperforms baseline MPC controllers that adopts a nominal model and fixed frequency.

% \begin{figure}[!t]
% 	\centering
% 	{\centering
% 		\resizebox{0.8\linewidth}{!}{\includegraphics[trim={0cm 1cm 0cm 5cm},clip]{figures/Exp/continuous/TO/TO_continuous.png}}
% 	}
% 	\caption{
% 	\textbf{Continuous jumping} with Full-body TO + feed-forward PD controller}
% 	\label{fig:TO_continuous}
% \end{figure}

==> cls/sym.tex <==
% Calligraphic fonts
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

% Fraktur fonts
\newcommand{\frakA}{{\mathfrak{A}}}
\newcommand{\frakB}{{\mathfrak{B}}}
\newcommand{\frakC}{{\mathfrak{C}}}
\newcommand{\frakD}{{\mathfrak{D}}}
\newcommand{\frakE}{{\mathfrak{E}}}
\newcommand{\frakF}{{\mathfrak{F}}}
\newcommand{\frakG}{{\mathfrak{G}}}
\newcommand{\frakH}{{\mathfrak{H}}}
\newcommand{\frakI}{{\mathfrak{I}}}
\newcommand{\frakJ}{{\mathfrak{J}}}
\newcommand{\frakK}{{\mathfrak{K}}}
\newcommand{\frakL}{{\mathfrak{L}}}
\newcommand{\frakM}{{\mathfrak{M}}}
\newcommand{\frakN}{{\mathfrak{N}}}
\newcommand{\frakO}{{\mathfrak{O}}}
\newcommand{\frakP}{{\mathfrak{P}}}
\newcommand{\frakQ}{{\mathfrak{Q}}}
\newcommand{\frakR}{{\mathfrak{R}}}
\newcommand{\frakS}{{\mathfrak{S}}}
\newcommand{\frakT}{{\mathfrak{T}}}
\newcommand{\frakU}{{\mathfrak{U}}}
\newcommand{\frakV}{{\mathfrak{V}}}
\newcommand{\frakW}{{\mathfrak{W}}}
\newcommand{\frakX}{{\mathfrak{X}}}
\newcommand{\frakY}{{\mathfrak{Y}}}
\newcommand{\frakZ}{{\mathfrak{Z}}}

\newcommand{\fraka}{{\mathfrak{a}}}
\newcommand{\frakb}{{\mathfrak{b}}}
\newcommand{\frakc}{{\mathfrak{c}}}
\newcommand{\frakd}{{\mathfrak{d}}}
\newcommand{\frake}{{\mathfrak{e}}}
\newcommand{\frakf}{{\mathfrak{f}}}
\newcommand{\frakg}{{\mathfrak{g}}}
\newcommand{\frakh}{{\mathfrak{h}}}
\newcommand{\fraki}{{\mathfrak{i}}}
\newcommand{\frakj}{{\mathfrak{j}}}
\newcommand{\frakk}{{\mathfrak{k}}}
\newcommand{\frakl}{{\mathfrak{l}}}
\newcommand{\frakm}{{\mathfrak{m}}}
\newcommand{\frakn}{{\mathfrak{n}}}
\newcommand{\frako}{{\mathfrak{o}}}
\newcommand{\frakp}{{\mathfrak{p}}}
\newcommand{\frakq}{{\mathfrak{q}}}
\newcommand{\frakr}{{\mathfrak{r}}}
\newcommand{\fraks}{{\mathfrak{s}}}
\newcommand{\frakt}{{\mathfrak{t}}}
\newcommand{\fraku}{{\mathfrak{u}}}
\newcommand{\frakv}{{\mathfrak{v}}}
\newcommand{\frakw}{{\mathfrak{w}}}
\newcommand{\frakx}{{\mathfrak{x}}}
\newcommand{\fraky}{{\mathfrak{y}}}
\newcommand{\frakz}{{\mathfrak{z}}}

% Sets:
\newcommand{\setA}{\textsf{A}}
\newcommand{\setB}{\textsf{B}}
\newcommand{\setC}{\textsf{C}}
\newcommand{\setD}{\textsf{D}}
\newcommand{\setE}{\textsf{E}}
\newcommand{\setF}{\textsf{F}}
\newcommand{\setG}{\textsf{G}}
\newcommand{\setH}{\textsf{H}}
\newcommand{\setI}{\textsf{I}}
\newcommand{\setJ}{\textsf{J}}
\newcommand{\setK}{\textsf{K}}
\newcommand{\setL}{\textsf{L}}
\newcommand{\setM}{\textsf{M}}
\newcommand{\setN}{\textsf{N}}
\newcommand{\setO}{\textsf{O}}
\newcommand{\setP}{\textsf{P}}
\newcommand{\setQ}{\textsf{Q}}
\newcommand{\setR}{\textsf{R}}
\newcommand{\setS}{\textsf{S}}
\newcommand{\setT}{\textsf{T}}
\newcommand{\setU}{\textsf{U}}
\newcommand{\setV}{\textsf{V}}
\newcommand{\setW}{\textsf{W}}
\newcommand{\setX}{\textsf{X}}
\newcommand{\setY}{\textsf{Y}}
\newcommand{\setZ}{\textsf{Z}}

% Vectors
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}


\newcommand{\bfalpha}{\boldsymbol{\alpha}}
\newcommand{\bfbeta}{\boldsymbol{\beta}}
\newcommand{\bfgamma}{\boldsymbol{\gamma}}
\newcommand{\bfdelta}{\boldsymbol{\delta}}
\newcommand{\bfepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bfzeta}{\boldsymbol{\zeta}}
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bftheta}{\boldsymbol{\theta}}
\newcommand{\bfiota}{\boldsymbol{\iota}}
\newcommand{\bfkappa}{\boldsymbol{\kappa}}
\newcommand{\bflambda}{\boldsymbol{\lambda}}
\newcommand{\bfmu}{\boldsymbol{\mu}}
\newcommand{\bfnu}{\boldsymbol{\nu}}
\newcommand{\bfomicron}{\boldsymbol{\omicron}}
\newcommand{\bfpi}{\boldsymbol{\pi}}
\newcommand{\bfrho}{\boldsymbol{\rho}}
\newcommand{\bfsigma}{\boldsymbol{\sigma}}
\newcommand{\bftau}{\boldsymbol{\tau}}
\newcommand{\bfupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bfphi}{\boldsymbol{\phi}}
\newcommand{\bfchi}{\boldsymbol{\chi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\bfomega}{\boldsymbol{\omega}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\bfell}{\boldsymbol{\ell}}

% Matrices
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}


\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\bfDelta}{\boldsymbol{\Delta}}
\newcommand{\bfTheta}{\boldsymbol{\Theta}}
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}
\newcommand{\bfPi}{\boldsymbol{\Pi}}
\newcommand{\bfSigma}{\boldsymbol{\Sigma}}
\newcommand{\bfUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bfPhi}{\boldsymbol{\Phi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfOmega}{\boldsymbol{\Omega}}


% Blackboard Bold:
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}




